Nonlinear Random Matrices and Applications to the Sum of Squares Hierarchy

We develop new tools in the theory of nonlinear random matrices and apply them to study the performance of the Sum of Squares (SoS) hierarchy on average-case problems. The SoS hierarchy is a powerful optimization technique that has achieved tremendous success for various problems in combinatorial optimization, robust statistics and machine learning. It's a family of convex relaxations that lets us smoothly trade off running time for approximation guarantees. In recent works, it's been shown to be extremely useful for recovering structure in high dimensional noisy data. It also remains our best approach towards refuting the notorious Unique Games Conjecture. In this work, we analyze the performance of the SoS hierarchy on fundamental problems stemming from statistics, theoretical computer science and statistical physics. In particular, we show subexponential-time SoS lower bounds for the problems of the Sherrington-Kirkpatrick Hamiltonian, Planted Slightly Denser Subgraph, Tensor Principal Components Analysis and Sparse Principal Components Analysis. These SoS lower bounds involve analyzing large random matrices, wherein lie our main contributions. These results offer strong evidence for the truth of and insight into the low-degree likelihood ratio hypothesis, an important conjecture that predicts the power of bounded-time algorithms for hypothesis testing. We also develop general-purpose tools for analyzing the behavior of random matrices which are functions of independent random variables. Towards this, we build on and generalize the matrix variant of the Efron-Stein inequalities. In particular, our general theorem on matrix concentration recovers various results that have appeared in the literature. We expect these random matrix theory ideas to have other significant applications.

==> machinery/chapter_notes.tex <==
This chapter is adapted from \cite{potechin2020machinery}, which is joint work with Aaron Potechin.

==> machinery/choosing_funcs.tex <==
In this subsection, we give functions $B_{norm}(\alpha)$, $B(\gamma)$, $N(\gamma)$, and $c(\alpha)$ which satisfy the conditions needed for our machinery.
%--------------------------------
\subsection{Theorem Statements}
%--------------------------------
Recall the following definitions from Section \ref{quantitativetheoremstatementsection}.
\begin{definition}
	We define $S_{\alpha}$ to be the leftmost minimum vertex separator of $\alpha$
\end{definition}
\begin{definition}[Simplified Isolated Vertices]
	Under our simplifying assumptions, we define 
	\[
	I_{\alpha} = \{v \in W_{\alpha}: v \text{ is not incident to any edges in } E(\alpha)\}
	\]
\end{definition}
\begin{theorem}[Simplified $B_{norm}(\alpha)$, $B(\gamma)$, $N(\gamma)$, and $c(\alpha)$]\label{simplifiedfunctionstheorem}
	Under our simplifying assumptions, for all $\epsilon, \epsilon' > 0$ and all $D_V \in \mathbb{N}$, if we take
	\begin{enumerate}
		\item $q = 3\left\lceil{{D_V}ln(n) + \frac{ln(\frac{1}{\epsilon})}{3} + {D_V}ln(5) + 3{D^2_V}ln(2)}\right\rceil$
		\item $B_{vertex} = 6{D_V}\sqrt[4]{2eq}$
		\item $B_{norm}(\alpha) = {B_{vertex}^{|V(\alpha) \setminus U_{\alpha}| + |V(\alpha) \setminus V_{\alpha}|}}n^{\frac{w(V(\alpha)) + w(I_{\alpha}) - w(S_{\alpha})}{2}}$
		\item $B(\gamma) = B_{vertex}^{|V(\gamma) \setminus U_{\gamma}| + |V(\gamma) \setminus V_{\gamma}|}n^{\frac{w(V(\gamma) \setminus U_{\gamma})}{2}}$
		\item $N(\gamma) = (3D_V)^{2|V(\gamma) \setminus V_{\gamma}| + |V(\gamma) \setminus U_{\gamma}|}$
		\item $c(\alpha) = \frac{5(3D_V)^{|U_{\alpha} \setminus V_{\alpha}| + |V_{\alpha} \setminus U_{\alpha}| + 2|E(\alpha)|}2^{|V(\alpha) \setminus (U_{\alpha} \cup V_{\alpha})|}}{\epsilon'}$
	\end{enumerate}
	then the following conditions hold:
	\begin{enumerate}
		\item With probability at least $(1-\epsilon)$, $\forall \alpha \in \mathcal{M}'$, $||M_{\alpha}|| \leq B_{norm}(\alpha)$
		\item For all $\tau \in \mathcal{M}'$, $\gamma \in \Gamma_{*,U_{\tau}} \cup \{Id_{U_{\tau}}\}$, $\gamma' \in \Gamma_{*,V_{\tau}} \cup \{Id_{V_{\tau}}\}$, and intersection patterns $P \in \mathcal{P}_{\gamma,\tau,\gamma'}$,  
		\[
		B_{norm}(\tau_{P}) \leq B(\gamma)B(\gamma')B_{norm}(\tau)
		\]
		\item For all composable $\gamma_1,\gamma_2$, $B(\gamma_1)B(\gamma_2) = B(\gamma_1 \circ \gamma_2)$.
		\item $\forall U \in \mathcal{I}_{mid}, \sum_{\gamma \in \Gamma_{U,*}}{\frac{1}{|Aut(U)|c(\gamma)}} < \epsilon'$ 
		\item $\forall V \in \mathcal{I}_{mid}, \sum_{\gamma \in \Gamma_{*,V}}{\frac{1}{|Aut(U_{\gamma})|c(\gamma)}} < \epsilon'$ 
		\item $\forall U \in \mathcal{I}_{mid}, \sum_{\tau \in \mathcal{M}_{U}}{\frac{1}{|Aut(U)|c(\tau)}} < \epsilon'$
		\item For all $\tau \in \mathcal{M}'$, $\gamma \in \Gamma_{*,U_{\tau}} \cup \{Id_{U_{\tau}}\}$, and $\gamma' \in \Gamma_{*,V_{\tau}} \cup \{Id_{V_{\tau}}\}$,
		\begin{align*}
			&\sum_{j>0}{\sum_{\gamma_1,\gamma'_1,\cdots,\gamma_j,\gamma'_j \in \Gamma_{\gamma,\gamma',j}}{\prod_{i:\gamma_i \text{ is non-trivial}}{\frac{1}{|Aut(U_{\gamma_i})|}}
					\prod_{i:\gamma'_i \text{ is non-trivial}}{\frac{1}{|Aut(U_{\gamma'_i})|}}}}\sum_{P_1,\cdots,P_j:P_i \in \mathcal{P}_{\gamma_i,\tau_{P_{i-1}},{\gamma'_i}^T}}{\left(\prod_{i=1}^{j}{N(P_i)}\right)} \\
			&\leq \frac{N(\gamma)N(\gamma')}
			{(|Aut(U_{\gamma})|)^{1_{\gamma \text{ is non-trivial}}}(|Aut(U_{\gamma'})|)^{1_{\gamma' \text{ is non-trivial}}}}
		\end{align*}
	\end{enumerate}
\end{theorem}
\subsubsection{General functions $B_{norm}(\alpha)$, $B(\gamma)$, $N(\gamma)$, and $c(\alpha)$*}
Recall the following definitions from Section \ref{generalmaintheoremstatementsection}.
\begin{definition}[$S_{\alpha,min}$ and $S_{\alpha,max}$]
	Given a shape $\alpha \in \mathcal{M}'$, define $S_{\alpha,min}$ to be the leftmost minimum vertex separator of $\alpha$ if all edges with multiplicity at least $2$ are deleted and define $S_{\alpha,max}$ to be the leftmost minimum vertex separator of $\alpha$ if all edges with multiplicity at least $2$ are present.
\end{definition}
\begin{definition}[General $I_{\alpha}$]
	Given a shape $\alpha$, define $I_{\alpha}$ to be the set of vertices in $V(\alpha) \setminus (U_{\alpha} \cup V_{\alpha})$ such that all edges incident with that vertex have multplicity at least $2$.
\end{definition}
\begin{definition}[$B_{\Omega}$]
	We take $B_{\Omega}(j)$ to be a non-decreasing function such that for all $j \in \mathbb{N}$, $E_{\Omega}[x^{j}] \leq B_{\Omega}(j)^{j}$ 
\end{definition}
\begin{definition}
	For all $i$, we define $h^{+}_i$ to be the polynomial $h_i$ where we make all of the coefficients have positive sign.
\end{definition}
\begin{lemma}
	If $\Omega = N(0,1)$ then we can take $B_{\Omega}(j) = \sqrt{j}$ and we have that 
\end{lemma}
%\begin{definition}[General Potentially Isolated Vertices]
%In general, we define
%\[
%I_{\alpha} = \{v \in W_{\alpha}: \text{ every edge in } E(\alpha) \text{ which is incident to } v \text{ has multiplicity at least } 2\}
%\]
%Note that the labels on these multiple edges can be arbitrary.
%\end{definition}
\begin{theorem}[General $B_{norm}(\alpha)$, $B(\gamma)$, $N(\gamma)$, and $c(\alpha)$]\label{generalfunctionstheorem}
	For all $\epsilon, \epsilon' > 0$ and all $D_V,D_E \in \mathbb{N}$, if we take
	\begin{enumerate}
		\item $q = \left\lceil{3{D_V}ln(n) + ln(\frac{1}{\epsilon}) + {(3D_V)^k}ln(D_E + 1) + 3{D_V}ln(5)}\right\rceil$
		\item $B_{vertex} = 6q{D_V}$
		\item $B_{edge}(e) = 2h^{+}_{l_e}(B_{\Omega}(6{D_V}D_E))
		\max_{j \in [0,3{D_V}D_E]}{\left\{\left(h^{+}_{j}(B_{\Omega}(2qj))\right)^{\frac{l_e}{\max{\{j,l_e\}}}}\right\}}$
		\item $B_{norm}(\alpha) = 
		2e{B_{vertex}^{|V(\alpha) \setminus U_{\alpha}| + |V(\alpha) \setminus V_{\alpha}|}}\left(\prod_{e \in E(\alpha)}{B_{edge}(e)}\right)n^{\frac{w(V(\alpha)) + w(I_{\alpha}) - w(S_{\alpha})}{2}}$
		\item $B(\gamma) = B_{vertex}^{|V(\gamma) \setminus U_{\gamma}| + |V(\gamma) \setminus V_{\gamma}|}\left(\prod_{e \in E(\gamma)}{B_{edge}(e)}\right)n^{\frac{w(V(\gamma) \setminus U_{\gamma})}{2}}$
		\item $N(\gamma) = (3D_V)^{2|V(\gamma) \setminus V_{\gamma}| + |V(\gamma) \setminus U_{\gamma}|}$
		\item $c(\alpha) = \frac{5(3{t_{max}}D_V)^{|U_{\alpha} \setminus V_{\alpha}| + |V_{\alpha} \setminus U_{\alpha}| + k|E(\alpha)|}(2t_{max})^{|V(\alpha) \setminus (U_{\alpha} \cup V_{\alpha})|}}{\epsilon'}$
	\end{enumerate}
	then the following conditions hold:
	\begin{enumerate}
		\item With probability at least $(1-\epsilon)$, $\forall \alpha \in \mathcal{M}'$, $||M_{\alpha}|| \leq B_{norm}(\alpha)$
		\item For all $\tau \in \mathcal{M}'$, $\gamma \in \Gamma_{*,U_{\tau}} \cup \{Id_{U_{\tau}}\}$, $\gamma' \in \Gamma_{*,V_{\tau}} \cup \{Id_{V_{\tau}}\}$, and intersection patterns $P \in \mathcal{P}_{\gamma,\tau,\gamma'}$,  
		\[
		B_{norm}(\tau_{P}) \leq B(\gamma)B(\gamma')B_{norm}(\tau)
		\]
		\item For all composable $\gamma_1,\gamma_2$, $B(\gamma_1)B(\gamma_2) = B(\gamma_1 \circ \gamma_2)$.
		\item $\forall U \in \mathcal{I}_{mid}, \sum_{\gamma \in \Gamma_{U,*}}{\frac{1}{|Aut(U)|c(\gamma)}} < \epsilon'$ 
		\item $\forall V \in \mathcal{I}_{mid}, \sum_{\gamma \in \Gamma_{*,V}}{\frac{1}{|Aut(U_{\gamma})|c(\gamma)}} < \epsilon'$ 
		\item $\forall U \in \mathcal{I}_{mid}, \sum_{\tau \in \mathcal{M}_{U}}{\frac{1}{|Aut(U)|c(\tau)}} < \epsilon'$
		\item For all $\tau \in \mathcal{M}'$, $\gamma \in \Gamma_{*,U_{\tau}} \cup \{Id_{U_{\tau}}\}$, and $\gamma' \in \Gamma_{*,V_{\tau}} \cup \{Id_{V_{\tau}}\}$,
		\begin{align*}
			&\sum_{j>0}{\sum_{\gamma_1,\gamma'_1,\cdots,\gamma_j,\gamma'_j \in \Gamma_{\gamma,\gamma',j}}{\prod_{i:\gamma_i \text{ is non-trivial}}{\frac{1}{|Aut(U_{\gamma_i})|}}
					\prod_{i:\gamma'_i \text{ is non-trivial}}{\frac{1}{|Aut(U_{\gamma'_i})|}}}}\sum_{P_1,\cdots,P_j:P_i \in \mathcal{P}_{\gamma_i,\tau_{P_{i-1}},{\gamma'_i}^T}}{\left(\prod_{i=1}^{j}{N(P_i)}\right)} \\
			&\leq \frac{N(\gamma)N(\gamma')}
			{(|Aut(U_{\gamma})|)^{1_{\gamma \text{ is non-trivial}}}(|Aut(U_{\gamma'})|)^{1_{\gamma' \text{ is non-trivial}}}}
		\end{align*}
	\end{enumerate}
\end{theorem}
\begin{remark}
	Recall that if $\Omega = N(0,1)$ then we may take $B_{\Omega}(j) = \sqrt{j}$ and we have that 
	\[
	h^{+}_j(x) \leq \frac{1}{\sqrt{j!}}(x^2 + j)^{\frac{j}{2}} \leq \left(\frac{e}{j}(x^2 + j)\right)^{\frac{j}{2}}
	\]
	Thus, when $\Omega = N(0,1)$ we can take 
	\[
	B_{edge}(e) = 2\left(\frac{e}{l_e}(6{D_V}D_E + l_e)\right)^{l_e}\left(e(6{D_V}{D_E}q + 1)\right)^{l_e} \leq \left(400{D^2_V}{D^2_E}q\right)^{l_e}
	\]
\end{remark}
\subsection{Choosing $B_{norm}(\alpha)$}
We need matrix norm bounds which hold for all $\alpha \in \mathcal{M}'$. For convenience, we recall the definition of $\mathcal{M}'$ below.
\begin{definition}[$\mathcal{M}'$]
	We define $\mathcal{M}'$ to be the set of all shapes $\alpha$ such that
	\begin{enumerate}
		\item[1.] $|V(\alpha)| \leq 3D_V$
		\item[2.*] $\forall e \in E(\alpha), l_e \leq D_E$
		\item[3.*] All edges $e \in E(\alpha)$ have multiplicity at most $3D_V$.
	\end{enumerate}
\end{definition}
To obtain such norm bounds, we start with the norm bounds in the graph matrix norm bound paper. We then modify these bounds as follows:
\begin{enumerate}
	\item We make the bounds more compatible with the conditions of our machinery. To do this, we upper bound many of the terms in the norm bound by $B_{vertex}^{|V(\alpha) \setminus U_{\alpha}| + |V(\alpha) \setminus V_{\alpha}|}$ where $B_{vertex}$ is a function of our parameters. In general, we will also need to upper bound some of the terms by $\prod_{e \in E(\alpha)}(B_{edge}(e))$ where $B_{edge}(e)$ is a function of $l_e$, $\Omega$, and our parameters.
	\item We generalize the bounds so that they apply to improper shapes as well as proper shapes. Under our simplifying assumptions, all we need to do here is to take isolated vertices into account. In general, we also need to handle multi-edges. 
\end{enumerate}
\subsubsection{Simplified $B_{norm}(\alpha)$}
Under our simplifying assumptions, we start with the following norm bound from the updated graph matrix norm bound paper \cite{AMP20}:
\begin{theorem}[Simplified Graph Matrix Norm Bounds]\label{originalsimplifiednormbounds}
	Under our simplifying assumptions, for all $\epsilon > 0$ and all proper shapes $\alpha$, taking $c_{\alpha} = |V(\alpha) \setminus (U_{\alpha} \cup V_{\alpha})| + |S_{\alpha} \setminus (U_{\alpha} \cap V_{\alpha})|$,
	\[
	Pr\left(||M_{\alpha}|| > (2|V_{\alpha} \setminus (U_{\alpha} \cap V_{\alpha})|)^{|V(\alpha) \setminus (U_{\alpha} \cap V_{\alpha})|}(2eq)^{\frac{c_{\alpha}}{2}}n^{\frac{w(V(\alpha)) - w(S_{\alpha})}{2}}\right) < \epsilon
	\]
	where $q = 3\left\lceil\frac{ln(\frac{n^{w(S_{\alpha})}}{\epsilon})}{3c_{\alpha}}\right\rceil$
\end{theorem}
\begin{corollary}\label{firsttweakedsimplifiednormbound}
	For all shapes $\alpha$ and all $\epsilon > 0$, 
	\[
	Pr\left(||M_{\alpha}|| > \left(2|V_{\alpha}|\sqrt[4]{2eq}\right)^{|V(\alpha) \setminus U_{\alpha}| + |V(\alpha) \setminus V_{\alpha}|}n^{\frac{w(V(\alpha)) + w(I_{\alpha}) - w(S_{\alpha})}{2}}\right) < \epsilon
	\]
	where $q = 3\left\lceil\frac{ln(\frac{n^{w(S_{\alpha})}}{\epsilon})}{3c_{\alpha}}\right\rceil$.
\end{corollary}

\begin{proof}
	Observe that adding an isolated vertex to $\alpha$ is equivalent to multiplying $M_{\alpha}$ by $n - |V(\alpha)|$. Thus, if the bound holds for all proper $\alpha$ then it will hold for improper $\alpha$ as well. 
	
	We now make the following observations:
	\begin{enumerate}
		\item $|S_{\alpha} \setminus (U_{\alpha} \cap V_{\alpha})| \leq |U_{\alpha} \setminus V_{\alpha}|$, so $c_{\alpha} = |W_{\alpha}| + |S_{\alpha} \setminus (U_{\alpha} \cap V_{\alpha})| \leq |V(\alpha) \setminus V_{\alpha}|$. Similarly, $|S_{\alpha} \setminus (U_{\alpha} \cap V_{\alpha})| \leq |V_{\alpha} \setminus U_{\alpha}|$, so $c_{\alpha} \leq |V(\alpha) \setminus U_{\alpha}|$. Thus, $c_{\alpha} \leq \frac{|V(\alpha) \setminus U_{\alpha}| + |V(\alpha) \setminus V_{\alpha}|}{2}$.
		\item $|V(\alpha) \setminus (U_{\alpha} \cap V_{\alpha})| \leq |V(\alpha) \setminus U_{\alpha}| + |V(\alpha) \setminus V_{\alpha}|$
	\end{enumerate}
	Thus, by Theorem \ref{originalsimplifiednormbounds}, for all proper shapes $\alpha$ and all $\epsilon > 0$, 
	\[
	Pr\left(||M_{\alpha}|| > \left(2|V_{\alpha}|\sqrt[4]{2eq}\right)^{|V(\alpha) \setminus U_{\alpha}| + |V(\alpha) \setminus V_{\alpha}|}n^{\frac{w(V(\alpha)) + w(I_{\alpha}) - w(S_{\alpha})}{2}}\right) < \epsilon''
	\]
	where $q = 3\left\lceil\frac{ln(\frac{n^{w(S_{\alpha})}}{\epsilon})}{3c_{\alpha}}\right\rceil$.
\end{proof}
\begin{corollary}\label{tweakedsimplifiednormbound}
	For all $z \in \mathbb{N}$ and all $\epsilon > 0$, taking $\epsilon'' = \frac{\epsilon}{5^{z}2^{z^2}}$, with probability at least $1-\epsilon$ we have that for all shapes $\alpha$ such that $|V(\alpha)| \leq z$, 
	\[
	||M_{\alpha}|| \leq \left(2|V_{\alpha}|\sqrt[4]{2eq}\right)^{|V(\alpha) \setminus U_{\alpha}| + |V(\alpha) \setminus V_{\alpha}|}n^{\frac{w(V(\alpha)) + w(I_{\alpha}) - w(S_{\alpha})}{2}}
	\]
	where $q = 3\left\lceil\frac{ln(\frac{n^{w(S_{\alpha})}}{\epsilon''})}{3c_{\alpha}}\right\rceil$.
\end{corollary}
\begin{proof}
	This result can be proved from Corollary \ref{firsttweakedsimplifiednormbound} using a union bound and the following proposition:
	\begin{proposition}\label{simplifiedcountingalpha}
		Under our simplifying assumptions, for all $z \in \mathbb{N}$, there are at most $5^{z}2^{z^2}$ proper shapes $\alpha$ such that $V(\alpha) \leq z$.
	\end{proposition}
	\begin{proof}
		Observe that we can construct any proper shape $\alpha$ with at most $m$ vertices as follows:
		\begin{enumerate}
			\item Start with $z$ vertices $v_1,\ldots,v_z$.
			\item For each vertex $v_i$, choose whether $v_i \in V(\alpha) \setminus U_{\alpha} \setminus V_{\alpha}$, $v_i \in U_{\alpha} \setminus V_{\alpha}$, $v_i \in V_{\alpha} \setminus U_{\alpha}$, $v_i \in U_{\alpha} \cap V_{\alpha}$, or $v_i \notin V(\alpha)$.
			\item For each pair of vertices $v_i,v_j \in V(\alpha)$, choose whether or not $(v_i,v_j) \in E(\alpha)$
		\end{enumerate}
	\end{proof}
\end{proof}
\begin{corollary}\label{finalsimplifiednormbound}
	For all $D_V \in \mathbb{N}$ and all $\epsilon > 0$, taking 
	\[
	q = 3\left\lceil\frac{ln(\frac{5^{3D_V}2^{9D^2_V}n^{3D_V}}{\epsilon})}{3}\right\rceil = 
	3\left\lceil{{D_V}ln(n) + \frac{ln(\frac{1}{\epsilon})}{3} + {D_V}ln(5) + 3{D^2_V}ln(2)}\right\rceil,
	\] 
	$B_{vertex} = 6{D_V}\sqrt[4]{2eq}$, and
	\[
	B_{norm}(\alpha) = {B_{vertex}^{|V(\alpha) \setminus U_{\alpha}| + |V(\alpha) \setminus V_{\alpha}|}}n^{\frac{w(V(\alpha)) + w(I_{\alpha}) - w(S_{\alpha})}{2}},
	\] 
	with probability at least $(1-\epsilon)$ we have that for all shapes $\alpha \in \mathcal{M}'$, $||M_{\alpha}|| \leq B_{norm}(\alpha)$
\end{corollary}
\begin{proof}
	This follows from Corollary \ref{tweakedsimplifiednormbound} and the fact that for all $\alpha \in \mathcal{M}'$, $w(S_{\alpha}) \leq |V(\alpha)| \leq3D_V$
\end{proof}
\subsubsection{General $B_{norm}(\alpha)$}
In general, we start with the following norm bound from the updated graph matrix norm bound paper \cite{AMP20}:
\begin{theorem}[General Graph Matrix Norm Bounds]\label{originalgeneralnormbounds}
	For all $\epsilon > 0$ and all proper shapes $\alpha$, taking $q = \lceil{ln(\frac{n^{w(S_{\alpha})}}{\epsilon})}\rceil$
	\[
	P\left(||M_{\alpha}|| > 2e(2q|V(\alpha)|)^{|V(\alpha) \setminus (U_{\alpha} \cap V_{\alpha})|}\left(\prod_{e \in E(\alpha)}{h^{+}_{l_{e}}(B_{\Omega}(2q{l_e}))}\right)
	n^{\frac{(w(V(\alpha)) - w(S_{\alpha}))}{2}}\right) < \epsilon
	\]
\end{theorem}
\begin{corollary}
	For all $\epsilon > 0$, for all $z,l_{max},m \in \mathbb{N}$, taking $\epsilon'' = \frac{\epsilon}{5^{z}(l_{max} + 1)^{z^k}}$, with probability at least $1-\epsilon$, for all shapes $\alpha$ such that 
	\begin{enumerate}
		\item $|V(\alpha)| \leq z$.
		\item All edges in $E(\alpha)$ have label at most $l_{max}$.
		\item All edges in $E(\alpha)$ have multiplicity at most $m$.
	\end{enumerate}, 
	\begin{align*}
		||M_{\alpha}|| \leq &2e(2q|V(\alpha)|)^{|V(\alpha) \setminus U_{\alpha}| + |V(\alpha) \setminus V_{\alpha}|}\left(\prod_{e \in E(\alpha)}{2h^{+}_{l_e}(B_{\Omega}(2ml_{max}))
			\max_{j \in [0,ml_{max}]}{\left\{\left(h^{+}_{j}(B_{\Omega}(2qj))\right)^{\frac{l_e}{\max{\{j,l_e\}}}}\right\}}}\right)\\
		&n^{\frac{w(V(\alpha)) + w(I_{\alpha}) - w(S_{\alpha,min})}{2}}
	\end{align*}
	where $q = \left\lceil{ln\left(\frac{n^{w(S_{\alpha,max})}}{\epsilon''}\right)}\right\rceil$
\end{corollary}
\begin{proof}
	Observe that for each $\alpha$ which has multi-edges, we can write $M_{\alpha} = \sum_{i}{{c_i}M_{\alpha_i}}$ where each $\alpha_i$ has no multiple edges. We first upper bound $\sum_{i}{|c_i|}$.
	\begin{lemma}
		For any $a_1,\ldots,a_m \in \mathbb{N} \cup \{0\}$, taking $p_{max} = \sum_{i=1}^{m}{a_i}$ and writing $\prod_{i=1}^{m}{h_{a_i}} = \sum_{k=0}^{p_{max}}{{c_k}h_k}$,
		\[
		\sum_{k=0}^{p_{max}}{|c_k|} \leq (p_{max}+1)\prod_{i=1}^{m}{h^{+}_{a_i}(B_{\Omega}(2p_{max}))} \leq \prod_{i=1}^{m}{2h^{+}_{a_i}(B_{\Omega}(2p_{max}))}
		\]
	\end{lemma}
	\begin{proof}
		Suppose $\prod_{i = 1}^m (h_{a_i}(x))^2 = \sum_{k = 0}^{2p_{max}} u_kx^k$ and $\prod_{i = 1}^m (h^+_{a_i}(x))^2 = \sum_{k = 0}^{p_{max}} v_kx^k$. Then, note that $|u_k| \le v_k$ and so,	\[E_{\Omega}[\prod_{i = 1}^{m}(h_{a_i}(x))^2] = \sum_{k = 0}^{2p_{max}} u_k E_{\Omega}[x^k] \le \sum_{k = 0}^{2p_{max}} v_k|E_{\Omega}[x^k]| \le \sum_{k = 0}^{2p_{max}} v_k(B_{\Omega}(2p_{max}))^k = \prod_{i = 1}^m (h_{a_i}^+(B_{\Omega}(2p_{max}))^2\]
		Therefore, using the fact that $h_k$ form an orthonormal basis,
		\[\sum_{k = 0}^{p_{max}} c_k^2 = E_{\Omega}[(\sum_{k = 0}^{p_{max}} c_kh_k(x))^2] = E_{\Omega}[\prod_{i = 1}^m (h_{a_i}(x))^2] \le  \prod_{i = 1}^m (h_{a_i}^+(B_{\Omega}(2p_{max}))^2\]
		
		This implies
		\[(\sum_{k = 0}^{p_{max}}|c_k|)^2 \le (p_{max} + 1)(\sum_{k = 0}^{p_{max}} c_k^2) \le  (p_{max} + 1)  \prod_{i = 1}^m (h_{a_i}^+(B_{\Omega}(2p_{max}))^2\]
		Taking square roots gives the inequality.
	\end{proof}
	\begin{corollary}
		For any shape $\alpha$ such that every edge of $\alpha$ has multiplicity at most $m$ and label at most $l_{max}$, if we write 
		$M_{\alpha} = \sum_{i}{{c_i}M_{\alpha_i}}$ where each $\alpha_i$ has no multi-edges then $\sum_{i}{|c_i|} \leq \prod_{e \in E(\alpha)}{2h^{+}_{l_e}(B_{\Omega}(2ml_{max}))}$
	\end{corollary}
	The result now follows from Theorem \ref{originalgeneralnormbounds} and the following observations:
	\begin{enumerate}
		\item $|V(\alpha) \setminus (U_{\alpha} \cap V_{\alpha})| \leq |V(\alpha) \setminus U_{\alpha}| + |V(\alpha) \setminus V_{\alpha}|$.
		\item For any $\alpha$, writing $M_{\alpha} = \sum_{i}{{c_i}M_{\alpha_i}}$ where each $\alpha_i$ has no multi-edges, for all $\alpha_i$,
		\[
		w(V(\alpha_i)) + w(I_{\alpha_i}) - w(S_{\alpha_i}) \leq w(V(\alpha)) + w(I_{\alpha}) - w(S_{\alpha,min})
		\]
		\item For any $a_1,\ldots,a_m \in \mathbb{N} \cup \{0\}$ such that $\forall i' \in [m], a_{i'} \leq l_{max}$, for all $j \in [0,ml_{max}]$
		\[
		h^{+}_{j}(B_{\Omega}(2qj)) \leq \prod_{i'=1}^{m}{\left(h^{+}_{j}(B_{\Omega}(2qj))\right)^{\frac{a_{i'}}{\max{\{j,a_{i'}\}}}}} \leq 
		\prod_{i'=1}^{m}{\max_{j' \in [0,ml_{max}]}{\left\{\left(h^{+}_{j'}(B_{\Omega}(2qj'))\right)^{\frac{a_{i'}}{\max{\{j',a_{i'}\}}}}\right\}}}
		\]
	\end{enumerate}
	\begin{proposition}
		For all $z,l_{max} \in \mathbb{N}$, there are at most $5^{z}(l_{max} + 1)^{z^k}$ proper shapes $\alpha$ such that $|V(\alpha)| \leq z$ and every edge in $E(\alpha)$.
	\end{proposition}
	\begin{proof}
		This can be proved in the same way as before. Observe that we can construct any proper shape $\alpha$ with at most $z$ vertices as follows:
		\begin{enumerate}
			\item Start with $z$ vertices $v_1,\ldots,v_z$.
			\item For each vertex $v_i$, choose whether $v_i \in V(\alpha) \setminus U_{\alpha} \setminus V_{\alpha}$, $v_i \in U_{\alpha} \setminus V_{\alpha}$, $v_i \in V_{\alpha} \setminus U_{\alpha}$, $v_i \in U_{\alpha} \cap V_{\alpha}$, or $v_i \notin V(\alpha)$.
			\item For each $k$ tuple of vertices in $V(\alpha)$, choose the label of the hyperedge between these vertices (or $0$ if the hyperedge is not in $E(\alpha)$).
		\end{enumerate}
	\end{proof}
\end{proof}
\begin{corollary}\label{finalgeneralnormbounds}
	For all $D_V,D_E \in \mathbb{N}$ and all $\epsilon > 0$, taking 
	\[
	B_{norm}(\alpha) = 2e{B_{vertex}^{|V(\alpha) \setminus U_{\alpha}| + |V(\alpha) \setminus V_{\alpha}|}}\left(\prod_{e \in E(\alpha)}{B_{edge}(e)}\right)n^{\frac{w(V(\alpha)) + w(I_{\alpha}) - w(S_{\alpha})}{2}}
	\] where 
	\begin{enumerate}
		\item $q = \left\lceil{ln\left(\frac{n^{3D_V}}{\epsilon''}\right)}\right\rceil = \left\lceil{3{D_V}ln(n) + ln(\frac{1}{\epsilon}) + {(3D_V)^k}ln(D_E + 1) + 3{D_V}ln(5)}\right\rceil$
		\item $B_{vertex} = 6q{D_V}$
		\item $B_{edge}(e) = 2h^{+}_{l_e}(B_{\Omega}(6{D_V}D_E))
		\max_{j \in [0,3{D_V}D_E]}{\left\{\left(h^{+}_{j}(B_{\Omega}(2qj))\right)^{\frac{l_e}{\max{\{j,l_e\}}}}\right\}}$
	\end{enumerate}
	with probability at least $(1-\epsilon)$, for all shapes $\alpha \in \mathcal{M}'$, $||M_{\alpha}|| \leq B_{norm}(\alpha)$.
\end{corollary}
\subsection{Choosing $B(\gamma)$}
We now describe how to choose the function $B(\gamma)$. Recall that we want the following conditions to hold:
\begin{enumerate}
	\item For all $\gamma, \tau, \gamma'$ and all intersection patterns $P \in \mathcal{P}_{\gamma,\tau,\gamma'}$, 
	\[
	B_{norm}(\tau_{P}) \leq B(\gamma)B(\gamma')B_{norm}(\tau)
	\]
	\item For all composable $\gamma_1,\gamma_2$, $B(\gamma_1)B(\gamma_2) = B(\gamma_1 \circ \gamma_2)$.
\end{enumerate}
The most important part of choosing $B(\gamma)$ is to make sure that the factors of $n$ are controlled. For this, we use the following intersection tradeoff lemma. Under our simplifying assumptions, this lemma follows from \cite[Lemma 7.12]{BHKKMP16}. We defer the general proof of this lemma to the end of this section.
\begin{lemma}[Intersection Tradeoff Lemma]
	For all $\gamma, \tau, \gamma'$ and all intersection patterns $P \in \mathcal{P}_{\gamma,\tau,\gamma'}$, 
	\[
	w(V(\tau_P)) + w(I_{\tau_P}) - w(S_{\tau_P,min}) \leq w(V(\tau)) + w(I_{\tau}) - w(S_{\tau,min})+ w(V(\gamma) \setminus U_{\gamma}) + w(V(\gamma') \setminus U_{\gamma'})
	\]
\end{lemma}
Based on this intersection tradeoff lemma, we can choose the function $B(\gamma)$ as follows.
\begin{corollary}
	If we take 
	\[
	B_{norm}(\alpha) = C \cdot B_{vertex}^{|V(\alpha) \setminus U_{\alpha}| + |V(\alpha) \setminus V_{\alpha}|}\left(\prod_{e \in E(\alpha)}{B_{edge}(e)}\right)n^{\frac{w(V(\alpha)) + w(I_{\alpha}) - w(S_{\alpha})}{2}}
	\] 
	for some constant $C > 0$ and take
	\[
	B(\gamma) = B_{vertex}^{|V(\gamma) \setminus U_{\gamma}| + |V(\gamma) \setminus V_{\gamma}|}\left(\prod_{e \in E(\gamma)}{B_{edge}(e)}\right)n^{\frac{w(V(\gamma) \setminus U_{\gamma})}{2}}
	\]
	then the following conditions hold:
	\begin{enumerate}
		\item For all $\gamma, \tau, \gamma'$ and all intersection patterns $P \in \mathcal{P}_{\gamma,\tau,\gamma'}$, 
		\[
		B_{norm}(\tau_{P}) \leq B(\gamma)B(\gamma')B_{norm}(\tau)
		\]
		\item For all composable $\gamma_1,\gamma_2$, $B(\gamma_1)B(\gamma_2) = B(\gamma_1 \circ \gamma_2)$.
	\end{enumerate}
\end{corollary}
\begin{proof}
	We have that 
	\[
	B_{norm}(\tau_{P}) = B_{vertex}^{|V(\tau_P) \setminus U_{\tau_P}| + |V(\tau_P) \setminus V_{\tau_P}|}\left(\prod_{e \in E(\tau_P)}{B_{edge}(e)}\right)n^{\frac{w(V(\tau_P)) + w(I_{\tau_P}) - w(S_{\tau_P})}{2}}
	\]
	and 
	\begin{align*}
		B(\gamma)B(\gamma')B_{norm}(\tau) &= B_{vertex}^{|V(\gamma) \setminus U_{\gamma}| + |V(\gamma) \setminus V_{\gamma}| + |V(\gamma') \setminus U_{\gamma'}| + |V(\gamma') \setminus V_{\gamma'}| + |V(\tau) \setminus U_{\tau}| + |V(\tau) \setminus V_{\tau}|} \\
		&\left(\prod_{e \in E(\gamma) \cup E(\gamma') \cup E(\tau)}{B_{edge}(e)}\right)n^{\frac{w(V(\gamma) \setminus U_{\gamma}) + w(V(\gamma') \setminus U_{\gamma'}) + 
				w(V(\tau)) + w(I_{\tau}) - w(S_{\tau})}{2}}
	\end{align*}
	The first condition now follows immediately from the following observations:
	\begin{enumerate}
		\item \begin{align*}
			&|V(\gamma) \setminus U_{\gamma}| + |V(\gamma) \setminus V_{\gamma}| + |V(\gamma') \setminus U_{\gamma'}| + |V(\gamma') \setminus V_{\gamma'}| + |V(\tau) \setminus U_{\tau}| + |V(\tau) \setminus V_{\tau}| \\
			&= |V(\gamma \circ \tau \circ {\gamma'}^T) \setminus U_{\gamma \circ \tau \circ {\gamma'}^T}| + |V(\gamma \circ \tau \circ {\gamma'}^T) \setminus V_{\gamma \circ \tau \circ {\gamma'}^T}| 
			\geq |V(\tau_P) \setminus U_{\tau_P}| + |V(\tau_P) \setminus V_{\tau_P}|
		\end{align*}
		\item $E(\tau_P) = E(\gamma) \cup E(\tau) \cup E({\gamma'}^T)$ so 
		$\prod_{e \in E(\tau_P)}{B_{edge}(e)} = \prod_{e \in E(\gamma) \cup E(\gamma') \cup E(\tau)}{B_{edge}(e)}$.
		\item By the intersection tradeoff lemma, 
		\[
		w(V(\tau_P)) + w(I_{\tau_P}) - w(S_{\tau_P}) \leq w(V(\tau)) + w(I_{\tau}) - w(S_{\tau}) + w(V(\gamma) \setminus U_{\gamma}) + w(V(\gamma') \setminus U_{\gamma'})
		\]
	\end{enumerate}
	The second condition follows  from the form of $B(\gamma)$.
\end{proof}
\subsection{Choosing $N(\gamma)$}
To choose $N(\gamma)$, we use the following lemma:
\begin{lemma}
	For all $D_V \in \mathbb{N}$, for all composable $\gamma,\tau,{\gamma'}^T$ such that $|V(\gamma)| \leq D_V$, $|V(\tau)| \leq D_V$, and $|V(\gamma')| \leq D_V$, 
	\begin{align*}
		&\sum_{j>0}{\sum_{\gamma_1,\gamma'_1,\cdots,\gamma_j,\gamma'_j \in \Gamma_{\gamma,\gamma',j}}{\prod_{i:\gamma_i \text{ is non-trivial}}{\frac{1}{|Aut(U_{\gamma_i})|}}
				\prod_{i:\gamma'_i \text{ is non-trivial}}{\frac{1}{|Aut(U_{\gamma'_i})|}}}}\sum_{P_1,\cdots,P_j:P_i \in \mathcal{P}_{\gamma_i,\tau_{P_{i-1}},{\gamma'_i}^T}}{\left(\prod_{i=1}^{j}{N(P_i)}\right)} \\
		&\leq \frac{{(3D_V)}^{2(|V(\gamma) \setminus V_{\gamma}| + |V(\gamma') \setminus V_{\gamma'}|) + (|V(\gamma) \setminus U_{\gamma}| + |V(\gamma') \setminus U_{\gamma'}|)}}
		{(|Aut(U_{\gamma})|)^{1_{\gamma \text{ is non-trivial}}}(|Aut(U_{\gamma'})|)^{1_{\gamma' \text{ is non-trivial}}}}
	\end{align*}
\end{lemma}
\begin{proof}[Proof sketch]
	Observe that aside from the orderings (which are canceled out by the $|Aut(U_{\gamma_i})|$ and $|Aut(U_{\gamma'_i})|$ factors), the intersection patterns $\{P_i: i \in [j]\}$ are determined by the following data on each vertex $v \in (V(\gamma) \setminus V_{\gamma}) \cup (V({\gamma'}^T) \setminus V_{{\gamma'}^T})$:
	\begin{enumerate}
		\item The first $i \in [j]$ such that $v \in (V(\gamma_i) \setminus V_{\gamma_i}) \cup (V({\gamma'_i}^T) \setminus V_{{\gamma'_i}^T})$. There are at most $j$ possibilities for this.
		\item A vertex $u$ (if one exists) in $V(\gamma_{i-1} \circ \ldots \circ \gamma_1 \circ \tau \circ {\gamma'_1}^T \ldots \circ {\gamma'_{i-1}}^T)$ such that $u$ and $v$ are equal. There are at most $3D_V$ possibilities for this.
	\end{enumerate}
	Using these observations and taking $j_{max} = |V(\gamma) \setminus V_{\gamma}| + |V(\gamma') \setminus V_{\gamma'}|$,
	\begin{align*}
		&\sum_{j > 0}{\sum_{\gamma_1,\gamma'_1,\cdots,\gamma_j,\gamma'_j \in \Gamma_{\gamma,\gamma',j}}{\prod_{i:\gamma_i \text{ is non-trivial}}{\frac{1}{|Aut(U_{\gamma_i})|}}
				\prod_{i:\gamma'_i \text{ is non-trivial}}{\frac{1}{|Aut(U_{\gamma'_i})|}}}}\sum_{P_1,\cdots,P_j:P_i \in \mathcal{P}_{\gamma_i,\tau_{P_{i-1}},{\gamma'_i}^T}}{1} \\
		&\leq \sum_{j =1}^{j_{max}}{\frac{{(3jD_V)}^{|V(\gamma) \setminus V_{\gamma}| + |V(\gamma') \setminus V_{\gamma'}|}}
			{(|Aut(U_{\gamma})|)^{1_{\gamma \text{ is non-trivial}}}(|Aut(U_{\gamma'})|)^{1_{\gamma' \text{ is non-trivial}}}}} \\
		&\leq j_{max}\left(\frac{2}{3}\right)^{j_{max}}\frac{{(3D_V)}^{2(|V(\gamma) \setminus V_{\gamma}| + |V(\gamma') \setminus V_{\gamma'}|)}}
		{(|Aut(U_{\gamma})|)^{1_{\gamma \text{ is non-trivial}}}(|Aut(U_{\gamma'})|)^{1_{\gamma' \text{ is non-trivial}}}} \\
		&< \frac{{(3D_V)}^{2(|V(\gamma) \setminus V_{\gamma}| + |V(\gamma') \setminus V_{\gamma'}|)}}
		{(|Aut(U_{\gamma})|)^{1_{\gamma \text{ is non-trivial}}}(|Aut(U_{\gamma'})|)^{1_{\gamma' \text{ is non-trivial}}}}
	\end{align*}
	Now recall that by Lemma ,
	for any $\gamma_i,\tau_{P_{i-1}},{\gamma'_i}^{T}$ and any intersection pattern $P_i \in \mathcal{P}_{\gamma_i,\tau_{P_{i-1}},{\gamma'_i}^T}$, 
	\[
	N(P_i) \leq |V(\tau_{P_i})|^{|V(\gamma_i) \setminus U_{\gamma_i}| + |V(\gamma'_i) \setminus U_{\gamma'_i}|}
	\]
	Thus, for any $P_1,\cdots,P_j:P_i \in \mathcal{P}_{\gamma_i,\tau_{P_{i-1}},{\gamma'_i}^T}$, $\prod_{i=1}^{j}{N(P_i)} \leq (3D_V)^{|V(\gamma) \setminus U_{\gamma}| + |V(\gamma') \setminus U_{\gamma'}|}$.
	Putting everything together, the result follows.
\end{proof}
\begin{corollary}
	For all $D_V \in \mathbb{N}$, if we take $N(\gamma) = (3D_V)^{2|V(\gamma) \setminus V_{\gamma}| + |V(\gamma) \setminus U_{\gamma}|}$ then for all composable $\gamma, \tau, {\gamma'}^T$ such that $|V(\gamma)| \leq D_V$, $|V(\tau)| \leq D_V$, and $|V(\gamma')| \leq D_V$, 
	\begin{align*}
		&\sum_{j>0}{\sum_{\gamma_1,\gamma'_1,\cdots,\gamma_j,\gamma'_j \in \Gamma_{\gamma,\gamma',j}}{\prod_{i:\gamma_i \text{ is non-trivial}}{\frac{1}{|Aut(U_{\gamma_i})|}}
				\prod_{i:\gamma'_i \text{ is non-trivial}}{\frac{1}{|Aut(U_{\gamma'_i})|}}}}\sum_{P_1,\cdots,P_j:P_i \in \mathcal{P}_{\gamma_i,\tau_{P_{i-1}},{\gamma'_i}^T}}{\left(\prod_{i=1}^{j}{N(P_i)}\right)} \\
		&\leq \frac{N(\gamma)N(\gamma')}
		{(|Aut(U_{\gamma})|)^{1_{\gamma \text{ is non-trivial}}}(|Aut(U_{\gamma'})|)^{1_{\gamma' \text{ is non-trivial}}}}
	\end{align*}
\end{corollary}
%Based on this, we can take $N(\gamma) = (3D_V)^{2|V(\gamma) \setminus V_{\gamma}| + |V(\gamma) \setminus U_{\gamma}|}$
\subsection{Choosing $c(\alpha)$}
In this section, we describe how to choose $c(\alpha)$. For simplicity, we first describe how to choose $c(\alpha)$ under our simplifying assumptions. We then describe the minor adjustments that are needed when we have hyperedges and multiple types of vertices.
\begin{lemma}\label{calphalemma}
	Under our simplifying assumptons, for all $U \in \mathcal{I}_{mid}$,
	\[
	\sum_{\alpha: U_{\alpha} \equiv U, \alpha \text{ is proper and non-trivial}}{\frac{1}{|Aut(U_{\alpha} \cap V_{\alpha})|(3D_V)^{|U_{\alpha} \setminus V_{\alpha}| + |V_{\alpha} \setminus U_{\alpha}| + 2|E(\alpha)|}2^{|V(\alpha) \setminus (U_{\alpha} \cup V_{\alpha})|}}} < 5
	\]
\end{lemma} 
\begin{proof}
	In order to choose $\alpha$, it is sufficient to choose the following:
	\begin{enumerate}
		\item The number $j_1$ of vertices in $U_{\alpha} \setminus V_{\alpha}$, the number $j_2$ of vertices in $V_{\alpha} \setminus U_{\alpha}$, and the number $j_3$ of vertices in $V(\alpha) \setminus (U_{\alpha} \cup V_{\alpha})$.
		\item A mapping in $Aut(U_{\alpha} \cap V_{\alpha})$ determining how the vertices in $U_{\alpha} \cap V_{\alpha}$ match up with each other.
		\item The position of each vertex $u \in U_{\alpha} \setminus V_{\alpha}$ within $U_{\alpha}$ (there are at most $|U_{\alpha}| \leq D_V$ choices for this).
		\item The position of each vertex $v \in V_{\alpha} \setminus U_{\alpha}$ within $V_{\alpha}$ (there are at most $|U_{\alpha}| \leq D_V$ choices for this).
		\item The number $j_4$ of edges in $E(\alpha)$.
		\item The endpoints of each edge in $E(\alpha)$.
	\end{enumerate}
	This implies that for all $j_1,j_2,j_3,j_4 \geq 0$
	\[
	\sum_{\alpha: U_{\alpha} \equiv U, |U_{\alpha} \setminus V_{\alpha}| = j_1, |V_{\alpha} \setminus U_{\alpha}| = j_2 \atop
		|V(\alpha) \setminus (U_{\alpha} \cup V_{\alpha})| = j_3, |E(\alpha)| = j_4}{\frac{1}{|Aut(U_{\alpha} \cap V_{\alpha})|(D_V)^{j_1 + j_2}
			(D_V)^{2j_4}}} \leq 1
	\]
	Using this, we have that
	\begin{align*}
		&\sum_{\alpha: U_{\alpha} \equiv U, \alpha \text{ is proper and non-trivial}}{\frac{1}{|Aut(U_{\alpha} \cap V_{\alpha})|(3D_V)^{|U_{\alpha} \setminus V_{\alpha}| + |V_{\alpha} \setminus U_{\alpha}| + 2|E(\alpha)|}2^{|V(\alpha) \setminus (U_{\alpha} \cup V_{\alpha})|}}} \\
		&\leq \sum_{j_1,j_2,j_3,j_4 \in \mathbb{N} \cup \{0\}: j_1 + j_2 + j_3 + j_4 \geq 1}{\frac{1}{3^{j_1 + j_2}9^{j_4}2^{j_3}}} \leq 2\left(\frac{3}{2}\right)^2\frac{9}{8} - 1 < 5
	\end{align*}
\end{proof}
\begin{corollary}
	For all $\epsilon' > 0$, if we take 
	\[
	c(\alpha) = \frac{5(3D_V)^{|U_{\alpha} \setminus V_{\alpha}| + |V_{\alpha} \setminus U_{\alpha}| + 2|E(\alpha)|}2^{|V(\alpha) \setminus (U_{\alpha} \cup V_{\alpha})|}}{\epsilon'}
	\]
	then
	\begin{enumerate}
		\item $\forall U \in \mathcal{I}_{mid}, \sum_{\gamma \in \Gamma_{U,*}}{\frac{1}{|Aut(U)|c(\gamma)}} < \epsilon'$ 
		\item $\forall V \in \mathcal{I}_{mid}, \sum_{\gamma \in \Gamma_{*,V}}{\frac{1}{|Aut(U_{\gamma})|c(\gamma)}} < \epsilon'$ 
		\item $\forall U \in \mathcal{I}_{mid}, \sum_{\tau \in \mathcal{M}_{U}}{\frac{1}{|Aut(U)|c(\tau)}} < \epsilon'$
	\end{enumerate}
\end{corollary}
\subsubsection{Choosing $c(\alpha)$ in general*}
When we have multiple types of vertices and hyperedges of arity $k$, Lemma \ref{calphalemma} can be generalized as follows:
\begin{lemma}
	Under our simplifying assumptons, for all $U \in \mathcal{I}_{mid}$,
	\[
	\sum_{\alpha: U_{\alpha} \equiv U, \alpha \text{ is proper and non-trivial}}{\frac{1}{|Aut(U_{\alpha} \cap V_{\alpha})|(3D_V{t_{max}})^{|U_{\alpha} \setminus V_{\alpha}| + |V_{\alpha} \setminus U_{\alpha}| + k|E(\alpha)|}(2t_{max})^{|V(\alpha) \setminus (U_{\alpha} \cup V_{\alpha})|}}} < 5
	\]
\end{lemma}
\begin{proof}[Proof sketch]
	This can be proved in the same way as Lemma \ref{calphalemma} with the following modifications:
	\begin{enumerate}
		\item In addition to choosing the number of vertices in $U_{\alpha} \setminus V_{\alpha}$, $V_{\alpha} \setminus U_{\alpha}$, and $V(\alpha) \setminus (U_{\alpha} \cap V_{\alpha})$, we also have to choose the types of these vertices.
		\item For each hyperedge, we have to choose $k$ endpoints rather than $2$ endpoints.
	\end{enumerate}
\end{proof}

\begin{corollary}\label{cor: calphachoice}
	For all $\eps' > 0$, if we take
	\[c(\alpha) = \frac{5(3{t_{max}}D_V)^{|U_{\alpha} \setminus V_{\alpha}| + |V_{\alpha} \setminus U_{\alpha}| + k|E(\alpha)|}(2t_{max})^{|V(\alpha) \setminus (U_{\alpha} \cup V_{\alpha})|}}{\epsilon'}\]
	then
	\begin{enumerate}
		\item $\forall U \in \mathcal{I}_{mid}, \sum_{\gamma \in \Gamma_{U,*}}{\frac{1}{|Aut(U)|c(\gamma)}} < \epsilon'$ 
		\item $\forall V \in \mathcal{I}_{mid}, \sum_{\gamma \in \Gamma_{*,V}}{\frac{1}{|Aut(U_{\gamma})|c(\gamma)}} < \epsilon'$ 
		\item $\forall U \in \mathcal{I}_{mid}, \sum_{\tau \in \mathcal{M}_{U}}{\frac{1}{|Aut(U)|c(\tau)}} < \epsilon'$
	\end{enumerate}
\end{corollary}

For technical reasons, we will need a more refined bound when the sum is over all shapes $\gamma$ of at least a prescribed size.

\begin{lemma}\label{lem: tpca_refined_bound}
	For all $\eps' > 0$, for the same choice of $c(\al)$ as in $\cref{cor: calphachoice}$, for any $U \in \calI_{mid}$ and integer $m \ge 1$, we have \[\sum_{\gam \in \Gam_{U, *}: |V(\gam)| \ge |U| + m} \frac{1}{|Aut(U)|c(\gam)} \le \frac{\eps'}{5\cdot 2^{m - 1}}\]
\end{lemma}

\begin{proof}[Proof sketch]
	The proof is similar to the proof of \cref{cor: calphachoice}, but we now have the extra condition $j_2 + j_3 \ge m$ in the proof of \cref{calphalemma}. Then,
	\[\sum_{j_1, j_2, j_3, j_4 \in \NN\cup \{0\}: j_2 + j_3 \ge m} \frac{1}{3^{j_1 + j_2}9^{j_4}2^{j_3}} \le \sum_{j_1, j_4 \in \NN\cup \{0\}} \frac{1}{2^m3^{j_1}9^{j_4}} = \frac{27}{16\cdot 2^m}\le \frac{1}{2^{m - 1}}\]
\end{proof}

\subsection{Proof of the Generalized Intersection Tradeoff Lemma}
We now prove the generalized intersection tradeoff lemma.
\begin{lemma}
	For all $\gamma, \tau, \gamma'$ and all intersection patterns $P \in \mathcal{P}_{\gamma,\tau,\gamma'}$, 
	\[
	w(V(\tau_P)) + w(I_{\tau_P}) - w(S_{\tau_P,min}) \leq w(V(\tau)) + w(I_{\tau}) - w(S_{\tau,min})+ w(V(\gamma) \setminus U_{\gamma}) + w(V(\gamma') \setminus U_{\gamma'})
	\]
\end{lemma}
\begin{proof}
	\begin{definition} \ 
		\begin{enumerate}
			\item We define $I_{LM}$ to be the set of vertices which, after intersections, touch $\gamma$ and $\tau$ but not ${\gamma'}^T$. In particular, $I_{LM}$ consists of the vertices which result from intersecting a pair of vertices in $V(\gamma) \setminus V_{\gamma}$ and $V(\tau) \setminus U_{\tau} \setminus V_{\tau}$ and the vertices which are in $U_{\tau} \setminus V_{\tau}$ and are not intersected with any other vertex.
			\item We define $I_{MR}$ to be the set of vertices which, after intersections, touch $\tau$ and ${\gamma'}^T$ but not $\gamma$. In particular, $I_{MR}$ consists of the vertices which result from intersecting a pair of vertices in $V(\tau) \setminus U_{\tau} \setminus V_{\tau}$ and $V({\gamma'}^T) \setminus U_{{\gamma'}^T}$ and the vertices which are in $V_{\tau} \setminus U_{\tau}$ and are not intersected with any other vertex.
			\item We define $I_{LR}$ to be the set of vertices which, after intersections, touch $\gamma$ and ${\gamma'}^T$ but not $\tau$. In particular, $I_{LR}$ consists of the vertices which result from intersecting a pair of vertices in $V(\gamma) \setminus V_{\gamma}$ and $V({\gamma'}^T) \setminus U_{{\gamma'}^T}$.
			\item We define $I_{LMR}$ to be the set of vertices which, after intersections, touch $\gamma$, $\tau$, and ${\gamma'}^T$. In particular, $I_{LMR}$ consists of the vertices which result from intersecting a triple of vertices in $V(\gamma) \setminus V_{\gamma}$,  $V(\tau) \setminus U_{\tau} \setminus V_{\tau}$, and $V({\gamma'}^T) \setminus U_{{\gamma'}^T}$, intersecting a pair of vertices in $V(\gamma) \setminus V_{\gamma}$ and $V_{\tau} \setminus U_{\tau}$, intersecting a pair of vertices in $U_{\tau} \setminus V_{\tau}$ and $V({\gamma'}^T) \setminus U_{{\gamma'}^T}$, and single vertices in $U_{\tau} \cap V_{\tau}$. 
		\end{enumerate}
	\end{definition}
	The main idea is as follows. A priori, any of the vertices in $I_{LM} \cup I_{MR} \cup I_{LR} \cup I_{LMR}$ could become isolated. We handle this by keeping track of the following types of flows:
	\begin{enumerate}
		\item Flows from $U_{\gamma}$ to $I_{LM} \cup I_{LR} \cup I_{LMR}$
		\item Flows from $I_{LR} \cup I_{MR} \cup I_{LMR}$ to $V_{{\gamma'}^T}$
		\item Flows from $I_{LM}$ to $I_{MR}$. For technical reasons, we also view vertices in $I_{LMR}$ as having flow to themselves.
	\end{enumerate}
	We then observe that flows to and from these vertices prevent these vertices from being isolated and can provide flow from $U_{\gamma}$ to $V_{{\gamma'}^T}$, which gives a lower bound on $w(S_{\tau_P})$.
	
	We now implement this idea.
	\begin{definition}[Flow Graph]
		Given a shape $\alpha$, we define the directed graph $H_{\alpha}$ as follows:
		\begin{enumerate}
			\item For each vertex $v \in V(\alpha)$, we create two vertices $v_{in}$ and $v_{out}$. We then create a directed edge from $v_{in}$ to $v_{out}$ with capacity $w(v)$
			\item For each pair of vertices $(v,w)$ which is an edge of multiplicity $1$ in $E(\alpha)$ (or part of a hyperedge of multiplicity $1$ in $E(\alpha)$), we create a directed edge with infinite capacity from $v_{out}$ to $w_{in}$ and we create a directed edge with infinite capacity from $w_{out}$ to $v_{in}$.
			\item We define $U_{H_{\alpha}}$ to be $U_{H_{\alpha}} = \{u_{in}: u \in U_{\alpha}\}$ and we define $V_{H_{\alpha}}$ to be $V_{H_{\alpha}} = \{v_{out}: v \in V_{\alpha}\}$
		\end{enumerate}
	\end{definition}
	\begin{lemma}
		The maximum flow from $U_{H_{\alpha}}$ to $V_{H_{\alpha}}$ is equal to the minimum weight of a separator between $U_{\alpha}$ and $V_{\alpha}$.
	\end{lemma}
	\begin{proof}
		This can be proved using the max flow min cut theorem.
	\end{proof}
	\begin{definition}[Modified Flow Graph]
		Given a shape $\alpha$ together with a set $I_L \subseteq V(\alpha)$ of vertices in $\alpha$ (which will be the vertices in $\alpha$ which are intersected with a vertex to the left of $\alpha$) and a set $I_R \subseteq V(\alpha)$ of vertices in $\alpha$ (which will be the vertices in $\alpha$ which are intersected with a vertex to the right of $\alpha$), we define the modified flow graph $H^{I_L,I_R}_{\alpha}$ as follows:
		\begin{enumerate}
			\item We start with the flow graph $H_{\alpha}$
			\item For each vertex $u \in I_L$, we delete all of the edges into $u_{in}$ and add $u_{in}$ to $U_{H_{\alpha}}$
			\item For each vertex $v \in I_R$, we delete all of the edges out of $v_{out}$ and add $v_{out}$ to $V_{H_{\alpha}}$
			\item We call the resulting graph $H^{I_L,I_R}_{\alpha}$ and the resulting sets $U_{H^{I_L,I_R}_{\alpha}}$ and $V_{H^{I_L,I_R}_{\alpha}}$
		\end{enumerate}
	\end{definition}
	\begin{lemma}\label{increasedflowlemma}
		The maximum flow from $U_{H^{I_L,I_R}_{\alpha}}$ to $V_{H^{I_L,I_R}_{\alpha}}$ in $H^{I_L,I_R}_{\alpha}$ is at least as large as the maximum flow from $U_{H_{\alpha}}$ to $V_{H_{\alpha}}$ in $H_{\alpha}$
	\end{lemma}
	\begin{proof}[Proof sketch]
		Observe that if we have a cut $C$ in $H^{I_L,I_R}_{\alpha}$ which separates $U_{H^{I_L,I_R}_{\alpha}}$ and $V_{H^{I_L,I_R}_{\alpha}}$ then $C$ separates $U_{H_{\alpha}}$ and $V_{H_{\alpha}}$ in $H_{\alpha}$
	\end{proof}
	Before the intersections, we have the following flows.
	\begin{enumerate}
		\item We take $F_1$ to be the maximum flow from $U_{\gamma}$ to $V_{\gamma}$ in $\gamma$. Note that $F_1$ has value $w(V_{\gamma})$
		\item We take $F_2$ to be the maximum flow from $U_{\tau}$ to $V_{\tau}$ in $\tau$. Note that $F_2$ has value $w(S_{\tau,min})$
		\item We take $F_3$ to be the maximum flow from $U_{{\gamma'}^T}$ to $V_{{\gamma'}^T}$ in ${\gamma'}^T$. Note that $F_1$ has value $w(U_{{\gamma'}^T})$
	\end{enumerate}
	After the intersections, we take the following flows:
	\begin{enumerate}
		\item We take $F'_1$ to be the maximum flow from $U_{H^{\emptyset,I_{LM} \cup I_{LR} \cup I_{LMR}}_{\gamma}}$ to $V_{H^{\emptyset,I_{LM} \cup I_{LR} \cup I_{LMR}}_{\gamma}}$ in \\
		$H^{\emptyset,I_{LM} \cup I_{LR} \cup I_{LMR}}_{\gamma}$.
		\item We take $F'_2$ to be the maximum flow from $U_{H^{I_{LM} \cup I_{LMR},I_{MR} \cup I_{LMR}}_{\tau}}$ to $V_{H^{I_{LM} \cup I_{LMR},I_{MR} \cup I_{LMR}}_{\tau}}$ in \\
		$H^{I_{LM} \cup I_{LMR},I_{MR} \cup I_{LMR}}_{\tau}$
		\item We take $F'_3$ to be the maximum flow from $U_{H^{I_{MR} \cup I_{LR} \cup I_{LMR},\emptyset}_{{\gamma'}^T}}$ to $V_{H^{I_{MR} \cup I_{LR} \cup I_{LMR},\emptyset}_{{\gamma'}^T}}$ in \\
		$H^{I_{MR} \cup I_{LR} \cup I_{LMR},\emptyset}_{{\gamma'}^T}$.
	\end{enumerate}
	Observe that because of how intersection patterns are defined, $val(F'_1) = w(U_{\gamma})$ and $val(F'_3) = w(V_{{\gamma'}^T})$. By Lemma \ref{increasedflowlemma}, the value of $F'_2$ is at least as large as the value of $F_2$, so $val(F'_2) \geq w(S_{\tau,min})$.
	
	We now consider $F'_1 + F'_2 + F'_3$. As is, this is not a flow, but we can fix this.
	\begin{definition}
		For each vertex $v \in V(\tau_P)$,
		\begin{enumerate}
			\item We define $f_{in}(v)$ to be the flow into $v_{in}$ in $F'_1 + F'_2 + F'_3$.
			\item We define $f_{out}(v)$ to be the flow out of $v_{out}$ in $F'_1 + F'_2 + F'_3$.
			\item We define $f_{through}(v)$ to be the flow from $v_{in}$ to $v_{out}$ in $F'_1 + F'_2 + F'_3$
			\item We define $f_{imbalance}(v)$ to be $f_{imbalance}(v) = |f_{in}(v) - f_{out}(v)|$
			\item We define $f_{excess}(v)$ to be $f_{excess}(v) = f_{through}(v) - max{\{f_{in}(v),f_{out}(v)\}}$
		\end{enumerate}
		With this information, we fix the flow $F'_1 + F'_2 + F'_3$ as follows. For each vertex $v \in V(\tau_P)$, 
		\begin{enumerate}
			\item If $f_{in}(v) > f_{out}(v)$ then we create a vertex $v_{supplemental,out}$ and an edge from $v_{out}$ to $v_{supplemental,out}$ with capacity $f_{imbalance}(v)$ and we route $f_{imbalance}(v)$ of flow along this edge. We then add $v_{supplemental,out}$ to a set of vertices $V_{supplemental}$.
			\item If $f_{in}(v) < f_{out}(v)$ then we create a vertex $v_{supplemental,in}$ and an edge from $v_{supplemental,in}$ to $v_{in}$ with capacity $f_{imbalance}(v)$ and we route $f_{imbalance}(v)$ of flow along this edge. We then add $v_{supplemental,out}$ to a set of vertices $V_{supplemental}$.
			\item We reduce the flow on the edge from $v_{in}$ to $v_{out}$ by $f_{excess}(v)$
		\end{enumerate}
		We call the resulting flow $F'$
	\end{definition}
	\begin{proposition}
		$F'$ is a flow from  $U_{H^{\emptyset,I_{LM} \cup I_{LR} \cup I_{LMR}}_{\gamma}} \cup U_{supplemental}$ to $V_{H^{I_{MR} \cup I_{LR} \cup I_{LMR},\emptyset}_{{\gamma'}^T}} \cup V_{supplemental}$ with value $val(F') = val(F'_1) + val(F'_2) + val(F'_3) - \sum_{v \in V(\tau)}{f_{excess}(v)}$
	\end{proposition}
	\begin{corollary}\label{fixedflowcorollary}
		There exists a flow $F''$ from $U_{H^{\emptyset,I_{LM} \cup I_{LR} \cup I_{LMR}}_{\gamma}}$ to $V_{H^{I_{MR} \cup I_{LR} \cup I_{LMR},\emptyset}_{{\gamma'}^T}}$ with value $val(F'') \geq val(F'_1) + val(F'_2) + val(F'_3) - \sum_{v \in V(\tau)}{(f_{excess}(v) + f_{imbalance}(v))}$
	\end{corollary}
	\begin{proof}
		Consider the minimum cut $C$ between $U_{H^{\emptyset,I_{LM} \cup I_{LR} \cup I_{LMR}}_{\gamma}}$ and $V_{H^{I_{MR} \cup I_{LR} \cup I_{LMR},\emptyset}_{{\gamma'}^T}}$. If we add all of the supplemental edges to $C$ then this gives a cut $C'$ between $U_{H^{\emptyset,I_{LM} \cup I_{LR} \cup I_{LMR}}_{\gamma}}$ and $V_{H^{I_{MR} \cup I_{LR} \cup I_{LMR},\emptyset}_{{\gamma'}^T}}$ with capacity 
		\[
		capacity(C') = capacity(C) + \sum_{v \in V(\tau)}{f_{imbalance}(v)} \geq val(F')
		\]
		Thus, $capacity(C) \geq val(F') - \sum_{v \in V(\tau)}{f_{imbalance}(v)}$ so there exists a flow $F''$ from $U_{H^{\emptyset,I_{LM} \cup I_{LR} \cup I_{LMR}}_{\gamma}}$ to $V_{H^{I_{MR} \cup I_{LR} \cup I_{LMR},\emptyset}_{{\gamma'}^T}}$ with value 
		\[
		val(F'') = capacity(C) \geq val(F'_1) + val(F'_2) + val(F'_3) - \sum_{v \in V(\tau)}{(f_{excess}(v) + f_{imbalance}(v))}
		\]
	\end{proof}
	We now make the following observations:
	\begin{lemma} \ 
		\begin{enumerate}
			\item For all vertices $v \notin I_{LM} \cup I_{MR} \cup I_{LR} \cup I_{LMR}$, $f_{excess}(v) = f_{imbalance}(v) = 0$ (and these vertices can never be isolated).
			\item For all vertices $v \in I_{LM}$, $f_{excess}(v) + f_{imbalance}(v) \leq w(v)$. Moreover, for all vertices $v \in I_{LM}$ which are isolated, $f_{excess}(v) = f_{imbalance}(v) = 0$.
			\item For all vertices $v \in I_{MR}$, $f_{excess}(v) + f_{imbalance}(v) \leq w(v)$. Moreover, for all vertices $v \in I_{LM}$ which are isolated, $f_{excess}(v) = f_{imbalance}(v) = 0$.
			\item For all vertices $v \in I_{LR}$, $f_{excess}(v) + f_{imbalance}(v) \leq w(v)$. Moreover, for all vertices $v \in I_{LM}$ which are isolated, $f_{excess}(v) = f_{imbalance}(v) = 0$.
			\item For all vertices $v \in I_{LMR}$, $f_{excess}(v) + f_{imbalance}(v) \leq 2w(v)$. Moreover, for all vertices $v \in I_{LMR}$ which are isolated, $f_{excess}(v) = w(v)$ and $f_{imbalance}(v) = 0$.
		\end{enumerate}
	\end{lemma}
	\begin{proof}
		For the first statement, observe that for vertices $v \notin I_{LM} \cup I_{MR} \cup I_{LR} \cup I_{LMR}$, neither $v_{in}$ nor $v_{out}$ is ever a sink or source so the flow into these vertices must equal the flow out of these vertices and thus $f_{in}(v) = f_{out}(v) = f_{through}(v)$.
		
		For the second statement, observe that for a vertex $v \in I_{LM}$, 
		\begin{enumerate}
			\item $F'_1$ will have a flow of $f_{in}(v)$ into $v_{in}$ and along the edge from $v_{in}$ to $v_{out}$ 
			\item $F'_2$ will have a flow of $f_{out}(v)$ along the edge from $v_{in}$ to $v_{out}$ and out of $v_{out}$.
		\end{enumerate}
		Thus, $f_{excess}(v) = f_{in}(v) + f_{out}(v) - \max\{f_{in}(v),f_{out}(v)\}$. Since $f_{imbalance}(v) = |f_{in}(v) - f_{out}(v)|$, 
		$f_{excess}(v) + f_{imbalance}(v) = f_{in}(v) + f_{out}(v) - \min\{f_{in}(v),f_{out}(v)\} \leq w(v)$.
		
		If $v$ is isolated then neither $F'_1$ nor $F'_2$ can have any flow to $v_{in}$ or out of $v_{out}$ so $f_{in}(v) = f_{through}(v) = f_{out}(v) = 0$
		
		The third and fourth statements can be proved in the same way as the second statement.
		
		For the fifth statement, observe that for a vertex $v \in I_{LMR}$, 
		\begin{enumerate}
			\item $F'_1$ will have a flow of $f_{in}(v)$ into $v_{in}$ and along the edge from $v_{in}$ to $v_{out}$.
			\item $F'_2$ will have a flow of $w(v)$ along the edge from $v_{in}$ to $v_{out}$
			\item $F'_3$ will have a flow of $f_{out}(v)$ along the edge from $v_{in}$ to $v_{out}$ and out of $v_{out}$.
		\end{enumerate}
		Thus, $f_{excess}(v) = w(v) + f_{in}(v) + f_{out}(v) - \max\{f_{in}(v),f_{out}(v)\}$. Since $f_{imbalance}(v) = |f_{in}(v) - f_{out}(v)|$, 
		$f_{excess}(v) + f_{imbalance}(v) = w(v) + f_{in}(v) + f_{out}(v) - \min\{f_{in}(v),f_{out}(v)\} \leq 2w(v)$.
		
		If $v$ is isolated then neither $F'_1$ nor $F'_3$ can have any flow to $v_{in}$ or out of $v_{out}$ so $f_{in}(v) = f_{out}(v) = 0$ and $f_{through}(v) = w(v)$.
	\end{proof}
	Putting everything together, we have the following corollary:
	\begin{corollary} \ 
		\[
		\sum_{v \in V(\tau_P)}{(f_{excess}(v) + f_{imbalance}(v))} \leq w(I_{LM}) + w(I_{LR}) + w(I_{MR}) + 2w(I_{LMR}) - (w(I_{\tau_P}) - w(I_{\tau}))
		\]
	\end{corollary}
	Combining this with Corollary \ref{fixedflowcorollary},
	\begin{align*}
		w(S_{\tau_P,min}) &\geq val(F'_1) + val(F'_2) + val(F'_3) - \sum_{v \in V(\tau_P)}{(f_{excess}(v) + f_{imbalance}(v))}\\
		&\geq w(U_{\gamma}) + w(S_{\tau,min}) + w(V_{{\gamma'}^T}) - w(I_{LM}) - w(I_{LR}) - w(I_{MR}) - 2w(I_{LMR}) + (w(I_{\tau_P}) - w(I_{\tau}))
	\end{align*}
	Since $w(V(\tau_P)) = w(V(\tau)) + w(V(\gamma)) + w(V(\gamma')) - w(I_{LM}) - w(I_{LR}) - w(I_{MR}) - 2w(I_{LMR})$, 
	\[
	w(S_{\tau_P,min}) \geq w(U_{\gamma}) + w(S_{\tau,min}) + w(V_{{\gamma'}^T}) + w(V(\tau_P)) - w(V(\tau)) - w(V(\gamma)) - w(V(\gamma')) + (w(I_{\tau_P}) - w(I_{\tau}))
	\]
	Rearranging this gives 
	\[
	w(V(\tau_P)) - w(S_{\tau_P,min}) + w(I_{\tau_P}) \leq w(V(\tau)) - w(S_{\tau,min}) + w(I_{\tau}) + w(V(\gamma) \setminus U_{\gamma}) + w(V(\gamma') \setminus U_{\gamma'})
	\]
	which is the generalized intersection tradeoff lemma.
\end{proof}


==> machinery/informal_statement.tex <==
In this section, we informally describe our machinery for proving sum of squares lower bounds on planted problems. Our goal for this section is to qualitatively state the conditions under which we can show that the moment matrix $\Lambda$ is PSD with high probability (see \cref{informalmaintheoremstatement}). For simplicity, in this section we restrict ourselves to the setting where the input is $\{-1,1\}^{\binom{n}{2}}$ (i.e. a random graph on $n$ vertices). We also defer the proofs of several important facts until \cref{sec: technical_def_and_main_theorem}. In \cref{sec: technical_def_and_main_theorem}, we give the general definitions, fill in the missing proofs, and give the full, quantitative statement of our main result (see \cref{generalmaintheorem}).

%In general, the moment matrix $\Lda$ usually constructed via pseudo-calibration is quite complicated and proving PSDness is a significant challenge. However, one key property of $\Lambda$ is that it is symmetric. 

% The goal of our machinery is to give conditions 
% on matrices $\Lambda$ which are sufficient for  
%In this section and those which follow, we study symmetric matrix-valued functions on subset-indexed product spaces which are \emph{almost positive semidefinite}.
%To warm up, here is a special case of the setting we study. Let $n,d,k \in \N$. We consider functions $\Lambda \, : \, \{\pm 1\}^{{n \choose k}} \rightarrow \R^{{n \choose d} \times {n \choose d}}$ which map the product space $\{\pm 1\}^{n \choose k}$ to real symmetric matrices.

%Notice that $\{\pm 1\}^{n \choose k}$ is indexed by \emph{subsets} of $[n]$, and $\R^{{n \choose d} \times {n \choose d}}$ is indexed by pairs of subsets of $[n]$.
%The permutation group $S_n$ has a natural action on both $\{\pm 1\}^{n \choose k}$ and $\R^{{n \choose d} \times {n \choose d}}$, and hence also it acts on $\Lambda$: suppose that $\Lambda$ is invariant under this action.
%That is, for every $\pi \in S_n$ it holds that $\pi \cdot \Lambda = \Lambda$.
%For instance, if $k=2$ and $d=1$, the function $\Lambda(x) = x + \Id$ is such a function, where $\Id$ is the $d \times d$ identity matrix.

%Symmetric functions $\Lambda$ of this type arise as the main players in the construction of SoS lower bounds for planted problems, where the goal is often to show that $\Lambda$ is positive semi-definite with high probability:
%\begin{align}\label{eq:goal}
%	\Lambda(x) \succeq 0 \text{ with probability at least } 1 - \littleoh(1) \text{ when } x \sim \{\pm 1\}^{n \choose k} \text{ uniformly.}
%\end{align}
%For instance, if $k = 2$, then $x \sim \{ \pm 1\}^{n \choose 2}$ chosen uniformly at random is in fact a sample from $G(n,\frac{1}{2})$; this recovers settings in which one might study optimization problems over random graphs, such as the planted clique problem.
%In the example case $k=2,d=1$, if $\Lambda(x) = x + 10\sqrt{n} \cdot \Id$ then \eqref{eq:goal} holds for $\Lambda$, since with high probability the $n \times n$ random matrix $x$ has spectral norm at most $2\sqrt{n}$.
%When $k > 2$, the space $\{ \pm 1\}^{n \choose k}$ is the set of $k$-tensors with $\pm 1$ entries, which puts us in the setting of our SoS lower bound for tensor principal component analysis.

%Our main result in this section is a sufficient condition on $\Lambda$ for \eqref{eq:goal} to hold.
%Together with the pseudo-calibration method (which supplies the function $\Lambda$ we employ to prove SoS lower bounds for planted problems), this condition suffices to prove our exponential lower bounds for component analysis problems.

%\paragraph{Setup overview}
%The sufficient condition we describe is Fourier-theoretic: that is, it concerns the pattern of decay in the coefficients of a Fourier expansion of $\Lambda$.
%Stating this condition, and hence our main theorem, requires some setup, as we have to establish enough definitions to do Fourier analysis on $S_n$-symmetric matrix-valued subset-indexed functions $\Lambda$.
%Our first task is to describe an explicit orthonormal basis for the set of functions $\{ \Lambda \, : \, \{ \pm 1\}^{n \choose k} \rightarrow \R^{{n \choose d} \times {n \choose d}} \, S_n \text{-symmetric} \}$.
%We establish a description of these basis functions in terms of combinatorial objects we call \emph{ribbons} and \emph{shapes} -- this will ultimately allow us to turn Fourier-theoretic statements into combinatorial ones, a connection which will be quite useful in our proofs.

%The basis functions we construct are of course themselves maps $M \, : \, \{ \pm 1\}^{n \choose k} \rightarrow \R^{{n \choose d} \times {n \choose d}}$.
%The basis functions have a factorization structure: that is, some basis functions $M_\alpha$ can be (approximately) factored into a product of two (or more) other basis functions: $M_\alpha(x) \approx M_\beta(x) M_\gamma(x)$, where we emphasize that $M_\beta(x) M_\gamma(x)$ are multiplied \emph{as matrices in $\R^{{n \choose d} \times {n \choose d}}$.}
%To state our main theorem we have to describe some basics of this factorization structure.

%\paragraph{Organization}
%We will give definitions and theorem statements in two rounds.
%As warm-ups, in the remainder of this section we offer definitions and a theorem statement which are simplified in two ways with respect to our main theorem: they concern just the case that the underlying product space is $\{ \pm 1\}^{n \choose 2}$, and they leave out some of the quantitative bounds necessary to apply the main theorem and prove SoS lower bounds.
%In the following section we make more general definitions and state our main theorem.
%The subsequent sections prove the main theorem.


%\paragraph{On generality}
%Since we will not be able to make a full statement of our main theorem until after some setup, we describe a couple features of the general setting which we have avoided in the special case considered so far.

%The challenges presented by these generalizations are primarily technical and definitional\gnote{Seems to downplay the machinery?}; the general setting is required, however, to obtain a theorem which can be used for SoS lower bounds outside Boolean settings and for less symmetric problems.

%First of all, we do not require that the underlying product space is $\{ \pm 1\}^{n \choose k}$.
%Instead, under mild conditions on a set $\Omega$ and a measure $\mu$ on it, our theorem applies to $\Lambda$ defined on $\Omega^{n \choose k}$.
%For instance, $\Omega = \R$ and $\mu = \cN(0,1)$ is another common setting.
%Second, if $n_1,\ldots,n_k \in \N$, our theorem applies also if the underlying product space is not indexed by subsets of $[n]$ but rather by tuples in $[n_1] \times [n_2] \times \ldots [n_k]$.
%In the example case $k=2$, this allows $\Omega^{n_1 \times n_2}$ to be the set of rectangular matrices with entries in $\Omega$.
%Then the required symmetry group of $\Lambda$ is $S_{n_1} \times \ldots \times S_{n_k}$ rather than $S_n$.

%Finally, we note that as far as we are aware simpler approaches to Fourier analysis of $\Lambda \, : \, \{ \pm 1\}^{n \choose k} \rightarrow \R^{{n \choose d} \times {n \choose d}}$ than we follow here do not suffice to prove results like our main theorem.
%It is tempting, for instance, to do more traditional Fourier analysis of scalar-valued functions on each entry of $\Lambda$.
%Unfortunately, this approach seems not to adequately take advantage of the matrix structure of $\Lambda$, and hence we suspect it cannot be used to prove spectral statements like $\Lambda(x) \succeq 0$.
% The goal of this section and the following two sections is to generalize the technical machinery used to prove the SOS lower bound for planted clique so that it can be used to prove SOS lower bounds on other planted problems. As the reader might imagine, this is very technical and many definitions are needed before we can even state our theorem. In this section, we describe our definitions and our result informally so that we can transmit the high level ideas without getting bogged down in the technical details.

% For this section, we assume that our input is a random $G(n,\frac{1}{2})$ graph, which is the case for planted clique and the variant of sparse PCA which we consider in this paper. In the next section, we will make our definitions more precise and generalize them to handle other possible random inputs.

\subsection{Fourier analysis for matrix-valued functions: ribbons, shapes, and graph matrices}
For our machinery, we need the definitions of ribbons, shapes, and graph matrices from \cite{AMP20}.

%In this section we construct an explicit orthonormal basis for $\{ \Lambda \, : \, \{ \pm 1\}^{n \choose 2} \rightarrow \R^{{\frac{n!}{(n - \frac{d}{2})!}} \times \frac{n!}{(n - \frac{d}{2})!}} \, S_n\text{-symmetric} \}$.

\subsubsection{Ribbons}
\emph{Ribbons} lift the usual Fourier basis for functions $\{ f \, : \, \{ \pm 1\}^{n \choose 2} \rightarrow \R \}$ to  matrix-valued functions.

%Because $\{ \pm 1\}^{n \choose 2}$ is (isomorphic to) the set of graphs on $n$ vertices, we denote its elements by $G$.
%Also, since ${n \choose d}$ is (isomorphic to) the set of multilinear monomials of degree $d$ in variables $x_1,\ldots,x_n$, we interchangebly consider $\Lambda$ to be indexed by $A \subseteq [n]$ or by monomials $x^A = \prod_{i \in A} x_i$.


% SAM: commented this out because same ground is now covered in introduction
% ------------------
%To prove our SOS lower bounds, we need to analyze a matrix $\Lambda$ which has the following properties:
%\begin{enumerate}
%\item The rows and columns of $\Lambda$ are indexed by multilinear monomials.
%\item The entries of $\Lambda$ are a function of a random $G(n,\frac{1}{2})$ graph.
%\end{enumerate}
%To analyze $\Lambda$, we use Fourier analysis on its entries. For this, our fundamental building block is a ribbon, which describes a Fourier character together with row and column indices.

%We start by recalling the usual Fourier characters for functions on the hypercube.
%\begin{definition}
%	For $n \in \N$ and $E \subseteq {n \choose 2}$, let $\chi_E \, : \, \{ \pm 1\}^{n \choose 2} \rightarrow \R$ be given by $\chi_E(G) = \prod_{(i,j) \in E} G_{ij}$.
%\end{definition}
%The functions $\{ \chi_E \}_{E \subseteq {n \choose 2}}$ form an orthonormal basis for $\{ f \, : \,\{ \pm 1\}^{n \choose 2} \rightarrow \R \}$ with respect to the uniform distribution on $\{ \pm 1\}^{n \choose 2}$ -- see e.g. \cite{odonnell-book}.

\begin{definition}[Simplified ribbons -- see \cref{def: ribbons}]
	Let $n \in \N$.
	A ribbon $R$ is a tuple $(E_R,A_R,B_R)$ where $E_R \subseteq {[n] \choose 2}$ and $A_R,B_R$ are tuples of elements in $[n]$.
%	To distinguish the components of one ribbon from those of another, we often write $E = E(R)$ and $A = A_R, B = B_R$.
	$R$ thus specifies:
	\begin{enumerate}
		\item A Fourier character $\chi_{E_R}$.
		\item Row and column indices $A_R$ and $B_R$.
	\end{enumerate}
	We think of $R$ as a graph with vertices
	\[
	V(R) = \{ \text{ endpoints of $(i,j) \in E_R$ } \} \cup A_R \cup B_R
	\]
	and edges $E(R) = E_R$, where $A_R, B_R$ are distinguished tuples of vertices.
\end{definition}

\begin{definition}[Matrix-valued function for a ribbon $R$]
	Given a ribbon $R$, we define the matrix valued function $M_R \, : \, \{ \pm 1\}^{n \choose 2} \rightarrow \R^{\frac{n!}{(n - |A_R|)!} \times \frac{n!}{(n - |B_R|)!}}$ to have entries $M_R(A_R,B_R) = \chi_{E_R}$ and $M_R(A',B') = 0$ whenever $A' \neq A_R$ or $B' \neq B_R$.
	%Notice that if $|A_R|$ or $|B_R|$ is not equal to $d$, the function $M_R$ assumes values in matrices of dimensions other than ${n \choose d} \times {n \choose d}$.
	%We will need to work with matrices of dimensions ${n \choose {d'}} \times {n \choose {d''}}$ because they will appear in factorizations of ${n \choose d} \times {n \choose d}$ matrices.
\end{definition}

The following proposition captures the main property of the matrix-valued functions $M_R$ -- they are an orthonormal basis. We leave the proof to the reader.
\begin{proposition}
	The matrix-valued functions $M_R$ form an orthonormal basis for the vector space of matrix valued functions with respect to the inner product 
	\[
	\iprod{M,M'} = \E_{G \sim \{ \pm 1\}^{n \choose 2} }\left[\Tr \left(M(G) (M'(G))^\top\right)\right].
	\]
\end{proposition}

We don't directly utilize this proposition in our work but this gives insight on to the structure of the matrix valued functions we define and motivates the definition of graph matrices, that we use extensively.

%\gnote{Do we need the above proposition? The beginning of the next section talks about it}

\begin{example}
    In \cref{fig: ribbon_shape}, consider the ribbon $R$ as shown. We have $A_R = (1, 3), B_R = (4), V(R) = \{1, 2, 3, 4\}, E_R = \{\{1, 2\}, \{3, 2\}, \{2, 4\}\}$. The Fourier character is $\chi_{E_R} = \chi_{1, 2}\chi_{3, 2}\chi_{2, 4}$. And finally, $M_R$ is a matrix with rows and columns indexed by tuples of length $|A_R| = 2$ and $|B_R| = 1$ respectively, with exactly one nonzero entry $M_R((1, 3), (4)) = \chi_{E_R}$. Succinctly, \[M_R =
%     \begin{blockarray}{c@{\hspace{5pt}}rr@{\hspace{5pt}}cl}
%     & \matindex{1} & \matindex{2} & & \\
%     \begin{block}{(c@{\hspace{5pt}}rr@{\hspace{5pt}}c)l}
%       & 100 &  b & & \matindex{row 1} \\
%       &   2 & 12 & & \matindex{row 2} \\
%       &   e &  f & & \matindex{ABDC} \\
%     \end{block}
%   \end{blockarray}$.
  \begin{blockarray}{rl@{}c@{}r}
    & & \makebox[0pt]{column $(4)$} \\[-0.5ex]
    & & \,\downarrow \\[-0.5ex]
    \begin{block}{r(l@{}c@{}r)}
    & \makebox[3.1em]{\Large $0$\bigstrut[t]} & \vdots &\makebox[4.2em]{\Large $0$} \\[-0.2ex]
    \text{row }(1, 3) \to \mkern-9mu & \raisebox{0.5ex}{\makebox[3.2em][l]{\dotfill}} & \chi_{1, 2}\chi_{3, 2}\chi_{2, 4} & \raisebox{0.5ex}{\makebox[4.2em][r]{\dotfill}} \\[+0ex]
    & \makebox[3.1em]{\Large $0$} & \vdots &\makebox[4.2em]{\bigstrut\Large $0$} \\
    \end{block}
  \end{blockarray}\]
\end{example}

\begin{figure}[!h]
    \centering
    \includegraphics[scale=.6, trim={0 5cm 2 5cm},clip]{machinery/images/ribbon_shape}
    \caption{Example of a ribbon and a shape}
    \label{fig: ribbon_shape}
\end{figure}


\subsubsection{Shapes and Graph Matrices}
As described above, \emph{ribbons} are an orthonormal basis for matrix-valued functions. However, we will need an orthogonal basis for the subset of those functions which are symmetric with respect to the action of $S_n$. For this, we use \emph{graph matrices}, which are described by \emph{shapes}. The idea is that each ribbon $R$ has a shape $\alpha$ which is obtained by replacing the vertices of $R$ with unspecified indices. Up to scaling, the graph matrix $M_{\alpha}$ is the average of $M_{\pi(R)}$ over all permutations $\pi \in S_n$.

%We will obtain such a basis by projecting the $M_R$ functions to the span of the symmetric functions; this just requires averaging each $M_R$ over its orbit under $S_n$ (then checking that the projected functions are still orthonormal, once we remove duplicates). As with ribbons, we will make use of a combinatorial description of the resulting matrix-valued functions; we call the combinatorial objects we use \emph{shapes}.

% We assume that the matrix $\Lambda$ we are analyzing is symmetric (as a function of the input) under permutations of $[1,n]$. We take advantage of this symmetry by grouping ribbons which are in the same orbit under permutations of $[1,n]$ together. 

\begin{definition}[Simplified shapes -- see \cref{def: shapes}]
	Informally, a shape $\alpha$ is just a ribbon $R$ where the vertices are specified by variables rather than having specific values in $[n]$. More precisely, a shape $\alpha = (V(\alpha),E(\alpha),U_{\alpha},V_{\alpha})$ is a graph on vertices $V(\alpha)$, with
	\begin{enumerate}
		\item Edges $E(\alpha) \subseteq {{V(\alpha)} \choose 2}$
		\item Distinguished tuples of vertices $U_\alpha = (u_1,u_2,\dots)$ and $V_\alpha = (v_1,v_2,\dots)$, where $u_i,v_i \in V(\alpha)$.
	\end{enumerate}
	(Note that $V(\alpha)$ and $V_\alpha$ are not the same object!)
\end{definition}

\begin{definition}[Shape transposes]
	Given a shape $\alpha$, we define $\alpha^{\top}$ to be the shape $\alpha$ with $U_{\alpha}$ and $V_{\alpha}$ swapped i.e. $U_{\sigma^{\top}} = V_{\sigma}$ and $V_{\sigma^{\top}} = U_{\sigma}$.
	Note that $M_{\alpha^{\top}} = M_\alpha^{\top}$, where $M_\alpha^{\top}$ is the usual transpose of the matrix-valued function $M_\alpha$.
\end{definition}
%Now we can define our basis functions, called \emph{graph matrices}, for the symmetric matrix-valued functions, by projecting the functions $M_R$.

\begin{definition}[Graph matrices]
	Let $\alpha$ be a shape.
	The graph matrix $M_{\alpha} \, : \, \{ \pm 1\}^{n \choose 2} \rightarrow \R^{\frac{n!}{(n - |U_{\alpha}|)!} \times \frac{n!}{(n - |V_{\alpha}|)!}}$ is defined to be the matrix-valued function with $A,B$-th entry
	\[
	M_{\alpha}(A,B) = \sum_{\substack{R \text{ s.t. } A_R = A, B_R = B \\ \exists \phi:V(\alpha) \to [n]: \\ \phi \text{ is injective}, \phi(\alpha) = R}}{\chi_{E_R}}
	\]
	In other words, $M_\alpha = \sum_{R} M_R$ where the sum is over ribbons $R$ which can be obtained by assigning each vertex in $V(\alpha)$ a label from $[n]$.
	%Up to scaling, $M_\alpha$ is the result of averaging each $M_R$ over the orbit of $R$.
\end{definition}

\begin{example}
In \cref{fig: ribbon_shape}, consider the shape $\al$ as shown. We have $U_{\al} = (u_1, u_2), V_{\al} = (v_1), V(\al) = \{u_1, u_2, v_1, w_1\}$ and $E(\al) = \{\{u_1, w_1\}, \{u_2, w_1\}, \{w_1, v_1\}\}$. $M_{\al}$ is a matrix with rows and columns indexed by tuples of length $|U_{\al}| = 2$ and $|V_{\al}| = 1$ respectively. The nonzero entries will have rows and columns indexed by $(a_1, a_2)$ and $b_1$ respectively for all distinct $a_1, a_2, b_1$, with the corresponding entry being $M_{\al}((a_1, a_2), (b_1)) = \sum_{c_1 \in [n] \setminus \{a_1, a_2, b_1\}} \chi_{a_1, c_1}\chi_{a_2, c_1}, \chi_{c_1, b_1}$. Here, the injective map $\phi$ maps $u_1, u_2, w_1, v_1$ to $a_1, a_2, c_1, b_1$ respectively and we sum over all such maps. Succinctly, \[M_{\al} =
%     \begin{blockarray}{c@{\hspace{5pt}}rr@{\hspace{5pt}}cl}
%     & \matindex{1} & \matindex{2} & & \\
%     \begin{block}{(c@{\hspace{5pt}}rr@{\hspace{5pt}}c)l}
%       & 100 &  b & & \matindex{row 1} \\
%       &   2 & 12 & & \matindex{row 2} \\
%       &   e &  f & & \matindex{ABDC} \\
%     \end{block}
%   \end{blockarray}$.
  \begin{blockarray}{rl@{}c@{}r}
    & & \makebox[0pt]{column $(c_1)$} \\[-0.5ex]
    & & \,\downarrow \\[-0.5ex]
    \begin{block}{r(l@{}c@{}r)}
    &  & \vdots & \\[-0.2ex]
    \text{row }(a_1, a_2) \to \mkern-9mu & \raisebox{0.5ex}{\makebox[3.2em][l]{\dotfill}} & \sum_{c_1 \in [n] \setminus \{a_1, a_2, b_1\}} \chi_{a_1, c_1}\chi_{a_2, c_1}, \chi_{c_1, b_1} & \raisebox{0.5ex}{\makebox[4.2em][r]{\dotfill}} \\[+.5ex]
    &  & \vdots & \\
    \end{block}
  \end{blockarray}\]
\end{example}

\begin{remk}
    The fact that we are summing over all "free" vertices in $V(\al) \setminus (U_{\al} \cup V_{\al})$ is how we are incorporating symmetry into the definition of these graph matrices.
\end{remk}

The following examples illustrate that simple matrices such as the adjacency matrix of a graph and the identity matrix are also graph matrices.

\begin{example}[Adjacency matrix]\label{ex:adj-matrix}
	Let $\alpha$ be the shape with two vertices $V(\alpha) = \{u_1,v_1\}$ and a single edge $E(\alpha) = \{\{ u_1,v_1\}\}$. The tuples $U_\alpha, V_\alpha$ are $(u_1), (v_1)$, respectively.
	Then $M_\alpha$ has entries $(M_\alpha)_{i,j}(G) = G_{ij}$ if $i \neq j$ and $(M_\alpha)_{i,i} = 0$.
	If $G \in \{ \pm 1\}^{n \choose 2}$ is thought of as a graph, then $M_\alpha$ is precisely its $\pm 1$ adjacency matrix with zeros on the diagonal.
\end{example}

\begin{example}[Identity matrix]
	If $V(\alpha) = \{u\}$ is a singleton, $E(\alpha) = \emptyset$, and $U_{\alpha} = V_{\alpha} = (u)$, then $M_\alpha(G)$ is identically equal to the $n \times n$ identity matrix, independent of $G$.
\end{example}

% \begin{example}\label{ex:adj-matrix}
% 	Suppose $d=1$, so that $M_\alpha \, : \, \{\pm 1\}^{n \choose 2} \rightarrow \R^{n \times n}$.
% 	Let $\alpha$ be the following shape.
% 	$V(\alpha) = \{u_1,v_1\}$ is a $2$-element set.
% 	$E(\alpha) = \{\{ u_1,v_1\}\}$ contains a single edge between vertices $u_1,v_1$.
% 	The tuples $U_\alpha, V_\alpha$ are $(u_1), (v_1)$, respectively.
% 	Then $M_\alpha$ has entries $(M_\alpha)_{i,j}(G) = G_{ij}$ if $i \neq j$ and $(M_\alpha)_{i,i} = 0$.
% 	If $G \in \{ \pm 1\}^{n \choose 2}$ is thought of as a graph, then $M_\alpha$ is its $\pm 1$ adjacency matrix with zeros on the diagonal.
% \end{example}

% \begin{example}
% 	If $V(\alpha) = \{u\}$ is a singleton, $E(\alpha) = \emptyset$, and $U_{\alpha} = V_{\alpha} = (u)$, then $M_\alpha(G)$ is a constant function with value always equal to the $n \times n$ identity matrix.
% \end{example}

For more examples of graph matrices and why they can be a useful tool to work with, see \cite{AMP20}.
\begin{remark}
As noted in \cite{AMP20}, we index graph matrices by tuples rather than sets so that they are symmetric (as a function of the input) under permutations of $[n]$.
\end{remark}

\subsection{Factoring Graph Matrices and Decomposing Shapes into Left, Middle, and Right Parts}

A crucial idea in our analysis is the idea from \cite{BHKKMP16} of decomposing each shape $\alpha$ into left, middle, and right parts. This will allow us to give an approximate factorization of each graph matrix $M_{\alpha}$.

\subsubsection{Leftmost and Rightmost Minimum Vertex Separators and Decomposition of Shapes into Left, Middle, and Right Parts}
For each shape $\alpha$ we will identify three other shapes, which we denote by $\sigma,\tau,{\sigma'}^T$ and call (for reasons we will see soon) the \emph{left, middle, and right parts of $\alpha$}, respectively.
The idea is that $M_{\alpha} \approx M_{\sigma} M_{\tau} M_{{\sigma'}^T}$.
We obtain $\sigma, \tau$, and ${\sigma'}^T$ by splitting the shape $\alpha$ along the \emph{leftmost and rightmost minimum vertex separators}.

\begin{definition}[Vertex Separators]
	We say that a set of vertices $S$ is a vertex separator of $\alpha$ if every path from $U_{\alpha}$ to $V_{\alpha}$ in $\alpha$ (including paths of length $0$) intersects $S$. Note that for any vertex separator $S$, $U_{\alpha} \cap V_{\alpha} \subseteq S$. 
\end{definition}

%\noindent We note one basic property of vertex separators; the proof is straightforward.

%\begin{proposition}
%	For any vertex separator $S$ of $\alpha$, $U_{\alpha} \cap V_{\alpha} \subseteq S$
%\end{proposition}

\begin{definition}[Minimum Vertex Separators]
	We say that $S$ is a minimum vertex separator of $\alpha$ if $S$ is a vertex separator of $\alpha$ and for any other vertex separator $S'$ of $\alpha$, $|S| \leq |S'|$.
\end{definition}

\begin{definition}[Leftmost and Rightmost Minimum Vertex Separators] \
	\begin{enumerate}
		\item We say that $S$ is the leftmost minimum vertex separator of $\alpha$ if $S$ is a minimum vertex separator of $\alpha$ and for every other minimum vertex separator $S'$ of $\alpha$, every path from $U_{\alpha}$ to $S'$ intersects $S$. 
		\item We say that $T$ is the rightmost minimum vertex separator of $\alpha$ if $T$ is a minimum vertex separator of $\alpha$ and for every other minimum vertex separator $S'$ of $\alpha$, every path from $S'$ to $V_{\alpha}$ intersects $T$. 
	\end{enumerate}
\end{definition}
It is not immediately obvious that leftmost and rightmost minimum vertex separators are well-defined. For the simplified setting we are considering here, this was shown by \cite{BHKKMP16}. We give a more general proof in \cref{separatorswelldefinedsection}.

We now describe how to split $\alpha$ into left, middle, and right parts $\sigma, \tau$, and ${\sigma'}^T$.

\begin{definition}[Decomposition Into Left, Middle, and Right Parts]
	Let $\alpha$ be a shape and let $S$ and $T$ be the leftmost and rightmost minimum vertex separators of $\alpha$. Given orderings $O_S$ and $O_T$ for $S$ and $T$, we decompose $\alpha$ into left, middle, and right parts $\sigma$, $\tau$, and ${\sigma'}^T$ as follows.
	%We will have $V(\sigma), V(\tau), V(\sigma') \subseteq V(\alpha)$ and $E(\sigma),E(\tau),E(\sigma') \subseteq E(\alpha)$, but the distinguished vertices $U_\sigma, V_\sigma$ and so on will differ from $U_\alpha, V_\alpha$.
	\begin{enumerate}
		\item The left part $\sigma$ of $\alpha$ is the part of $\alpha$ reachable from $U_\alpha$ without passing through $S$. It includes $S$ but excludes all edges which are entirely within $S$.
		More formally, 
		\begin{enumerate}
		    \item $V(\sigma) = \{u \in V(\alpha): \text{ there is a path } P \text{ from } U_{\alpha} \text{ to } u \text{ in } \alpha \text{ such that } (V(P) \setminus \{u\}) \cap S = \emptyset\}$
		    \item $U_\sigma = U_\alpha$ and $V_\sigma = S$ with the ordering $O_S$
		    \item $E(\sigma) = \{\{u,v\} \in E(\alpha): u,v \in V(\sigma), u \notin S \text{ or } v \notin S\}$
		\end{enumerate}
		\item %The right part ${\sigma'}^T$ of $\alpha$ is like the left part with the roles of $S$ and $T$ interchanged.
		The right part ${\sigma'}^T$ of $\alpha$ is the part of $\alpha$ reachable from $V_\alpha$ without intersecting $T$ more than once. It includes $T$ but excludes all edges which are entirely within $T$.
		More formally, 		
		\begin{enumerate}
		    \item $V({\sigma'}^T) = \{u \in V(\alpha): \text{ there is a path } P \text{ from } V_{\alpha} \text{ to } u \text{ in } \alpha \text{ such that } (V(P) \setminus \{u\}) \cap T = \emptyset\}$
		    \item $U_{{\sigma'}^T} = T$ with the ordering $O_T$ and $V_{{\sigma'}^T} = V_\alpha$.
		    \item $E({\sigma'}^T) = \{\{u,v\} \in E(\alpha): u,v \in V({\sigma'}^T), u \notin T \text{ or } v \notin T\}$
		\end{enumerate}
		\item The middle part $\tau$ of $\alpha$ is, informally, the part of $\alpha$ between $S$ and $T$ (including $S$ and $T$ and all edges which are entirely within $S$ or within $T$).
		More formally, let $U_\tau = S$ with the ordering $O_S$, let $V_\tau = T$ with the ordering $O_T$, and let $E(\tau) = E(\alpha) \setminus (E(\sigma) \cup E(\sigma'))$ be all of the edges of $E(\alpha)$ which do not appear in $E(\sigma)$ or $E(\sigma')$.
		Then $V(\tau)$ is all of the vertices incident to edges in $E(\tau)$ together with $S, T$.
	\end{enumerate}
\end{definition}

\begin{example}
    \cref{fig: basic_shape_comp} illustrates an example decomposition.
    \begin{enumerate}
        \item If we start with the shape $\al$ denoted as $\sig \circ \sig'^T$, observe that there is a unique minimum vertex separator, which consists of the middle vertex of degree $5$, i.e. the one that's not in either $U_{\sig \circ \sig'^T}$ or $V_{\sig \circ \sig'^T}$.
        Then, $\al$ is decomposed in to the left part $\sig$, a trivial middle part $\tau$ (not shown in this figure) which has $V(\tau) = \{u\}, U_{\tau} = V_{\tau} = (u), E(\tau) = \emptyset$, and the right part $\sig'^T$.
        \item If we start with the shape $\al$ denoted as $\sig \circ \tau \circ \sig'^T$, then the leftmost minimum vertex separator is the vertex of degree $4$ and the rightmost minimum vertex separator is the vertex of degree $5$. Then, $\al$ is decomposed into the left part $\sig$, the middle part $\tau$ and the right part $\sig'^T$, which are all shown in this figure.
    \end{enumerate}
\end{example}

\begin{remark}
Note that the decomposition into left, middle, and right parts depends on the ordering for the vertices in $S$ and $T$. As we will discuss later (see Section \ref{fullcoefficientmatrixsubsection}), we will use all possible orderings simultaneously and then scale things by an appropriate constant.
\end{remark}

\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.45, trim={4.5cm 2cm 0 2cm},clip]{machinery/images/basic_shape_comp}
    \caption{Illustration of shape composition and decomposition.}
    \label{fig: basic_shape_comp}
\end{figure}


\noindent Because of the minimality and leftmost/rightmost-ness of the vertex separators $S,T$ used to define $\sigma, \tau, \sigma'$, the shapes $\sigma, \tau, \sigma'$ have some special combinatorial structure, which we capture in the following proposition. We defer the proof until \cref{sec: technical_def_and_main_theorem} where we state a generalized version.

\begin{proposition}
	$\sigma$, $\tau$, and ${\sigma'}^{T}$ have the following properties:
	\begin{enumerate}
		\item $V_{\sigma} = S$ is the unique minimum vertex separator of $\sigma$.
		\item $S$ and $T$ are the leftmost and rightmost minimum vertex separators of $\tau$.
		\item $T = U_{{\sigma'}^T}$ is the unique minimum vertex separator of ${\sigma'}^T$.
	\end{enumerate}
\end{proposition}

\noindent Based on this, we define sets of shapes which can appear as left, middle, or right parts.

\begin{definition}[Left, Middle, and Right Parts] Let $\alpha$ be a shape.
	\begin{enumerate}
		\item We say that $\alpha$ is a left part if $V_{\alpha}$ is the unique minimum vertex separator of $\alpha$, all vertices of $\alpha$ are reachable from $U_{\alpha}$ without passing through $V_{\alpha}$, and $E(\alpha)$ has no edges which are entirely contained in $V_{\alpha}$.
		\item We say that $\alpha$ is a proper middle part if $U_{\alpha}$ is the leftmost minimum vertex separator of $\alpha$ and $V_{\alpha}$ is the rightmost minimum vertex separator of $\alpha$
		\item We say that $\alpha$ is a right part if $U_{\alpha}$ is the unique minimum vertex separator of $\alpha$, all vertices of $\alpha$ are reachable from $V_{\alpha}$ without passing through $U_{\alpha}$, and $E(\alpha)$ has no edges which are entirely contained in $U_{\alpha}$.
	\end{enumerate}
\end{definition}
\begin{remark}
	For technical reasons, later on we will need to consider improper middle parts $\tau$ where $U_{\tau}$ and $V_{\tau}$ are not the leftmost and rightmost minimum vertex separators of $\tau$, which is why we make this distinction here.
\end{remark}

\noindent The following proposition is also straightforward from the definitions.

\begin{proposition}
	A shape $\sigma$ is a left part if and only if $\sigma^{T}$ is a right part
\end{proposition}
%Examples should be added.\gnote{**}

\subsubsection{Products of Graph Matrices}
We now analyze what happens when we take the products of graph matrices. Roughly speaking, we will have that if $\alpha$ can be decomposed into left, middle, and right parts $\sigma$, $\tau$, and ${\sigma'}^{T}$ then $M_{\alpha} \approx M_{\sigma}M_{\tau}M_{{\sigma'}^T}$. However, this is only an approximation rather than an equality, and this will be the source of considerable technical difficulties.

We begin with a concatenation operation on ribbons.
\begin{definition}[Ribbon Concatenation]
	If $R_1$ and $R_2$ are two ribbons such that $V(R_1) \cap V(R_2) = B_{R_1} = A_{R_2}$ and either $R_1$ or $R_2$ contains no edges entirely within $B_{R_1} = A_{R_2}$ then we define $R_1 \circ R_2$ to be the ribbon formed by glueing together $R_1$ and $R_2$ along $B_{R_1} = A_{R_2}$.
	In other words,
	\begin{enumerate}
		\item $V(R_1 \circ R_2) = V(R_1) \cup V(R_2)$
		\item $E(R_1 \circ R_2) = E(R_1) \cup E(R_2)$
		\item $A_{R_1 \circ R_2} = A_{R_1}$ and $B_{R_1 \circ R_2} = B_{R_2}$.
	\end{enumerate}
\end{definition}

\noindent The following proposition is easy to check.

\begin{proposition}
	Whenever $R_1, R_2$ are ribbons such that $R_1 \circ R_2$ is defined, $M_{R_1}M_{R_2} = M_{R_1 \circ R_2}$
\end{proposition}

\noindent We have an analogous definition for concatenating shapes:

\begin{definition}[Shape Concatenation]
	If $\alpha_1$ and $\alpha_2$ are two shapes such that $V(\alpha_1) \cap V(\alpha_2) = V_{\alpha_1} = U_{\alpha_2}$ and either $\alpha_1$ or $\alpha_2$ contains no edges entirely within $V_{\alpha_1} = U_{\alpha_2}$ then we define $\alpha_1 \circ \alpha_2$ to be the shape formed by glueing together $\alpha_1$ and $\alpha_2$ along $V_{\alpha_1} = U_{\alpha_2}$. In other words,
	\begin{enumerate}
		\item $V(\alpha_1 \circ \alpha_2) = V(\alpha_1) \cup V(\alpha_2)$
		\item $E(\alpha_1 \circ \alpha_2) = E(\alpha_1) \cup E(\alpha_2)$
		\item $U_{\alpha_1 \circ \alpha_2} = U_{\alpha_1}$ and $V_{\alpha_1 \circ \alpha_2} = V_{\alpha_2}$.
	\end{enumerate}
\end{definition}

\begin{example}
    \cref{fig: basic_shape_comp} illustrates an example of shape composition. Observe how the shapes $\sig \circ \sig'^T$ and $\sig \circ \tau \circ \sig'^T$ are obtained from the shapes $\sig, \tau$ and $\sig'^T$.
\end{example}

\noindent The next proposition, again easy to check, shows that the shape concatenation operation respects the left/middle/right part decomposition.

\begin{proposition}
	If $\alpha$ can be decomposed into left, middle, and right parts $\sigma,\tau,{\sigma'}^{T}$ then $\alpha = \sigma \circ \tau \circ {\sigma'}^T$.
\end{proposition}

We now discuss why $M_\alpha = M_{\sigma \circ \tau \circ {\sigma'}^T} \approx M_\sigma M_\tau M_{{\sigma'}^T}$ is only an approximation rather than an equality. Consider the difference $M_{\sigma}M_\tau M_{{\sigma'}^T} - M_{\sigma \circ \tau \circ {\sigma'}^T}$. The graph matrix $M_{\sigma \circ \tau \circ {\sigma'}^T}$ decomposes (by definition) into a sum over injective maps $\phi \, : \, V(\sigma \circ \tau \circ {\sigma'}^T) \rightarrow [n]$. Also by expanding definitions, the product $M_{\sigma}M_\tau M_{{\sigma'}^T}$ expands into a sum over triples of injective maps $(\phi_1, \phi_2, \phi_3)$, where $\phi_1 \, : \, V(\sigma) \rightarrow [n], \phi_2 \, : \, V(\tau) \rightarrow [n], \phi_3 \, : \, V(\sigma') \rightarrow [n]$ where $\phi_1$ and $\phi_2$ agree on $V_{\sigma} = U_{\tau}$ and $\phi_2$ and $\phi_3$ agree on $V_{\tau} = U_{{\sigma'}^T}$.

If they are combined into one map $\phi: V(\sigma \cup \tau \cup {\sigma'} ) \to [n]$, the resulting $\phi$ may not be injective because $\phi_1(V(\sigma)), \phi_2(V(\tau)), \phi_3(V({\sigma'}^T))$ may have nontrivial intersection (beyond $\phi_1(V_\sigma)$ and $\phi_2(V_\tau)$).
We call the resulting terms \emph{intersection terms} and handling them properly is a major part of the technical analysis.
\begin{remark}
    Actually, the approximation $M_\alpha = M_{\sigma \circ \tau \circ {\sigma'}^T} \approx M_\sigma M_\tau M_{{\sigma'}^T}$ is also off by a multiplicative constant because there is also a subtle issue involving the automorphism groups of these shapes. For now, we ignore this issue. For details about this issue, see Lemma \ref{lm:morthsimplereexpression}.
\end{remark}


% Sam: this is not really a proposition; it is more like flavor text. "intersection terms" isn't well-defined here, is the issue.
%\begin{proposition}[Approximate Decomposition of Graph Matrices]
%If $\sigma,\tau,{\sigma'}^{T}$ are the left, middle, and rights parts for $\alpha$ then 
%\[
%M_{\alpha} = M_{\sigma}M_{\tau}M_{{\sigma'}^T} + \text{intersection terms}
%\]
%\end{proposition}

%
%\begin{remark}
%It would be nice if we had that $M_{\alpha} = M_{\sigma}M_{\tau}M_{{\sigma'}^T}$. The reason this isn't quite true is as follows. If we take injective maps $\phi_{1}: V(\sigma) \to [1,n]$, $\phi_{2}: V(\tau) \to [1,n]$, $\phi_{3}: V({\sigma'}^T) \to [1,n]$ (where $\phi_1$ and $\phi_2$ agree on $V_{\sigma} = U_{\tau}$ and $\phi_2$ and $\phi_3$ agree on $V_{\tau} = U_{{\sigma'}^T}$) and combine them, the resulting map $\phi: V(\alpha) \to [1,n]$ may not be injective because $\phi_1(V(\sigma)), \phi_2(V(\tau)), \phi_3(V({\sigma'}^T))$ may have additional intersections. We call the resulting terms \emph{intersection terms} and handling them properly is a major part of the technical analysis.
%\end{remark}

\subsection{Shape Coefficient Matrices}
The idea for our analysis is as follows. Given a matrix-valued function $\Lambda$ which is symmetric under permutations of $[n]$, we write $\Lambda = \sum_{\alpha}{\lambda_{\alpha}M_{\alpha}}$. We then break each shape $\alpha$ up into left, middle, and right parts $\sigma$, $\tau$, and ${\sigma'}^{T}$.

For this analysis, we use \emph{shape coefficient matrices} $H_{\tau}$ whose rows and columns are indexed by left shapes and whose entries depend on the coefficients $\lambda_{\alpha}$. We choose these matrices so that 
\[
\Lambda = \sum_{\tau}{H_{\tau}(\sigma,\sigma')M_{\sigma \circ \tau \circ {\sigma'}^T}} \approx \sum_{\tau}{H_{\tau}(\sigma,\sigma')M_{\sigma}M_{\tau}M_{{\sigma'}^T}}
\]
To set this up, we separate the possible middle parts $\tau$ into groups based on the size of $U_{\tau}$ and whether or not they are trivial.
\begin{definition}
    We define $\mathcal{I}_{mid}$ to be the set of all possible $U_{\tau}$. Here $\mathcal{I}_{mid}$ is the set of tuples of unspecified vertices of the form $U = (u_1,\ldots,u_k)$ where $0 \leq k \leq d$.
\end{definition}
\begin{definition}
    We say that a proper middle shape $\tau$ is trivial if $E(\tau) = \emptyset$ and $|U_{\tau} \cap V_{\tau}| = |U_{\tau}| = |V_{\tau}|$ (i.e. $V_{\tau}$ is a permutation of $U_{\tau}$).
\end{definition}
For simplicity, the only proper trivial middle parts $\tau$ we consider are shapes $Id_U$ corresponding to identity matrices. 
\begin{definition}
    Given a tuple of unspecified vertices $U = (u_1,\ldots,u_{|U|})$ We define $Id_U$ to be the shape where $V(Id_U) = U$, $U_{Id_U} = V_{Id_U} = U$, and $E(Id_U) = \emptyset$.
\end{definition}
We group all of the proper non-trivial middle parts $\tau$ into sets $\mathcal{M}_U$ based on the size of $U_{\tau}$.
\begin{definition}
    Given a tuple of unspecified vertices $U = (u_1,\ldots,u_{|U|})$, we define $\mathcal{M}_U$ to be the set of proper non-trivial middle parts $\tau$ such that $U_{\tau}$ and $V_{\tau}$ have the same size as $U$. Note that $U_{\tau}$ and $V_{\tau}$ may intersect each other arbitrarily.
\end{definition}
With these definitions, we can now define our shape coefficient matrices.
\begin{definition}
    Given $U \in \mathcal{I}_{mid}$, we define $\mathcal{L}_U$ to be the set of left shapes $\sigma$ such that $|V_{\sigma}| = |U|$.
\end{definition}
\begin{definition}
    For each $U \in \mathcal{I}_{mid}$, we define the shape coefficient matrix $H_{Id_U}$ to be the matrix indexed by left shapes $\sigma,\sigma' \in \mathcal{L}_{U}$ with entries $H_{Id_U}(\sigma,\sigma') = \frac{1}{|U|!}\lambda_{\sigma \circ {\sigma'}^T}$
\end{definition}
\begin{definition}
    For each $U \in \mathcal{I}_{mid}$, for each $\tau \in \mathcal{M}_{U}$, we define the shape coefficient matrix $H_{\tau}$ to be the matrix indexed by left shapes $\sigma,\sigma' \in \mathcal{L}_{U}$ with entries $H_{\tau}(\sigma,\sigma') = \frac{1}{(|U|!)^2}\lambda_{\sigma \circ \tau \circ {\sigma'}^T}$
\end{definition}
With these shape coefficient matrices, we have the following decomposition of $\Lambda = \sum_{\alpha}{\lambda_{\alpha}M_{\alpha}}$.
\begin{lemma}
$\Lambda = \sum_{U \in \mathcal{I}_{mid}}{\sum_{\sigma,\sigma' \in \mathcal{L}_U}{H_{Id_U}(\sigma,\sigma')M_{\sigma \circ {\sigma'}^T}}} + \sum_{U \in \mathcal{I}_{mid}}{\sum_{\tau \in \mathcal{M}_{U}}{\sum_{\sigma,\sigma' \in \mathcal{L}_U}{H_{\tau}(\sigma,\sigma')M_{\sigma \circ \tau \circ  {\sigma'}^T}}}}$
\end{lemma}
We defer the proof of this lemma to \cref{lm:determiningcoefficientmatrices}.

For technical reasons, we need to define one more operation to handle intersection terms. We call this operation \emph{the $-\gamma,\gamma$ operation.}

\begin{definition}
Given $U,V \in \mathcal{I}_{mid}$ where $|U| > |V|$, we define $\Gamma_{U,V}$ to be the set of left parts $\gamma$ such that $|U_{\gamma}| = |U|$ and $|V_{\gamma}| = |V|$.
\end{definition}
\begin{definition}
	Given $U,V \in \mathcal{I}_{mid}$ where $|U| > |V|$, a shape coefficient matrix $H_{Id_V}$, and a $\gamma \in \Gamma_{U,V}$, we define the shape coefficient matrix $H^{-\gamma,\gamma}_{Id_V}$ to be the matrix indexed by left shapes $\sigma,\sigma' \in \mathcal{L}_{U}$ with entries $H^{-\gamma,\gamma}_{Id_V}(\sigma,\sigma') = H(\sigma \circ \gamma, \sigma' \circ \gamma)$
\end{definition}

\subsection{Informal Theorem Statement}

We are now ready to state a simplified, qualitative version of our main theorem. For the full, quantitative version of our main theorem, see \cref{simplifiedmaintheorem}.
%\begin{itemize}
%	\item Quantitative bounds needed for the applications to SoS lower bounds (in particular, quantitative expressions for $f(\gamma)$ and $f(\tau)$.
%	\item Generalization beyond the setting $k=2$ or to the case that the underlying product space is $\Omega^{n \choose k}$ for som $\Omega \neq \{\pm 1\}$.
%	\item Generalization to the asymmeric setting that the underlying product space is $\Omega^{n_1 \times n_2 \times \ldots \times n_k}$.
%\end{itemize}

\begin{theorem}\label{informalmaintheoremstatement}
	There exist functions $f(\tau): \mathcal{M}_U \rightarrow \R$ and $f(\gamma): \Gamma_{U,V} \rightarrow \R$ depending on $n$ and other parameters such that if $\Lambda = \sum_{\alpha}{\lambda_{\alpha}M_{\alpha}}$ and the following conditions hold:
	\begin{enumerate}
		\item For all $U \in \mathcal{I}_{mid}$,  $H_{Id_U} \succeq 0$
		\item For all $U \in \mathcal{I}_{mid}$ and all $\tau \in \mathcal{M}_{U}$,
		\[
		\left[ {\begin{array}{cc}
				H_{Id_U} & f(\tau)H_{\tau} \\
				f(\tau)H^T_{\tau} & H_{Id_U}
		\end{array}} \right] \succeq 0
		\]
		%If the matrices $H_{\tau}$ are always symmetric, this reduces to the condition that $f(\tau)H_{\tau} \preceq H_{Id_r}$
		\item For all $U,V \in \mathcal{I}_{mid}$ such that $|U| > |V|$ and all $\gamma \in \Gamma_{U,V}$, $H^{-\gamma,\gamma}_{Id_{V_{\gamma}}} \preceq f(\gamma)H_{Id_{U_{\gamma}}}$
	\end{enumerate}
	then with probability at least $1-o(1)$ over $G \sim \{ \pm 1\}^{n \choose 2}$ it holds that $\Lambda(G) \succeq 0$.
\end{theorem}

\begin{remark}
	Condition $1$ of \cref{informalmaintheoremstatement} will follow from condition $2$ but we state it explicitly since it will correspond to the dominating terms of the approximate PSD decomposition. And in applications, it will be both easy to verify and will shed light on the structure of the coefficients which in turn will be useful for verifying conditions $2$ and $3$.
\end{remark}

\begin{remark}
As we will demonstrate in the remainder of this paper, our machinery works well when the coefficients $\lambda_{\alpha}$ has a polynomial decay for each vertex or edge in the shape. In many settings, this can be done quite easily by adding noise to the distribution, such as resampling part of the input, or by lowering the parameters slightly, such as $m \le n^{k/4 - \eps}$ instead of $m \le n^{k/4}$. That said, it's possible to optimize many of our functions so that a significantly better bound can be obtained (say for example $m \le n^{k/4} / polylog(n)$ is potentially feasible), we do not attempt this in this work.
% However, since our machinery is highly technical with many different parts, it does not work as well if the coefficients have a different kind of decay.
\end{remark}

\subsubsection{Choice of functions $f(\tau)$ and $f(\gam)$, upto lower order terms}

In a rough sense, $f(\tau)$ measures the blow-up in the norm by using $M_{\tau}$ instead of $M_{Id_U}$ in the corresponding term of the Fourier decomposition. So we choose $f(\tau)$ to be $\norm{M_{\tau}}$, upto lower order terms. Our second condition verifies that the coefficients that arise because of this $\tau$ (which are encoded in $H_{\tau}$) are sufficiently small to overpower this norm blowup.

The fact that $\norm{M_{\tau}}$ is equal to $\tilde{O}(n^{\frac{|V(\tau)|-|U_{\tau}|}{2}})$ has been shown in previous works \cite{BHKKMP16, AMP20}. So, we choose $f(\tau)$ to be $\tilde{O}(n^{\frac{|V(\tau)|-|U_{\tau}|}{2}})$ where the problem instance is on $G_{n, 1/2}$. For problems with Gaussian or other inputs, similar forms of $f(\tau)$ can be used, which have been shown formally in the work of \cite{AMP20}. When we state the main theorem in general, we use a single $f(\tau)$ that incorporates all of these settings.

$f(\gam)$ is a bit trickier to describe. In our analysis, we roughly collect intersection terms from the approximate PSD decomposition and charge them to shapes of the form $\sig \circ \gam \circ \gam^T \circ \sig'^T$. Using the same idea as the previous step, we charge these to shapes with trivial middle shapes. Roughly, $f(\gam)$ for a fixed $\gam$ upper bounds the blowup from the norms of the original shape as compared to the new intersection shape. And the third condition argues that the the original coefficients are sufficiently small to compensate for these blowups.

For problems on $G_{n, 1/2}$, we set $f(\gam) = \tilde{O}(n^{|V(\gamma) \setminus U_{\gamma}|})$. For problems with Gaussian inputs, we choose essentially the same function, but they fall under the umbrella of generalized graph matrices, where $V(\gam)$ and $U_{\gam}$ are defined accordingly. Indeed, in our main theorem, we encompass both these settings with a single choice of $f(\gam)$.

\subsection{An informal application to planted clique}
Before we move on to further definitions needed for a more complete statement of the main theorem, we present an informal example.

\begin{example}
	When the pseudo-calibration method is applied to prove an SoS lower bound for the planted clique problem in $n$ node graphs with clique size $k$, as in \cite{BHKKMP16}, the matrix-valued function which results is $\Lambda =  \sum_{\alpha \, : \, |V(\alpha)| \leq t}{\left(\frac{k}{n}\right)^{|V(\alpha)|}M_{\alpha}}$ where $t \approx \log(n)$.
	One may then compute that the matrices $H_{Id_U}$ and $H_{\tau}$ are as follows (at least so long as $|V(\sigma)|,|V(\tau)|,|V(\sigma')| \ll t$; we ignore this detail for now).
	For all $r \in [0,\frac{d}{2}]$,
	\begin{enumerate}
		\item For $U$ with $|U|  = r$, $H_{Id_U}(\sigma,\sigma') = \left(\frac{k}{n}\right)^{|V(\sigma)| + |V(\sigma')| - r}$
		\item For all proper, non-trivial middle shapes $\tau$ such that $|U_{\tau}| = |V_{\tau}| = r$, 
		\[
		H_{\tau}(\sigma,\sigma') = \left(\frac{k}{n}\right)^{|V(\sigma)| + |V(\sigma')| + |V(\tau)|- 2r}
		\]
	\end{enumerate}
	Defining $v_r$ to be the vector such that $v_r(\sigma) = \left(\frac{k}{n}\right)^{|V(\sigma)| - \frac{r}{2}}$, we have that 
	\begin{enumerate}
		\item For $U$ with $|U|  = r$, $H_{Id_U} = {v_{|U|}}{v^T_{|U|}}$
		\item For all proper, non-trivial middle shapes $\tau$ such that $|U_{\tau}| = |V_{\tau}| = r$, $H_{\tau} = \left(\frac{k}{n}\right)^{|V(\tau)|- r}{v_r}{v^T_r}$
		\item For all left parts $\gamma$, $H^{-\gamma,\gamma}_{Id_{V_{\gamma}}} = \left(\frac{k}{n}\right)^{2|V(\gamma)| - |U_{\gamma}| - |V_{\gamma}|}v_{|U_{\gamma}|}v^{T}_{|U_{\gamma}|}$
	\end{enumerate}
	It turns out in this setting that we can take $f(\tau)$ to be $\tilde{O}(n^{\frac{|V(\tau)|-|U_{\tau}|}{2}})$ and $f(\gamma)$ to be $\tilde{O}(n^{|V(\gamma) \setminus U_{\gamma}|})$. Thus, as long as $k \ll \sqrt{n}$,
	\begin{enumerate}
		\item For any $U$ and all $\tau$ such that $V_{\tau} \neq U_{\tau}$ with $|U_{\tau}| = |V_{\tau}| = |U|$, $f(\tau)H_{\tau} \preceq H_{Id_U}$.
		\item For all non-trivial left parts $\gamma$, $H^{-\gamma,\gamma}_{Id_{V_{\gamma}}} \preceq f(\gamma)H_{Id_{U_{\gamma}}}$
	\end{enumerate}
\end{example}
\begin{remark}\label{rmk: planted_clique_failure}
This does not quite satisfy the conditions of Theorem \ref{informalmaintheoremstatement} because there are $\tau$ such that $V_{\tau} = U_{\tau}$ but which are non-trivial because $E(\tau) \neq \emptyset$. For these $\tau$, condition 2 of Theorem \ref{informalmaintheoremstatement} fails. In order to prove their SoS lower bounds for planted clique, \cite{BHKKMP16} handle this issue by grouping together all of the $\tau$ where $V_{\tau} = U_{\tau}$ into the indicator function for whether $V_{\tau} = U_{\tau}$ is a clique.

Since this issue is specific to planted clique, we don't try to incorporate it into the machinery to avoid losing generality.
%	It should be noted that this theorem as stated (even with $f(\tau), f(\gamma)$ made quantitative) is not quite enough to prove the planted clique SoS lower bound of \cite{BHKKMP16}.

%In this paper, we get around this issue by instead considering the planted slightly denser subgraph problem. This introduces an edge decay into the coefficients. For details, see Section \ref{sec: plds_qual}.
\end{remark}

For the sake of exposition, a detailed analysis with figures of all the shapes and all the coefficient matrices that appear for the degree-$4$ SoS lower bound for planted clique is given in \cref{sec: deg_4_planted_clique}.

\subsection{Generalizing the machinery}
In this section, we restricted ourselves to the case when the input is from $\{-1,1\}^{\binom{n}{2}}$ for simplicity. However, for our results we will need to handle more general types of inputs. We now briefly describe which kinds of inputs we will need to handle and how we handle them.
\begin{enumerate}
    \item In general, the entries of the input may be labeled by more than $2$ indices. For example, for tensor PCA on order $3$ tensors, the entries of the input are indexed by $3$ indices. To handle this, we will have shapes which have hyperedges rather than edges.
    \item In general, the entries of the input will come from a distribution $\Omega$ rather than being $\pm{1}$. To handle this, we will take an orthonormal basis $\{h_k\}$ for $\Omega$. We will then give each edge/hyperedge a label $l$ to specify which polynomial $h_l$ should be applied to that entry of the input.   
    \item In general, there may be $t$ different types of indices rather than just one type of index. In this case, the symmetry group will be $S_{n_1} \times \ldots \times S_{n_t}$ rather than $S_n$. To handle this, we will have shapes with different types of vertices.
\end{enumerate}
We formally make these generalizations in \cref{sec: technical_def_and_main_theorem}.

\subsection{Further definitions needed for our applications}

We will describe some more notations and definitions that will be useful to us to describe the qualitative bounds for our applications. For each of our applications, we will describe the corresponding modifications needed to the definitions already in place and present new definitions where necessary.

\subsubsection{Planted slightly denser subgraph}

Since the input is a graph $G \in \{-1, 1\}^{\binom{[n]}{2}}$, most of what we introduced already apply to this setting. To describe the moment matrix, we need to define the truncation parameter.

\begin{definition}[Truncation parameters]
For integers $D_{sos}, D_V \ge 0$, say that a shape $\al$ satisfies the truncation parameters $D_{sos}, D_V$ if
\begin{itemize}
    \item The degrees of the monomials that $U_{\al}$ and $V_{\al}$ correspond to, are at most $\frac{D_{sos}}{2}$
    \item The left part $\sig$, the middle part $\tau$ and the right part $\sig'$ of $\al$ satisfy $|V(\sig)|, |V(\tau)|, |V(\sig')| \le D_V$
\end{itemize}
\end{definition}

\subsubsection{Tensor PCA}

We consider the input to be a tensor $A \in \RR^{[n]^k}$. The input entries are now sampled from the distribution $\GN(0, 1)$ instead of $\{-1, 1\}$. So, we will work with the Hermite basis of polynomials.

Let the standard unnormalized Hermite polynomials be denoted as $h_0(x) = 1, h_1(x) = x, h_2(x) = x^2 - 1, \ldots$. Then, we work with the basis $h_a(A) \defeq \prod_{e \in [n]^k} h_e(A_e)$ over $a \in \NN^{[n]^k}$. Accordingly, we will modify the graphs that represent ribbons (and by extension, shapes), to have labeled hyperedges of arity $k$. So, an hyperedge $e$ with a label $t$ will correspond to the hermite polynomial $h_t(A_e)$.

\begin{definition}[Hyperedges]
Instead of standard edges, we will have labeled hyperedges of arity $k$ in the underlying graphs for our ribbons as well as shapes. The label for an hyperedge $e$, denoted $l_e$, is an element of $\NN$ which will correspond to the Hermite polynomial being evaluated on that entry.
\end{definition}

Note that our hyperedges are ordered since the tensor $A$ is not necessarily symmetric.

For variables $x_1, \ldots, x_n$, the rows and columns of our moment matrix will now correspond to monomials of the form $\prod_{i \le n} x_i^{p_i}$ for $p_i \ge 0$. To capture this, we use the notion of index shape pieces and index shapes. Informally, we split the above monomial product into groups based on their powers and each such group will form an index shape piece.

\begin{definition}[Index shape piece]
    An index shape piece $U_i= ((U_{i, 1}, \ldots, U_{i, t}), p_i)$ is a tuple of indices $(U_{i, 1}, \ldots, U_{i, t})$ along with a power $p_i \in \NN$. Let $V(U_i)$ be the set $\{U_{i, 1}, \ldots, U_{i, t}\}$ of vertices of this index shape piece. When clear from context, we use $U_i$ instead of $V(U_i)$.
\end{definition}

If we realize $U_{i, 1}, \ldots, U_{i, t}$ to be indices $a_1, \ldots, a_t \in [n]$, then, this realization of this index shape piece corresponds to the monomial $\prod_{j \le t} x_{a_j}^{p_i}$.

\begin{definition}[Index shape]
An index shape $U$ is a set of index shape pieces $U_i$ that have different powers. Let $V(U)$ be the set of vertices $\cup_i V(U_i)$. When clear from context, we use $U$ instead of $V(U)$.
\end{definition}

Observe that each realization of an index shape corresponds to a row or column of the moment matrix.

\begin{definition}
For two index shapes $U, V$, we write $U \equiv V$ if for all powers $p$, the index shape pieces of power $p$ in $U$ and $V$ have the same length.
\end{definition}

\begin{definition}
Define $\calI_{mid}$ to be the set of all index shapes $U$ that contain only index shape pieces of power $1$.
\end{definition}

In the definition of shapes, the distinguished set of vertices should now be replaced by index shapes.

\begin{definition}[Shapes]
Shapes are tuples $\al = (H_{\al}, U_{\al}, V_{\al})$ where $H_{\al}$ is a graph with hyperedges of arity $k$ and $U_{\al}, V_{\al}$ are index shapes such that $U_{\al}, V_{\al} \subseteq V(H_{\al})$.
\end{definition}

\begin{definition}[Proper shape]
A shape $\al$ is proper if it has no isolated vertices outside $U_{\al} \cup V_{\al}$, no multi-edges and all the edges have a nonzero label.
\end{definition}

To define the notion of vertex separators, we modify the notion of paths for hyperedges.

\begin{definition}[Path]
A path is a sequence of vertices $u_1, \ldots, u_t$ such that $u_i, u_{i + 1}$ are in the same hyperedge, for all $i \le t - 1$.
\end{definition}

The notions of vertex separator and decomposition into left, middle and right parts are identically defined with the above notion of hyperedges and paths. In \cref{sec: technical_def_and_main_theorem}, we will show that they are well defined.

In the definition of trivial shape $\tau$, we now require $U_{\tau} \equiv V_{\tau}$. For $U \in \calI_{mid}$, $\calM_U$ will be the set of proper non-trivial middle parts $\tau$ with $U_{\tau} \equiv V_{\tau} \equiv U$ and $\calL_U$ will be the set of left parts $\sig$ such that $V_{\sig} \equiv U$. Similarly, for $U, V \in \calI_{mid}$, $\calL_{U, V}$ will be the set of left parts $\gam$ such that $U_{\gam} \equiv U$ and $V_{\gam} \equiv V$.

In order to define the moment matrix, we need to truncate our shapes based on the number of vertices and the labels on our hyperedges. So, we make the following definition.

\begin{definition}[Truncation parameters]
For integers $D_{sos}, D_V, D_E \ge 0$, say that a shape $\al$ satisfies the truncation parameters $D_{sos}, D_V, D_E$ if
\begin{itemize}
    \item The degrees of the monomials that $U_{\al}$ and $V_{\al}$ correspond to, are at most $\frac{D_{sos}}{2}$
    \item The left part $\sig$, the middle part $\tau$ and the right part $\sig'^T$ of $\al$ satisfy $|V(\sig)|, |V(\tau)|, |V(\sig'^T)| \le D_V$
    \item For each $e \in E(\al)$, $l_e \le D_E$.
\end{itemize}
\end{definition}

\subsubsection{Sparse PCA}

We consider the $m$ vectors $v_1, \ldots, v_m \in \RR^d$ to be the input. Similar to Tensor PCA, we will work with the Hermite basis of polynomials since the entries are sampled from the distribution $\GN(0, 1)$.

In particular, if we denote the unnormalized Hermite polynomials by $h_0(x) = 1, h_1(x) = x, h_2(x) = x^2 - 1, \ldots$, then, we work with the basis $h_a(v) \defeq \prod_{i \in [m], j \in [n]} h_{a_{i, j}}(v_{i, j})$ over $a \in \NN^{m \times n}$. To capture these bases, we will modify the graphs that represent ribbons (and by extension, shapes), to be bipartite graphs with two types of vertices, and have labeled edges that go across vertices of different types. So, an edge $(i, j)$ with label $t$ between a vertex $i$ of type $1$ and a vertex $j$ of type $2$ will correspond to $h_t(v_{i, j})$.

\begin{definition}[Vertices]
We will have two types of vertices, the vertices corresponding to the $m$ input vectors that we call type $1$ vertices and the vertices corresponding to ambient dimension of the space that we call type $2$ vertices.
\end{definition}

\begin{definition}[Edges]
Edges will go across vertices of different types, thereby forming a bipartite graph. An edge between a type $1$ vertex $i$ and a type 2 vertex $j$ corresonds to the input entry $v_{i, j}$. Each edge will have a label in $\NN$ corresponding to the Hermite polynomial evaluated on that entry.
\end{definition}

We will have variables $x_1, \ldots, x_n$ in our SoS program, so we will work with index shape pieces and index shapes as in Tensor PCA, since the rows and columns of our moment matrix will now correspond to monomials of the form $\prod_{i \le n} x_i^{p_i}$ for $p_i \ge 0$. But since in our decompositions into left, right and middle parts, we will have type $2$ vertices as well in the vertex separators, we will define a generalized notion of index shape pieces and index shapes.

\begin{definition}[Index shape piece]
    An index shape piece $U_i= ((U_{i, 1}, \ldots, U_{i, t}), t_i, p_i)$ is a tuple of indices $(U_{i, 1}, \ldots, U_{i, t})$ along a type $t_i \in \{1, 2\}$ with a power $p_i \in \NN$. Let $V(U_i)$ be the set $\{U_{i, 1}, \ldots, U_{i, t}\}$ of vertices of this index shape piece. When clear from context, we use $U_i$ instead of $V(U_i)$.
\end{definition}

For an index shape piece $((U_{i, 1}, \ldots, U_{i, t}), t_i, p_i)$ with type $t_i = 2$, if we realize $U_{i_1}, \ldots, U_{i_t}$ to be indices $a_1, \ldots, a_t \in [n]$, then, this index shape pieces correspond this to the monomial $\prod_{j \le n} x_{a_j}^{p_i}$.

\begin{definition}[Index shape]
An index shape $U$ is a set of index shape pieces $U_i$ that have either have different types or different powers. Let $V(U)$ be the set of vertices $\cup_i V(U_i)$. When clear from context, we use $U$ instead of $V(U)$.
\end{definition}

Observe that each realization of an index shape corresponds to a row or column of the moment matrix. For our moment matrix, the only nonzero rows correspond to index shapes that have only index shape pieces of type $2$, since the only SoS variables are $x_1 \ldots, x_n$, but in order to do our analysis, we need to work with the generalized notion of index shapes that allow index shape pieces of both types.

\begin{definition}
For two index shapes $U, V$, we write $U \equiv V$ if for all types $t$ and all powers $p$, the index shape pieces of type $t$ and power $p$ in $U$ and $V$ have the same length.
\end{definition}

\begin{definition}
Define $\calI_{mid}$ to be the set of all index shapes $U$ that contain only index shape pieces of power $1$.
\end{definition}

Since we are working with standard graphs, the notion of path and vertex separator need no modifications, but we will now use the minimum weight vertex separator instead of the minimum vertex separator where we define the weight as follows.

\begin{definition}[Weight of an index shape]
Suppose we have an index shape $U = \{U_1, U_2\} \in \calI_{mid}$ where $U_1 = ((U_{1, 1}, \ldots, U_{1, |U_1|}), 1, 1)$ is an index shape piece of type $1$ and $U_2 = ((U_{2, 1}, \ldots, U_{2, |U_2|}), 2, 1)$ is an index shape piece of type $2$. Then, define the weight of this index shape to be $w(U) = \sqrt{m}^{|U_1|}\sqrt{n}^{|U_2|}$.
\end{definition}

We now give the modified definition of shapes.

\begin{definition}[Shapes]
Shapes are tuples $\al = (H_{\al}, U_{\al}, V_{\al})$ where $H_{\al}$ is a graph with two types of vertices, has labeled edges only across vertices of different types and $U_{\al}, V_{\al}$ are index shapes such that $U_{\al}, V_{\al} \subseteq V(H_{\al})$.
\end{definition}

\begin{definition}[Proper shape]
A shape $\al$ is proper if it has no isolated vertices outside $U_{\al} \cup V_{\al}$, no multi-edges and all the edges have a nonzero label.
\end{definition}

In \cref{sec: technical_def_and_main_theorem}, we will show that with this new definition of weight and shapes, any shape $\al$ has a unique decomposition into $\sig \circ \tau \circ \sig'^T$ where $\sig, \tau, \sig'^T$ are left, middle and right parts respectively. Here, $\tau$ may possibly be improper.

In the definition of trivial shape $\tau$, we now require $U_{\tau} \equiv V_{\tau}$. For $U \in \calI_{mid}$, $\calM_U$ will be the set of proper non-trivial middle parts $\tau$ with $U_{\tau} \equiv V_{\tau} \equiv U$ and $\calL_U$ will be the set of left parts $\sig$ such that $V_{\sig} \equiv U$. Similarly, for $U, V \in \calI_{mid}$, $\calL_{U, V}$ will be the set of left parts $\gam$ such that $U_{\gam} \equiv U$ and $V_{\gam} \equiv V$.

Finally, in order to define the moment matrix, we need to truncate our shapes based on the number of vertices and the labels on our edges. So, we make the following definition.

\begin{definition}[Truncation parameters]
For integers $D_{sos}, D_V, D_E \ge 0$, say that a shape $\al$ satisfies the truncation parameters $D_{sos}, D_V, D_E$ if
\begin{itemize}
    \item The degrees of the monomials that $U_{\al}$ and $V_{\al}$ correspond to, are at most $\frac{D_{sos}}{2}$
    \item The left part $\sig$, the middle part $\tau$ and the right part $\sig'^T$ of $\al$ satisfy $|V(\sig)|, |V(\tau)|, |V(\sig'^T)| \le D_V$
    \item For each $e \in E(\al)$, $l_e \le D_E$.
\end{itemize}
\end{definition}

\subsubsection{Relaxing the third condition}\label{sec: hgamma_qual}

In \cref{informalmaintheoremstatement}, the third qualitative condition we'd like to show is as follows:
For all $U,V \in \mathcal{I}_{mid}$ such that $|U| > |V|$ and all $\gamma \in \Gamma_{U,V}$, $H^{-\gamma,\gamma}_{Id_{V_{\gamma}}} \preceq f(\gamma)H_{Id_{U_{\gamma}}}$.

For technical reasons, we won't be able to show this directly. To handle this, we instead work with a slight modification of $H_{Id_{U_{\gamma}}}$, a matrix $H_{\gamma}'$ that's very close to $H_{Id_{U_{\gamma}}}$. So, what we will end up showing is:
For all $U,V \in \mathcal{I}_{mid}$ such that $|U| > |V|$ and all $\gamma \in \Gamma_{U,V}$, $H^{-\gamma,\gamma}_{Id_{V_{\gamma}}} \preceq f(\gamma)H'_{\gamma}$

Let $D_V$ be the truncation parameter. A canonical choice for $H'_{\gamma}$ is to take 
\begin{enumerate}
	\item $H'_{\gamma}(\sigma,\sigma') = H_{Id_U}(\sigma, \sigma')$ whenever $|V(\sigma \circ \gamma)| \leq D_V$ and $|V(\sigma' \circ \gamma)| \leq D_V$.
	\item $H'_{\gamma}(\sigma,\sigma') = 0$ whenever $|V(\sigma \circ \gamma)| > D_V$ or $|V(\sigma' \circ \gamma)| > D_V$.
\end{enumerate}

With this choice, $H_{\gamma}'$ is the same as $H_{Id_{U_{\gamma}}}$ upto truncation error. We will formally bound the errors in the quantitative sections after we introduce the full machinery.

==> machinery/intro.tex <==
The Sum-of-Squares (SoS) hierarchy is an optimization technique that harnesses the power of semidefinite programming to solve optimization tasks. For polynomial optimization problems, the SoS hierarchy, first independently investigated by Shor \cite{shor1987approach}, Nesterov \cite{nesterov2000squared}, Parillo \cite{parrilo2000structured}, Lasserre \cite{lasserre2001global} and Grigoriev \cite{grigoriev2001complexity, Grigoriev01}, offers a sequence of convex relaxations parameterized by an integer called the degree of the SoS hierarchy. As we increase the degree $d$ of the hierarchy, we get progressively stronger convex relaxations which are solvable in $n^{O(d)}$ time\footnote{There is a caveat, see \cite{o2017sos}}. This has paved the way for the SoS hierarchy to be a powerful tool in algorithm design both in the worst case and the average case settings. Indeed, there has been tremendous success in using the SoS hierarchy to obtain efficient algorithms for combinatorial optimization problems (e.g., \cite{GW94, AroraRV04, GuruswamiS11, raghavendra2017strongly}) as well as problems stemming from Statistics and Machine Learning (e.g., \cite{BarakBHKSZ12, bks15, HopSS15, pot17, kothari2017outlier}). In fact, SoS achieves the state-of-the-art approximation guarantees for many fundamental problems such as Sparsest Cut \cite{AroraRV04}, MaxCut \cite{GW94}, Tensor PCA \cite{HopSS15} and all Max-$k$-CSPs \cite{Raghavendra08}. Moreover, for a large class of problems, it's been shown that SoS relaxations are the most efficient among all semidefinite programming relaxations \cite{lrs15}.

On the flip side, some problems have remained intractable beyond a certain threshold even by considering higher degrees of the SoS hierarchy \cite{BHKKMP16, KothariMOW17, MRX20, sklowerbounds}. For example, consider the Planted Clique problem where we have to distinguish a random graph sampled from the \Erdos-\Renyi model $G(n, \frac{1}{2})$ from a random graph which is obtained by first sampling a graph from $G(n, \frac{1}{2})$ and then planting a clique of size $n^{\frac{1}{2} - \eps}$ for a small constant $\eps > 0$. It was shown in \cite{BHKKMP16} that with high probability degree $o(\log n)$ SoS fails to solve this distinguishing problem.


There are many reasons for why studying lower bounds against the SoS hierarchy is important. SoS is a generic proof system that captures a broad class of algorithmic reasoning \cite{FKP19}. In particular, SoS captures statistical query algorithms and algorithms based on low degree polynomials. Therefore, SoS lower bounds indicate to the algorithm designer the intrinsic hardness of the problem and suggest that if they want to break the algorithmic barrier, they need to search for algorithms that are not captured by SoS. Secondly, in average case problem settings, standard complexity theoretic assumptions such as P $\neq$ NP have not been shown to give insight into the limits of efficient algorithms. Instead, lower bounds against powerful proof systems such as SoS have served as strong evidence of computational hardness \cite{hop17, hop18}. Thus, understanding the power of the SoS hierarchy on these problems is an important step towards understanding the approximability of these problems.
%Note importantly that SoS lower bounds imply lower bounds on sample complexity, algorithms based on low-degree polynomials and statistical query algorithms. Unsurprisingly, SoS hardness results turn out to be harder to show.

\subsection{Our contributions}

In this paper, we consider the following general category of problems: Given a random input, can we certify that it does not contain a given structure?

Some important examples of this kind of problem are as follows.
\begin{enumerate}
    \item Planted clique: Can we certify that a random graph does not have a large clique?
    \item Tensor PCA: Given an order $k$ tensor $T$ with random independent Gaussian entries, can we certify that there is no unit vector $x$ such that $\ip{T}{x \otimes\ldots\otimes x}$ is large?
    \item Wishart model of sparse PCA: Given an $m \times d$ matrix $S$ with random independent Gaussian entries (which corresponds to taking $m$ samples from $\GN(0, I_d)$), can we certify that there is no $k$-sparse unit vector $x$ such that $\norm{Sx}$ is large?
\end{enumerate}

These kinds of problems, known as certification problems, are closely related to their optimization or estimation variants. A certification algorithm is required to produce a proof/certificate of a bound that holds for \textit{all} inputs, as opposed to most inputs. The Sum-of-Squares hierarchy provides such certificates in a canonical way for a wide variety of such problems, so analyzing SoS paves the way towards understanding the certification complexity of these problems. We investigate the following question.

\begin{quote}
    \em{For certification problems, what are the best bounds that SoS can certify?}
\end{quote}

In this work, we build general machinery for proving probabilistic Sum of Squares lower bounds on certification problems. To build our machinery, we generalize the techniques pioneered by \cite{BHKKMP16} for proving Sum of Squares lower bounds for planted clique. We start with the standard framework for proving probabilistic Sum of Squares lower bounds:
\begin{enumerate}
    \item Construct candidate pseudo-expectation values $\pE$ and the corresponding moment matrix $\Lambda$ (see \cref{subsec: sos}).
    \item Show that with high probability, $\Lambda \succeq 0$.
\end{enumerate}
For planted clique, \cite{BHKKMP16} constructed $\pE$ and the corresponding moment matrix $\Lambda$ by introducing the pseudo-calibration technique (see \cref{subsec: pseudocalibration}). They then showed through a careful and highly technical analysis that with high probability $\Lambda \succeq 0$. 

In this paper, we investigate how generally the techniques used for planted clique can be applied. We show that by constructing coefficient matrices based on the coefficients obtained by pseudo-calibration, we can give relatively simple conditions on these coefficient matrices which are sufficient to ensure that the moment matrix $\Lda$ is PSD with high probability. %This generality allows us to handle problems such as the Wishart model of sparse PCA which were beyond previous analyses.

%In this paper, by significantly generalizing the techniques used in this analysis, we give general conditions which are sufficient to show that a candidate moment matrix $\Lambda$ is positive-semidefinite (PSD) with high probability. These conditions, which are our main result, are stated informally in \cref{informalmaintheoremstatement} and stated formally in \cref{simplifiedmaintheorem} and \cref{generalmaintheorem}. 

By abstracting out a lot of the technical analysis that goes into sum of squares lower bound proofs with a general framework, we pave the way for future works on SoS lower bounds to use our machinery as a blackbox and instead focus on the analysis of the problem specific structure. We exhibit the usefulness of our machinery by achieving strong SoS lower bounds for the problems of Tensor PCA, Sparse PCA and a problem closely related to the Planted Clique problem that we call Planted Slightly Denser Subgraph. We do this with relative ease once the machinery is in place. The Sparse PCA lower bounds complement a long line of work on algorithmic guarantees that stretches for over two decades (the most recent one being \cite{sparse_pca_focs20}), giving a complete picture (up to polylogarithmic factors) for the approximability-inapproximability thresholds for Sparse PCA.

\subsubsection{A brief summary of pseudo-calibration}
A natural way to prove lower bounds on a certification problem is as follows.
\begin{enumerate}
    \item Construct a "maximum entropy" planted distribution of inputs which has the given structure.
    \item Show that we cannot distinguish between the random and planted distributions and thus cannot certify that a random input does not have the given structure.
\end{enumerate}
Based on this idea, the pseudo-calibration technique introduced  by \cite{BHKKMP16} constructs candidate pseudo-expectation values $\pE$ so that as far as low degree tests are concerned, $\pE$ for the random distribution mimics the behavior of the given structure for the planted distribution (for details, see \cref{subsec: pseudocalibration}). This gives a candidate moment matrix $\Lambda$ which we can then analyze with our machinery. A majority of known high-degree average-case SoS lower bounds in the literature have pseudo-expectation values that were either obtained by, or could be obtained by pseudocalibration, e.g., Planted Clique \cite{BHKKMP16}, Max-$k$-CSPs \cite{KothariMOW17}, Max-Cut on regular graphs \cite{MRX20}, Sherrington-Kirkpatrick problem \cite{sklowerbounds, MRX20}. It has also been successful for Densest-$k$-subgraph but for the weaker Sherali-Adams Hierarchy \cite{chlamtavc2018sherali}.

Naturally, pseudocalibration is the starting point for our SoS lower bounds. That said, our machinery is quite general and can be applied even if the candidate moment matrix $\Lambda$ is not obtained via pseudo-calibration.

\subsubsection{Our results on Tensor PCA, Sparse PCA, and Planted Slightly Denser Subgraph}
In this section, we formally state the main hardness theorems we show by applying our machinery. We defer discussing prior work, how we improve on them, and other related work to \cref{sec: prior_work}.

We describe the planted distributions we use to show our SoS lower bounds for planted slightly denser subgraph, tensor PCA, and the the Wishart model of sparse PCA. We also state the random distributions for completeness and for contrast. We then state our results.

\paragraph{Planted slightly denser subgraph}
We use the following distributions.
\begin{restatable}{itemize}{PLDSdistributions}
% \begin{itemize}
    \item Random distribution: Sample $G$ from $G(n, \frac{1}{2})$
    \item Planted distribution: Let $k$ be an integer and let $p > \frac{1}{2}$. Sample a graph $G'$ from $G(n, \frac{1}{2})$. Choose a random subset $S$ of the vertices, where each vertex is picked independently with probability $\frac{k}{n}$. For all pairs $i, j$ of vertices in $S$, rerandomize the edge $(i, j)$ where the probability of $(i, j)$ being in the graph is now $p$. Set $G$ to be the resulting graph.
% \end{itemize}
\end{restatable}
In \cref{sec: plds_qual}, we compute the candidate moment matrix $\Lambda$ obtained by using pseudo-calibration on this planted distribution.

\begin{restatable}{theorem}{PLDSmain}\label{thm: plds_main}
Let $C_p > 0$. There exists a constant $C > 0$ such that for all sufficiently small constants $\eps > 0$, if $k \le n^{\frac{1}{2} - \eps}$ and $p =  \frac{1}{2} + \frac{n^{-C_p\eps}}{2}$, then with high probability, the candidate moment matrix $\Lda$ given by pseudo-calibraton for degree $n^{C\eps}$ Sum-of-Squares is PSD.
\end{restatable}

\begin{corollary}\label{cor: plds_main}
Let $C_p > 0$. There exists a constant $C > 0$ such that for all sufficiently small constants $\eps > 0$, if $k \le n^{\frac{1}{2} - \eps}$ and $p =  \frac{1}{2} + \frac{n^{-C_p\eps}}{2}$, then with high probability, degree $n^{C\eps}$ Sum-of-Squares cannot certify that a random graph $G$ from $G(n, \frac{1}{2})$ does not have a subgraph of size $\approx k$ with edge density $\approx p$.
\end{corollary}

\paragraph{Tensor PCA}
Let $k \ge 2$ be an integer. We use the following distributions.
\begin{restatable}{itemize}{TPCAdistributions}
% \begin{itemize}
    \item Random distribution: Sample $A$ from $\GN(0, I_{[n]^k})$.
	\item Planted distribution: Let $\lda,\Delta > 0$. Sample $u$ from $\{-\frac{1}{\sqrt{\Delta n}}, 0, \frac{1}{\sqrt{\Delta n}}\}^n$ where the values are taken with probabilites $\frac{\Delta}{2}, 1 - \Delta, \frac{\Delta}{2}$ respectively. Then sample $B$ from $\GN(0, I_{[n]^k})$. Set $A = B + \lda \tens{u}{k}$.
% \end{itemize}
\end{restatable}

In \cref{sec: tpca_qual}, we compute the candidate moment matrix $\Lambda$ obtained by using pseudo-calibration on this planted distribution.

\begin{restatable}{theorem}{TPCAmain}\label{thm: tpca_main}
    Let $k \ge 2$ be an integer. There exist constants $C,C_{\Del} > 0$ such that for all sufficiently small constants $\eps > 0$, if $\lda \le n^{\frac{k}{4} - \eps}$ and $\Del = n^{-C_{\Del}\eps}$ then with high probability, the candidate moment matrix $\Lambda$ given by pseudo-calibration for degree $n^{C\eps}$ Sum-of-Squares is PSD.
\end{restatable}
\begin{corollary}\label{cor: tpca_main}
    Let $k \ge 2$ be an integer. There exists a constant $C > 0$ such that for all sufficiently small constants $\eps > 0$, if $\lda \le n^{\frac{k}{4} - \eps}$, then with high probability, degree $n^{C\eps}$ Sum-of-Squares cannot certify that for a random tensor $A$ from $\GN(0, I_{[n]^k})$, there is no vector $u$ such that $\norm{u} \approx 1$ and $\ip{A}{\underbrace{x \otimes\ldots\otimes x}_{\text{k times}}} \approx \lambda$.
\end{corollary}

\paragraph{Wishart model of Sparse PCA}
We use the following distributions.
\begin{restatable}{itemize}{SPCAdistributions}
% \begin{itemize}
    \item Random distribution: $v_1, \ldots, v_m$ are sampled from $\GN(0, I_d)$ and we take $S$ to be the $m \times d$ matrix with rows $v_1, \ldots, v_m$.
	\item Planted distribution: Sample $u$ from $\{-\frac{1}{\sqrt{k}}, 0, \frac{1}{\sqrt{k}}\}^d$ where the values are taken with probabilites $\frac{k}{2d}, 1 - \frac{k}{d}, \frac{k}{2d}$ respectively. Then sample $v_1, \ldots, v_m$ as follows. For each $i \in [m]$, with probability $\Delta$, sample $v_i$ from $\GN(0, I_d + \lda uu^T)$ and with probability $1 - \Delta$, sample $v_i$ from $\GN(0, I_d)$. Finally, take $S$ to be the $m \times d$ matrix with rows $v_1, \ldots, v_m$.
% \end{itemize}
\end{restatable}

In \cref{sec: spca_qual}, we compute the candidate moment matrix $\Lambda$ obtained by using pseudo-calibration on this planted distribution.

\begin{restatable}{theorem}{SPCAmain}\label{thm: spca_main}
    There exists a constant $C > 0$ such that for all sufficiently small constants $\eps > 0$, if $m \le \frac{d^{1 - \eps}}{\lda^2}, m \le \frac{k^{2 - \eps}}{\lda^2}$, and there exists a constant $A$ such that $0 < A < \frac{1}{4}$, $d^{4A} \le k \le d^{1 - A\eps}$, and $\frac{\sqrt{\lda}}{\sqrt{k}} \le d^{-A\eps}$, then with high probability, the candidate moment matrix $\Lambda$ given by pseudo-calibration for degree $d^{C\eps}$ Sum-of-Squares is PSD.
\end{restatable}

\begin{corollary}\label{cor: spca_main}
    There exists a constant $C > 0$ such that for all sufficiently small constants $\eps > 0$, if $m \le \frac{d^{1 - \eps}}{\lda^2}, m \le \frac{k^{2 - \eps}}{\lda^2}$, and there exists a constant $A$ such that $0 < A < \frac{1}{4}$, $d^{4A} \le k \le d^{1 - A\eps}$, and $\frac{\sqrt{\lda}}{\sqrt{k}} \le d^{-A\eps}$, then with high probability, the degree $d^{C\eps}$ degree Sum-of-Squares cannot certify that for a random $m \times d$ matrix $S$ with Gaussian entries, there is no vector $u$ such that $u$ has $\approx k$ nonzero entries, $\norm{u} \approx 1$, and $\norm{Su}^2 \approx m + m{\Delta}\lambda$.
\end{corollary}

\begin{remark}
Note that our planted distributions only approximately satisfy constraints such as having a subgraph of size $k$, having a unit vector $u$, and having $u$ be $k$-sparse. While we would like to use planted distributions which satisfy such constraints exactly, these distributions don't quite satisfy the conditions of our machinery. This same issue appeared in the SoS lower bounds for planted clique \cite{BHKKMP16}. Resolving this issue is a subtle but important open problem.
\end{remark}

\subsection{Relation to prior work on Planted Clique/Dense Subgraph, Tensor PCA, and Sparse PCA}\label{sec: prior_work}

\subsubsection{Planted Dense Subgraph}\label{sec: plds}

In the planted dense subgraph problem, we are given a random graph $G$ where a dense subgraph of size $k$ has been planted and we are asked to find this planted dense subgraph.
%This is related to the problem of detecting the densest subgraph on $k$ vertices in a given random graph on $n$ vertices. 
This is a natural generalization of the $k$-clique problem \cite{karp1972reducibility} and has been subject to a long line of work over the years (e.g. \cite{feige1997densest, feige2001dense, khot2006ruling, bhaskara2010detecting, bhaskara2012polynomial, braverman2017eth, manurangsi2017almost}).
In this work, we consider the following certification variant of planted dense subgraph.

% \paragraph{Densest $k$-subgraph of a random graph}
\begin{quote}
\em{Given a random graph $G$ sampled from the \Erdos-\Renyi model $G(n, \frac{1}{2})$, certify an upper bound on the edge density of the densest subgraph on $k$ vertices.}
\end{quote}

For many different parameter regimes of the random and planted distributions (an example being planting $G_{k, q}$ in $G_{n, p}$ for constants $p < q$), and when $k = o(\sqrt{n})$, the hardness of the easier distinguishing version of planted dense subgraph problem has been posed as formal conjecture (often referred to as the PDS conjecture) before in the literature (see e.g., \cite{hajek2015computational, chen2014statistical, brennan2018reducibility, brennan2019universality}). This has also led to many reductions to other problems \cite{brennan2019optimal}, although it's not clear if these reductions can be made in the SoS framework without loss in the parameter dependence.

In our case, we consider the slightly planted denser subgraph version where for $k \le n^{\frac{1}{2} - \eps}$, we plant a subgraph of density $\frac{1}{2} + \frac{1}{n^{O(\eps)}}$, i.e. $p = \frac{1}{2}, q = \frac{1}{2} + \frac{1}{n^{O(\eps)}}$. This has been widely believed to require sub-exponential time. Our work provides strong evidence towards this by exhibiting unconditional lower bounds against the powerful SoS hierarchy, even if we consider $n^{O(\eps)}$ levels, which corresponds to $n^{n^{O(\eps)}}$ running time! We expect this to lead to this problem being used as a natural starting point for reductions to show sub-exponential time hardness for various problems.

Within the SoS literature, \cite{BHKKMP16} show that for $k \le n^{\frac{1}{2} - \eps}$ for a constant $\eps > 0$, the degree $o(\log n)$ Sum-of-Squares cannot distinguish between a fully random graph sampled from $G(n, \frac{1}{2})$ from a random graph which has a planted $k$-clique. This implies that degree $o(\log n)$ SoS cannot certify an edge density better than $1$ for the densest $k$-subgraph if $k \le n^{\frac{1}{2} - \eps}$.

In \cref{cor: plds_main}, we show that for $k \le n^{\frac{1}{2} - \eps}$ for a constant $\eps > 0$, degree $n^{\Omega(\eps)}$ SoS cannot certify an edge density better than $\frac{1}{2} + \frac{1}{n^{O(\eps)}}$. The degree of SoS in our setting, $n^{\Omega(\eps)}$ is vastly higher than the earlier known result which uses degree $o(\log n)$. To the best of our knowledge, this is the first result that proves such a high degree lower bound. %When the SoS degree is only $o(\log n)$, our result is not as strong as the work of \cite{BHKKMP16}.

We remark that when we take $k = n^{\frac{1}{2} - \eps}$,  the true edge density of the densest $k$-subgraph is $\frac{1}{2} + \frac{\sqrt{\log(n/k)}}{\sqrt{k}} + \littleoh(\frac{1}{\sqrt{k}}) \approx \frac{1}{2} + \frac{1}{n^{1/4 - \eps/2}}$ as was shown in \cite[Corollary 2]{gamarnik2019landscape} whereas, by \cref{cor: plds_main}, the SoS optimum is as large as $\frac{1}{2} + \frac{1}{n^{\eps}}$. This highlights a significant difference in the optimum value.

\subsubsection{Tensor PCA}

The Tensor Principal Component Analysis problem, originally introduced by \cite{richard2014statistical}, is a generalization of the PCA problem from machine learning to higher order tensors. Given an order $k$ tensor of the form $\lda u^{\otimes k} + B$ where $u \in \RR^n$ is a unit vector and $B \in \RR^{[n]^k}$ has independent Gaussian entries, we would like to recover $u$. Here, $\lda$ is known as the signal-to-noise ratio.

This can be equivalently considered to be the problem of optimizing a homogenous degree $k$ polynomial $f(x)$, with random Gaussian coefficients over the unit sphere $\norm{x} = 1$. In general, polynomial optimization over the unit sphere is a fundamental primitive with a lot of connections to other areas of optimization (e.g. \cite{frieze2008new, brubaker2009random,brandao2017quantum, barak2014rounding, bks15, bhattiprolu2017weak}). Tensor PCA is an average case version of the above problem and has been studied before in the literature \cite{richard2014statistical, HopSS15, tensorpca16, hop17}. In this work, we consider the certification version of this average case problem.

\begin{quote}
\em{For an integer $k \ge 2$, given a random tensor $A \in \RR^{[n]^k}$ with entries sampled independently from $\GN(0, 1)$, certify an upper bound on $\ip{A}{x^{\otimes k}}$ over unit vectors $x$.}
\end{quote}

In \cite{tensorpca16}, it was shown that $q \le n$ levels of SoS certifies an upper bound of $\frac{2^{O(k)} (n \cdot \text{polylog}(n))^{k/4}}{q^{k/4 - 1/2}}$ for the Tensor PCA problem. When $q = n^{\eps}$ for sufficiently small $\eps$, this gives an upper bound of $n^{\frac{k}{4} - O(\eps)}$. \cref{cor: tpca_main} shows that this is tight.

In \cite{hop17}, they state a theorem similar to \cref{cor: tpca_main} and observe that it can be proved by applying the techniques used to prove the SoS lower bounds for planted clique. However, they do not give an explicit proof. Also, while they consider the setting where the random distribution has entries from $\{-1, 1\}$, we work with the more natural setting where the distribution is $\GN(0, 1)$. We remark that our machinery can also easily recover their result with the entries being restricted to $\{-1, 1\}$.

When $k = 2$, the maximum value of $\ip{\tens{x}{k}}{A}$ over the unit sphere $\norm{x}^2 = 1$ is precisely the largest eigenvalue of $(A + A^T)/2$ which is $\Theta(\sqrt{n})$ with high probability. For any integer $k \ge 2$, the true maximum of $\ip{\tens{x}{k}}{A}$ over $\norm{x}^2 = 1$ is $O(\sqrt{n})$ with high probability \cite{tomioka2014}. In contrast, by \cref{cor: tpca_main}, the optimum value of the degree $n^{\eps}$ SoS is as large as $n^{\frac{k}{4} - O(\eps)}$. This exhibits an integrality gap of $n^{\frac{k}{4} - \frac{1}{2} - O(\eps)}$.

\subsubsection{Wishart model of Sparse PCA}

The Wishart model of Sparse PCA, also known as the Spiked Covariance model, was originally proposed by \cite{johnstone_lu2009}. In this problem, we observe $m$ vectors $v_1, \ldots, v_m \in \RR^d$ from the distribution $\GN(0, I_d + \lda uu^T)$ where $u$ is a $k$-sparse unit vector, and we would like to recover $u$. Here, the sparsity of a vector is the number of nonzero entries and $\lda$ is known as the signal-to-noise ratio.

Sparse PCA is a fundamental problem that has applications in a diverse range of fields (e.g. \cite{wang2012online, naikal2011informative, majumdar2009image, tan2014classification, chun2009expression, allen2011sparse}). It's known that vanilla PCA does not yield good estimators in high dimensional settings \cite{baik2005phase, paul2007asymptotics, johnstone_lu2009}. A large volume of work has gone into studying Sparse PCA and it's variants, both from an algorithmic perspective (e.g. \cite{amini_wainwright2008, ma2013sparse, krauthgamer2015, deshpande2016, wang2016statistical}) as well as from an inapproximability perspective (e.g. \cite{berthet2013complexity, ma_wigderson_15, diakonikolas2017statistical, hop17, brennan2019optimal}).

Given the decades of research on this problem and how fundamental it is for a multitude of applications and disciplines, understanding the computational threshold behavior of the Wishart model of Sparse PCA is an extremely important research topic in statistics. In particular, prior works have explored statistical query lower bounds, SDP lower bounds, lower bounds by reductions from widely believed conjectures, etc. On the other hand, there have only been two prior works on lower bounds against SoS, specifically only for degree $2$ and degree $4$ SoS, which can be attributed to the difficulty in proving such lower bounds. In this paper, we vastly strengthen these lower bounds and show almost-tight lower bounds for the SoS hierarchy of degree $d^{\eps}$ which corresponds to a running time of $d^{d^{O(\eps)}}$.
%Nevertheless, it's an important research direction because SoS is a powerful proof system, so showing lower bounds against it provides compelling evidence of average-case hardness against many standard algorithmic techniques and reasoning. We undertake this here, and show almost-tight lower bounds for the SoS hierarchy of degree $d^{\eps}$ which corresponds to a running time of $d^{d^{O(\eps)}}$.

Between this work and prior works, we completely understand the parameter regimes where sparse PCA is easy or conjectured to be hard up to polylogarithmic factors. In \cref{fig: spca_thresholds}, we classify the different parameter regimes into the following categories.
\begin{itemize}
    \item DT: In this regime, Diagonal thresholding \cite{johnstone_lu2009, amini_wainwright2008} recovers the sparse vector. Covariance thresholding \cite{krauthgamer2015, deshpande2016} and SoS \cite{sparse_pca_focs20} can also be used in this regime. Covariance thresholding has better dependence on logarithmic factors and SoS works in the presence of adversarial errors.
    \item PCA: Vanilla PCA can recover the vector, i.e. we do not need to use the fact that the vector is sparse (see e.g. \cite{berthet2013, sparse_pca_focs20}).
    \item Spectral: An efficient spectral algorithm recovers the sparse vector (see e.g. \cite{sparse_pca_focs20}).
    \item Spectral*: A simple spectral algorithm distinguishes the planted distribution from the random distribution but it is information theoretically impossible to recover the sparse vector \cite[Appendix E]{sparse_pca_focs20}.
    \item Hard: A regime where it is conjectured to be hard to distinguish between the random and the planted distributions. We discuss this in more detail below.
\end{itemize}

% \begin{figure}[!h]
%     \centering
%     \includegraphics[scale=.67, trim={0 2cm 0 2cm},clip]{spca_graph}
%     \caption{The threshold behavior of the Wishart model of Sparse PCA with respect to $m$, the number of samples}
%     \label{fig: spca_thresholds}
% \end{figure}

\begin{figure}[!ht]
    \centering
    \includegraphics[scale=.6]{machinery/images/spca_graph_2}
    \caption{The threshold behavior of the Wishart model of Sparse PCA where the $x$-axis is $d$, the ambient dimension and the $y$-axis is $k$, the sparsity of the hidden vector. [*] indicates the regime studied in this paper.}
    \label{fig: spca_thresholds}
\end{figure}

% \begin{itemize}
%     \item If $m \gg \frac{k^2}{\lda^2}$ then the sparse vector can be recovered by diagonal thresholding\cite{johnstone_lu2009, amini_wainwright2008}, covariance thresholding \cite{krauthgamer2015, deshpande2016}, or SoS \cite{sparse_pca_focs20}. 
%     \item If $m \geq d$ and $m \gg \frac{d}{\lda^2}$ or $m \leq d$ and $m \gg \frac{d}{\lda}$ then vanilla PCA can recover the sparse vector (i.e. we do not need to use the fact that the vector is sparse) (e.g. \cite{berthet2013, sparse_pca_focs20}).
%     \item If $m \leq d$, $\frac{d}{\lda^2} \ll m \ll \frac{d}{\lda}$, and $m \gg \frac{k}{\lda}$ then there is an efficient spectral algorithm to recover the sparse vector (e.g. \cite{sparse_pca_focs20}).
%     \item If $m \leq d$, $\frac{d}{\lda^2} \ll m \ll \frac{d}{\lda}$, and $m \ll \frac{k}{\lda}$ then there is a simple spectral algorithm which distinguishes the planted distribution from the random distribution but it is information theoretically impossible to recover the sparse vector \cite[Appendix E]{sparse_pca_focs20}.
%     \item If $m \ll \frac{k^2}{\lda^2}$ and $m \ll \frac{d}{\lda^2}$ then it is conjectured to be hard to distinguish between the random and the planted distributions. We discuss the evidence for this below.
% \end{itemize}

In the \textit{Hard} parameter regime where $m \ll \frac{k^2}{\lda^2}$ and $m \ll \frac{d}{\lda^2}$, degree $2$ and degree $4$ SoS lower bounds have been shown in prior works, while we handle degree $d^{O(\eps)}$. In particular, the works \cite{krauthgamer2015, berthet2013} obtain degree $2$ SoS lower bounds. \cite{ma_wigderson_15} obtain degree $4$ SoS lower bounds using an ad-hoc construction. It's not clear if their construction can be generalized for higher degrees. Moreover, the bounds they obtain are tight up to polylogarithmic factors when $\lda$ is a constant but are not tight when $\lda$ is not a constant, so we improve their bounds even in the degree $4$ case. We subsume all these earlier known results in this work with \cref{cor: spca_main}. This is a vast improvement over prior known sum of squares lower bounds and provides compelling evidence for the hardness of Sparse PCA in this parameter range.

The work \cite{hop17} considers the related but qualitatively different Wigner model of Sparse PCA and they state degree $d^{\eps}$ SoS lower bounds, without explicitly proving these bounds. The techniques in that work do not recover our results because the matrix formed by the random samples in the Wishart model is asymmetric, and handling it correctly is far from being a mere technicality. On the other hand, our machinery can recover the results on the Wigner model as well, though we only analyze the Wishart model in this paper.

In \cite{sparse_pca_focs20}, they prove that if $m \le \frac{d}{\lda^2}$ and $m \le \left(\frac{k^2}{\lda^2}\right)^{1 - \Omega(\eps)}$, then degree $n^{\eps}$ polynomials cannot distinguish the random and planted distributions. %(see \cref{subsec: related_techniques} for a discussion).
\cref{cor: spca_main} says that under mildly stronger assumptions, degree $n^{\eps}$ Sum-of-Squares cannot distinguish the random and planted distributions, so we confirm that SoS is no more powerful than low degree polynomials in this setting. 
%This is interesting because on the surface, SoS is seemingly capable of way more reasoning than low degree polynomials, but this work ascertains that this is not the case for Sparse PCA. This suggests that perhaps this is a special case of a global phenomenon, which we leave for future work.

There have also been direct reductions from planted clique to Sparse PCA \cite{brennan2019optimal}, and it's natural to ask if these reductions can obtain SoS lower bounds on Sparse PCA from the known SoS lower bounds on planted clique \cite{BHKKMP16}. To the best of our knowledge, no such reduction is known and constructing such a reduction would be challenging as it would have to be captured by SoS and avoid losing too much in the parameters. Still, it may well be possible to construct such a reduction.

%However, it is unknown if there is such a reduction which is captured by SoS. Also, since the planted clique lower bounds are only for logarithmic degree SoS, such a reduction would only be able to prove logarithmic degree SoS lower bounds on Sparse PCA. % \cite{BHKKMP16} can be directly reduced to prove SoS lower bounds for Sparse PCA.
%Moreover, based on our work, we suspect even this will require new ideas. %\gnote{is this ok?}

%If we assume the input vectors form the rows of a $m \times d$ matrix $S$ then the most natural approach is to find the $k$-sparse unit vector $x$ that maximizes $x^TS^TSx = \norm{Sx}^2$. Hence, we can frame the average case certification problem as follows.

%\begin{quote}
%\em{Given an $m \times d$ matrix $S$ where each entry is chosen independently from $\GN(0, 1)$, certify an upper bound on $\norm{Sx}$ over $k$-sparse unit vectors $x$.}
%\end{quote}

%Recently, \cite{sparse_pca_focs20} studied upper bounds on the performance of a slightly modified SoS program and used them to design robust algorithms for the Wishart model of Sparse PCA. In particular, in the weak signal regime $m \lesssim \frac{d}{\lda^2}$ that we assume in \cref{cor: spca_main}, they show that degree $t$ SoS roughly certifies $\norm{Sx}^2 \le m + k \sqrt{\frac{m\log d}{t}}$. Since we also assume $m \le \frac{k^2}{\lda^2}$ in \cref{cor: spca_main}, we observe that our lower bound tightly matches this upper bound, up to lower order terms.

% \cite{sparse_pca_focs20} also obtain SoS upper bounds in the strong signal regime $m \gtrsim \frac{d}{\lda^2}$ where they prove that if $m \le \tilde{O}(d^{\frac{1}{t}})$, then degree $t$ SoS certifies an upper bound of $O(\sqrt{kt}\left(\frac{d}{k}\right)^{\frac{1}{2t}})$.

%We remark that if $m$ does not satisfy the bounds in \cref{cor: spca_main}, i.e., if $m \gtrsim \frac{d}{\lda^2}$ or $m \gtrsim  \frac{k^{2}}{\lda^2}$, then efficient algorithms exist that almost match the guarantees of the best statistical algorithms for the Wishart model of Sparse PCA.
%Concretely, if we assume $m \ge \tilde{\Omega}(\frac{k^2}{\lda^2})$, then there exist efficient algorithms for Sparse PCA (e.g. \cite{johnstone_lu2009, d2004direct, amini_wainwright2008, krauthgamer2015, deshpande2016, sparse_pca_focs20}).
%On the other hand, if $m \gtrsim \frac{d}{\lda^2}$, then a simple spectral algorithm can be shown to be statistically optimal (e.g. \cite{berthet2013, sparse_pca_focs20}).

\subsection{An overview of the machinery: All three results from a single main theorem}

Now that we have described our results, 
%seen a flavor of the kind of results we are aiming to show
we want to highlight that all three results are obtained via applications of one main theorem, which we call the machinery. \cref{thm: plds_main}, \cref{thm: tpca_main} and \cref{thm: spca_main} all essentially boil down to showing that a large moment matrix $\Lda$ is PSD. To show this, the machinery constructs certain \emph{coefficient matrices} from $\Lda$ and gives conditions on these coefficient matrices which are sufficient to guarantee that $\Lda$ is PSD with high probability. In this section, we give an informal sketch of the machinery and how it generalizes the techniques used to prove the SoS lower bound for planted clique \cite{BHKKMP16}. We also motivate some of the conditions that arise in the machinery.
\subsubsection{Shapes and graph matrices}
Before we can describe how our machinery works, we need to describe shapes and graph matrices, which were originally introduced by \cite{BHKKMP16, medarametla2016bounds} and later generalized in \cite{AMP20}. Both the planted clique analysis and our analysis use shapes and graph matrices.

%Both the analyses use the notion of shapes and graph matrices which were originally introduced by \cite{BHKKMP16, medarametla2016bounds} and later generalized in \cite{AMP20}. We use the generalized graph matrices in our analysis. 

Shapes $\al$ are graphs that contain extra information about the vertices. Corresponding to each shape $\al$, there is a matrix-valued function (i.e. a matrix whose entries depend on the input) $M_{\al}$ that we call a graph matrix. Graph matrices are analogous to a Fourier basis, but for matrix-valued functions that exhibit a certain kind of symmetry. In our setting, $\Lda$ will be such a matrix-valued function, so we can decompose $\Lda$ as a linear combination of graph matrices.

Shapes and graph matrices have several properties which make them very useful to work with. First, $\norm{M_{\al}}$ can be bounded with high probability in terms of simple combinatorial properties of the shape $\al$. Second, if two shapes $\alpha$ and $\beta$ match up in a certain way, we can combine them to form a larger shape $\alpha \circ \beta$. We call this operation shape composition. Third, each shape $\al$ has a canonical decomposition into three shapes, the left, middle and right parts of $\al$, which we call $\sigma$, $\tau$, and ${\sigma'}^T$. For this canonical decomposition, we have that $\alpha = \sigma \circ \tau \circ {\sigma'}^T$ and $M_{\alpha} \approx M_{\sigma}M_{\tau}M_{{\sigma'}^T}$ \footnote{Actually, due to a technical issue related to automorphism groups, this equation is off by a multiplicative constant. For details, see Lemma \ref{lm:morthsimplereexpression}.}. This decomposition turns out to be crucial for both the planted clique analysis and our analysis.
\subsubsection{Summary of the SoS lower bound for planted clique and the machinery}
%The machinery compared to the SoS lower bound proof in Planted Clique \cite{BHKKMP16}}
We now give a brief summary of the techniques for the SoS lower bound for planted clique and for our machinery. We elaborate on these steps in \cref{ideadescriptionsubsection}, we formally describe these steps in \cref{sec: informal_statement}, and we carry out these steps in full generality in \cref{sec: technical_def_and_main_theorem} and \cref{sec: proof_of_main}.


%This will be useful for our analysis because the product of the graph matrices corresponding to the three parts will be approximately $M_{\al}$.

%When working with SoS matrices, it's convenient to decompose them into "graph matrices". Graph matrices $M_{\al}$ indexed by "shapes" $\al$, are analogous to a Fourier basis, but for matrix valued functions that exhibit a certain kind of symmetry. Here, the shapes $\al$ are essentially simple graphs that contain extra information about the vertices. Importantly, each $\al$ will correspond to a unique matrix $M_{\al}$ and the fact that a large matrix $M_{\al}$ can be represented graphically will be of great use.

%There is also a canonical way to split the shape $\al$ into three other shapes called the left part $\sig$, middle part $\tau$ and the right part $\sig'^T$. They are graphically easy to describe, induce many nice properties of the corresponding matrices and the corresponding matrices will satisfy the approximately equality $M_{\al} \approx M_{\sig}M_{\tau}M_{\sig'^T}$.

%Graph matrices have been studied and used in many works such as \cite{medarametla2016bounds, BHKKMP16, AMP20, sklowerbounds, cai2020spectrum}. We will formally define them in \cref{sec: informal_statement}.

For planted clique, the SoS lower bound analysis works as follows%\footnote{actually, the planted clique paper keeps everything in terms of sums of ribbons (see***) and only combines them into graph matrices at the end.}
\begin{enumerate}
	\item Using the technique of pseudo-calibration, construct a candidate moment matrix $\Lda$.
	\item Decompose the moment matrix $\Lda$ as a linear combination $\Lda = \sum_{\text{shapes } \alpha}{\lambda_{\alpha}M_{\alpha}}$ of graph matrices $M_{\alpha}$.
	\item For each shape $\alpha$, decompose $\alpha$ into a left part $\sigma$, a middle part $\tau$, and a right part ${\sigma'}^T$. % based on its leftmost and rightmost minimum vertex separators. 
	We then have that $M_{\alpha} \approx M_{\sigma}M_{\tau}M_{{\sigma'}^T}$. 
	%More precisely, with high probability, 
	%\[
	%\norm{M_{\alpha} - M_{\sigma}M_{\tau}M_{{\sigma'}^T}} \ll \norm{M_{\alpha}}
	%\]
	\item Using the approximate decompositions $M_{\alpha} \approx M_{\sigma}M_{\tau}M_{{\sigma'}^T}$, give an approximate decomposition $\Lda \approx LQL^T$ of $M$ where $Q \succeq 0$ with high probability.
	\item Show that with high probability, $\Lda = LQL^T - (LQL^T - M) \succeq 0$ by carefully analyzing the difference $LQL^T - M$ using similar techniques.
\end{enumerate}

For our machinery, we use a similar framework. The key innovation of our machinery is that we introduce coefficient matrices (step 4) and carry out the analysis in terms of these coefficient matrices.
\begin{enumerate}
	\item Construct a candidate moment matrix $\Lda$. This can be done either using pseudo-calibration or in a more ad-hoc manner.
	\item Decompose the moment matrix $\Lda$ as a linear combination $\Lda = \sum_{\text{shapes } \alpha}{\lambda_{\alpha}M_{\alpha}}$ of graph matrices $M_{\alpha}$.%, akin to Fourier decomposition. 
	\item For each shape $\alpha$, decompose $\alpha$ into a left part $\sigma$, a middle part $\tau$, and a right part ${\sigma'}^T$.
	\item Based on the coefficients $\lambda_{\alpha}$ and the decompositions of the shapes $\alpha$ into left, middle, and right parts, construct coefficient matrices $H_{Id_U}$ and $H_{\tau}$.
	%, which just rearrange these Fourier coefficients in different matrices.
	\item Based on the coefficient matrices $H_{Id_U}$ and $H_{\tau}$, obtain an approximate PSD decomposition of $\Lda$.
	\item Show that the error terms (which we call intersection terms) can be bounded by the approximate PSD decomposition of $\Lda$.
\end{enumerate}
We show that this analysis will succeed as long as three conditions on the coefficient matrices are satisfied (see \cref{sec: informal_statement} for a qualitative statement of these conditions and \cref{sec: technical_def_and_main_theorem} for the precise statement of these conditions). Thus, in order to use our machinery to prove sum of squares lower bounds, it is sufficient to do the following.
\begin{enumerate}
    \item Construct a candidate moment matrix $\Lda$.
    \item Decompose the moment matrix $\Lda$ as a linear combination $\Lda = \sum_{\text{shapes } \alpha}{\lambda_{\alpha}M_{\alpha}}$ of graph matrices $M_{\alpha}$ (akin to Fourier decomposition) and find the corresponding coefficient matrices.
    \item Verify the required conditions on the coefficient matrices.
\end{enumerate}
%\subsubsection{The machinery}

%In this paper, we investigate how generally the techniques used for planted clique can be applied. We show that by constructing coefficient matrices containing the coefficients $\lambda_{\alpha}$, we can give relatively simple conditions on these coefficient matrices which are sufficient to ensure that the moment matrix $\Lda$ is PSD with high probability. We show that these conditions can be applied with the same generality as the vastly generalized graph matrices studied in \cite{AMP20}, which will be formally defined in \cref{sec: technical_def_and_main_theorem}. This generality allows the machinery to handle problems such as the Wishart model of sparse PCA which were beyond previous analyses.

%Our machinery can be used as follows to prove sum of squares lower bounds as follows.
%\begin{enumerate}
%	\item Construct a candidate moment matrix $\Lda$. This can often be done using pseudo-calibration, but it can also be done in a more ad-hoc manner.
%	\item Decompose the moment matrix $\Lda$ as a linear combination $\Lda = \sum_{\text{shapes } \alpha}{\lambda_{\alpha}M_{\alpha}}$ of graph matrices, akin to Fourier decomposition. 
%	\item Based on the coefficients $\lambda_{\alpha}$, construct coefficient matrices $H_{Id_U}$ and $H_{\tau}$, which just rearrange these Fourier coefficients in different matrices.
%	\item Verify the required conditions on these coefficient matrices.
%\end{enumerate}

%We highlight that the notion of coefficient matrices, is a key difference from prior works and is an important conceptual contribution of our work, that makes this entire PSDness pipeline almost mechanical for many problems.

\subsubsection{A sketch of the intuition behind the machinery conditions}\label{ideadescriptionsubsection}

%In this section, we describe some ideas behind our machinery, that will help motivate the coefficient matrices and the conditions that appear in the machinery.

%For showing SoS lower bounds, we have a candidate moment matrix $\Lda$ and our goal is to show $\Lda \succeq 0$ with high probability. For example, in the case of planted clique, $\Lda$ has rows and columns indexed by sub-tuples of $[n]$ of size at most $d$, such that
%\[\Lda[I, J] = \sum_{E:E \text{ is small}} \left(\frac{k}{n}\right)^{|I \cup J \cup V(E)|} \chi_E\]
%for all sub-tuples $I, J$ of $[n]$ of size at most $d$. We would like to prove that $\Lda \succeq 0$ with high probability.

%The machinery gives a set of conditions under which we can show that $\Lda \succeq 0$ with high probability. Our first step will be to decompose $\Lda$ into a linear combination of graph matrices.
\begin{comment}
\paragraph{Graph matrices}

Graph matrices were originally introduced by \cite{BHKKMP16, medarametla2016bounds} and later generalized in \cite{AMP20}. We use the generalized graph matrices in our analysis.

Each graph matrix is a matrix valued function of the input, that can be identified by a graph with labeled edges that we call a shape. Informally, graph matrices will form a basis for all matrix valued functions of the input that have a certain symmetry. In particular, $\Lda$ is one such matrix valued function and can thus be decomposed into graph matrices. For a shape $\al$, the graph matrix associated to $\al$ is denoted by $M_{\al}$.

Graph matrices have several useful properties. Firstly, $\norm{M_{\al}}$ can be bounded with high probability in terms of simple combinatorial properties of the shape $\al$. Secondly, when we multiply two graph matrices $M_{\al}, M_{\beta}$ corresponding to shapes $\al, \beta$, it approximately equals the graph matrix $M_{\al \circ \beta}$ where the shape $\al \circ \beta$, called the composition of the two shapes $\al$ and $\beta$, is easy to describe combinatorially.

These makes graph matrices a convenient tool to analyze the moment matrix. In our setting, the moment matrix decomposes as $\Lda = \sum \lda_{\al} M_{\al}$ where the sum is over all shapes $\al$ and $\lda_{\al} \in \RR$ are the coefficients that arise from pseudo-calibration.

\paragraph{Decomposing Shapes}

For graph matrices $\al, \beta$, $M_{\al}M_{\beta} \approx M_{\al \circ \beta}$ where we define the composition of two shapes $\al \circ \beta$ to be a larger shape that is obtained by concatenating the shapes $\al, \beta$. This equality is only approximate and handling it precisely is a significant source of difficulty in our analysis. Shape composition is also associative, hence we can define composition of three or more shapes.

A crucial idea for our machinery is that for any shape $\al$, there exists a canonical and unique decomposition of $\al$ as $\sig \circ \tau \circ \sig'^T$ satisfying some nice structural properties, for shapes $\sig, \tau$ and $\sig'^T$. Here, $\sig, \tau, \sig'^T$ are called the left part, the middle part and the right part of $\al$ respectively.
Using this, our moment matrix can be written as
\[\Lda = \sum_{\al}\lda_{\al}M_{\al} = \sum_{\sig, \tau, \sig'} \lda_{\sig\circ\tau\circ\sig'^T}M_{\sig\circ\tau\circ\sig'^T}\]
\end{comment}

\paragraph{Giving an approximate PSD factorization}
As discussed above, we decompose the moment matrix $\Lda$ as a linear combination $\Lda = \sum_{\text{shapes } \alpha}{\lambda_{\alpha}M_{\alpha}}$ of graph matrices $M_{\alpha}$. We then decompose each $\alpha$ into left, middle, and right parts $\sigma$, $\tau$, and ${\sigma'}^T$. We now have that 
\[
\Lda = \sum_{\alpha = \sigma \circ \tau \circ {\sigma'}^T}{\lambda_{\sigma \circ \tau \circ {\sigma'}^T}M_{\sigma \circ \tau \circ {\sigma'}^T}}
\]

We first consider the terms $\sum_{\sig, \sig'} \lda_{\sig \circ \sig'^T}M_{\sig \circ \sig'^T} \approx \sum_{\sig, \sig'} \lda_{\sig \circ \sig'^T}M_{\sig} M_{\sig'^T}$ where $\tau$ corresponds to an identity matrix and can be ignored. 

If there existed real numbers $v_{\sig}$ for all left shapes $\sig$ such that $\lda_{\sig \circ \sig'^T} = v_{\sig}v_{\sig'}$, then we would have
\[
\sum_{\sig, \sig'} \lda_{\sig \circ \sig'^T}M_{\sig} M_{\sig'^T} = \sum_{\sig, \sig'} v_{\sig}v_{\sig'}M_{\sig} M_{\sig'^T} = (\sum_{\sig} v_{\sig}M_{\sig})(\sum_{\sig} v_{\sig}M_{\sig})^T \succeq 0
\]
which shows that the contribution from these terms is positive semidefinite. In fact, this turns out to be the case for the planted clique analysis. However, this may not hold in general. To handle this, we note that the existence of $v_{\sig}$ can be relaxed as follows: Let $H$ be the matrix with rows and columns indexed by left shapes $\sig$ such that $H(\sig, \sig') = \lda_{\sig \circ \sig'^T}$. Up to scaling, $H$ will be one of our coefficient matrices. If $H$ is positive semidefinite then the contribution from these terms will also be positive semidefinite. In fact, this will be the first condition of our main theorem, the qualitative version of which can be found in \cref{informalmaintheoremstatement}.

\paragraph{Handling terms with a non-trivial middle part}

Unfortunately, we also have terms $\lda_{\sig \circ \tau \circ \sig'^T}M_{\sig \circ \tau \circ \sig'^T}$ where $\tau$ is non-trivial. Our strategy will be to charge these terms to other terms.

For the sake of simplicity, we will describe how to handle one term. A starting point is the following inequality. For a left shape $\sig$, a middle shape $\tau$, a right shape $\sig'^T$, and real numbers $a, b$,
\[(a M_{\sig} - bM_{\sig'}M_{\tau^T})(a M_{\sig} - bM_{\sig'}M_{\tau^T})^T \succeq 0\]
which rearranges to
\begin{align*}
ab(M_{\sig}M_{\tau}M_{\sig'^T} + (M_{\sig}M_{\tau}M_{\sig'^T})^T) &\preceq a^2M_{\sig}M_{\sig^T} + b^2M_{\sig'}M_{\tau^T}M_{\tau}M_{\sig'^T}\\
&\preceq a^2M_{\sig}M_{\sig^T} + b^2\norm{M_{\tau}}^2M_{\sig'}M_{\sig'^T}
\end{align*}

If $\lda_{\sig \circ \tau \circ \sig'^T}^2\norm{M_{\tau}}^2 \le \lda_{\sig \circ \sig^T}\lda_{\sig' \circ \sig'^T}$, then we can choose $a, b$ such that $a^2 \le \lda_{\sig \circ \sig^T}, b^2 \norm{M_{\tau}}^2 \le \lda_{\sig' \circ \sig'^T}$ and $ab = \lda_{\sig \circ \tau \circ \sig'^T}$. This will approximately imply
\[\lda_{\sig \circ \tau \circ \sig'^T}(M_{\sig \circ \tau \circ \sig'^T} + M_{\sig \circ \tau \circ \sig'^T}^T) \preceq \lda_{\sig \circ \sig^T}M_{\sig \circ \sig^T} + \lda_{\sig' \circ \sig'^T}M_{\sig' \circ \sig'^T}\]
which will give us a way to charge terms with a nontrivial middle part against terms with a trivial middle part.

While we could try to apply this inequality term by term, it is not strong enough to give us our results. Instead, we generalize this inequality to work with the entire set of shapes $\sig, \sig'$ for a fixed $\tau$. This will lead us to the second condition of our main theorem, the qualitative version of which can be found in \cref{informalmaintheoremstatement}.

\paragraph{Handing intersection terms}

There's one important technicality in the above heuristic calculations. Whenever we decompose $\alpha$ into left, middle, and right parts $\sigma$, $\tau$, and ${\sigma'}^T$, $M_{\sigma}M_{\tau}M_{{\sigma'}^T}$ is only approximately equal to $M_{\alpha} = M_{\sigma \circ \tau \circ {\sigma'}^T}$. All the other error terms have to be carefully handled in our analysis. We call these terms intersection terms.

These intersection terms themselves turn out to be graph matrices and our strategy is to now recursively decompose them into $\sig_2 \circ \tau_2 \circ \sig_2'^T$ and apply the previous ideas. To do this methodically, we employ several ideas such as the notion of intersection patterns and the generalized intersection tradeoff lemma (see \cref{sec: proof_of_main}). Properly handling the intersection terms is one of the most technically intensive parts of our work. %\gnote{...but this paper has done the work so future works don't have to} 
This analysis leads us to the third condition of the main theorem, the qualitative version of which can be found in \cref{informalmaintheoremstatement}.

\paragraph{Applying the machinery}

To apply the machinery to our problems of interest, we verify the spectral conditions that our coefficients should satisfy and then we can use our main theorem. The Planted slightly denser subgraph application is straightforward and will serve as a good warmup to understand our machinery. In the applications to Tensor PCA and Sparse PCA, the shapes corresponding to the graph matrices with nonzero coefficients have nice structural properties that will be crucial for our analysis. We exploit this structure and use novel charging arguments to verify the conditions of our machinery.

\subsubsection{A summary of our contributions}
\begin{comment}
\subsubsection{Power and limitations of the machinery}
We note that our machinery has the same level of generality as the generalized graph matrices in \cite{AMP20}, which is quite general. In particular, our machinery can handle inputs This generality allows our machinery to handle problems such as the Wishart model of Sparse PCA which were outside the range of previous lower bound analyses for sum of squares. 

That said, in our experience, in order for the machinery to work well, we need the coefficients $\lambda_{\alpha}$ to decay exponentially in the number of vertices and edges of $\alpha$ and we need this decay to be precise. This is an important reason why our machinery has trouble handling hard global constraints

It is an interesting question whether or not our machinery can be applied to problems on sparse inputs. On the one hand, qualitatively, there is 
\end{comment}
\paragraph{The machinery} In this work, we have attempted to drastically simplify the notoriously hard task of proving PSDness for SoS lower bounds to verifying relatively simple conditions that are assembled from the candidate moment matrix. Coefficient matrices are simple matrices whose entries are filled in a specific but well defined manner with the Fourier coefficients of $\Lda$, i.e. coefficients $\lda_{\al}$ for which we can write $\Lda = \sum_{\al} \lda_{\al} M_{\al}$. Here, $M_{\al}$ are called graph matrices, that will play the part of a Fourier basis. Indeed, they can be thought of as an analogue for the Fourier basis for large matrices that satisfy a certain type of symmetry.

The conditions, which are relatively easy to verify for specific applications, moreover give the right tradeoffs for SoS lower bounds that can be shown via coefficient decay techniques. That is, the bounds  $\lda \ll n^{k/4}$ for Tensor PCA or the bound $m \ll \min(d / \lda^2, k^2/\lda^2)$ for the Wishart model of Sparse PCA, almost naturally appear when applying the machinery on these problems. Moreover, as we saw in \cref{sec: prior_work}, these thresholds in fact match the best known algorithmic guarantees, thereby giving conclusive evidence of the correct computational threshold behavior of these problems.

\paragraph{Applicability to certification problems}
The machinery works well for problems where the Fourier coefficients of the candidate moment matrix exhibit a sort of decay behavior. This is akin to saying larger Fourier coefficients should be smaller in the Fourier decomposition. Such coefficient decay is present in many standard certification problems once we find a good planted distribution. Sometimes, noise can be easily introduced to the problem instance to force such kinds of decay, at a cost of slightly lowering the integrality gap we set out to prove, say from $n^{k/4}$ to $n^{k/4 - \eps}$ for a small $\eps > 0$.

The machinery in this work applies for both dense and sparse problems alike. Dense problems include certification problems on $G_{n, 1/2}$ or statistics problems with inputs being standard Gaussian inputs. Sparse problems include problems on $G_{n, p}$ for $p = n^{\eps}$ or statistics problems with inputs having bounded sub-Gaussian norm. While we have optimized our functions for dense problems, the general main theorem is readily applicable, with almost no modifications, for sparse problems as well. For sparse problems, to get the tightest possible tradeoffs, the functions might have to be optimized even further to reflect the behavior of random matrices on these sparse inputs but we haven't attempted this in this work. % but recent work has obtained such optimized functions and we expect them to work well with the machinery. %\gnote{keep this last sentence?}

\paragraph{Other contributions}
While the machinery builds on ideas from the work on Planted Clique, the kind of matrices they use, known as graph matrices are not powerful enough to handle problems on tensors or Gaussian inputs. This is addressed in the work of \cite{AMP20} who introduce the notion of generalized graph matrices. When trying to apply generally the same techniques, there are numerous difficulties that have to be overcome and we systematically handle them using both new ideas and by significantly generalizing known techniques.

We introduce and use the notion of coefficient matrices which attempt to abstract out the precise conditions that are needed in such SoS lower bound proofs. By making the dominant and non-dominant terms in the PSD decomposition explicit, the coefficient matrices shed light on the intrinsic structure of the problem at hand, to prevent getting lost in the technical details.

%We emphasize again that $\Lda$ is obtained via pseudo-calibration in our applications, but it's not necessary that that be the case.

%\gnote{To be added: Any other contributions we want to highlight early on}

\subsection{Comparison to Other Sum-of-Squares Lower Bounds on Certification Problems}
\cite{BHKKMP16} proved sum of squares lower bounds for the planted clique problem. Our machinery vastly generalizes the techniques of their paper. For a specific technical reason, our machinery actually doesn't recover the same lower bounds as planted clique in particular (See \cref{rmk: planted_clique_failure}). That said, this is because we have attempted to keep our framework as general as possible so that it is applicable to other problems, at the cost of losing a specific technicality that's needed for planted clique in particular.

\cite{hop17} remarked that the techniques used in \cite{BHKKMP16} can be used to give Sum-of-Squares lower bounds for $\pm{1}$ variants of tensor PCA and sparse PCA, though this is not made explicit. In this paper, we use our machinery to make these lower bounds explicit. We also handle the Wishart model of sparse PCA, which is more natural and significantly harder to prove lower bounds for. In particular, the bounds we prove do not follow solely from the techniques used in prior works.

\cite{KothariMOW17} proved that for random constraint satisfaction problems (CSPs) where the predicate has a balanced pairwise independent distribution of solutions, with high probability, degree $\Omega(n)$ SoS is required to certify that these CSPs do not have a solution. While they don't state it in this manner, the pseudo-expectation values used by \cite{KothariMOW17} can also be derived using pseudo-calibration \cite{rajendran2018combinatorial, brown2020extended}. The analysis for showing that the moment matrix is PSD is very different. It is an interesting question whether or not it is possible to unify these analyses.

\cite{MRX20} showed that it's possible to lift degree $2$ SoS solutions to degree $4$ SoS solutions under suitable conditions, and used it to obtain degree $4$ SoS lower bounds for average case $d$-regular Max-Cut and the Sherrington Kirkpatrick problem. Their construction is inspired by pseudo-calibration and their analysis also goes via graph matrices.

Recently, \cite{sklowerbounds} proved degree $n^{\eps}$ SoS lower bounds for the Sherrington-Kirkpatrick problem via an intermediate problem known as Planted Affine Planes. Their construction and analysis also goes via pseudo-calibration and graph matrices, but since the constructed moment matrix had a nontrivial nullspace, they had to use different techniques to handle them. However, once this nullspace is taken into account, the moment matrix is dominated by its expected value. After this preprocessing, our machinery would imply their result but using it would be overkill.

\cite{kunisky2020} recently proposed a technique to lift degree $2$ SoS lower bounds to higher levels and applied it to construct degree $6$ lower bounds for the Sherrington-Kirkpatrick problem. Interestingly, their construction does not go via pseudo-calibration.

\subsection{Related Algorithmic Techniques}\label{subsec: related_techniques}

\paragraph{Low degree polynomials} Consider a problem where the input is sampled from one of two distributions and we would like to identify which distribution it was sampled from. Usually, one distribution is the completely random distribution while the other is a planted distribution that contains a given structure not present in the random distribution. In this setting, a closely related method is to use low degree polynomials to try and distinguish the two distributions. More precisely, if there is a low degree polynomial such that its expected value on the random distribution is very different than its expected value on the planted distribution, this distinguishes the two distributions.
%Roughly speaking, this method corresponds to checking whether $\pE[1]$ is well-behaved or not as a function of the input (see Appendix ***\gnote{*} for a brief discussion). 
Recently, this method has been shown to be an excellent heuristic, as it recovers the conjectured hardness thresholds for several problems and is considerably easier to analyze \cite{hop17, hop18, kunisky19notes}.

Under some conditions, the SoS hierarchy is at least as powerful as low degree polynomials \cite{hop17}. It is an important open question whether low degree polynomials generally have the same power as the SoS hierarchy or if there are situations where the SoS hierarchy is more powerful. On the one hand, we know of very few examples where low degree polynomials fail yet some polynomial time algorithm succeeds and the examples we do know of are somewhat contrived \cite{holmgren2020counterexamples}. On the other hand, to the best of our knowledge there is no known way to obtain sum of squares lower bounds from low degree polynomial lower bounds. In this paper, we confirm that for tensor PCA and the Wishart model of sparse PCA with slightly adjusted planted distributions, the SoS hierarchy is no more powerful than low-degree polynomials. %This is a surprising result considering the vast expressability of SoS compared to low degree polynomials.

\paragraph{The Statistical Query Model}
The statistical query model is another popular restricted class of algorithms introduced by \cite{kearns1998efficient}. In this model, for an underlying distribution, we can access it by querying expected value of functions of the distribution. Concretely, for a distribution $D$ on $\RR^n$, we have access to it via an oracle that given as query a function $f: \RR^n \to [-1, 1]$ returns $\EE_{x \sim D} f(x)$ upto some additive adversarial error. SQ algorithms capture a broad class of algorithms in statistics and machine learning and has also been used to study information-computation tradeoffs. There has also been significant work trying to understand the limits of SQ algorithms (e.g. \cite{feldman2017statistical, feldman2018complexity, diakonikolas2017statistical}). The recent work \cite{brennan2020statistical} showed that low degree polynomials and statistical query algorithms have equivalent power under mild conditions. It's an interesting open question whether or not SQ algorithms have the same power as Sum-of-Squares algorithms. An important distinction to note is that SQ algorithms do not take into account the complexity of the oracle whereas SoS studies the whole computational aspect of the problem. Therefore, with our current knowledge, SoS lower bounds are strictly stronger evidence of intrinsic hardness of problems.

\subsection{Organization of the paper}

In this work, we occasionally distinguish between the qualitative and quantitative versions of theorem statements. Qualitative theorem statements capture the essence of the inequalities we prove, and serve to illustrate the main forms of the bounds we desire, without getting lost in the details. Quantitative theorems on the other hand build on their qualitative counterparts by stating the precise bounds that are needed.

The remainder of this paper is organized as follows. In \cref{sec: prelim}, we give some preliminaries. In particular, we describe the Sum-of-Squares hierarchy and present a brief overview of the machinery and some proof techniques that we use. In \cref{sec: informal_statement}, we present the informal statement of the main theorem. In \cref{sec: plds_qual}, \cref{sec: tpca_qual} and \cref{sec: spca_qual}, we qualitatively verify the conditions of the machinery for planted slightly denser subgraph, tensor PCA, and sparse PCA respectively. While these sections only verify the qualitative conditions, the results in these sections are precise and will be reused in \cref{sec: plds_quant}, \cref{sec: tpca_quant} and \cref{sec: spca_quant} to fully verify the conditions of the machinery. In \cref{sec: technical_def_and_main_theorem}, we introduce all the formal definitions and state the main theorem in full generality. In \cref{sec: proof_of_main}, we prove the main theorem while abstracting out the choice of several functions. In \cref{sec: choosing_funcs}, we choose these functions so that that they satisfy the conditions needed for our main theorem. In Section \ref{sec: showing_positivity}, we give tools for verifying a technical condition of our machinery which is related to truncation error. Finally, in \cref{sec: plds_quant}, \cref{sec: tpca_quant} and \cref{sec: spca_quant}, we verify all the conditions necessary to prove \cref{thm: plds_main}, \cref{thm: tpca_main} and \cref{thm: spca_main} respectively.

%\gnote{We may need to add a suggested reading for a first pass.}
For a first pass, the reader is encouraged to read the informal description of the machinery as outlined in \cref{sec: informal_statement}. Then, they can read any of the qualitative bounds \cref{sec: plds_qual}, \cref{sec: tpca_qual}, \cref{sec: spca_qual} to get a sense of how the machinery can be applied to these problems qualitatively. For readers interested in seeing complete proofs of the main applications, they can read parts of the quantitative bounds sections of their favorite problem(s) from among \cref{sec: plds_quant}, \cref{sec: tpca_quant}, \cref{sec: spca_quant}. To understand the details of the machinery, the reader may then read the formal definitions and theorem statement in \cref{sec: technical_def_and_main_theorem} whose proof follows in section \cref{sec: proof_of_main}. In \cref{sec: technical_def_and_main_theorem}, for the sake of clarity, the reader is given a choice of generality in the definitions and theorem statement.

==> machinery/preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%% FLAG FOR CONFERENCE VERSION %%%%%
\def\confversion{0}
\def\ifconf{\ifnum\confversion=1}
\def\ifnotconf{\ifnum\confversion=0}

%\documentclass[11 pt]{article}
%%%%%%%%% options for the file macros.tex

%\def\showauthornotes{0}
%\def\showkeys{0}
%\def\showdraftbox{0}

%\input{macros}
\let\pref=\prettyref

%\usepackage{tikz}
%\usetikzlibrary{shapes.geometric}
%\usepackage{float}
%
%\usepackage{thm-restate}
\usepackage{titlesec}
\usepackage{comment}

%%%%%%% Additional macros for this paper

\usepackage{scalerel,stackengine}
\stackMath
\newcommand\reallywidehat[1]{%
	\savestack{\tmpbox}{\stretchto{%
			\scaleto{%
				\scalerel*[\widthof{\ensuremath{#1}}]{\kern-.6pt\bigwedge\kern-.6pt}%
				{\rule[-\textheight/2]{1ex}{\textheight}}%WIDTH-LIMITED BIG WEDGE
			}{\textheight}% 
		}{0.5ex}}%
	\stackon[1pt]{#1}{\tmpbox}%
}
\parskip 1ex

%\newcommand{\RR}{\mathbb{R}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\CZ}{\mathcal{Z}}
\newcommand{\EE}{\mathop{\mathbb{E}}}
\newcommand{\GN}{\mathcal{N}}
\newcommand{\MM}{\mathcal{M}}
\newcommand{\sig}{\sigma}
\newcommand{\Sig}{\Sigma}
\newcommand{\al}{\alpha}
\newcommand{\lda}{\lambda}
\newcommand{\Lda}{\Lambda}
\newcommand{\Gam}{\Gamma}
\newcommand{\gam}{\gamma}
\newcommand{\Del}{\Delta}
\newcommand{\del}{\delta}

\newcommand{\matindex}[1]{\mbox{\scriptsize#1}}% Matrix index

\newcommand{\tens}[2] {\ensuremath{#1 ^ {\otimes #2}}}

\newcommand{\cN}{\mathcal{N}}
\def\ZZ{{\mathbb Z}}
\def\QQ{{\mathbb Q}}
%\def\RR{{\mathbb R}}
\def\TT{{\mathcal{C} T}}
\def\KK{{\mathcal{C} K}}
\newcommand{\hus}{\hfill\break}
\newcommand{\bull}{\textbullet\;\;}
\def\iso{{\operatorname{\ \approx \ }}}   % isomorphism
\def\im{{\operatorname{im}}}              % image
\def\Hom{{\operatorname{Hom}}}           % homomorphisms
\def\line{{\operatorname{line} \,}}       % line graph
\def\sd{{\operatorname{sd \,}}}           % first edge subdivision graph
\def\coker{{\operatorname{coker}}}        % cokernel
\def\lcm{{\operatorname{lcm}}}             % least common multiple
\newcommand{\gcdd}{\gamma}              
% \def\del{{\partial}}                      % signed incidence matrix
\def\<{{\langle}} \def\>{{\rangle}}       % Inner product
\def\ZC{{Z^\#}}                           % cycle space
\setlength{\textheight}{9in}               
%\setlength{\textwidth}{6in}               % width of text
%\setlength{\oddsidemargin}{0in}           % odd page left margin
%\setlength{\evensidemargin}{0in}          % even page left margin 

\DeclareMathOperator{\Id}{Id}
\newcommand{\iprod}[1]{\langle #1 \rangle}
\DeclareMathOperator{\Tr}{Tr}

%\allowdisplaybreaks

\newtheorem{propn}[theorem]{Proposition}

%\newcommand{\unif}{\in_{\text{R}}}
%\newcommand{\T}{\intercal}
%\let\mod\relax
%\DeclareMathOperator{\mod}{mod}
%\DeclareMathOperator{\GOE}{GOE}
%\DeclareMathOperator{\linspan}{span}
%\DeclareMathOperator{\nullspace}{Null}
%\DeclareMathOperator{\parents}{parents}
%\renewcommand{\E}{\mathop{\mathbb{E}}}

%\newcommand{\pE}{\tilde{\EE}}


%%%%%%%%%%%%%% No bullets
\renewcommand{\labelitemi}{-}

\renewcommand*{\circle}[1]{\scalebox{0.85}{\footnotesize
		\tikz[baseline=(char.base)]{
			\node[shape=circle,draw,inner sep=1.5pt](char) {   \ifx&#1&
				\color{white} $i$
				\else
				$#1$
				\fi};
}}}
\renewcommand*{\square}[1]{\scalebox{0.85}{\footnotesize
		\tikz[baseline=(char.base), square/.style={regular polygon,regular polygon sides=4}]{
			\node[draw,square, inner sep=0.5pt](char) {
				\ifx&#1&
				\color{white} $t$
				\else
				$#1$
				\fi};
}}}

%%%%%%%%%%%%%%% Author Notes	

%\usepackage[top=1in, bottom=1in, left=1in, right=1in]{geometry}


%% \usepackage{fullpage}
%% \usepackage{color,xcolor}

%% % math packages
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{ytableau}
\usepackage{mathtools}
\usepackage{blkarray}
\usepackage{bigstrut}

\usepackage{amsmath,amsthm,amssymb,amscd,epsfig,url}
\usepackage{fullpage}
\usepackage{times}
\usepackage{xcolor}

\usepackage{pgfplots}
\pgfplotsset{compat=1.15}
\usepackage{mathrsfs}
\usetikzlibrary{arrows}
% \pagestyle{empty}

%
%\newcommand{\anote}[1]{\textcolor{blue}{ {\textbf{(Aaron: #1)}}}}
%\newcommand{\gnote}[1]{\textcolor{magenta}{ {\textbf{(Goutham: #1)}}}}

==> machinery/prelim.tex <==
\subsection{The Sum of Squares Hierarchy}\label{subsec: sos}

The SoS hierarchy is a powerful class of algorithms parameterized by it's degree. As we increase the degree, we get progressively stronger algorithms (with longer running times). It's been shown formally to obtain the state-of-the art guarantees for many problems both in the worst case and the average case setting. 
For constant degree SoS, the hierarchy can be optimized in polynomial time\footnote{There is a caveat, see \cite{o2017sos}}. In general, for degree-$d$ SoS, we can solve it in $n^{O(d)}$ time. Most of our applications in this paper focus on showing hardness for the SoS hierarchy when the degree is $n^{\eps}$, which corresponds to a subexponential running time.

We now formally describe the sum of squares hierarchy.
%Here, we describe the hierarchy formally and set up the notation we will use throughout this paper.

\begin{definition}[Pseudo-expectation values]\label{def: pseudoexpectation}
Given polynomial constraints $g_1 = 0$,\ldots,$g_m = 0$, degree $d$ pseudo-expectation values are a linear map $\pE$ from polynomials of degree at most $d$ to $\mathbb{R}$ satisfying the following conditions:
  \begin{enumerate}
    \item $\pE[1] = 1$, \label{pe:normalized}
%    \item $\pE$ is an $\RR$-linear operator, i.e., $\pE[f+cg] = \pE[f] + c\pE[g]$ for every $f,g \in \RR^{\le d}[x_1,\dots,x_n], c \in \RR$, \label{pe:linear}
    \item $\pE[f \cdot g_i] = 0$ for every $i \in [m]$ and polynomial $f$ such that $\deg(f \cdot g_i) \leq d$. \label{pe:feasible}
    \item $\pE[f^2] \geq 0$ for every polynomial $f$ such that $\deg(f^2) \le d$. \label{pe:psdness}
  \end{enumerate}
\end{definition}
The intuition behind pseudo-expectation values is that the conditions on the pseudo-expectation values are conditions that would be satisfied by any actual expected values over a distribution of solutions, so optimizing over pseudo-expectation values gives a relaxation of the problem. Moreover, the conditions on pseudo-expectation values can be captured by a semidefinite program.

In particular, \cref{pe:psdness} in \cref{def: pseudoexpectation} can be reexpressed in terms of a matrix called the moment matrix.

\begin{definition}[Moment Matrix of $\pE$]
Given degree $d$ pseudo-expectation values $\pE$, define the associated moment matrix $\Lda$ to be a matrix with rows and columns indexed by monomials $p$ and $q$ such that the entry corresponding to row $p$ and column $q$ is
  \[
  \Lda[p, q] \defeq \pE\left[pq\right].
  \]
\end{definition}

It is easy to verify that \cref{pe:psdness} in~\cref{def: pseudoexpectation} equivalent to $\Lda \succeq 0$.

For our setting, we are investigating the following kind of question. Given polynomial constraints $g_1 = 0$,\ldots,$g_m = 0$, can degree $d$ SoS certify that some other polynomial $h$ has value at most $c$?

If there do not exist pseudo-expectation values $\pE$ satisfying the conditions in~\cref{def: pseudoexpectation} such that $\pE[h] > c$ then degree $d$ SoS certifies that $\pE[h] \leq c$. More precisely, by duality, there exists a degree $d$ SoS/Positivstellensatz proof that $h \leq c$.

On the other hand, if there exist degree $d$ pseudo-expectation values $\pE$ satisfying the conditions in~\cref{def: pseudoexpectation} such that $\pE[h] > c$ then degree $d$ SoS fails to certify that $h \leq c$. This is what we need to show in order to prove SoS lower bounds on certification problems.

\begin{comment}

We will first introduce the notion of a pseudoexpectation operator for a set of polynomial constraints and then describe the Sum-of-Squares relaxation for a polynomial optimization problem.

For an integer $d$, Let $\RR^{\le d}[x_1, \ldots, x_n]$ be the set of polynomials on $x_1 \ldots, x_n$ of degree at most $d$. We denote the degree of a polynomial
$f \in \RR[x_1,\dots,x_n]$ by $\deg(f)$.

\begin{definition}[Pseudoexpectation operator]\label{def: pseudoexpectation}
  Given polynomial constraints $g_1(x) = 0, \ldots, g_m(x) = 0$ on variables $x_1,\dots,x_n$ such that $deg(g_i) \le D$ for an integer $D \ge 0$. For an even integer $d \ge D$, a degree-$d$ pseudoexpectation operator $\pE$ satisfying these constraints is an operator
  $\pE \colon \RR^{\le d}[x_1,\dots,x_n] \to \mathbb{R}$ satisfying:
  \begin{enumerate}
    \item $\pE[1] = 1$, \label{pe:normalized}
    \item $\pE$ is an $\RR$-linear operator, i.e., $\pE[f+cg] = \pE[f] + c\pE[g]$ for every $f,g \in \RR^{\le d}[x_1,\dots,x_n], c \in \RR$, \label{pe:linear}
    \item $\pE[g_i \cdot f] = 0$ for every $i = 1, \ldots, m$ and $f \in \RR^{\le d}[x_1,\dots,x_n]$ with $\deg(f \cdot g_i) \le d$. \label{pe:feasible}
    \item $\pE[f^2] \ge 0$ for every $f \in \RR^{\le d}[x_1,\dots,x_n]$ with $\deg(f^2) \le d$. \label{pe:psdness}
  \end{enumerate}
\end{definition}

The notion of $\pE$ generalizes the standard expectation operator. The idea is that optimizing over this larger space of pseudoexpectation operators can be formulated as a semidefinite programming problem and hence, will serve as a relaxation of our program that can be solved efficiently.

Formally, consider an optimization task on $n$ variables $x_1, \ldots, x_n \in \RR$ formulated as maximizing a polynomial $f(x)$ subject to polynomial constraints $g_1(x) = 0, \ldots, g_m(x) = 0$. Suppose all the polynomials $f, g_1, \ldots, g_m$ have degree at most $D$.  Then, for an even integer $d \ge D$, the degree $d$ Sum-of-Squares relaxation of this program is as follows: Over all pseudoexpectation operators $\pE$ satisfying $\pE[g_1(x)] = 0, \ldots, \pE[g_m(x)] = 0$, output the maximum value of $\pE[f(x)]$.

To prove an SoS lower bound, we need to exhibit an operator $\pE$ that satisfies these constraints with optimum value of $\pE[f(x)]$ being far away from the true optimum.

In most cases, when constructing $\pE$, the condition \cref{pe:psdness} in \cref{def: pseudoexpectation} is the most technically challenging condition to satisfy. It can be equivalently stated as a positive semidefiniteness condition of an associated matrix called the moment matrix.

To define the moment matrix, we need to set up some more notation.

For an integer $d \ge 0$, let $\calI_d$ denote the set of all tuples $(t_1, \ldots, t_n)$ such that $t_i \ge 0$ for all $i$ and $\sum t_i \le d$. For $I = (t_1, \ldots, t_n) \in \calI_d$, denote by $x^I := x_1^{t_1}x_2^{t_2} \ldots x_n^{t_n}$.

\begin{definition}[Moment Matrix of $\pE$]
For a degree $2d$ pseudoexpectation operator $\pE$ on variables $x_1, \ldots, x_n$, define the associated moment matrix $\Lda$ to be a matrix with rows and columns indexed by $\calI_d$ such that the entry corresponding to row $I$ and column $J$ is
  \[
  \Lda[I, J] \defeq \pE\left[ x^I \cdot x^J \right].
  \]
\end{definition}

It is easy to verify that \cref{pe:psdness} in~\cref{def: pseudoexpectation} equivalent to $\Lda \succeq 0$.

The machinery in this paper provides general conditions under which we can show that with high probability, $\Lda \succeq 0$.
\end{comment}
\subsection{Pseudo-calibration}\label{subsec: pseudocalibration}

To obtain SoS integrality gaps on random instances, we need to construct valid pseudo-expectation values for a random input instance of an optimization problem. Naturally, these pseudo-expectation values will depend on the input. Psuedo-calibration is a heuristic introduced by \cite{BHKKMP16} to construct such candidate pseudo-expectation values almost mechanically by considering a planted distribution supported on instances of the problem with large objective value and using this planted distribution as a guide to construct the pseudo-expectation values. 

Unfortunately, psuedo-calibration doesn't guarantee feasibility of these candidate pseudo-expectation values and the corresponding moment matrix and this has to be verified separately for different problems. This verification of feasibility is relatively easy except for the PSDness condition, which often leads to highly technical and involved analyses. The machinery attempts to mitigate this problem by providing easily verifiable conditions to prove PSDness, regardless of whether the moment matrix was obtained via pseudo-calibration.

For our applications, psuedocalibration is used to obtain a candidate pseudoexpectation operator $\pE$ and a corresponding moment matrix $\Lda$
%, to prove Sum-of-Squares lower bounds 
from the random vs planted problem. This will be the starting point for all our applications. Here, we do not attempt to motivate and describe it in great detail. Instead, we will briefly describe the heuristic, the intuition behind it and show an example of how to use it. A detailed treatment can be found in \cite{BHKKMP16}.

Let $\nu$ denote the random distribution and $\mu$ denote the planted distribution. Let $v$ denote the input and $x$ denote the variables for our SoS relaxation. The main idea is that, for an input $v$ sampled from $\nu$ and any polynomial $f(x)$ of degree at most the SoS degree, pseudo-calibration proposes that for any low-degree test $g(v)$, the correlation of $\pE[f]$ should match in the planted and random distributions. That is,
\[\EE_{v \sim \nu}[\pE[f(x)]g(v)] = \EE_{(x, v) \sim \mu}[f(x)g(v)]\]

Here, the notation $(x, v) \sim \mu$ means that in the planted distribution $\mu$, the input is $v$ and $x$ denotes the planted structure in that instance. For example, in planted clique, $x$ would be the indicator vector of the clique. If there are multiple, pick an arbitrary one.

Let $\calF$ denote the Fourier basis of polynomials for the input $v$. By choosing different basis functions from $\calF$ as choices for $g$ such that the degree is at most $n^{\eps}$ (hence the term low-degree test), we get all lower order Fourier coefficients for $\pE[f(x)]$ when considered as a function of $v$. Furthermore, the higher order coefficients are set to be $0$ so that the candidate pseudoexpectation operator can be written as
\[\pE f(x) = \sum_{\substack{g \in \calF\\deg(g) \le n^{\eps}}} \EE_{v \sim \nu}[\pE[f(x)]g(v)] g(v) = \sum_{\substack{g \in \calF\\deg(g) \le n^{\eps}}} \EE_{(x, v) \sim \mu}[[f(x)]g(v)] g(v)\]

The coefficients $\EE_{(x, v) \sim \mu}[[f(x)]g(v)]$ can be explicitly computed in many settings, which therefore gives an explicit pseudoexpectation operator $\pE$.

One intuition for pseudo-calibration is as follows. The planted distribution is usually chosen to be a maximum entropy distribution which still has the planted structure. This conforms to the philosophy that random instances are hard for SoS, such as the uniform Bernoulli distribution for planted clique or the Gaussian distribution for Tensor PCA. By conditioning on the lower order moments matching such a planted distribution, pseudo-calibration can be interpreted as sort of interpolating between the random and planted distributions by only looking at lower order Fourier characters. This intuition has proven to be successful, since pseudo-calibration been successfully exploited to construct SoS lower bounds for a wide variety of dense as well as sparse problems.

An advantage of pseudo-calibration is that this construction automatically satisfies some nice properties that the pseudoexpectation $\pE$ should satisfy. It's linear in $v$ by construction. For all polynomial equalities of the form $f(x) = 0$ that is satisfied in the planted distribution, it's true that $\pE[f(x)] = 0$. For other polynomial equalities of the form $f(x, v) = 0$ that are satisfied in the planted distribution, the equality $\pE[f(x, v)] = 0$ is approximately satisfied. In most cases, $\pE$ can be mildly adjusted to satisfy these exactly.

The condition $\pE[1] = 1$ is not automatically satisfied but in most applications, we usually require that $\pE[1] = 1 \pm \littleoh(1)$. Indeed, this has been the case for all known successful applications of pseudo-calibration. Once we have this, we simply set our final pseudoexpectation operator to be $\pE'$ defined as $\pE'[f(x)] = \pE[f(x)] / \pE[1]$.

We remark that the condition $\pE[1] = 1 \pm \littleoh(1)$ has been quite successful in predicting the right thresholds between approximability and inapproximability\cite{hop17, hop18, kunisky19notes}.

\paragraph{Example: Planted Clique} 
As an warmup, we review the pseudo-calibration calculation for planted clique. Here, the random distribution $\nu$ is $G(n, \frac{1}{2})$.

The planted distribution $\mu$ is as follows. For a given integer $k$, first sample $G'$ from $G(n, \frac{1}{2})$, then choose a random subset $S$ of the vertices where each vertex is picked independently with probability $\frac{k}{n}$. For all pairs $i, j$ of distinct vertices in $S$, add the edge $(i, j)$ to the graph if not already present. Set $G$ to be the resulting graph.

The input is given by $G \in \{-1, 1\}^{\binom{[n]}{2}}$ where $G_{i, j}$ is $1$ if the edge $(i, j)$ is present and $-1$ otherwise. Let $x_1, \ldots, x_n$ be the boolean variables for our SoS program such that $x_i$ indicates if $i$ is in the clique.

\begin{definition}
Given a set of vertices $V \subseteq [n]$, define $x_V = \prod_{v \in V}{x_v}$.
\end{definition}
\begin{definition}
Given a set of possible edges $E \subseteq \binom{[n]}{2}$, define $\chi_E = (-1)^{|E \setminus E(G)|} = \prod_{(i, j) \in E}G_{i, j}$.
\end{definition}

Pseudo-calibration says that for all small $V$ and $E$,
\[
\EE_{G \sim \nu}\left[\tilde{E}[x_V]\chi_E\right] = \EE_{\mu}\left[x_V{\chi_E}\right]
\]
Using standard Fourier analysis, this implies that if we take 
\[
c_E = \EE_{\mu}\left[x_V{\chi_E}\right] = \left(\frac{k}{n}\right)^{|V \cup V(E)|}
\]
where $V(E)$ is the set of the endpoints of the edges in $E$, then for all small $V$,
\[
\pE[x_V] = \sum_{E:E \text{ is small}}{{c_E}\chi_E} = \sum_{E:E \text{ is small}}{\left(\frac{k}{n}\right)^{|V \cup V(E)|}\chi_E}
\]

Since the values of $\pE[x_V]$ are known, by multi-linearity, this can be naturally extended to obtain values $\pE[f(x)]$ for any polynomial $f$ of degree at most the SoS degree.

%\subsection{Using the machinery}
%
%To apply the machinery to a problem of interest, the intended strategy, at a high level, is as follows
%\begin{enumerate}
%	\item A candidate moment matrix $\Lda$ should be constructed, that has the desired integrality gap. For this purpose, pseudo-calibration can be a useful approach, but ad-hoc constructions have also been shown to be useful.
%	\item We then decompose $\Lda$ into a linear combination of graph matrices $\Lda = \sum_{\al} \lda_{\al}M_{\al}$, akin to decomposing a boolean function in the Fourier basis. In many cases where the input is obtained by independently sampling from a distribution (for example, in $G_{n, 1/2}$, each edge is sampled i.i.d. from the uniform distribution on $\{+1, -1\}$), this is a standard computation.
%	\item The machinery handles the case when the coefficients have a decay term for each new vertex or edge that appears in the shape. This is analogous to larger Fourier coefficients being smaller, in Fourier analysis. So, such a coefficient decay should be present in our setting. In many applications, if the coefficients intrinsically don't have such a decay, this can be amended by adding noise to the underlying distribution. This comes at the cost of losing a factor of say $n^{\eps}$ in the integrality gap, where the instance has size $poly(n)$.
%	\item Because of the coefficient decay, it's natural to expect the dominant terms in the decomposition $\sum_{\al}\lda_{\al}M_{\al}$ to be $\sum_{\sig \circ \sig'^T} \lda_{\sig \circ \sig'^T}M_{\sig \circ \sig'^T}$ and the non-dominant terms to be $\sum_{\sig \circ \tau \circ \sig'^T} \lda_{\sig \circ \tau \circ \sig'^T}M_{\sig \circ \tau \circ \sig'^T}$. Indeed, the machinery gives a set of Fourier theoretic conditions to check, under which this indeed is the case.
%	\item The coefficients $\lda_{\al}$ naturally define shape coefficient matrices $H_{\tau}$ that are just matrices constructed from these coefficients.
%	\item The first step would be to check whether the conjectured dominant term $\sum_{\sig, \sig'^T} \lda_{\sig \circ \sig'^T}M_{\sig \circ \sig'^T}$ is actually PSD. This is done by checking if $H_{Id_U} \succeq 0$ for all $U$, which is the first conditon of \cref{informalmaintheoremstatement}.
%	\item Informally, the second step would to verify if $\lda_{\sig \circ \tau \circ \sig'^T} M_{\sig \circ \tau \circ \sig'^T}$ is dominated by $\lda_{\sig \circ \sig'^T} M_{\sig \circ \sig'^T}$ for all nontrivial $\tau$. For a first back-of-the-hand qualitative calculation, we can ignore all lower order terms and simply check if $B_{norm}(\tau)H_{\tau} \preceq H_{Id_U}$, which is essentially the second condition of \cref{informalmaintheoremstatement}. This inequality captures the intuition we had about dominant and non-dominant terms that we are attempting to prove.
%	\item In the above inequality, we know the coefficients $\lda_{\al}$ and hence the matrices $H_{Id_U}$ and $H_{\tau}$. The remaining term is $B_{norm}(\tau)$. As described earlier, we ignore all lower order terms and instead focus on the power of $n$ (where the input size is $poly(n)$) that arises in this norm bound. For input distributions arising from uniform boolean inputs or standard Gaussians, $B_{norm}(\tau)$ is essentially $\sqrt{n}^{|V(\tau)|-|U_{\tau}|}$, as was shown in \cite{AMP20}. These kind of settings give rise to dense problems that we study in this paper. For input distributions arising from biased distributions such as graphs sampled from $G_{n, p}$ where $p = o(1)$, we can use tighter norm bounds.\gnote{Cite independent-set paper}
%	\item The third main condition we have to verify is the technical condition that arises from intersection terms. That is, we have to check that for all left shapes $\gam$ that arise from intersection terms, we have $H^{-\gamma,\gamma}_{Id_{V_{\gamma}}} \preceq f(\gamma)H_{Id_{U_{\gamma}}}$ for an appropriate $f(\gam)$. In this paper, upto lower order terms, we will essentially set $f(\gam)$ to be $n^{|V(\gam)| - |U_{\gam}|}$. We expect this choice to work for other dense problems as well. But for sparse problems, we need to be more careful in our choice of $f(\gam)$ since it has to carefully balanced against the $B_{norm}(\tau)$ that we use. In such situations, it's advised to directly attempt to use \cref{maintheoremviaproperties}.
%	\item If all the above conditions go through upto lower order terms, then we would be in great shape to carry out the full analysis. We simply have to invoke the main theorems, \cref{simplifiedmaintheorem} and \cref{generalmaintheorem}, to ultimately help us show PSDness of the moment matrix. Much of the nitty-gritties that are involved in the full PSDness proof via this approach, are handled in the background by the machinery.
%\end{enumerate}

==> machinery/proof_of_main.tex <==
In this section, we prove the main theorem under the assumption that the functions $B_{norm}(\alpha)$, $B(\gamma)$, $N(\gamma)$, and $c(\alpha)$ have certain properties. More precisely, we prove the following theorem. 
\begin{theorem}\label{maintheoremviaproperties}
	For all $\epsilon > 0$ and all $\epsilon' \in (0,\frac{1}{20}]$, for any moment matrix 
	\[
	\Lambda = \sum_{U \in \mathcal{I}_{mid}}{M^{orth}_{Id_U}(H_{Id_U})} + \sum_{U \in \mathcal{I}_{mid}}{\sum_{\tau \in \mathcal{M}_U}{M^{orth}_{\tau}(H_{\tau})}},
	\]
	if $B_{norm}(\alpha)$, $B(\gamma)$, $N(\gamma)$, and $c(\alpha)$ are functions such that 
	\begin{enumerate}
		\item With probability at least $(1-\epsilon)$, for all shapes $\alpha \in \mathcal{M}', ||M_{\alpha}|| \leq B_{norm}(\alpha)$.
		\item For all $\tau \in \mathcal{M}'$, $\gamma \in \Gamma_{*,U_{\tau}}$, $\gamma' \in \Gamma_{*,V_{\tau}}$, and all intersection patterns $P \in \mathcal{P}_{\gamma,\tau,\gamma'}$, 
		\[
		B_{norm}(\tau_{P}) \leq B(\gamma)B(\gamma')B_{norm}(\tau)
		\]
		Note: Intersection patterns and $\mathcal{P}_{\gamma,\tau,\gamma'}$ will be defined later, see Definitions \ref{intersectionpatternroughdef} and \ref{setPdefinition}.
		\item For all composable $\gamma_1,\gamma_2$, $B(\gamma_1)B(\gamma_2) = B(\gamma_1 \circ \gamma_2)$.
		\item $\forall U \in \mathcal{I}_{mid}, \sum_{\gamma \in \Gamma_{U,*}}{\frac{1}{|Aut(U)|c(\gamma)}} < \epsilon'$ 
		\item $\forall V \in \mathcal{I}_{mid}, \sum_{\gamma \in \Gamma_{*,V}}{\frac{1}{|Aut(U_{\gamma})|c(\gamma)}} < \epsilon'$ 
		\item $\forall U \in \mathcal{I}_{mid}, \sum_{\tau \in \mathcal{M}_{U}}{\frac{1}{|Aut(U)|c(\tau)}} < \epsilon'$
		\item For all $\tau \in \mathcal{M}'$, $\gamma \in \Gamma_{*,U_{\tau}} \cup \{Id_{U_{\tau}}\}$, and $\gamma' \in \Gamma_{*,V_{\tau}} \cup \{Id_{V_{\tau}}\}$,
		\begin{align*}
			&\sum_{j>0}{\sum_{\gamma_1,\gamma'_1,\cdots,\gamma_j,\gamma'_j \in \Gamma_{\gamma,\gamma',j}}{\prod_{i:\gamma_i \text{ is non-trivial}}{\frac{1}{|Aut(U_{\gamma_i})|}}
					\prod_{i:\gamma'_i \text{ is non-trivial}}{\frac{1}{|Aut(U_{\gamma'_i})|}}}}\sum_{P_1,\cdots,P_j:P_i \in \mathcal{P}_{\gamma_i,\tau_{P_{i-1}},{\gamma'_i}^T}}{\left(\prod_{i=1}^{j}{N(P_i)}\right)} \\
			&\leq \frac{N(\gamma)N(\gamma')}
			{(|Aut(U_{\gamma})|)^{1_{\gamma \text{ is non-trivial}}}(|Aut(U_{\gamma'})|)^{1_{\gamma' \text{ is non-trivial}}}}
		\end{align*}
		Note: $\Gamma_{\gamma,\gamma',j}$ will be defined later, see Definition \ref{multigammadefinition}.
	\end{enumerate}
	and we have SOS-symmetric coefficient matrices $\{H'_{\gamma}: \gamma \in \Gamma\}$ such that the following conditions hold:
	\begin{enumerate}
		\item For all $U \in \mathcal{I}_{mid}$,  $H_{Id_{U}} \succeq 0$
		\item For all $U \in \mathcal{I}_{mid}$ and $\tau \in \mathcal{M}_U$,
		\[
		\left[ {\begin{array}{cc}
				\frac{1}{|Aut(U)|c(\tau)}H_{Id_{U}} & B_{norm}(\tau)H_{\tau} \\
				B_{norm}(\tau)H^T_{\tau} & \frac{1}{|Aut(U)|c(\tau)}H_{Id_{U}}
		\end{array}} \right] \succeq 0
		\]
		\item For all $U,V \in \mathcal{I}_{mid}$ where $w(U) > w(V)$ and all $\gamma \in \Gamma_{U,V}$, 
		\[
		c(\gamma)^2{N(\gamma)}^2{B(\gamma)^2}H^{-\gamma,\gamma}_{Id_{V}} \preceq H'_{\gamma}
		\]
	\end{enumerate}
	then with probability at least $1 - \epsilon$, 
	\[
	\Lambda \succeq \frac{1}{2}\left(\sum_{U \in \mathcal{I}_{mid}}{M^{fact}_{Id_U}{(H_{Id_U})}}\right) - 3\left(\sum_{U \in \mathcal{I}_{mid}}{\sum_{\gamma \in \Gamma_{U,*}}{\frac{d_{Id_{U}}(H'_{\gamma},H_{Id_{U}})}{|Aut(U)|c(\gamma)}}}\right)Id_{sym}
	\]
	If it is also true that whenever $||M_{\alpha}|| \leq B_{norm}(\alpha)$ for all $\alpha \in \mathcal{M}'$, 
	\[
	\sum_{U \in \mathcal{I}_{mid}}{M^{fact}_{Id_U}{(H_{Id_U})}} \succeq 6\left(\sum_{U \in \mathcal{I}_{mid}}{\sum_{\gamma \in \Gamma_{U,*}}{\frac{d_{Id_{U}}(H'_{\gamma},H_{Id_{U}})}{|Aut(U)|c(\gamma)}}}\right)Id_{sym}
	\]
	then with probability at least $1 - \epsilon$, $\Lambda \succeq 0$.
\end{theorem}
Throughout this section, we assume that we have functions $B_{norm}(\alpha)$, $B(\gamma)$, $N(\gamma)$, and $c(\alpha)$. If $\forall \alpha \in \mathcal{M}', ||M_{\alpha}|| \leq B_{norm}(\alpha)$ then we say that the norm bounds hold. For the other properties of these functions, we will either restate these properties in our intermediate results to highlight where these properties are needed or just state that the conditions on these functions are satisfied for brevity.
\subsection{Warm-up: Analysis with no intersection terms}
In this subsection, we show how the analysis works if we ignore the difference between $M^{fact}$ and $M^{orth}$
\begin{theorem}\label{thm:nointersectionanalysis}
	For all $\epsilon' \in (0,\frac{1}{2}]$, if the norm bounds hold and the following conditions hold
	\begin{enumerate}
		\item For all $U \in \mathcal{I}_{mid}$,  $H_{Id_{U}} \succeq 0$
		\item For all $U \in \mathcal{I}_{mid}$ and all $\tau \in \mathcal{M}_U$
		\[
		\left[ {\begin{array}{cc}
				\frac{1}{|Aut(U)|c(\tau)}H_{Id_{U}} & B_{norm}(\tau)H_{\tau} \\
				B_{norm}(\tau)H^T_{\tau} & \frac{1}{|Aut(U)|c(\tau)}H_{Id_{U}}
		\end{array}} \right] \succeq 0
		\]
		\item $\forall U \in \mathcal{I}_{mid}, \sum_{\tau \in \mathcal{M}_U}{\frac{1}{|Aut(U)|c(\tau)}} \leq \epsilon'$.
	\end{enumerate}
	then
	\[
	\sum_{U \in \mathcal{I}_{mid}}{M^{fact}_{Id_U}(H_{Id_U})} + \sum_{U \in \mathcal{I}_{mid}}{\sum_{\tau \in \mathcal{M}_U}{M^{fact}_{\tau}(H_{\tau})} \succeq (1-2\epsilon')\sum_{U \in \mathcal{I}_{mid}}{M^{fact}_{Id_U}(H_{Id_U})}} \succeq 0
	\]
\end{theorem}
\begin{proof}
	We first show how a single term $M_{\sigma}M_{\tau}M_{{\sigma'}^T}$ plus its transpose $M_{\sigma'}M_{{\tau}^T}M_{{\sigma}^T}$ can be bounded.
	\begin{lemma}
		If the norm bounds hold then for all $\tau \in \mathcal{M}'$ and shapes $\sigma,\sigma'$ such that $\sigma,\tau,{\sigma'}^T$ are composable, for all $a,b$ such that $a > 0$, $b > 0$, and $ab = B_{norm}(\tau)^2$,
		\[
		M_{\sigma}M_{\tau}M_{{\sigma'}^T} + M_{\sigma'}M_{{\tau}^T}M_{{\sigma}^T} \preceq aM_{\sigma}M_{\sigma^T} + bM_{\sigma'}M_{{\sigma'}^T}
		\]
	\end{lemma}
	\begin{proof}
		Observe that 
		\begin{align*}
			0 \preceq &\left(\sqrt{a}M_{\sigma} - \frac{\sqrt{b}}{B_{norm}(\tau)}M_{{\sigma'}}M_{\tau^T}\right)\left(\sqrt{a}M_{\sigma} - \frac{\sqrt{b}}{B_{norm}(\tau)}M_{{\sigma'}}M_{\tau^T}\right)^T = \\
			&\left(\sqrt{a}M_{\sigma} - \frac{\sqrt{b}}{B_{norm}(\tau)}M_{{\sigma'}}M_{\tau}\right)\left(\sqrt{a}M_{{\sigma}^T} - \frac{\sqrt{b}}{B_{norm}(\tau)}M_{{\tau}}M_{{\sigma'}^T}\right) = \\
			&aM_{\sigma}M_{\sigma^T} - M_{\sigma}M_{\tau}M_{{\sigma'}^T} - M_{\sigma'}M_{{\tau}^T}M_{{\sigma}^T} + \frac{b}{B_{norm}(\tau)^2}M_{\sigma'}M_{\tau^{T}}M_{\tau}M_{{\sigma'}^T} \preceq \\
			&aM_{\sigma}M_{\sigma^T} - M_{\sigma}M_{\tau}M_{{\sigma'}^T} - M_{\sigma'}M_{{\tau}^T}M_{{\sigma}^T} + \frac{b}{B_{norm}(\tau)^2}M_{\sigma'}(B_{norm}(\tau)^2{Id})M_{{\sigma'}^T}
		\end{align*}
		Thus, $M_{\sigma}M_{\tau}M_{{\sigma'}^T} + M_{\sigma'}M_{{\tau}^T}M_{{\sigma}^T} \preceq aM_{\sigma}M_{\sigma^T} + bM_{\sigma'}M_{{\sigma'}^T}$, as needed.
	\end{proof}
	%\begin{figure}[ht]
	%\centerline{\includegraphics[height=8cm]{GraphMatrixComparison100517}}
	%\caption{To be added}
	%\end{figure}
	Unfortunately, if we try to bound everything term by term, there may be too many terms to bound. Instead, we generalize this argument for vectors and coefficient matrices.
	\begin{definition}
		Let $\tau$ be a shape. We say that a vector $v$ is a left $\tau$-vector if the coordinates of $v$ are indexed by left shapes $\sigma \in \mathcal{L}_{U_{\tau}}$. We say that a vector $w$ is a right $\tau$-vector if the coordinates of $w$ are indexed by left shapes $\sigma' \in \mathcal{L}_{V_{\tau}}$.
	\end{definition}
	\begin{lemma}\label{lm:rankonetosquares}
		For all $\tau \in \mathcal{M}'$, if the norm bounds hold, $v$ is a left $\tau$-vector, and $w$ is a right $\tau$-vector then 
		\[
		M^{fact}_{\tau}(vw^T) + M^{fact}_{{\tau}^T}(wv^T) \preceq B_{norm}(\tau)\left(M^{fact}_{Id_{U_{\tau}}}(vv^T) + M^{fact}_{Id_{V_{\tau}}}(ww^T)\right)
		\]
		and 
		\[
		-M^{fact}_{\tau}(vw^T) - M^{fact}_{{\tau}^T}(wv^T) \preceq B_{norm}(\tau)\left(M^{fact}_{Id_{U_{\tau}}}(vv^T) + M^{fact}_{Id_{V_{\tau}}}(ww^T)\right)
		\]
	\end{lemma}
	\begin{proof}
		Observe that 
		\begin{align*}
			0 \preceq &\left(\sum_{\sigma}{v_{\sigma}M_{\sigma} \mp \frac{w_{\sigma}M_{\sigma}M_{{\tau}^T}}{B_{norm}(\tau)}}\right)
			\left(\sum_{\sigma'}{v_{\sigma'}M_{\sigma'} \mp \frac{w_{\sigma'}M_{\sigma'}M_{{\tau}^T}}{B_{norm}(\tau)}}\right)^T = \\
			&\left(\sum_{\sigma}{v_{\sigma}M_{\sigma} \mp \frac{w_{\sigma}M_{\sigma}M_{{\tau}^T}}{B_{norm}(\tau)}}\right)\left(\sum_{\sigma'}{v_{\sigma'}M_{{\sigma'}^T} \mp \frac{w_{{\sigma'}}M_{\tau}M_{{\sigma'}^T}}{B_{norm}(\tau)}}\right) = \\
			&\sum_{\sigma,\sigma'}{\left(v_{\sigma}v_{\sigma'}\right)M_{\sigma}M_{{\sigma'}^T}} \mp \sum_{\sigma,\sigma'}{\frac{\left(v_{\sigma}w_{\sigma'}\right)}{B_{norm}(\tau)}M_{\sigma}M_{\tau}M_{\sigma'}} \\
			&\mp \sum_{\sigma,\sigma'}{\frac{\left(w_{\sigma}v_{\sigma'}\right)}{B_{norm}(\tau)}M_{\sigma}M_{{\tau}^T}M_{\sigma'}} + 
			\frac{1}{B_{norm}(\tau)^2}\sum_{\sigma,\sigma'}{\left(v_{\sigma}v_{\sigma'}\right)M_{\sigma}M_{\tau}M_{{\tau}^T}M_{{\sigma'}^T}}
		\end{align*}
		Further observe that 
		\begin{enumerate}
			\item $\sum_{\sigma,\sigma'}{\left(v_{\sigma}v_{\sigma'}\right)M_{\sigma}M_{{\sigma'}^T}} = M^{fact}_{Id_{U_{\tau}}}(vv^T)$
			\item $\sum_{\sigma,\sigma'}{\left(v_{\sigma}w_{\sigma'}\right)M_{\sigma}M_{\tau}M_{{\sigma'}^T}} = M^{fact}_{\tau}(vw^T)$
			\item $\sum_{\sigma,\sigma'}{\left(w_{\sigma}v_{\sigma'}\right)M_{\sigma}M_{{\tau}^T}M_{{\sigma'}^T}} = M^{fact}_{{\tau}^T}(wv^T)$
			\item 
			\begin{align*}
				\sum_{\sigma,\sigma'}{\left(w_{\sigma}w_{\sigma'}\right)M_{\sigma}M_{\tau}M_{{\tau}^T}M_{{\sigma'}^T}} 
				&= \left(\sum_{\sigma}{w_{\sigma}M_{\sigma}}\right)M_{\tau}M_{{\tau}^T}\left(\sum_{\sigma}{w_{\sigma}M_{\sigma}}\right)^T \\
				&\preceq \left(\sum_{\sigma}{w_{\sigma}M_{\sigma}}\right)B_{norm}(\tau)^2{Id}\left(\sum_{\sigma}{w_{\sigma}M_{\sigma}}\right)^T \\
				&= B_{norm}(\tau)^2\sum_{\sigma,\sigma'}{\left(w_{\sigma}w_{\sigma'}\right)M_{\sigma}M_{{\sigma'}^T}} \\
				&= {B_{norm}(\tau)^2}M^{fact}_{Id_{V_{\tau}}}(ww^T)
			\end{align*}
		\end{enumerate}
		Putting everything together, 
		\[
		\frac{M^{fact}_{\tau}(vw^T) + M^{fact}_{{\tau}^T}(wv^T)}{B_{norm}(\tau)} \preceq M^{fact}_{Id_{U_{\tau}}}(vv^T) + M^{fact}_{Id_{V_{\tau}}}(ww^T)
		\] 
		and 
		\[
		-\frac{M^{fact}_{\tau}(vw^T) + M^{fact}_{{\tau}^T}(wv^T)}{B_{norm}(\tau)} \preceq M^{fact}_{Id_{U_{\tau}}}(vv^T) + M^{fact}_{Id_{V_{\tau}}}(ww^T)
		\] 
		as needed.
	\end{proof}
	\begin{corollary}\label{cor:factorizedmatrixbound}
		For all $\tau \in \mathcal{M}'$, if the norm bounds hold and $H_U$ and $H_V$ are matrices such that 
		\[
		\left[ {\begin{array}{cc}
				H_{U} & B_{norm}(\tau)H_{\tau} \\
				B_{norm}(\tau)H^T_{\tau} & H_{V}
		\end{array}} \right] \succeq 0
		\]
		then $M^{fact}_{\tau}(H_{\tau}) + M^{fact}_{{\tau}^T}(H_{\tau^T}) \preceq M^{fact}_{Id_{U_{\tau}}}(H_{U}) + M^{fact}_{Id_{V_{\tau}}}(H_{V})$
	\end{corollary}
	\begin{proof}
		If $            \left[ {\begin{array}{cc}
				H_{U} & B_{norm}(\tau)H_{\tau} \\
				B_{norm}(\tau)H^T_{\tau} & H_{V}
		\end{array}} \right] \succeq 0$ then we can write 
		\[            \left[ {\begin{array}{cc}
				H_{U} & B_{norm}(\tau)H_{\tau} \\
				B_{norm}(\tau)H^T_{\tau} & H_{V}
		\end{array}} \right] = \sum_{i}{(v_i,w_i)(v_i,w_i)^T}
		\]
		Since the $M^{fact}$ operations are linear, the result now follows by summing the equation
		\[
		M^{fact}_{\tau}({v_i}w_i^T) + M^{fact}_{{\tau}^T}({w_i}v_i^T) \preceq B_{norm}(\tau)\left(M^{fact}_{Id_{U_{\tau}}}({v_i}v_i^T) + M^{fact}_{Id_{V_{\tau}}}({w_i}w_i^T)\right)
		\]
		over all $i$.
	\end{proof}
	Theorem \ref{thm:nointersectionanalysis} now follows directly. For all $U \in \mathcal{I}_{mid}$ and all $\tau \in \mathcal{M}_U$, using Corollary \ref{cor:factorizedmatrixbound} with $H_U = H_V = \frac{1}{|Aut(U)|c(\tau)}H_{Id_{U}}$,
	\[
	M^{fact}_{\tau}(H_{\tau}) + M^{fact}_{{\tau}^T}(H_{\tau^T}) \preceq \frac{1}{|Aut(U)|c(\tau)}M^{fact}_{Id_{U}}(H_{Id_{U}}) + \frac{1}{|Aut(U)|c(\tau)}M^{fact}_{Id_{U}}(H_{Id_{U}})
	\]
	Summing this equation over all $U \in \mathcal{I}_{mid}$ and all $\tau \in \mathcal{M}_U$, we obtain that 
	\[
	\sum_{U \in \mathcal{I}_{mid}}{\sum_{\tau \in \mathcal{M}_U}{M^{fact}_{\tau}(H_{\tau})}} \preceq 2\epsilon'\sum_{U \in \mathcal{I}_{mid}}{M^{fact}_{Id_U}(H_{Id_U})}
	\] as needed.
\end{proof}
\subsection{Intersection Term Analysis Strategy}\label{qualitativeintersectionpatternssection}
As we saw in the previous subsection, the analysis works out nicely if we work with $M^{fact}$. Unfortunately, our matrices are expressed in terms of $M^{orth}$. In this subsection, we describe our strategy for analyzing the difference between $M^{fact}$ and $M^{orth}$.

Recall the following expressions for $\left(M^{fact}_{\tau}(H)\right)(A,B)$ and $\left(M^{orth}_{\tau}(H)\right)(A,B)$ where $A$ has shape $U_{\tau}$ and $B$ has shape $V_{\tau}$:
\[
\left(M^{fact}_{\tau}(H)\right)(A,B) = \sum_{\sigma \in \mathcal{L}_{U_{\tau}}, \sigma' \in \mathcal{L}_{V_{\tau}}}{H(\sigma,\sigma')\sum_{A',B'}{
		\sum_{R_1 \in \mathcal{R}(\sigma,A,A'), R_2 \in \mathcal{R}(\tau,A',B'), \atop R_3 \in \mathcal{R}({\sigma'}^T,B',B)}M_{R_1}(A,A')M_{R_2}(A',B')M_{R_3}(B',B)}}
\]
\begin{align*}
	&\left(M^{orth}_{\tau}(H)\right)(A,B) \\
	&= \sum_{\sigma \in \mathcal{L}_{U_{\tau}}, \sigma' \in \mathcal{L}_{V_{\tau}}}{H(\sigma,\sigma')\sum_{A',B'}{
			\sum_{R_1 \in \mathcal{R}(\sigma,A,A'), R_2 \in \mathcal{R}(\tau,A',B'), \atop {R_3 \in \mathcal{R}({\sigma'}^T,B',B), R_1,R_2,R_3 \text{ are properly composable}}}M_{R_1}(A,A')M_{R_2}(A',B')M_{R_3}(B',B)}} 
\end{align*}
This implies that $\left(M^{fact}_{\tau}(H)\right)(A,B) - \left(M^{orth}_{\tau}(H)\right)(A,B)$ is equal to
\[
\sum_{\sigma \in \mathcal{L}_{U_{\tau}}, \sigma' \in \mathcal{L}_{V_{\tau}}}{H(\sigma,\sigma')\sum_{A',B'}{
		\sum_{R_1 \in \mathcal{R}(\sigma,A,A'), R_2 \in \mathcal{R}(\tau,A',B'), \text{ and } R_3 \in \mathcal{R}({\sigma'}^T,B',B) \atop R_1,R_2,R_3 \text{ are not properly composable}}M_{R_1}(A,A')M_{R_2}(A',B')M_{R_3}(B',B)}} 
\]
%\begin{figure}[ht]
%\centerline{\includegraphics[height=8cm]{IntersectionTermsExampleOne100517}}
%\caption{To be added}
%\end{figure}
Thus, to understand the difference between $M^{fact}$ and $M^{orth}$, we need to analyze the terms $\chi_{R_1}\chi_{R_2}\chi_{R_3} = \chi_{R_1 \circ R_2 \circ R_3}$ for ribbons $R_1,R_2,R_3$ which are composable but not properly composable. These terms, which we call intersection terms, are not negligible and must be analyzed carefully. In particular, we decompose each resulting ribbon $R = R_1 \circ R_2 \circ R_3$ into new left, middle, and right parts. We do this as follows:
\begin{enumerate}
	\item Let $V_{*}$ be the set of vertices which appear more than once in $V(R_1 \circ R_2 \circ R_3)$. In other words, $V_{*}$ is the set of vertices involved in the intersections between $R_1$, $R_2$, and $R_3$ (not counting the facts that $B_{R_1} = A_{R_2}$ and $B_{R_2} = A_{R_3}$ because we expect these intersections).
	\item Let $A'$ be the leftmost minimum vertex separator of $A_{R_1}$ and $B_{R_1} \cup V_{*}$ in $R_1$. We turn $A'$ into a matrix index by specifying an ordering $O_{A'}$ for the vertices in $A'$.
	\item Let $B'$ be the leftmost minimum vertex separator of $A_{R_3} \cup V_{*}$ and $B_{R_3}$ in $R_2$. We turn $B'$ into a matrix index by specifying an ordering $O_{B'}$ for the vertices in $B'$.
	\item Decompose $R_1$ as $R_1 = {R'}_1 \cup R_4$ where ${R'}_1$ is the part of $R_1$ between $A_{R_1}$ and $A'$ and $R_4$ is the part of $R_1$ between $B'$ and $B_{R_1} = A_{R_2}$. Similarly, decompose 
	$R_3$ as $R_3 = R_5 \cup {R'}_3 $ where $R_5$ is the part of $R_3$ between $B_{R_1} = A_{R_2}$ and $B'$ and ${R'}_3$ is the part of $R_3$ between $B'$ and $B_{R_3}$.
	\item Take $R'_2 = R_4 \circ R_2 \circ R_5$ and note that $R'_1 \circ R'_2 \circ R'_3 = R_1 \circ R_2 \circ R_3$. We view $R'_1,R'_2,R'_3$ as the left, middle, and right parts of $R = R_1 \circ R_2 \circ R_3$
\end{enumerate}
While we will verify our analysis by checking the coefficients of the ribbons, we want to express everything in terms of shapes. We use the following conventions for the names of the shapes:
\begin{enumerate}
	\item As usual, we let $\sigma$, $\tau$, and ${\sigma'}^T$ be the shapes of $R_1$, $R_2$, and $R_3$.
	\item We let $\gamma$ and ${\gamma'}^T$ be the shapes of $R_4$ and $R_5$.
	\item We let $\sigma_2$, $\tau_{P}$, and ${\sigma'_2}^T$ be the shapes of $R'_1$, $R'_2$, and $R'_3$. Here $P$ is the intersection pattern induced by $R_4$, $R_2$, and $R_5$ which we define in the next subsection.
\end{enumerate}
\begin{remark}
	A key feature of our analysis is that it will work the same way regardless of the shapes $\sigma_2,{\sigma'_2}^T$ of $R'_1$ and $R'_3$. In other words, if we replace $\sigma_2$ by $\sigma_{2a}$ and $\sigma'_2$ by $\sigma'_{2a}$ for a given intersection term, this just replaces $\sigma = \sigma_2 \cup \gamma$ with  $\sigma_{a} = \sigma_{2a} \cup \gamma$ and $\sigma' = \sigma'_2 \cup \gamma'$ with  $\sigma'_{a} = \sigma'_{2a} \cup \gamma'$. This allows us to focus on the shapes $\gamma$, $\tau$, and ${\gamma'}^T$ and is the reason why the $-\gamma,\gamma$ operation appears in our results.
\end{remark}
\subsection{Intersection Term Analysis}\label{intersectiontermanalysissection}
In this section, we implement our strategy for analyzing intersection terms. For simplicity, we only give rough definitions and proof sketches here. For a more rigorous treatment, see Apendix \ref{canonicalmapsection}.

We begin by defining intersection patterns which describe how the ribbons $R_1$, $R_2$, and $R_3$ intersect. 
\begin{definition}[Rough Definition of Intersection Patterns]\label{intersectionpatternroughdef}
	Given $\tau \in \mathcal{M}'$, $\gamma \in \Gamma_{*,U_{\tau}} \cup \{Id_{U_{\tau}}\}$, $\gamma' \in \Gamma_{*,V_{\tau}} \cup \{Id_{V_{\tau}}\}$, and ribbons $R_1$, $R_2$, and $R_3$ of shapes $\gamma$, $\tau$, and ${\gamma'}^T$ which are composable but not properly composable, we define the intersection pattern $P$ induced by $R_1$, $R_2$, and $R_3$ and the resulting shape $\tau_P$ as follows:
	\begin{enumerate}
		\item We take $V(P) = V(\gamma \circ \tau \circ {\gamma'}^T)$.
		\item We take $E(P)$ to be the set of edges $(u,v)$ such that $u,v$ are distinct vertices in $V(\sigma \circ \tau \circ {\sigma'}^T)$ but $u$ and $v$ correspond to the same vertex in $R_1 \circ R_2 \circ R_3$
		\item We define $\tau_{P}$ to be the shape of the ribbon $R = R_1 \circ R_2 \circ R_3$
	\end{enumerate}
\end{definition}
\begin{definition}\label{setPdefinition}
	Given $\tau \in \mathcal{M}'$, $\gamma \in \Gamma_{*,U_{\tau}} \cup \{Id_{U_{\tau}}\}$, and $\gamma' \in \Gamma_{*,V_{\tau}} \cup \{Id_{V_{\tau}}\}$, we define $\mathcal{P}_{\gamma,\tau,{\gamma'}^T}$ to be the set of all possible intersection patterns $P$ which can be induced by ribbons $R_1$, $R_2$, and $R_3$ of shapes $\gamma$, $\tau$, and ${\gamma'}^T$.
\end{definition}
\begin{remark}
	Note that if $\gamma = Id_{U_{\tau}}$ and $\gamma' = Id_{V_{\tau}}$ then $\mathcal{P}_{\gamma,\tau,{\gamma'}^T} = \emptyset$ as every intersection pattern must have an unexpected intersection so either $\gamma$ or $\gamma'$ must be non-trivial.
\end{remark}
%\begin{figure}[ht]
%\centerline{\includegraphics[height=8cm]{IntersectionTermComparison100517}}
%\caption{To be added}
%\end{figure}
It would be nice if the intersection pattern $P$ together with the ribbon $R$ allowed us to recover the original ribbons $R_1$, $R_2$, and $R_3$. Unfortunately, it is possible for different triples of ribbons to result in the same intersection pattern $P$ and ribbon $R$. That said, the number of such triples cannot be too large, and this is sufficient for our purposes.
\begin{definition}
	Given an intersection pattern $P \in \mathcal{P}_{\gamma,\tau,{\gamma'}^T}$, let $R$ be a ribbon of shape $\tau_{P}$. We define $N(P)$ to be the number of different triples of ribbons $R_1,R_2,R_3$ such that $R_1 \circ R_2 \circ R_3 = R$ and $R_1,R_2,R_3$ induce the intersection pattern $P$.
\end{definition}
\begin{lemma}
	For all intersection patterns $P \in \mathcal{P}_{\gamma,\tau,{\gamma'}^T}$, $N(P) \leq |V(\tau_{P})|^{|V(\gamma) \setminus U_{\gamma}| + |V(\gamma') \setminus U_{\gamma'}|}$
\end{lemma}
\begin{proof}[Proof sketch]
	This can be proved by making the following observations:
	\begin{enumerate}
		\item $A_{R_1} = A_{R}$ and $B_{R_3} = B_{R}$.
		\item All of the remining vertices in $V(R_1)$ and $V(R_3)$ must be equal to some vertex in $V(R)$.
		\item Once $R_1$ and $R_3$ are determined, there is at most one ribbon $R_2$ such that $R_1,R_2,R_3$ are composable, $R = R_1 \circ R_2 \circ R_3$, and $R_1,R_2,R_3$ induce the intersection pattern $P$.
	\end{enumerate}
\end{proof}
With these definitions, we can now analyze the intersection terms.
\begin{definition}
	Given a left shape $\sigma$, define $e_{\sigma}$ to be the vector which has a $1$ in coordinate $\sigma$ and has a $0$ in all other coordinates.
\end{definition}
\begin{lemma}\label{lm:singleshapeintersections}
	For all $\tau \in \mathcal{M}'$, $\sigma \in \mathcal{L}_{U_{\tau}}$, and $\sigma' \in \mathcal{L}_{V_{\tau}}$, 
	\begin{align*}
		&M^{fact}_{\tau}(e_{\sigma}e^T_{\sigma'}) - M^{orth}_{\tau}(e_{\sigma}e^T_{\sigma'}) = \sum_{\sigma_2 \in \mathcal{L}, \gamma \in \Gamma: \sigma_2 \circ \gamma = \sigma}{\frac{1}{|Aut(U_{\gamma})|}\sum_{P \in \mathcal{P}_{\gamma,\tau,Id_{V_{\tau}}}}N(P)M^{orth}_{\tau_P}(e_{\sigma_2}e^T_{\sigma'})} \\
		&+ \sum_{\sigma'_2 \in \mathcal{L}, \gamma' \in \Gamma: \sigma'_2 \circ \gamma' = \sigma'}{\frac{1}{|Aut(U_{\gamma'})|}\sum_{P \in \mathcal{P}_{Id_{U_{\tau}},\tau,{\gamma'}^T}}N(P)M^{orth}_{\tau_P}(e_{\sigma}e^T_{\sigma'_2})} \\
		&+ \sum_{\sigma_2 \in \mathcal{L}, \gamma \in \Gamma: \sigma_2 \circ \gamma = \sigma}{\sum_{\sigma'_2 \in \mathcal{L}, \gamma' \in \Gamma: \sigma'_2 \circ \gamma' = \sigma'}{
				\frac{1}{|Aut(U_{\gamma})|\cdot|Aut(U_{\gamma'})|}\sum_{P \in \mathcal{P}_{\gamma,\tau,{\gamma'}^T}}N(P)M^{orth}_{\tau_P}(e_{\sigma_2}e^T_{\sigma'_2})}}
	\end{align*}
\end{lemma}
\begin{proof}[Proof sketch]
	This lemma follows from the following bijection. Consider the third term
	\[
	\sum_{\sigma_2 \in \mathcal{L}, \gamma \in \Gamma: \sigma_2 \circ \gamma = \sigma}{\sum_{\sigma'_2 \in \mathcal{L}, \gamma' \in \Gamma: \sigma'_2 \circ \gamma' = \sigma'}{
			\frac{1}{|Aut(U_{\gamma})|\cdot|Aut(U_{\gamma'})|}\sum_{P \in \mathcal{P}_{\gamma,\tau,{\gamma'}^T}}N(P)M^{orth}_{\tau_P}(e_{\sigma_2}e^T_{\sigma'_2})}}
	\]
	On one side, we have the following data:
	\begin{enumerate}
		\item Ribbons $R_1$, $R_2$, and $R_3$ of shapes $\gamma,\tau,{\gamma'}^T$ such that $R_1,R_2,R_3$ are composable but $R_1$ and $R_2 \circ R_3$ are not properly composable (i.e. $R_1$ has an unexpected intersection with $R_2$ and/or $R_3$) and $R_1 \circ R_2$ and $R_3$ are not properly composable (i.e. $R_3$ has an unexpected intersection with $R_1$ and/or $R_2$).
		\item An ordering $O_{A'}$ on the leftmost minimum vertex separator $A'$ of $A_{R_1}$ and $V_{*} \cup B_{R_1}$ (recall that $V_{*}$ is the set of vertices which appear more than once in $V(R_1 \circ R_2 \circ R_3)$).
		\item An ordering $O_{B'}$ on the rightmost minimum vertex separator $B'$ of $V_{*} \cup A_{R_3}$ and $B_{R_3}$.
	\end{enumerate}
	On the other side, we have the following data
	\begin{enumerate}
		\item An intersection pattern $P \in \mathcal{P}_{\gamma,\tau,{\gamma'}^T}$ where $\gamma$ and ${\gamma'}^T$ are non-trivial.
		\item Ribbons $R'_1$, $R'_2$, $R'_3$ of shapes $\sigma_2$, $\tau_P$, ${\sigma'_2}^T$ which are properly composable
		\item A number in $[N(P)]$ describing which possible triple of ribbons resulted in the intersection pattern $P$ and the ribbon $R'_2$.
	\end{enumerate}
	To see this bijection, note that given the data on the first side, we can recover the ribbons $R'_1$, $R'_2$, and $R'_3$ as follows:
	\begin{enumerate}
		\item We decompose $R_1$ as $R_1 = R'_1 \circ R_4$ where $B_{R'_1} = A_{R_4} = A'$ with the ordering $O_{A'}$.
		\item We decompose $R_3$ as $R_3 = R_5 \circ R'_3$ where  where $B_{R_5} = A_{R'_3} = B'$ with the ordering $O_{B'}$.
		\item We take $R'_2 = R_4 \circ R_2 \circ R_5$.
	\end{enumerate}
	The intersection pattern $P$ and the number in $[N(P)]$ can be obtained from $R_1$, $R_2$, and $R_3$.
	
	Conversely, with the data on the other side, we can recover the data on the first side as follows:
	\begin{enumerate}
		\item $R'_2$ gives an ordering $O_{A'}$ for $A' = A_{R'_2}$ and an ordering $O_{B'}$ for $B' = B_{R'_2}$.
		\item The ribbon $R'_2$, intersection pattern $P$, and number in $[N(P)]$ allow us to recover $R_4$, $R_2$, and $R_5$.
		\item We take $R_1 = R'_1 \circ R_4$ and $R_3 = R_5 \circ R'_3$.
	\end{enumerate}
	Thus, both sides have the same coefficient for each ribbon.
	
	The analysis for the the first term is the same except that when $\gamma'$ is trivial, we always take $\gamma' = Id_{V_{\tau}}$. Thus, we always have that $B' = B_{R'_2} = B_{R_2}$ (with the same ordering) and $R'_3 = R_3 = Id_{B'}$. Because of this, there is no need to specify $R_3$, $R'_3$, $R_5$, or an ordering on $B'$.
	
	Similarly, the analysis for the the second term is the same except that when $\gamma$ is trivial, we always take $\gamma = Id_{U_{\tau}}$. Thus, we always have that $A' = A_{R'_2} = A_{R_2}$ (with the same ordering) and $R'_1 = R_1 = Id_{A'}$. Because of this, there is no need to specify $R_1$, $R'_1$, $R_4$, or an ordering on $A'$.
\end{proof}
Applying Lemma \ref{lm:singleshapeintersections} for all $\sigma$ and $\sigma'$ simultaneously, we obtain the following corollary.
\begin{definition}
	For all $U,V \in \mathcal{I}_{mid}$, given a $\gamma \in \Gamma_{U,V}$ and a vector $v$ indexed by left shapes $\sigma \in \mathcal{L}_V$, define $v^{-\gamma}$ to be the vector indexed by left shapes $\sigma_2 \in \mathcal{L}_{U}$ such that $v^{-\gamma}(\sigma_2) = v(\sigma_2 \circ \gamma)$ if $\sigma_2 \circ \gamma \in \mathcal{L}_V$ and $v^{-\gamma}(\sigma_2) = 0$ otherwise.
\end{definition}
\begin{proposition}
	For all composable $\gamma_2,\gamma_1 \in \Gamma$ and all vectors $v$ indexed by left shapes in $\mathcal{L}_{V_{\gamma_1}}$, $(v^{-\gamma_1})^{-\gamma_2} = v^{-\gamma_2 \circ \gamma_1}$
\end{proposition}
\begin{corollary}\label{cor:singlestepintersections}
	For all $\tau \in \mathcal{M}'$, for all left $\tau$-vectors $v$ and all right $\tau$-vectors $w$, 
	\begin{align*}
		&M^{orth}_{\tau}(vw^T) = M^{fact}_{\tau}(vw^T) - \sum_{\gamma \in \Gamma_{*,U_{\tau}}}{\frac{1}{|Aut(U_{\gamma})|}\sum_{P \in \mathcal{P}_{\gamma,\tau,Id_{V_{\tau}}}}N(P)M^{orth}_{\tau_P}(v^{-\gamma}w^T)} \\
		&- \sum_{\gamma' \in \Gamma_{*,V_{\tau}}}{\frac{1}{|Aut(U_{\gamma'})|}\sum_{P \in \mathcal{P}_{Id_{U_{\tau}},\tau,{\gamma'}^T}}N(P)M^{orth}_{\tau_P}(v(w^{-\gamma})^T)} \\
		&- \sum_{\gamma \in \Gamma_{*,U_{\tau}}}{\sum_{\gamma' \in \Gamma_{*,V_{\tau}}}{
				\frac{1}{|Aut(U_{\gamma})|\cdot|Aut(U_{\gamma'})|}\sum_{P \in \mathcal{P}_{\gamma,\tau,{\gamma'}^T}}N(P)M^{orth}_{\tau_P}(v^{-\gamma}(w^{-\gamma'})^T)}}
	\end{align*}
\end{corollary}
Applying Corollary \ref{cor:singlestepintersections} iteratively, we obtain the following theorem:
\begin{definition}\label{multigammadefinition}
	Given $\gamma,\gamma' \in \Gamma \cup \{Id_U:U \in \mathcal{I}_{mid}\}$ and $j > 0$, let $\Gamma_{\gamma,\gamma',j}$ be the set of all $\gamma_1,\gamma'_1,\cdots,\gamma_j,\gamma'_j \in \Gamma \cup \{Id_U:U \in \mathcal{I}_{mid}\}$ such that:
	\begin{enumerate}
		\item $\gamma_j,\ldots,\gamma_1$ are composable and $\gamma_j \circ \ldots \circ \gamma_1 = \gamma$
		\item $\gamma'_j,\ldots,\gamma'_1$ are composable and $\gamma'_j \circ \ldots \circ \gamma'_1 = \gamma'$
		\item For all $i \in [1,j]$, $\gamma_i$ or $\gamma'_i$ is non-trivial (i.e. $\gamma_i \neq Id_{U_{\gamma_i}}$ or $\gamma'_i \neq Id_{U_{\gamma'_i}}$).
	\end{enumerate}
\end{definition}
\begin{remark}
	Note that if $\gamma = Id_{U}$ and $\gamma' = Id_{V}$ then for all $j > 0$, $\Gamma_{\gamma,\gamma',j} = \emptyset$.
\end{remark}
\begin{theorem}\label{thm:mfactmorthdifference}
	For all $\tau \in \mathcal{M}'$, left $\tau$-vectors $v$, and right $\tau$-vectors $w$, 
	\begin{align*}
		&M^{orth}_{\tau}(v{w^T}) = M^{fact}_{\tau}(v{w^T}) + \\
		&\sum_{\gamma \in \Gamma_{*,U_{\tau}} \cup \{Id_{U_{\tau}}\},\gamma' \in \Gamma_{*,V_{\tau}} \cup \{Id_{V_{\tau}}\}: \atop \gamma \text{ or } \gamma' \text{ is non-trivial }}\sum_{j>0}{(-1)^{j}\sum_{\gamma_1,\gamma'_1,\cdots,\gamma_j,\gamma'_j \in \Gamma_{\gamma,\gamma',j}}{\prod_{i:\gamma_i \text{ is non-trivial}}{\frac{1}{|Aut(U_{\gamma_i})|}}
				\prod_{i:\gamma'_i \text{ is non-trivial}}{\frac{1}{|Aut(U_{\gamma'_i})|}}}} \\
		&\sum_{P_1,\cdots,P_j:P_i \in \mathcal{P}_{\gamma_i,\tau_{P_{i-1}},{\gamma'_i}^T}}{\left(\prod_{i=1}^{j}{N(P_i)}\right)M^{fact}_{\tau_{P_j}}(v^{-\gamma}{(w^{-\gamma'})^T})}
	\end{align*}
	where we take $\tau_{P_0} = \tau$.
\end{theorem}
\subsection{Bounding the difference between $M^{fact}$ and $M^{orth}$}\label{boundingdifferencesection}
In this subsection, we bound the difference between $M^{fact}_{\tau}(H_{\tau})$ and $M^{orth}_{\tau}(H_{\tau})$. We recall the following conditions on $B(\gamma)$, $N(\gamma)$, and $c(\gamma)$:
\begin{enumerate}
	\item For all $\tau \in \mathcal{M}'$, $\gamma \in \Gamma_{*,U_{\tau}} \cup \{Id_{U_{\tau}}\}$, and $\gamma' \in \Gamma_{*,V_{\tau}} \cup \{Id_{V_{\tau}}\}$,
	\begin{align*}
		&\sum_{j>0}{\sum_{\gamma_1,\gamma'_1,\cdots,\gamma_j,\gamma'_j \in \Gamma_{\gamma,\gamma',j}}{\left(\prod_{i:\gamma_i \text{ is non-trivial}}{\frac{1}{|Aut(U_{\gamma_i})|}}\right)
				\left(\prod_{i:\gamma'_i \text{ is non-trivial}}{\frac{1}{|Aut(U_{\gamma'_i})|}}\right)}}\\
		&\sum_{P_1,\cdots,P_j:P_i \in \mathcal{P}_{\gamma_i,\tau_{P_{i-1}},{\gamma'_i}^T}}{\left(\prod_{i=1}^{j}{N(P_i)}\right)} \leq \frac{N(\gamma)N(\gamma')}{(|Aut(U_{\gamma})|)^{1_{\gamma \text{ is non-trivial}}}(|Aut(U_{\gamma'})|)^{1_{\gamma' \text{ is non-trivial}}}}
	\end{align*}
	\item For all $\tau \in \mathcal{M}'$, $\gamma \in \Gamma_{*,U_{\tau}}$, and $\gamma' \in \Gamma_{*,V_{\tau}}$, for all $P \in \mathcal{P}_{\gamma,\tau,{\gamma'}^T}$, 
	$B_{norm}(\tau_{P}) \leq B(\gamma)B(\gamma')B_{norm}(\tau)$
	\item $\forall V \in \mathcal{I}_{mid}, \sum_{\gamma \in \Gamma_{*,V}}{\frac{1}{|Aut(U_{\gamma})|c(\gamma)}} \leq \epsilon' \leq \frac{1}{20}$
\end{enumerate}
With these conditions, we can now bound the difference between $M^{fact}$ and $M^{orth}$.
\begin{lemma}\label{keyboundinglemma}
	If the norm bounds and the conditions on $B(\gamma)$, $N(\gamma)$, and $c(\gamma)$ hold then for all $\tau \in \mathcal{M}'$, left $\tau$-vectors $v$, and right $\tau$-vectors $w$, 
	\begin{align*}
		&\left(M^{fact}_{\tau}(v{w^T}) + M^{fact}_{{\tau}^T}(w{v^T})\right) - \left(M^{orth}_{\tau}(v{w^T}) + M^{orth}_{{\tau}^T}(w{v^T})\right) \preceq \\
		&\\
		&{\epsilon'}B_{norm}(\tau)M^{fact}_{Id_{U_{\tau}}}(vv^{T}) + 
		2\sum_{\gamma \in \Gamma_{*,U_{\tau}}}{\frac{B(\gamma)^{2}N(\gamma)^{2}B_{norm}(\tau){c(\gamma)}}{|Aut(U_{\gamma})|}M^{fact}_{Id_{U_{\gamma}}}(v^{-\gamma}(v^{-\gamma})^T)} + \\
		&{\epsilon'}B_{norm}(\tau)M^{fact}_{Id_{V_{\tau}}}(ww^{T}) + 
		2\sum_{\gamma' \in \Gamma_{*,V_{\tau}}}{\frac{B(\gamma')^{2}N(\gamma')^{2}B_{norm}(\tau){c(\gamma')}}{|Aut(U_{\gamma'})|}M^{fact}_{Id_{U_{\gamma'}}}(w^{-\gamma'}(w^{-\gamma'})^T)}
	\end{align*}
\end{lemma}
\begin{proof}
	By Theorem \ref{thm:mfactmorthdifference}, taking $\tau_{P_0} = \tau$, 
	\begin{align*}
		&M^{orth}_{\tau}(v{w^T}) = M^{fact}_{\tau}(v{w^T}) + \\
		&\sum_{\gamma \in \Gamma_{*,U_{\tau}} \cup \{Id_{U_{\tau}}\},\gamma' \in \Gamma_{*,V_{\tau}} \cup \{Id_{V_{\tau}}\}: \atop \gamma \text{ or } \gamma' \text{ is non-trivial }}\sum_{j>0}{(-1)^{j}\sum_{\gamma_1,\gamma'_1,\cdots,\gamma_j,\gamma'_j \in \Gamma_{\gamma,\gamma',j}}{\prod_{i:\gamma_i \text{ is non-trivial}}{\frac{1}{|Aut(U_{\gamma_i})|}}
				\prod_{i:\gamma'_i \text{ is non-trivial}}{\frac{1}{|Aut(U_{\gamma'_i})|}}}} \\
		&\sum_{P_1,\cdots,P_j:P_i \in \mathcal{P}_{\gamma_i,\tau_{P_{i-1}},{\gamma'_i}^T}}{\left(\prod_{i=1}^{j}{N(P_i)}\right)M^{fact}_{\tau_{P_j}}(v^{-\gamma}{(w^{-\gamma'})^T})}
	\end{align*}
	Taking the transpose of this equation gives
	\begin{align*}
		&M^{orth}_{{\tau}^T}(w{v^T}) = M^{fact}_{{\tau}^T}(w{v^T}) + \\
		&\sum_{\gamma \in \Gamma_{*,U_{\tau}} \cup \{Id_{U_{\tau}}\},\gamma' \in \Gamma_{*,V_{\tau}} \cup \{Id_{V_{\tau}}\}: \atop \gamma \text{ or } \gamma' \text{ is non-trivial }}\sum_{j>0}{(-1)^{j}\sum_{\gamma_1,\gamma'_1,\cdots,\gamma_j,\gamma'_j \in \Gamma_{\gamma,\gamma',j}}{\prod_{i:\gamma_i \text{ is non-trivial}}{\frac{1}{|Aut(U_{\gamma_i})|}}
				\prod_{i:\gamma'_i \text{ is non-trivial}}{\frac{1}{|Aut(U_{\gamma'_i})|}}}} \\
		&\sum_{P_1,\cdots,P_j:P_i \in \mathcal{P}_{\gamma_i,\tau_{P_{i-1}},{\gamma'_i}^T}}{\left(\prod_{i=1}^{j}{N(P_i)}\right)M^{fact}_{\tau^{T}_{P_j}}({w^{-\gamma'}(v^{-\gamma})^T})}
	\end{align*}
	Now observe that by Lemma \ref{lm:rankonetosquares}, if the norm bounds hold, 
	\begin{align*}
		&{\pm}\left(M^{fact}_{\tau_{P_j}}(v^{-\gamma}{(w^{-\gamma'})^T}) + M^{fact}_{\tau^{T}_{P_j}}({w^{-\gamma'}(v^{-\gamma})^T})\right) = \\
		&{\pm}M^{fact}_{\tau_{P_j}}\left(\left(\sqrt{\frac{N(\gamma)B(\gamma){c(\gamma)}}{N(\gamma')B(\gamma'){c(\gamma')}}}v^{-\gamma}\right)
		\left(\sqrt{\frac{N(\gamma')B(\gamma'){c(\gamma')}}{N(\gamma)B(\gamma){c(\gamma)}}}{(w^{-\gamma'})^T}\right)\right) \pm \\
		&M^{fact}_{\tau^{T}_{P_j}}\left(\left(\sqrt{\frac{N(\gamma')B(\gamma'){c(\gamma')}}{N(\gamma)B(\gamma){c(\gamma)}}}w^{-\gamma'}\right)
		\left(\sqrt{\frac{N(\gamma)B(\gamma){c(\gamma)}}{N(\gamma')B(\gamma'){c(\gamma')}}}{(v^{-\gamma})^T}\right)\right) \preceq \\
		&B_{norm}(\tau_{P_j})\left(\frac{N(\gamma)B(\gamma){c(\gamma)}}{N(\gamma')B(\gamma'){c(\gamma')}}M^{fact}_{Id_{U_{\gamma}}}(v^{-\gamma}(v^{-\gamma})^T) + 
		\frac{N(\gamma')B(\gamma'){c(\gamma')}}{N(\gamma)B(\gamma){c(\gamma)}}M^{fact}_{Id_{U_{\gamma'}}}(w^{-\gamma'}(w^{-\gamma'})^T)\right)
	\end{align*}
	Combining these equations,
	\begin{align*}
		&\left(M^{fact}_{\tau}(v{w^T}) + M^{fact}_{{\tau}^T}(w{v^T})\right) - \left(M^{orth}_{\tau}(v{w^T}) + M^{orth}_{{\tau}^T}(w{v^T})\right) \preceq \\
		&\sum_{\gamma \in \Gamma_{*,U_{\tau}} \cup \{Id_{U_{\tau}}\},\gamma' \in \Gamma_{*,V_{\tau}} \cup \{Id_{V_{\tau}}\}: \atop \gamma \text{ or } \gamma' \text{ is non-trivial }}\sum_{j>0}{\sum_{\gamma_1,\gamma'_1,\cdots,\gamma_j,\gamma'_j \in \Gamma_{\gamma,\gamma',j}}{\prod_{i:\gamma_i \text{ is non-trivial}}{\frac{1}{|Aut(U_{\gamma_i})|}}
				\prod_{i:\gamma'_i \text{ is non-trivial}}{\frac{1}{|Aut(U_{\gamma'_i})|}}}} \\
		&\sum_{P_1,\cdots,P_j:P_i \in \mathcal{P}_{\gamma_i,\tau_{P_{i-1}},{\gamma'_i}^T}}{\left(\prod_{i=1}^{j}{N(P_i)}\right)
			B_{norm}(\tau_{P_j})} \\
		&\left(\frac{N(\gamma)B(\gamma){c(\gamma)}}{N(\gamma')B(\gamma'){c(\gamma')}}M^{fact}_{Id_{U_{\gamma}}}(v^{-\gamma}(v^{-\gamma})^T) + 
		\frac{N(\gamma')B(\gamma'){c(\gamma')}}{N(\gamma)B(\gamma){c(\gamma)}}M^{fact}_{Id_{U_{\gamma'}}}(w^{-\gamma'}(w^{-\gamma'})^T)\right)
	\end{align*}
	From the conditions on $B(\gamma)$ and $N(\gamma)$, 
	\begin{enumerate}
		\item $B_{norm}(\tau_{P_j}) \leq B(\gamma)B(\gamma')B_{norm}(\tau)$
		\item
		\begin{align*}
			&\sum_{j>0}{\sum_{\gamma_1,\gamma'_1,\cdots,\gamma_j,\gamma'_j \in \Gamma_{\gamma,\gamma',j}}{\left(\prod_{i:\gamma_i \text{ is non-trivial}}{\frac{1}{|Aut(U_{\gamma_i})|}}\right)
					\left(\prod_{i:\gamma'_i \text{ is non-trivial}}{\frac{1}{|Aut(U_{\gamma'_i})|}}\right)}}\\
			&\sum_{P_1,\cdots,P_j:P_i \in \mathcal{P}_{\gamma_i,\tau_{P_{i-1}},{\gamma'_i}^T}}{\left(\prod_{i=1}^{j}{N(P_i)}\right)} \leq \frac{N(\gamma)N(\gamma')}{(|Aut(U_{\gamma})|)^{1_{\gamma \text{ is non-trivial}}}(|Aut(U_{\gamma'})|)^{1_{\gamma' \text{ is non-trivial}}}}
		\end{align*}
	\end{enumerate}
	Putting these equations together, 
	\begin{align*}
		&\left(M^{fact}_{\tau}(v{w^T}) + M^{fact}_{{\tau}^T}(w{v^T})\right) - \left(M^{orth}_{\tau}(v{w^T}) + M^{orth}_{{\tau}^T}(w{v^T})\right) \preceq \\
		&\sum_{\gamma \in \Gamma_{*,U_{\tau}} \cup \{Id_{U_{\tau}}\},\gamma' \in \Gamma_{*,V_{\tau}} \cup \{Id_{V_{\tau}}\}: \atop \gamma \text{ or } \gamma' \text{ is non-trivial }}{\frac{B(\gamma)^{2}N(\gamma)^{2}B_{norm}(\tau){c(\gamma)}}{(|Aut(U_{\gamma})|)^{1_{\gamma \text{ is non-trivial}}}(|Aut(U_{\gamma'})|)^{1_{\gamma' \text{ is non-trivial}}}{c(\gamma')}}M^{fact}_{Id_{U_{\gamma}}}(v^{-\gamma}(v^{-\gamma})^T)} + \\
		&\sum_{\gamma \in \Gamma_{*,U_{\tau}} \cup \{Id_{U_{\tau}}\},\gamma' \in \Gamma_{*,V_{\tau}} \cup \{Id_{V_{\tau}}\}: \atop \gamma \text{ or } \gamma' \text{ is non-trivial }}{\frac{B(\gamma')^{2}N(\gamma')^{2}B_{norm}(\tau){c(\gamma')}}{(|Aut(U_{\gamma})|)^{1_{\gamma \text{ is non-trivial}}}(|Aut(U_{\gamma'})|)^{1_{\gamma' \text{ is non-trivial}}}{c(\gamma)}}M^{fact}_{Id_{U_{\gamma'}}}(w^{-\gamma'}(w^{-\gamma'})^T)}
	\end{align*}
	Now observe that
	\begin{align*}
		&\sum_{\gamma \in \Gamma_{*,U_{\tau}} \cup \{Id_{U_{\tau}}\},\gamma' \in \Gamma_{*,V_{\tau}} \cup \{Id_{V_{\tau}}\}: \atop \gamma \text{ or } \gamma' \text{ is non-trivial }}{\frac{B(\gamma)^{2}N(\gamma)^{2}B_{norm}(\tau){c(\gamma)}}{(|Aut(U_{\gamma})|)^{1_{\gamma \text{ is non-trivial}}}(|Aut(U_{\gamma'})|)^{1_{\gamma' \text{ is non-trivial}}}{c(\gamma')}}M^{fact}_{Id_{U_{\gamma}}}(v^{-\gamma}(v^{-\gamma})^T)} \preceq \\
		&\left(\sum_{\gamma' \in \Gamma_{*,V_{\tau}}}{\frac{1}{|Aut(U_{\gamma'})|{c(\gamma')}}}\right)B_{norm}(\tau)M^{fact}_{Id_{U_{\tau}}}(vv^{T}) + \\
		&\sum_{\gamma \in \Gamma_{*,U_{\tau}}}{\left(\sum_{\gamma' \in \Gamma_{*,V_{\tau}} \cup \{Id_{V_{\tau}}\}}{\frac{1}{(|Aut(U_{\gamma'})|)^{1_{\gamma' \text{ is non-trivial}}}{c(\gamma')}}}\right)\frac{B(\gamma)^{2}N(\gamma)^{2}B_{norm}(\tau){c(\gamma)}}{(|Aut(U_{\gamma})|)^{1_{\gamma \text{ is non-trivial}}}}M^{fact}_{Id_{U_{\gamma}}}(v^{-\gamma}(v^{-\gamma})^T)}  \preceq \\
		&{\epsilon'}B_{norm}(\tau)M^{fact}_{Id_{U_{\tau}}}(vv^{T}) + 
		2\sum_{\gamma \in \Gamma_{*,U_{\tau}}}{\frac{B(\gamma)^{2}N(\gamma)^{2}B_{norm}(\tau){c(\gamma)}}{|Aut(U_{\gamma})|}M^{fact}_{Id_{U_{\gamma}}}(v^{-\gamma}(v^{-\gamma})^T)}
	\end{align*}
	Following similar logic, 
	\begin{align*}
		&\sum_{\gamma \in \Gamma_{*,U_{\tau}} \cup \{Id_{U_{\tau}}\},\gamma' \in \Gamma_{*,V_{\tau}} \cup \{Id_{V_{\tau}}\}: \atop \gamma \text{ or } \gamma' \text{ is non-trivial }}{\frac{B(\gamma')^{2}N(\gamma')^{2}B_{norm}(\tau){c(\gamma')}}{(|Aut(U_{\gamma})|)^{1_{\gamma \text{ is non-trivial}}}(|Aut(U_{\gamma'})|)^{1_{\gamma' \text{ is non-trivial}}}{c(\gamma)}}M^{fact}_{Id_{U_{\gamma'}}}(w^{-\gamma'}(w^{-\gamma'})^T)} \preceq \\
		&{\epsilon'}B_{norm}(\tau)M^{fact}_{Id_{V_{\tau}}}(ww^{T}) + 
		2\sum_{\gamma' \in \Gamma_{*,V_{\tau}}}{\frac{B(\gamma')^{2}N(\gamma')^{2}B_{norm}(\tau){c(\gamma')}}{|Aut(U_{\gamma'})|}M^{fact}_{Id_{U_{\gamma'}}}(w^{-\gamma'}(w^{-\gamma'})^T)}
	\end{align*}
	Putting everything together,
	\begin{align*}
		&\left(M^{fact}_{\tau}(v{w^T}) + M^{fact}_{{\tau}^T}(w{v^T})\right) - \left(M^{orth}_{\tau}(v{w^T}) + M^{orth}_{{\tau}^T}(w{v^T})\right) \preceq \\
		&\\
		&{\epsilon'}B_{norm}(\tau)M^{fact}_{Id_{U_{\tau}}}(vv^{T}) + 
		2\sum_{\gamma \in \Gamma_{*,U_{\tau}}}{\frac{B(\gamma)^{2}N(\gamma)^{2}B_{norm}(\tau){c(\gamma)}}{|Aut(U_{\gamma})|}M^{fact}_{Id_{U_{\gamma}}}(v^{-\gamma}(v^{-\gamma})^T)} + \\
		&{\epsilon'}B_{norm}(\tau)M^{fact}_{Id_{V_{\tau}}}(ww^{T}) + 
		2\sum_{\gamma' \in \Gamma_{*,V_{\tau}}}{\frac{B(\gamma')^{2}N(\gamma')^{2}B_{norm}(\tau){c(\gamma')}}{|Aut(U_{\gamma'})|}M^{fact}_{Id_{U_{\gamma'}}}(w^{-\gamma'}(w^{-\gamma'})^T)}
	\end{align*}
	as needed.
\end{proof}
Using Lemma \ref{keyboundinglemma} we have the following corollaries:
\begin{corollary}\label{notauintersectiontermcorollary}
	For all $U \in \mathcal{I}_{mid}$, if the norm bounds and the conditions on $B(\gamma)$, $N(\gamma)$, and $c(\gamma)$ hold and $H_{Id_U} \succeq 0$ then  
	\[
	M^{fact}_{Id_{U}}(H_{Id_U}) - M^{orth}_{Id_{U}}(H_{Id_U}) \preceq {\epsilon'}M^{fact}_{Id_{U}}(H_{Id_U}) + 
	2\sum_{\gamma \in \Gamma_{*,U}}{\frac{B(\gamma)^{2}N(\gamma)^{2}{c(\gamma)}}{|Aut(U_{\gamma})|}M^{fact}_{Id_{U_{\gamma}}}(H^{-\gamma,\gamma}_{Id_{U}})}
	\]
\end{corollary}
\begin{corollary}\label{yestauintersectiontermcorollary}
	For all $U \in \mathcal{I}_{mid}$ and all $\tau \in \mathcal{M}_{U}$, if the norm bounds and the conditions on $B(\gamma)$, $N(\gamma)$, and $c(\gamma)$ hold and 
	\[
	\left[ {\begin{array}{cc}
			\frac{1}{|Aut(U)|c(\tau)}H_{Id_U} & B_{norm}(\tau)H_{\tau} \\
			B_{norm}(\tau)H^T_{\tau} & \frac{1}{|Aut(U)|c(\tau)}H_{Id_U}
	\end{array}} \right] \succeq 0
	\]
	then
	\begin{align*}
		&\left(M^{fact}_{\tau}(H_{\tau}) + M^{fact}_{{\tau}^T}(H^{T}_{\tau})\right) - \left(M^{orth}_{\tau}(H_{\tau}) + M^{orth}_{{\tau}^T}(H^{T}_{\tau})\right) \preceq \\
		&\\
		&2{\epsilon'}\frac{1}{|Aut(U)|c(\tau)}M^{fact}_{Id_{U}}(H_{Id_U}) + 
		4\sum_{\gamma \in \Gamma_{*,U}}{\frac{B(\gamma)^{2}N(\gamma)^{2}{c(\gamma)}}{|Aut(U_{\gamma})|\cdot|Aut(U)|c(\tau)}M^{fact}_{Id_{U_{\gamma}}}(H_{Id_{U}}^{-\gamma,\gamma}})
	\end{align*}
\end{corollary}
\subsection{Proof of the Main Theorem}
We now prove the following theorem which is a slight modification of Theorem \ref{maintheoremviaproperties} and which implies Theorem \ref{maintheoremviaproperties}.
\begin{theorem}\label{maintheoremviapropertiescopy}
	For all $\epsilon > 0$ and all $\epsilon' \in (0,\frac{1}{20}]$, for any moment matrix 
	\[
	\Lambda = \sum_{U \in \mathcal{I}_{mid}}{M^{orth}_{Id_U}(H_{Id_U})} + \sum_{U \in \mathcal{I}_{mid}}{\sum_{\tau \in \mathcal{M}_U}{M^{orth}_{\tau}(H_{\tau})}},
	\]
	if we have that for all $\alpha \in \mathcal{M}', ||M_{\alpha}|| \leq B_{norm}(\alpha)$ and $B(\gamma)$, $N(\gamma)$, and $c(\alpha)$ are functions such that 
	\begin{enumerate}
		\item For all $\tau \in \mathcal{M}'$, $\gamma \in \Gamma_{*,U_{\tau}}$, $\gamma' \in \Gamma_{*,V_{\tau}}$, and all intersection patterns $P \in \mathcal{P}_{\gamma,\tau,\gamma'}$, 
		\[
		B_{norm}(\tau_{P}) \leq B(\gamma)B(\gamma')B_{norm}(\tau)
		\]
		\item For all composable $\gamma_1,\gamma_2$, $B(\gamma_1)B(\gamma_2) = B(\gamma_1 \circ \gamma_2)$.
		\item $\forall U \in \mathcal{I}_{mid}, \sum_{\gamma \in \Gamma_{U,*}}{\frac{1}{|Aut(U)|c(\gamma)}} < \epsilon'$ 
		\item $\forall V \in \mathcal{I}_{mid}, \sum_{\gamma \in \Gamma_{*,V}}{\frac{1}{|Aut(U_{\gamma})|c(\gamma)}} < \epsilon'$ 
		\item $\forall U \in \mathcal{I}_{mid}, \sum_{\tau \in \mathcal{M}_{U}}{\frac{1}{|Aut(U)|c(\tau)}} < \epsilon'$
		\item For all $\tau \in \mathcal{M}'$, $\gamma \in \Gamma_{*,U_{\tau}} \cup \{Id_{U_{\tau}}\}$, and $\gamma' \in \Gamma_{*,V_{\tau}} \cup \{Id_{V_{\tau}}\}$,
		\begin{align*}
			&\sum_{j>0}{\sum_{\gamma_1,\gamma'_1,\cdots,\gamma_j,\gamma'_j \in \Gamma_{\gamma,\gamma',j}}{\prod_{i:\gamma_i \text{ is non-trivial}}{\frac{1}{|Aut(U_{\gamma_i})|}}
					\prod_{i:\gamma'_i \text{ is non-trivial}}{\frac{1}{|Aut(U_{\gamma'_i})|}}}}\sum_{P_1,\cdots,P_j:P_i \in \mathcal{P}_{\gamma_i,\tau_{P_{i-1}},{\gamma'_i}^T}}{\left(\prod_{i=1}^{j}{N(P_i)}\right)} \\
			&\leq \frac{N(\gamma)N(\gamma')}
			{(|Aut(U_{\gamma})|)^{1_{\gamma \text{ is non-trivial}}}(|Aut(U_{\gamma'})|)^{1_{\gamma' \text{ is non-trivial}}}}
		\end{align*}
	\end{enumerate}
	and we have SOS-symmetric coefficient matrices $\{H'_{\gamma}: \gamma \in \Gamma\}$ such that the following conditions hold:
	\begin{enumerate}
		\item For all $U \in \mathcal{I}_{mid}$,  $H_{Id_{U}} \succeq 0$
		\item For all $U \in \mathcal{I}_{mid}$ and $\tau \in \mathcal{M}_U$,
		\[
		\left[ {\begin{array}{cc}
				\frac{1}{|Aut(U)|c(\tau)}H_{Id_{U}} & B_{norm}(\tau)H_{\tau} \\
				B_{norm}(\tau)H^T_{\tau} & \frac{1}{|Aut(U)|c(\tau)}H_{Id_{U}}
		\end{array}} \right] \succeq 0
		\]
		\item For all $U,V \in \mathcal{I}_{mid}$ where $w(U) > w(V)$ and all $\gamma \in \Gamma_{U,V}$, 
		\[
		c(\gamma)^2{N(\gamma)}^2{B(\gamma)^2}H^{-\gamma,\gamma}_{Id_{V}} \preceq H'_{\gamma}
		\]
	\end{enumerate}
	then 
	\[
	\Lambda \succeq \frac{1}{2}\left(\sum_{U \in \mathcal{I}_{mid}}{M^{fact}_{Id_U}{(H_{Id_U})}}\right) - 3\left(\sum_{U \in \mathcal{I}_{mid}}{\sum_{\gamma \in \Gamma_{U,*}}{\frac{d_{Id_{U}}(H'_{\gamma},H_{Id_{U}})}{|Aut(U)|c(\gamma)}}}\right)Id_{sym}
	\]
	If it is also true that 
	\[
	\sum_{U \in \mathcal{I}_{mid}}{M^{fact}_{Id_U}{(H_{Id_U})}} \succeq 6\left(\sum_{U \in \mathcal{I}_{mid}}{\sum_{\gamma \in \Gamma_{U,*}}{\frac{d_{Id_{U}}(H'_{\gamma},H_{Id_{U}})}{|Aut(U)|c(\gamma)}}}\right)Id_{sym}
	\]
	then $\Lambda \succeq 0$.
\end{theorem}
\begin{proof}
	We make the following observations:
	\begin{enumerate}
		\item By Theorem \ref{thm:nointersectionanalysis},
		\[
		\sum_{U \in \mathcal{I}_{mid}}{M^{fact}_{Id_U}(H_{Id_U})} + \sum_{U \in \mathcal{I}_{mid}}{\sum_{\tau \in \mathcal{M}_U}{M^{fact}_{\tau}(H_{\tau})} \succeq (1-2\epsilon')\sum_{U \in \mathcal{I}_{mid}}{M^{fact}_{Id_U}(H_{Id_U})}}
		\]
		\item By Corollary \ref{notauintersectiontermcorollary}, 
		\[
		\sum_{U \in \mathcal{I}_{mid}}{\left(M^{fact}_{Id_{U}}(H_{Id_U}) - M^{orth}_{Id_{U}}(H_{Id_U})\right)} \preceq {\epsilon'}\sum_{U \in \mathcal{I}_{mid}}{M^{fact}_{Id_{U}}(H_{Id_U})} + 
		2\sum_{U \in \mathcal{I}_{mid}}{\sum_{\gamma \in \Gamma_{*,U}}{\frac{M^{fact}_{Id_{U_{\gamma}}}(H'_{\gamma})}{c(\gamma)|Aut(U_{\gamma})|}}}
		\]
		\item By Corollary \ref{yestauintersectiontermcorollary}, 
		\begin{align*}
			&\sum_{U \in \mathcal{I}_{mid}}{\sum_{\tau \in \mathcal{M}_U}{\left(M^{fact}_{\tau}(H_{\tau}) - M^{orth}_{\tau}(H_{\tau})\right)}} \preceq \\
			&\\
			&\sum_{U \in \mathcal{I}_{mid}}{\sum_{\tau \in \mathcal{M}_U}{\left(\frac{2{\epsilon'}}{|Aut(U)|c(\tau)}M^{fact}_{Id_{U}}(H_{Id_U}) + 
					4\sum_{\gamma \in \Gamma_{*,U}}{\frac{B(\gamma)^{2}N(\gamma)^{2}{c(\gamma)}}{|Aut(U_{\gamma})|\cdot|Aut(U)|c(\tau)}M^{fact}_{Id_{U_{\gamma}}}(H_{Id_{U}}^{-\gamma,\gamma})}\right)}} \preceq \\
			&2{\epsilon'}^2\sum_{U \in \mathcal{I}_{mid}}{M^{fact}_{Id_{U}}(H_{Id_U})} + 
			4{\epsilon'}\sum_{U \in \mathcal{I}_{mid}}{\sum_{\gamma \in \Gamma_{*,U}}{\frac{M^{fact}_{Id_{U_{\gamma}}}(H'_{\gamma})}{c(\gamma)|Aut(U_{\gamma})|}}}
		\end{align*}
		\item
		\begin{align*}
			&\sum_{U \in \mathcal{I}_{mid}}{\sum_{\gamma \in \Gamma_{*,U}}{\frac{M^{fact}_{Id_{U_{\gamma}}}(H'_{\gamma})}{c(\gamma)|Aut(U_{\gamma})|}}} = 
			\sum_{U \in \mathcal{I}_{mid}}{\sum_{\gamma \in \Gamma_{*,U}}{\frac{M^{fact}_{Id_{U_{\gamma}}}(H_{Id_{U_\gamma}}) + \left(M^{fact}_{Id_{U_{\gamma}}}(H'_{\gamma}) - M^{fact}_{Id_{U_{\gamma}}}(H_{Id_{U_\gamma}})\right)}{c(\gamma)|Aut(U_{\gamma})|}}} \preceq \\
			&\sum_{U \in \mathcal{I}_{mid}}{\sum_{\gamma \in \Gamma_{*,U}}{\frac{M^{fact}_{Id_{U_{\gamma}}}(H_{Id_{U_{\gamma}}})}{c(\gamma)|Aut(U_{\gamma})|}}} + 
			\left(\sum_{U \in \mathcal{I}_{mid}}{\sum_{\gamma \in \Gamma_{U,*}}{\frac{d_{Id_{U_{\gamma}}}(H'_{\gamma},H_{Id_{U_{\gamma}}})}{|Aut(U_{\gamma})|c(\gamma)}}}\right)Id_{sym} \preceq \\
			&{\epsilon'}\sum_{U \in \mathcal{I}_{mid}}{M^{fact}_{U}(H_{Id_{U}})} + 
			\left(\sum_{U \in \mathcal{I}_{mid}}{\sum_{\gamma \in \Gamma_{U,*}}{\frac{d_{Id_{U_{\gamma}}}(H'_{\gamma},H_{Id_{U_{\gamma}}})}{|Aut(U_{\gamma})|c(\gamma)}}}\right)Id_{sym}
		\end{align*}
	\end{enumerate}
	Putting everything together, 
	\begin{align*}
		&\Lambda = \sum_{U \in \mathcal{I}_{mid}}{M^{orth}_{Id_U}(H_{Id_U})} + \sum_{U \in \mathcal{I}_{mid}}{\sum_{\tau \in \mathcal{M}_U}{M^{orth}_{\tau}(H_{\tau})}} = \\
		&\sum_{U \in \mathcal{I}_{mid}}{M^{fact}_{Id_U}(H_{Id_U})} + \sum_{U \in \mathcal{I}_{mid}}{\sum_{\tau \in \mathcal{M}_U}{M^{fact}_{\tau}(H_{\tau})}} + 
		\sum_{U \in \mathcal{I}_{mid}}{\left(M^{fact}_{Id_{U}}(H_{Id_U}) - M^{orth}_{Id_{U}}(H_{Id_U})\right)} + \\
		&\sum_{U \in \mathcal{I}_{mid}}{\sum_{\tau \in \mathcal{M}_U}{\left(M^{fact}_{\tau}(H_{\tau}) - M^{orth}_{\tau}(H_{\tau}) \right)}} \succeq \\
		&(1 - 3{\epsilon'} - 2{\epsilon'}^2)\sum_{U \in \mathcal{I}_{mid}}{M^{fact}_{Id_U}(H_{Id_U})} - 
		(2 + 4\epsilon')\sum_{U \in \mathcal{I}_{mid}}{\sum_{\gamma \in \Gamma_{*,U}}{\frac{M^{fact}_{Id_{U_{\gamma}}}(H'_{\gamma})}{c(\gamma)|Aut(U_{\gamma})|}}} \succeq \\
		&(1 - 5{\epsilon'} - 6{\epsilon'}^2)\sum_{U \in \mathcal{I}_{mid}}{M^{fact}_{Id_U}(H_{Id_U})} - 
		(2 + 4\epsilon')\left(\sum_{U \in \mathcal{I}_{mid}}{\sum_{\gamma \in \Gamma_{U,*}}{\frac{d_{Id_{U_{\gamma}}}(H'_{\gamma},H_{Id_{U_{\gamma}}})}{|Aut(U_{\gamma})|c(\gamma)}}}\right)Id_{sym} \succeq \\
		&\frac{1}{2}\sum_{U \in \mathcal{I}_{mid}}{M^{fact}_{Id_U}(H_{Id_U})} - 
		3\left(\sum_{U \in \mathcal{I}_{mid}}{\sum_{\gamma \in \Gamma_{U,*}}{\frac{d_{Id_{U_{\gamma}}}(H'_{\gamma},H_{Id_{U_{\gamma}}})}{|Aut(U_{\gamma})|c(\gamma)}}}\right)Id_{sym}
	\end{align*}
\end{proof}

==> machinery/showing_positivity.tex <==
\subsection{General strategy to lower bound $\sum_{V \in \mathcal{I}_{mid}}{M^{fact}(H_{Id_V})}$}\label{subsec: positivity_lower_bound_strategy}

In this section, we describe how to show that $\sum_{V \in \mathcal{I}_{mid}}{M^{fact}(H_{Id_V})} \succeq {\delta}Id_{Sym}$ for some $\delta > 0$ where $\delta$ will depend on $n$ and other parameters. For now, we assume that the indices of $\Lambda$ are multilinear monomials. We will then describe the adjustments that are needed to handle non-multilinear matrix indices.

We start with a few more definitions.
\begin{definition}
	For all $V \in \mathcal{I}_{mid}$ we define $Id_{Sym,V}$ to be the matrix such that 
	\begin{enumerate}
		\item $Id_{Sym,V}(A,B) = 1$ if $A$ and $B$ both have index shape $V$.
		\item Otherwise, $Id_{Sym,V}(A,B) = 0$.
	\end{enumerate}
\end{definition}
\begin{proposition}
	$Id_{Sym} = \sum_{V \in \mathcal{I}_{mid}}{Id_{Sym,V}}$
\end{proposition}
\begin{definition}
	For all $V \in \mathcal{I}_{mid}$ we define $\lambda_V = |Aut(V)|H_{Id_V}(Id_V,Id_V)$
\end{definition}
We now describe our strategy for showing $\sum_{V \in \mathcal{I}_{mid}}{M^{fact}(H_{Id_V})} \succeq {\delta}Id_{Sym}$. The idea is as follows. We will consider the index shapes $V \in \mathcal{I}_{mid}$ from largest weight to smallest weight and we will show that for each $V \in \mathcal{I}_{mid}$, there exists a $\delta_V > 0$ such that $\sum_{V \in \mathcal{I}_{mid}}{M^{fact}(H_{Id_V})} \succeq \delta_{V}\sum_{U \in \mathcal{I}_{mid}: w(U) \geq w(V)}{Id_{Sym,U}}$.

For the first step, letting $V_{max}$ be the maximum weight index shape in $\mathcal{I}_{mid}$, $M^{fact}(H_{Id_{V_{max}}}) = \lambda_{V_{max}}Id_{Sym,V_{max}}$ because there are no non-trivial left shapes $\sigma$ such that $V_{\sigma} = V_{max}$. For other $V \in \mathcal{I}_{mid}$, $\lambda_{V}Id_{Sym,V}$ is a part of $M^{fact}(H_{Id_V})$ but $M^{fact}(H_{Id_V})$ will also contain terms of the form $H_{Id_V}(\sigma,\sigma')M_{\sigma}M_{{\sigma'}^T}$ where $U_{\sigma} \neq V$ or $U_{\sigma'} \neq V$. 

We can handle the terms $H_{Id_V}(\sigma,\sigma')M_{\sigma}M_{{\sigma'}^T}$ where $U_{\sigma} \neq V$ and $U_{\sigma'} \neq V$ by bounding these terms in terms of $Id_{Sym,U_{\sigma}}$ and $Id_{Sym,U_{\sigma'}}$. Since $w(U_{\sigma}) > w(V)$ and $w(U_{\sigma'}) > w(V)$, $Id_{Sym,U_{\sigma}}$ and $Id_{Sym,U_{\sigma'}}$ are already available to us. To handle the terms $H_{Id_V}(\sigma,\sigma')M_{\sigma}M_{{\sigma'}^T}$ where exactly one of $U_{\sigma}$ and $U_{\sigma'}$ are equal to $V$, we use the following trick.
\begin{definition}
	Given $V \in \mathcal{I}_{mid}$, define $H''_{Id_V}$ to be the coefficient matrix such that 
	\begin{enumerate}
		\item If $U_{\sigma} = U_{\sigma'} = V$ then $H''_{Id_V}(\sigma,\sigma') = \frac{1}{2}H_{Id_V}(\sigma,\sigma')$
		\item If exactly one of $U_{\sigma}$ and $U_{\sigma'}$ are equal to $V$ then $H''_{Id_V}(\sigma,\sigma') = H_{Id_V}(\sigma,\sigma')$
		\item If $U_{\sigma} \neq V$ and $U_{\sigma'} \neq V$ then $H''_{Id_V}(\sigma,\sigma') = 2H_{Id_V}(\sigma,\sigma')$
	\end{enumerate}
\end{definition}
\begin{proposition}
	$M^{fact}(H''_{Id_V}) \succeq 0$
\end{proposition}
\begin{proof}
	Since $H_{Id_V} \succeq 0$, $H''_{Id_V} \succeq 0$ and thus $M^{fact}(H''_{Id_V}) \succeq 0$.
\end{proof}
\begin{corollary}\label{cor: showing_positivity_corollary}
	For all $V \in \mathcal{I}_{mid}$, 
	\[
	M^{fact}(H_{Id_V}) + \sum_{\sigma,\sigma' \in \mathcal{L}_V: U_{\sigma} \neq V, U_{\sigma'} \neq V}{H_{Id_V}(\sigma,\sigma')M_{\sigma}M_{{\sigma'}^T}} \succeq \frac{\lambda_V}{2}Id_{Sym,V}
	\]
\end{corollary}
\begin{proof}
	Observe that 
	\[
	M^{fact}(H_{Id_V})  -  \frac{\lambda_V}{2}Id_{Sym,V} + \sum_{\sigma,\sigma' \in \mathcal{L}_V: U_{\sigma} \neq V, U_{\sigma'} \neq V}{H_{Id_V}(\sigma,\sigma')M_{\sigma}M_{{\sigma'}^T}} = 
	M^{fact}(H''_{Id_V}) \succeq 0
	\]
\end{proof}
We now analyze the terms $ \sum_{\sigma,\sigma' \in \mathcal{L}_V: U_{\sigma} \neq V, U_{\sigma'} \neq V}{H_{Id_V}(\sigma,\sigma')M_{\sigma}M_{{\sigma'}^T}}$.
\begin{definition}
	Given $U,V \in \mathcal{I}$ with $w(U) > w(V)$, we define $W(U,V)$ to be
	\[
	W(U,V) = \frac{1}{|Aut(U)|}\sum_{\sigma \in \mathcal{L}_{V}: U_{\sigma} = U}{\sum_{\sigma' \in \mathcal{L}_{V}: U_{\sigma'} \neq V}{B_{norm}(\sigma)B_{norm}(\sigma')H_{Id_V}(\sigma,\sigma')}}
	\]
\end{definition}
\begin{lemma}\label{showingpositivitylemma}
	For all $V \in \mathcal{I}_{mid}$, 
	\[
	\sum_{\sigma,\sigma' \in \mathcal{L}_V: U_{\sigma} \neq V, U_{\sigma'} \neq V}{H_{Id_V}(\sigma,\sigma')M_{\sigma}M_{{\sigma'}^T}} \preceq \sum_{U \in \mathcal{I}_{mid}: w(U) > w(V)}{W(U,V)Id_{Sym,U}}
	\]
\end{lemma}
\begin{proof}
	Observe that for all $\sigma,\sigma' \in \mathcal{L}_{V}$ such that $U_{\sigma} \neq V$ and $U_{\sigma'} \neq V$, $||M_{\sigma}M_{{\sigma'}^T}|| \leq B_{norm}(\sigma)B_{norm}(\sigma')$ and thus 
	\[
	\frac{1}{2}\left(M_{\sigma}M_{{\sigma'}^T} + M_{\sigma'}M_{{\sigma}^T}\right) \preceq \frac{1}{2}B_{norm}(\sigma)B_{norm}(\sigma')\left(M_{Id_{U_{\sigma}}} + M_{Id_{U_{\sigma'}}}\right)
	\]
	Summing this equation over all $\sigma,\sigma' \in \mathcal{L}_{V}$ such that $U_{\sigma} \neq V$ and $U_{\sigma'} \neq V$,
	\begin{align*}
		&\sum_{\sigma,\sigma' \in \mathcal{L}_V: U_{\sigma} \neq V, U_{\sigma'} \neq V}{H_{Id_U}(\sigma,\sigma')M_{\sigma}M_{{\sigma'}^T}} \preceq 
		\sum_{\sigma,\sigma' \in \mathcal{L}_V: U_{\sigma} \neq V, U_{\sigma'} \neq V}{B_{norm}(\sigma)B_{norm}(\sigma')M_{Id_{U_{\sigma}}}} \\
		&\preceq \sum_{U \in \mathcal{I}_{mid}: w(U) > w(V)}{\sum_{\sigma \in \mathcal{L}_{V}: U_{\sigma} = U}{\sum_{\sigma' \in \mathcal{L}_{V}: V_{\sigma} \neq V}{B_{norm}(\sigma)B_{norm}(\sigma')H_{Id_U}(\sigma,\sigma')M_{Id_U}}}} \\
		&\preceq \sum_{U \in \mathcal{I}_{mid}: w(U) > w(V)}|Aut(U)|W(U,V)M_{Id_U}
	\end{align*}
	Since all of the coefficient matrices have SOS-symmetry, we can replace $M_{Id_U}$ by $\frac{1}{|Aut(U)|}Id_{Sym,U}$ and this completes the proof.
\end{proof}
Using this lemma, we can show the following theorem:
\begin{theorem}
	Let $G$ be the following directed graph:
	\begin{enumerate}
		\item The vertices of $G$ are the index shapes $V \in \mathcal{I}_{mid}$
		\item For each $U,V \in \mathcal{I}_{mid}$ such that $w(U) > w(V)$, we have an edge $e = (V,U)$ with weight $w(e) = \frac{2W(U,V)}{\lambda_V}$
	\end{enumerate}
	For all $V \in \mathcal{I}_{mid}$,
	\[
	Id_{Sym,V} \preceq 2\sum_{U \in \mathcal{I}_{mid}: w(U) \geq w(V)}{\left(\sum_{P: P \text{ is a path from V to U in } G}{\prod_{e \in E(P)}{w(e)}}\right)\frac{1}{{\lambda_{U}}}M^{fact}(H_{Id_{U}})}
	\]
\end{theorem}
\begin{proof}[Proof sketch]
	This can be proved by starting with \cref{cor: showing_positivity_corollary} and iteratively applying Lemma \ref{showingpositivitylemma} and \cref{cor: showing_positivity_corollary}.
\end{proof}
\subsubsection{Handling Non-multilinear Matrix Indices*}
In order to handle non-multilinear matrix indices, we need to make a few adjustments. First, we need to modify the definition of $Id_{Sym,V}$.
\begin{definition}
    For all $V \in \mathcal{I}_{mid}$ we define $Id_{Sym,V}$ to be the matrix such that 
	\begin{enumerate}
		\item $Id_{Sym,V}(A,B) = 1$ if $A$ and $B$ have the same index shape $U$ and $U$ has the same number of each type of vertex as $V$. Note that $B$ may be a permutation of $A$ and $U$ may have different powers than $V$.
		\item Otherwise, $Id_{Sym,V}(A,B) = 0$.
	\end{enumerate}
\end{definition}

Observe that with this modified definition, we will still have $Id_{Sym} = \sum_{V \in \mathcal{I}_{mid}}{Id_{Sym,V}}$.

We also need to adjust how we define $\lambda_V$ as there are left shapes $\sigma$ such that $U_{\sigma}$ and $V_{\sigma}$ have the same numbers and types of vertices but $U_{\sigma}$ has different powers.
\begin{definition}
Given $V \in \mathcal{I}_{mid}$, we define $\mathcal{T}_V \subseteq \mathcal{L}_V$ to be the set of left shapes $\sigma \in \mathcal{L}_V$ such that $U_{\sigma}$ has the same numbers and types of vertices as $V$ (which automatically implies that $E(\sigma) = \emptyset$).
\end{definition}

\begin{definition}
Define $Id^{*}_{Sym,V}$ to be the matrix indexed by left shapes $\sigma,\sigma' \in \mathcal{T}_V$ such that $Id^{*}_{Sym,V}(\sigma,\sigma') = \frac{1}{|Aut(V)|}$ if $U_{\sigma} \equiv U_{\sigma'}$ and $Id^{*}_{Sym,V}(\sigma,\sigma') = 0$ otherwise.
\end{definition}
\begin{proposition}
$M^{fact}(Id^{*}_{Sym,V}) = Id_{Sym,V}$
\end{proposition}
\begin{definition}
Let $H'_{Id_V}$ be the matrix $H_{Id_V}$ restricted to rows and columns $\sigma,\sigma'$ where $\sigma,\sigma' \in \mathcal{T}_V$. We define $\lambda_V$ to be the largest constant $\lda$ such that $H'_{Id_V} \succeq {\lambda}Id^{*}_{Sym,V}$
\end{definition}

Finally, whenever we have the condition that $U_{\sigma} \neq V$, it should instead be the condition that $U_{\sigma}$ does not have the same number of each type of vertex as $V$. With these adjustments, the same arguments go through.
\subsection{Strategy to prove positivity in our applications}

Now, we will illustrate the final ingredients needed to show positivity for our applications.

To use \cref{generalmaintheorem}, we would need to prove a statement of the form: Whenever $\norm{M_{\alpha}} \le B_{norm}(\alpha)$ for all $\alpha \in \mathcal{M}'$,
\[
	\sum_{U \in \mathcal{I}_{mid}}{M^{fact}_{Id_U}{(H_{Id_U})}} \succeq 6\left(\sum_{U \in \mathcal{I}_{mid}}{\sum_{\gamma \in \Gamma_{U,*}}{\frac{d_{Id_{U}}(H'_{\gamma},H_{Id_{U}})}{|Aut(U)|c(\gamma)}}}\right)Id_{sym}
\]

We will sketch the strategy we use to prove this. Let $D_{sos}$ be the degree of the SoS program.

For the left hand side, we will prove a lower bound of the form: Whenever $\norm{M_{\al}} \le B_{norm}(\al)$ for all $\al \in \calM'$,
\[
\sum_{U \in \mathcal{I}_{mid}}{M^{fact}_{Id_U}{(H_{Id_U})}} \succeq \frac{1}{n^{K_1D_{sos}^2}} Id_{sym}
\]
for a constant $K_1 > 0$. For this, we use the strategy from \cref{subsec: positivity_lower_bound_strategy}. Then, we prove an upper bound on the right hand side of the form
\[\sum_{U\in \calI_{mid}} \sum_{\gam \in \Gam_{U, *}} \frac{d_{Id_{U}}(H_{Id_{U}}, H'_{\gam})}{|Aut(U)|c(\gam)} \le \frac{n^{K_2D_{sos}}}{2^{D_V}}\]
for a constant $K_2 > 0$.

Now, we put these two together. Using the fact that $Id_{Sym} \succeq 0$, by simply setting $\frac{1}{n^{K_1D_{sos}^2}} > \frac{n^{K_2D_{sos}}}{2^{D_V}}$ which can be obtained by choosing $D_{sos}$ small enough, we obtain the desired result.

We will also need the following bound that says that  that lets us sum over all shapes if we have sufficient decay for each vertex, then, the sum of this decay, over all shapes $\sig \circ \sig'$ for $\sig, \sig' \in \calL_U'$, is bounded.

\begin{definition}
	For $U \in \calI_{mid}$, let $\calL_{U}' \subset \calL_U$ be the set of non-trivial shapes in $\calL_U$.
\end{definition}

\begin{lemma}\label{lem: gp_sum}
    Suppose $D_V = n^{C_V\eps}, D_E = n^{C_E\eps}$ for constants $C_V, C_E > 0$, are the truncation parameters for our shapes. For any $U \in \calI_{mid}$, 
	\begin{align*}
	\sum_{U\in \calI_{mid}} \sum_{\sig, \sig' \in \calL'_U} \frac{1}{D_{sos}^{D_{sos}}n^{F \eps|V(\sig \circ \sig')|}} \le 1
	\end{align*}
	for a constant $F > 0$ that depends only on $C_V, C_E$. In particular, by setting $C_V, C_E$ small enough, we can make this constant arbitrarily small.
\end{lemma}

\begin{proof}
	For a given $j = |U|$, the number of ways to choose $U$ is at most $t_{max}^j$. For a given $U \in \calI_{mid}$, we will bound the number of ways to choose $\sig, \sig' \in \calL_U'$. To choose $\sig, \sig'\in \calL'_U$, it is sufficient to choose
	\begin{itemize}
		\item The number of vertices $j_1 \ge 1$ (resp. $j_1' \ge 1$) in $U_{\sig} \setminus V_{\sig}$ (resp. $U_{\sig'} \setminus V_{\sig'}$), their types of which there are at most $t_{max}$, and their powers which have at most $D_{sos}$ choices.
		\item The number of vertices $j_2$ (resp. $j_2'$) in $V(\sig) \setminus (U_{\sig} \cup V_{\sig})$ (resp. $V(\sig') \setminus (U_{\sig'} \cup V_{\sig'})$) and also their types, of which there are at most $t_{max}$.
		\item The position of each vertex $i$ in $U_{\sig} \setminus V_{\sig}$ (resp. $U_{\sig'} \setminus V_{\sig'}$) within $U_{\sig}$ (resp. $U_{\sig'}$). There are at most $D_V$ choices for each vertex.
		\item The subset of $U_{\sig}$ (resp. $U_{\sig'}$) that is in $V_{\sig}$ (resp. $V_{\sig'}$) and a mapping in $Aut(U_{\sig} \cap V_{\sig})$ (resp. $Aut(U_{\sig'} \cap V_{\sig'})$) that determines the matching between the vertices in $U_{\sig} \cap V_{\sig}$ (resp. $U_{\sig'} \cap V_{\sig'}$).
		\item The number $j_3$ (resp. $j_3'$) of edges in $E(\sig)$ (resp. $E(\sig')$). and the $k$ endpoints of each edge. Each endpoint has at most $D_V$ choices.
	\end{itemize}
	Therefore, for all $j \ge 0, j_1, j_1' \ge 1, j_2, j_2', j_3, j_3' \ge 0$, we have
	\begin{align*}
	\sum_{U \in \calI_{mid}}\sum_{\substack{\sig, \sig' \in \calL'_U \\ |U_{\sig} \setminus V_{\sig}| = j_1, |U_{\sig'} \setminus V_{\sig'}| = j_1' \\ |V(\sig) \setminus (U_{\sig} \cup V_{\sig})| = j_2, |V(\sig') \setminus (U_{\sig'} \cup V_{\sig'})| = j_2'\\ |E(\sig)| = j_3, |E(\sig')| = j_3'}} \frac{1}{|Aut(U_{\sig'} \cap V_{\sig'})||Aut(U_{\sig} \cap V_{\sig})|(2t_{max})^{j + j_2 + j_2'}(D_Vt_{max}D_{sos})^{j_1 + j_1'}(D_V)^{kj_3}} \le 1
	\end{align*}
	This implies that
	\begin{align*}
	\sum_{U\in \calI_{mid}} \sum_{\sig, \sig' \in \calL'_U} \frac{1}{D_{sos}^{D_{sos}}n^{F \eps|V(\sig \circ \sig')|}} \le 1
	\end{align*}
	for a constant $F > 0$ that only depends on $C_V, C_E$.
\end{proof}

==> machinery/technical_def_and_main_theorem.tex <==
\begin{comment}

In this section, we give the precise definitions needed to state the main theorem statement of the machinery. An informal theorem statement can be found in \cite{potechin2020machinery}.

As we have already seen in \cref{chap: sk}, the general idea to show SoS lower bounds in this work is to decompose the moment matrix into graph matrices, which are matrix-valued functions of the input entries, and show PSDness using various norm bounds. The machinery takes a similar approach and provides an approximate PSD decomposition, using certain decay properties of the Fourier coefficients.

In general, the machinery handles problems where one or more of the following is true:
\begin{enumerate}
	\item The input entries correspond to hyperedges rather than edges.
	\item We have different types of indices.
	\item The alphabet $\Omega$ is a more complicated distribution than $\{-1,+1\}$.
	\item We have to consider matrix indices which are not multilinear.
\end{enumerate}

Throughout this section, we give the reader a choice for the level of generality of this machinery. In particular, we will first state the definition for the simpler case when the input is $\{-1,+1\}^{\binom{n}{2}}$ and we only consider multilinear indices. We will then discuss how this simpler definition generalizes. We denote these generalizations with an asterisk $*$.
\subsubsection{Additional Parameters for the General Case*}
In the general case we will need a few additional parameters which we define here.
\begin{definition} \
	\begin{enumerate}
		\item We define $k$ to be the arity of the hyperedges corresponding to the input.
		\item We define $t_{max}$ to be the number of different types of indices. We define $n_i$ to be the number of possibilities for indices of type $i$ and we define $n = \max{\{n_i: i \in [t_{max]}\}}$.
	\end{enumerate}
\end{definition}
\subsection{Indices, Input Entries, Vertices, and Edges}
Note: For this section, we use $X$ to denote the input, we use $x$ to denote entries of the input and we use $y$ to denote solution variables.
\begin{definition}[Vertices: Simplified Case]
	When the input and solution variables are indexed by one type of index which takes values in $[n]$ then we represent the index $i$ by a vertex labeled $i$.

	If we want to leave an index unspecified, we instead represent it by a vertex labeled with a variable (we will generally use $u$, $v$, or $w$ for these variables).
\end{definition}
\begin{definition}[Vertices: General Case*]
	When the input and solution variables are indexed by several types of indices where indices of type $t$ take values in $[n_t]$, we represent an index of type $t$ with value $i$ as a vertex labeled by the tuple $(t,i)$. We say that such a vertex has type $t$.

	If we want to leave an index of type $t$ unspecified, we instead represent it by a vertex labeled with a tuple $(t,?)$ where $?$ is a variable (which will generally be $u$, $v$, or $w$).
\end{definition}
\begin{definition}[Edges: Simplified Case]
	When the input is $X \in \{-1,+1\}^{\binom{n}{2}}$, we represent the entries of the input by the undirected edges $\{(i,j): i < j \in [n]\}$. Given an edge $e = (i,j)$, we take $x_e = x_{ij}$ to be the input entry corresponding to $e$.
\end{definition}
\begin{definition}[Edges: General Case*]
	In general, we represent the entries of the input by hyperedges whose form depends on nature of the input. We still take $x_e$ to be the input entry corresponding to $e$.
\end{definition}
\begin{example}
	If the input is an $n_1 \times n_2$ matrix $X$ then we will have two types of indices, one for the row and one for the column. Thus, we will have the vertices $\{(1,i): i \in [n_1]\} \cup \{(2,j): j \in [n_2]\}$. In this case, we have an edge $((1,i),(2,j))$ for each entry $x_{ij}$ of the input.
\end{example}
\begin{example}
	If the input is an $n \times n$ matrix $X$ which is not symmetric then we only need the indices $[n]$. In this case, we have a directed edge $(i,j)$ for each entry $x_{ij}$ where $i \neq j$. If the entries $x_{ii}$ are also part of the input than we also have loops $(i,i)$ for these entries.
\end{example}
\begin{example}
	If our input is a symmetric $n \times n \times n$ tensor $X$ (i.e. $x_{ijk} = x_{ikj} = x_{jik} = x_{jki} = x_{kij} = x_{kji}$) and $x_{ijk} = 0$ whenever $i,j,k$ are not distinct then we only need the indices $[n]$. In this case, we have an undirected hyperedge $e = (i,j,k)$ for each entry $x_{e} = x_{ijk}$ of the input where $i,j,k$ are distinct.
\end{example}
\begin{example}
	If the input is an $n_1 \times n_2 \times n_3$ tensor $X$ then we will have three types of indices. Thus, we will have the vertices $\{(1,i): i \in [n_1]\} \cup \{(2,j): j \in [n_2]\} \cup \{(3,k): k \in [n_3]\}$. In this case, we have a hyperedge $e = ((1,i),(2,j),(3,k))$ for each entry $x_e = x_{ijk}$ of the input.
\end{example}
\subsection{Matrix Indices and Monomials}
In this subsection, we discuss how our matrices are indexed and how we associate matrix indices with monomials. We also describe the automorphism groups of matrix indices.
\begin{definition}[Matrix Indices: Simplified Case]
	If there is only one type of index and we have the constraints $y^2_i = 1$ or $y^2_i = y_i$ on the solution variables then we define a matrix index $A$ to be a tuple of indices $(a_1,\ldots,a_{|A|})$. We make the following definitions about matrix indices:
	\begin{enumerate}
		\item We associate the monomial $\prod_{j=1}^{|A|}{y_{a_j}}$ to $A$.
		\item We define $V(A)$ to be the set of vertices $\{a_i: i \in [|A|]\}$. For brevity, we will often write $A$ instead of $V(A)$ when it is clear from context that we are referring to $A$ as a set of vertices rather than a matrix index.
		\item We take the automorphism group of $A$ to be $Aut(A) = S_{|A|}$ (the permutations of the elements of $A$)
	\end{enumerate}
\end{definition}
\begin{example}
	The matrix index $A = (4,6,1)$ represents the monomial ${y_4}{y_6}{y_1} = {y_1}{y_4}{y_6}$ and $Aut(A) = S_3$
\end{example}
\begin{remark}
	We take $A$ to be an ordered tuple rather than a set for technical reasons.
\end{remark}
In general, we need a more intricate definition for matrix indices. We start by defining matrix index pieces
\begin{definition}[Matrix Index Piece Definition*]
	We define a matrix index piece $A_i = ((a_{i1},\ldots,a_{i|A_i|}), t_i, p_i)$ to be a tuple of indices $(a_{i1},\ldots,a_{i|A_i|})$ together with a type $t_i$ and a power $p_i$. We make the following definitions about matrix index pieces:
	\begin{enumerate}
		\item We associate the monomial $p_{A_i} = \prod_{j = 1}^{|A_i|}{y^{p_i}_{{t_i}j}}$ with $A_i$.
		\item We define $V(A_i)$ to be the set of vertices $\{(t_i,a_{ij}): j \in [|A_i|]\}$.
		\item We take the automorphism group of $A_i$ to be $Aut(A_i) = S_{|A_i|}$
		\item We say that $A_i$ and $A_j$ are disjoint if $V(A_i) \cap V(A_j) = \emptyset$ (i.e. $t_i \neq t_j$ or $\{a_{i1},\ldots,a_{i|A_i|}\} \cap \{a_{j1},\ldots,a_{j|A_j|}\} = \emptyset$)
	\end{enumerate}
\end{definition}
\begin{definition}[General Matrix Index Definition*]
	We define a matrix index $A = \{A_i\}$ to be a set of disjoint matrix index pieces. We make the following definitions about matrix indices:
	\begin{enumerate}
		\item We associate the monomial $p_{A} = \prod_{A_i \in A}{p(A_i)}$ with $A$.
		\item We define $V(A)$ to be the set of vertices $\cup_{A_i \in A}{V(A_i)}$. For brevity, we will often write $A$ instead of $V(A)$ when it is clear from context that we are referring to $A$ as a set of vertices rather than a matrix index.
		\item We take the automorphism group of $A$ to be $Aut(A) = \prod_{A_i \in A}{Aut(A_i)}$
	\end{enumerate}
\end{definition}
\begin{example}[*]
	If $A_1 = ((2),1,1)$, $A_2 = ((3,1),1,2)$, and $A_3 = ((1,2,3),2,1)$ then $A = \{A_1,A_2,A_3\}$ represesents the monomial $p = {y_{12}}{y^2_{13}}{y^2_{11}}{y_{21}}{y_{22}}{y_{23}}$ and we have $Aut(A) = S_1 \times S_2 \times S_3$
\end{example}
\subsection{Fourier Characters and Ribbons}
A key idea is to analyze Fourier characters of the input.
\begin{definition}[Simplified Fourier Characters]
	If the input distribution is $\Omega = \{-1,1\}$ then given a multi-set of edges $E$, we define $\chi_{E}(X) = \prod_{e \in E}{x_e}$.
\end{definition}
\begin{example}
	If the input is a graph $G \in \{-1,1\}^{\binom{n}{2}}$ and $E$ is a set of potential edges of $G$ (with no multiple edges) then $\chi_E(G) = (-1)^{|E \setminus E(G)|}$.
\end{example}
In general, the Fourier characters are somewhat more complicated.
\begin{definition}[Orthonormal Basis for ${\Omega}$*]
	We define the polynomials $\{h_i: i \in \mathbb{Z} \cap [0,|supp(\Omega)|-1]\}$ to be the unique polynomials (which can be found through the Gram-Schmidt process) such that
	\begin{enumerate}
		\item $\forall i, E_{\Omega}[h^2_i(x)] = 1$
		\item $\forall i \neq j, E_{\Omega}[h_i(x)h_j(x)] = 0$
		\item For all $i$, the leading coefficient of $h_i(x)$ is positive.
	\end{enumerate}
\end{definition}
\begin{example}\label{example: hermite_basis}
	If $\Omega$ is the normal distribution then the polynomials $\{h_i\}$ are the Hermite polynomials with the appropriate normalization so that for all $i$, $E_{\Omega}[h^2_i(x)] = 1$. In particular, $h_0(x) = 1$, $h_1(x) = x$, $h_2(x) = \frac{x^2 - 1}{\sqrt{2!}}$, $h_3(x) = \frac{x^3 - 3x}{\sqrt{3!}}$, etc.
\end{example}
\begin{definition}[General Fourier Characters*]
	Given a multi-set of hyperedges $E$, each of which has a label $l(e) \in [|support(\Omega)|-1]$ (or $\mathbb{N}$ if $\Omega$ has infinite support), we define $\chi_E = \prod_{e \in E}{h_{l(e)}{(X_e)}}$.

	We say that such a multi-set of hyperedges $E$ is proper if it contains no duplicate hyperedges, i.e. it is a set (though the labels on the hyperedges can be arbitrary non-negative integers). Otherwise, we say that $E$ is improper.
\end{definition}
\begin{remark}
	The Fourier characters are $\{\chi_{E}: E \text{ is proper}\}$. For improper $E$, $\chi_{E}$ can be decomposed as a linear combination of $\chi_{E_j}$ where each $E_j$ is proper. We allow improper $E$ because it is sometimes more convenient to have improper $E$ in the middle of the analysis and then do this decomposition at the end.
\end{remark}
\begin{definition}[Ribbons]\label{def: ribbons}
	A ribbon $R$ is a tuple $(H_R,A_R,B_R)$ where $H_R$ is a multi-graph (*or multi-hypergraph with labeled edges in the general case) whose vertices are indices of the input and $A_R$ and $B_R$ are matrix indices such that $V(A_R) \subseteq V(H_R)$ and $V(B_R) \subseteq V(H_R)$. We make the following definitions about ribbons:
	\begin{enumerate}
		\item We define $V(R) = V(H_R)$ and $E(R) = E(H_R)$
		\item We define $\chi_R = \chi_{E(R)}$.
		\item We define $M_R$ to be the matrix such that $(M_R)_{{A_R}{B_R}} = \chi_R$ and $M_{AB} = 0$ whenever $A \neq A_R$ or $B \neq B_R$.
	\end{enumerate}
	We say that $R$ is a proper ribbon if $H_R$ contains no isolated vertices outside of $A_R \cup B_R$ and $E(R)$ is proper. If there is an isolated vertex in $(V(R) \setminus A_R) \setminus B_R$ or $E(R)$ is improper then we say that $R$ is an improper ribbon.
\end{definition}
Proper ribbons are useful because they give an orthonormal basis for the space of matrix valued functions.
\begin{definition}[Inner products of matrix functions]
	For a pair of real matrices $M_1,M_2$ of the same dimension, we write $\langle{M_1,M_2}\rangle = tr({M_1}{M_2}^T)$ (i.e. $\langle{M_1,M_2}\rangle$ is the entrywise dot product of $M_1$ and $M_2$). For a pair of matrix-valued functions $M_1, M_2$ (of the same dimensions), we define
	\[
	\langle{M_1,M_2}\rangle = E_{X}\left[\langle{M_1(X),M_2(X)}\rangle\right]
	\]
\end{definition}
\begin{proposition}
	If $R$ and $R'$ are two proper ribbons then $\langle{M_R,M_{R'}}\rangle = 1$ if $R = R'$ and is $0$ otherwise.
\end{proposition}
We have already seen examples of ribbons in earlier chapters, but we provide an example here for convenience.
For more examples, see \cite{AMP20}.

\begin{example}[Simplified Ribbon]
    In \cref{fig: ribbon_shape}, consider the ribbon $R$ as shown. We have $A_R = (1, 3), B_R = (4), V(R) = \{1, 2, 3, 4\}, E_R = \{\{1, 2\}, \{3, 2\}, \{2, 4\}\}$. The Fourier character is $\chi_{E_R} = \chi_{1, 2}\chi_{3, 2}\chi_{2, 4}$. And finally, $M_R$ is a matrix with rows and columns indexed by tuples of length $|A_R| = 2$ and $|B_R| = 1$ respectively, with exactly one nonzero entry $M_R((1, 3), (4)) = \chi_{E_R}$. Succinctly, \[M_R =
    %     \begin{blockarray}{c@{\hspace{5pt}}rr@{\hspace{5pt}}cl}
        %     & \matindex{1} & \matindex{2} & & \\
        %     \begin{block}{(c@{\hspace{5pt}}rr@{\hspace{5pt}}c)l}
            %       & 100 &  b & & \matindex{row 1} \\
            %       &   2 & 12 & & \matindex{row 2} \\
            %       &   e &  f & & \matindex{ABDC} \\
            %     \end{block}
        %   \end{blockarray}$.
    \begin{blockarray}{rl@{}c@{}r}
        & & \makebox[0pt]{column $(4)$} \\[-0.5ex]
        & & \,\downarrow \\[-0.5ex]
        \begin{block}{r(l@{}c@{}r)}
            & \makebox[3.1em]{\Large $0$\bigstrut[t]} & \vdots &\makebox[4.2em]{\Large $0$} \\[-0.2ex]
            \text{row }(1, 3) \to \mkern-9mu & \raisebox{0.5ex}{\makebox[3.2em][l]{\dotfill}} & \chi_{1, 2}\chi_{3, 2}\chi_{2, 4} & \raisebox{0.5ex}{\makebox[4.2em][r]{\dotfill}} \\[+0ex]
            & \makebox[3.1em]{\Large $0$} & \vdots &\makebox[4.2em]{\bigstrut\Large $0$} \\
        \end{block}
    \end{blockarray}\]
\end{example}

\begin{figure}[!h]
    \centering
    \includegraphics[scale=.6, trim={0 5cm 2 5cm},clip]{machinery/images/ribbon_shape}
    \caption{Example of a ribbon and a shape}
    \label{fig: ribbon_shape}
\end{figure}

\subsection{Shapes}
In this subsection, we describe a basis for $S$-invariant matrix valued functions where each matrix in this basis can be described by a relatively small \emph{shape} $\alpha$. The fundamental idea behind shapes is that we keep the structure of the objects we are working with but leave the elements of the object unspecified.
\subsubsection{Simplified Index Shapes}
\begin{definition}[Simplified Index shapes]
	With our simplifying assumptions, an index shape $U$ is a tuple of unspecified indices $(u_1,\cdots,u_{|U|})$. We make the following definitions about index shapes:
	\begin{enumerate}
		\item We define $V(U)$ to be the set of vertices $\{u_i: i \in [|U|]\}$. For brevity, we will often write $U$ instead of $V(U)$ when it is clear from context that we are referring to $U$ as a set of vertices rather than an index shape.
		\item We define the weight of $U$ to be $w(U) = |U|$.
		\item We take the automorphism group of $U$ to be $Aut(U) = S_{|U|}$ (the permutations of the elements of $U$)
	\end{enumerate}
\end{definition}
\begin{definition}
	We say that a matrix index $A = (a_1,\ldots,a_{|A|})$ has index shape $U = (u_1,\ldots,u_{|U|})$ if $|U| = |A|$. Note that in this case, if we take the map $\phi: \{u_j: j \in [|U|]\} \to [n]$ where $\phi(u_j) = a_j$ then $\phi(U) = (\phi(u_1),\ldots,\phi(u_{|U|})) = (a_1,\ldots,a_{|A|}) = A$
\end{definition}
\begin{definition}
	We say that index shapes $U = (u_1,\ldots,u_{|U|})$ and $V = (v_1,\ldots,v_{|V|})$ are equivalent (which we write as $U \equiv V$) if $|U| = |V|$. If $U \equiv V$ then we can set $U = V$ by setting $v_j = u_j$ for all $j \in [|U|]$.
\end{definition}
\begin{example}
	The matrix index $A = \{4,6,1\}$ has shape $U = \{u_1,u_2,u_3\}$ which has weight $3$.
\end{example}
\subsubsection{General Index Shapes*}
In general, we define general index shapes in the same way that we defined general matrix indices (just with unspecified indices)
\begin{definition}[Index Shape Piece Definition]
	We define a index shape piece $U_i = ((u_{i1},\ldots,u_{i|U_i|}), t_i, p_i)$ to be a tuple of indices $(u_{i1},\ldots,u_{i|A_i|})$ together with a type $t_i$ and a power $p_i$. We make the following definitions about index shape pieces:
	\begin{enumerate}
		\item We define $V(U_i)$ to be the set of vertices $\{(t_i,u_{ij}): j \in [|U_i|]\}$.
		\item We define $w(U_i) = |U_i|log_{n}(n_{t_i})$
		\item We take the automorphism group of $U_i$ to be $Aut(U_i) = S_{|U_i|}$
	\end{enumerate}
\end{definition}
\begin{definition}[General Index Shape Definition]
	We define an index shape $U = \{U_i\}$ to be a set of index shape pieces such that for all $i' \neq i$, either $t_{i'} \neq t_i$ or $p_{i'} \neq p_i$. We make the following definitions about index shapes:
	\begin{enumerate}
		\item We define $V(U)$ to be the set of vertices $\cup_{U_i \in U}{V(U_i)}$. For brevity, we will often write $U$ instead of $V(U)$ when it is clear from context that we are referring to $U$ as a set of vertices rather than an index shape.
		\item We define $w(U)$ to be $w(U) = \sum_{U_i \in U}{w(U_i)}$
		\item We take the automorphism group of $U$ to be $Aut(U) = \prod_{U_i \in U}{Aut(U_i)}$
	\end{enumerate}
\end{definition}
\begin{remark}
	For technical reasons, we want to ensure that if two index shapes $U$ and $U'$ have the same weight then $U$ and $U'$ have the same number of each type of vertex. To ensure this, we add an infinitesimal perturbation to each $n_i$ if necessary.
\end{remark}
\begin{definition}
	We say that a matrix index $A$ has index shape $U$ if there is an assignment of values to the unspecified indices of $U$ which results in $A$. More precisely, we say that $A$ has index shape $U$ if there is a map $\phi: \{u_{ij}\} \to \mathbb{N}$ such that if we define $\phi(U_i)$ to be $\phi(U_i) = ((\phi(u_{i1}),\ldots,\phi(u_{i|U_i|})),t_i,p_i)$ then $\phi(U) = \{\phi(U_i)\} = \{A_i\} = A$.
\end{definition}
\begin{definition}
	If $U$ and $V$ are two index shapes, we say that $U$ is equivalent to $V$ (which we write as $U \equiv V$) if $U$ and $V$ have the same number of index shape pieces and we can order the index shape pieces of $U$ and $V$ so that writing $U = \{U_i\}$ and $V = \{V_i\}$ where $U_i = ((u_{i1},\ldots,u_{i|U_i|}), t_i, p_i)$ and $V_{i} = ((v_{i1},\ldots,v_{i|V_i|}), t'_i, p'_i)$, we have that for all $i$, $|V_i| = |U_i|$, $t'_i = t_i$, and $p'_i = p_i$. If $U \equiv V$ then we can set $U = V$ by setting $u_{ij} = v_{ij}$ for all $i$ and all $j \in [|U_i|]$.
\end{definition}
\subsubsection{Ribbon Shapes}
With these definitions, we are now ready to define shapes and the matrices associated to them.
\begin{definition}[Shapes]\label{def: shapes}
	A ribbon shape $\alpha$ (which we call a shape for brevity) is a tuple $\alpha = (H_{\alpha},U_{\alpha},V_{\alpha})$ where $H_{\alpha}$ is a multi-graph (*or multi-hypergraph with labeled edges in the general case) whose vertices are unspecified distinct indices of the input (*whose type is specified in the general case) and $U_{\alpha}$ and $V_{\alpha}$ are index shapes such that $V(U_{\alpha}) \subseteq V(H_\alpha)$ and $V(V_{\alpha}) \subseteq V(H_\alpha)$. We make the following definitions about shapes:
	\begin{enumerate}
		\item We define $V(\alpha) = V(H_{\alpha})$ (note that $V(\alpha)$ and $V_{\alpha}$ are not the same thing) and we define $E(\alpha) = E(H_{\alpha})$.
		\item We say that a shape $\alpha$ is proper if it contains no isolated vertices outside of $V(U_{\alpha}) \cup V(V_{\alpha})$, $E(\alpha)$ has no multiple edges/hyperedges and edges in $E(\al)$ do not have label $0$. If there is an isolated vertex in $V(\alpha) \setminus V(U_{\alpha}) \setminus V(V_{\alpha})$ or $E(\alpha)$ has a multiple edge/hyperedge then we say that $\alpha$ is an improper shape.
	\end{enumerate}
	Note: For brevity, we will often write $U_{\alpha}$ and $V_{\alpha}$ instead of $V(U_{\alpha})$ and $V(V_{\alpha})$ when it is clear from context that we are referring to $U_{\alpha}$ and $V_{\alpha}$ as sets of vertices rather than index shapes.
\end{definition}
%While $U_{\alpha}$ and $V_{\alpha}$ can intersect, vertices in $U_{\alpha} \cap V_{\alpha}$ can be ignored for several parts of the analysis. Thus, we make the following definitions.
%\begin{definition}
%We define $V_{red}(\alpha) = V(\alpha) \setminus (U_{\alpha} \cap V_{\alpha})$
%\end{definition}
\begin{definition}[Trivial shapes]
	We say that a shape $\alpha$ is trivial if $V(\alpha) = V(U_{\alpha}) = V(V_{\alpha})$ and $E(\alpha) = \emptyset$. Otherwise, we say that $\alpha$ is non-trivial.
\end{definition}
\begin{remark}
	Note that all trivial shapes can do is permute the order of the vertices in $V(U_{\alpha}) = V(V_{\alpha})$.
\end{remark}
\begin{definition}
	Informally, we say that a ribbon $R$ has shape $\alpha$ if replacing the indices in $R$ with unspecified labels results in $\alpha$. Formally, we say that $R$ has shape $\alpha$ if there is an injective mapping $\phi:V(\alpha) \to [n]$ (*or $[t_{max}] \times [n]$ in the general case) such that $\phi(\alpha) = R$, i.e. $\phi(H_{\alpha}) = H_R$, $\phi(U_{\alpha}) = A_R$, and $\phi(V_{\alpha}) = B_R$
\end{definition}
\begin{definition}
	We say that two shapes $\alpha$ and $\beta$ are equivalent (which we write as $\alpha \equiv \beta$) if they are the same up to renaming their indices. More precisely, we say that $\alpha \equiv \beta$ if there is a bijective map $\pi: V(H_\alpha) \to V(H_\beta)$ such that $\pi(H_\alpha) = H_{\beta}$, $\pi(U_{\alpha}) = U_{\beta}$, and $\pi(V_{\alpha}) = V_{\beta}$.
\end{definition}
\begin{definition}
	Given a shape $\alpha$ and matrix indices $A,B$ of shapes $U_\alpha$ and $V_\alpha$ respectively, we define $\mathcal{R}(\alpha,A,B)$ to be the set of ribbons $R$ such that $R$ \emph{has shape $\alpha$}, $A_R = A$, and $B_R = B$.
\end{definition}
\begin{definition}
	For a shape $\alpha$, we define the matrix-valued function $M_\alpha$ to have entries $M_{\alpha}(A,B)$ given by
	\[
	(M_\alpha)_{A,B}(X) = \sum_{R \in \mathcal{R}(\alpha, A,B )} \chi_R(X)
	\]
\end{definition}

We have seen examples of shapes in earlier chapters, but we provide one here for convenience.
For more examples, see \cite{AMP20}.

\begin{example}[Simplified Shape]
    In \cref{fig: ribbon_shape}, consider the shape $\al$ as shown. We have $U_{\al} = (u_1, u_2), V_{\al} = (v_1), V(\al) = \{u_1, u_2, v_1, w_1\}$ and $E(\al) = \{\{u_1, w_1\}, \{u_2, w_1\}, \{w_1, v_1\}\}$. $M_{\al}$ is a matrix with rows and columns indexed by tuples of length $|U_{\al}| = 2$ and $|V_{\al}| = 1$ respectively. The nonzero entries will have rows and columns indexed by $(a_1, a_2)$ and $b_1$ respectively for all distinct $a_1, a_2, b_1$, with the corresponding entry being $M_{\al}((a_1, a_2), (b_1)) = \sum_{c_1 \in [n] \setminus \{a_1, a_2, b_1\}} \chi_{a_1, c_1}\chi_{a_2, c_1} \chi_{c_1, b_1}$. Here, the injective map $\phi$ maps $u_1, u_2, w_1, v_1$ to $a_1, a_2, c_1, b_1$ respectively and we sum over all such maps. Succinctly, \[M_{\al} =
    %     \begin{blockarray}{c@{\hspace{5pt}}rr@{\hspace{5pt}}cl}
        %     & \matindex{1} & \matindex{2} & & \\
        %     \begin{block}{(c@{\hspace{5pt}}rr@{\hspace{5pt}}c)l}
            %       & 100 &  b & & \matindex{row 1} \\
            %       &   2 & 12 & & \matindex{row 2} \\
            %       &   e &  f & & \matindex{ABDC} \\
            %     \end{block}
        %   \end{blockarray}$.
    \begin{blockarray}{rl@{}c@{}r}
        & & \makebox[0pt]{column $(c_1)$} \\[-0.5ex]
        & & \,\downarrow \\[-0.5ex]
        \begin{block}{r(l@{}c@{}r)}
            &  & \vdots & \\[-0.2ex]
            \text{row }(a_1, a_2) \to \mkern-9mu & \raisebox{0.5ex}{\makebox[3.2em][l]{\dotfill}} & \sum_{c_1 \in [n] \setminus \{a_1, a_2, b_1\}} \chi_{a_1, c_1}\chi_{a_2, c_1} \chi_{c_1, b_1} & \raisebox{0.5ex}{\makebox[4.2em][r]{\dotfill}} \\[+.5ex]
            &  & \vdots & \\
        \end{block}
    \end{blockarray}\]
\end{example}

\begin{proposition}
    The $M_\alpha$'s for proper shapes $\alpha$ are an orthogonal basis for the $S$-invariant functions.\footnote{
        Because of orthogonality of the underlying Fourier characters, it is not hard to check that when $\alpha \neq \alpha'$ and $M_\alpha, M_{\alpha'}$ have the same dimensions, $\langle{M_\alpha, M_{\alpha'}}\rangle = 0$.}
\end{proposition}
\begin{remark}
    Conceptually, one may think of forming an orthonormal basis for this space with the functions $M_\alpha / \sqrt{\langle{M_\alpha, M_\alpha}\rangle}$, but for technical reasons it is easiest to work with these functions without normalizing them to $1$.
    By orthogonality and the fact that every Boolean function is a polynomial, any $S$-invariant matrix-valued function $\Lambda$ is expressible as
    \[
    \Lambda = \sum_{\alpha} \frac{\langle{\Lambda, M_\alpha}\rangle}{\langle{M_\alpha, M_\alpha}\rangle} \cdot M_\alpha
    \]
\end{remark}

%In the proof of our main theorem, we encounter improper shapes. We can handle them by decomposing them into proper shapes using basic Fourier analysis. For now, we will illustrate how this can be done via an example.
%
%\begin{example}[Reducing improper shape to proper shapes*]
%Consider the case when the input distribution is Gaussian and there is only one type of vertex. Consider the improper shape $\alpha$ where $U_{\alpha} = (u_1,u_2,u_3)$, $V_{\alpha} = (v_1,v_2,v_3)$, and $V(\alpha) = U_{\alpha} \cup V_{\alpha} \cup \{w_1,w_2,w_3,w_4\}$ with edges
%\begin{align*} E(\alpha) = &\{(u_1,w_1),(u_2,w_1),(u_3,w_1),(u_1,w_2),(u_2,w_2),(u_3,w_2)\} \\
%&\cup \{(w_1,w_3), (w_1,w_3), (w_2,w_4), (w_2,w_4)\} \\
%&\cup \{(w_3,v_1), (w_3,v_2), (w_3,v_3), (w_4,v_1), (w_4,v_2), (w_4,v_3)\}
%\end{align*}
%where all edges have label $1$.
%$M_{\alpha}$ can be decomposed into a linear combination $M_{\alpha_1}$, $M_{\alpha_2}$, and $M_{\alpha_3}$ for the following proper shapes $\alpha_1$, $\alpha_2$, and $\alpha_3$
%\begin{enumerate}
%\item $\alpha_1$ is the same as $\alpha$ except that the edges $\{(w_1,w_3), (w_1,w_3), (w_2,w_4), (w_2,w_4)\}$ are replaced by $\{(w_1,w_3)_2, (w_2,w_4)_2\}$. The subscript notation means that we replaced the multiedge by a single edge with label $2$ so the edge now corresponds to the Hermite polynomial $h_2(x)$ as in \cref{example: hermite_basis}.
%\item $\alpha_2$ is the same as $\alpha$ except that the edges $\{(w_1,w_3), (w_1,w_3), (w_2,w_4), (w_2,w_4)\}$ are replaced by $\{(w_1,w_3)_2\}$.
%\item $\alpha_3$ is the same as $\alpha$ except that the edges $\{(w_1,w_3), (w_1,w_3), (w_2,w_4), (w_2,w_4)\}$ are deleted.
%\end{enumerate}
%With our definition of graph matrices
%\[
%M_{\alpha} = 2M_{\alpha_1} + \sqrt{2}M_{\alpha_2} + 2M_{\alpha_3}
%\]
%% With the alternative definition of graph matrices,
%% \[
%% M_{\alpha} = 2M_{\alpha_1} + 2\sqrt{2}M_{\alpha_2} + M_{\alpha_3}
%% \]
%\end{example}

\subsection{Composing Ribbons and Shapes}
\begin{definition}[Composing Ribbons]
	We say that ribbons $R_1$ and $R_2$ are composable if $B_{R_1} = A_{R_2}$. Note that this definition is not symmetric so we may have that $R_1$ and $R_2$ are composable but $R_2$ and $R_1$ are not composable.

	We say that $R_1$ and $R_2$ are properly composable if we also have that $V(R_1) \cap V(R_2) = V(B_{R_1}) = V(A_{R_2})$ (there are no unexpected intersections between $R_1$ and $R_2$).

	If $R_1$ and $R_2$ are composable ribbons then we define the composition of $R_1$ and $R_2$ to be the ribbon $R_1 \circ R_2$ such that
	\begin{enumerate}
		\item $A_{R_1 \circ R_2} = A_{R_1}$ and $B_{R_1 \circ R_2} = B_{R_2}$
		\item $V(R_1 \circ R_2) = V(R_1) \cup V(R_2)$
		\item $E(R_1 \circ R_2) = E(R_1) \cup E(R_2)$ (and thus $\chi_{R_1 \circ R_2} = \chi_{R_1}\chi_{R_2}$)
	\end{enumerate}
	We say that ribbons $R_1,\ldots,R_k$ are composable/properly composable if for all $j \in [k-1]$, $R_1 \circ \ldots \circ R_j$ and $R_{j+1}$ are composable/properly composable. If $R_1,\ldots,R_k$ are composable then we define $R_1 \circ \ldots \circ R_k$ to be
	$R_1 \circ \ldots \circ R_k = (R_1 \circ \ldots \circ R_{k-1}) \circ R_k$
\end{definition}
\begin{proposition}
	Ribbon composition is associative, i.e. if $R_1,R_2,R_3$ are composable/properly composable ribbons then $R_2, R_3$ are composable/properly composable, $R_1, (R_2 \circ R_3)$ are composable/properly composable, and $R_1 \circ (R_2 \circ R_3) = (R_1 \circ R_2) \circ R_3$
\end{proposition}
\begin{proposition}
	If $R_1$ and $R_2$ are composable ribbons then $M_{R_1 \cup R_2} = M_{R_1}M_{R_2}$.
\end{proposition}
We have similar definitions for composing shapes.
\begin{definition}[Composing Shapes]
	We say that shapes $\alpha$ and $\beta$ are composable if $U_{\beta} \equiv V_{\alpha}$. Note that this definition is not symmetric so we may have that $\alpha$ and $\beta$ are composable but $\beta$ and $\alpha$ are not composable.

	If $\alpha$ and $\beta$ are composable shapes then we define the composition of $\alpha$ and $\beta$ to be the shape $\alpha \circ \beta$ such that
	\begin{enumerate}
		\item $U_{\alpha \circ \beta} = U_{\alpha}$ and $V_{\alpha \circ \beta} = V_{\beta}$
		\item After setting $U_{\beta} = V_{\alpha}$, we take $V(\alpha \circ \beta) = V(\alpha) \cup V(\beta)$
		\item $E(\alpha \circ \beta) = E(\alpha) \cup E(\beta)$
	\end{enumerate}
	We say that shapes $\alpha_1,\ldots,\alpha_k$ are composable if for all $j \in [k-1]$, $\alpha_1 \circ \ldots \circ \alpha_j$ and $\alpha_{j+1}$ are composable. If $\alpha_1,\ldots,\alpha_k$ are composable then we define the shape $\alpha_1 \circ \ldots \circ \alpha_k$ to be
	$\alpha_1 \circ \ldots \circ \alpha_k = (\alpha_1 \circ \ldots \circ \alpha_{k-1}) \circ \alpha_k$
\end{definition}
\begin{proposition}
	Shape composition is associative, i.e. if $\alpha_1,\alpha_2,\alpha_3$ are composable shapes then $\alpha_2, \alpha_3$ are composable, $\alpha_1, (\alpha_2 \circ \alpha_3)$ are composable, and $\alpha_1 \circ (\alpha_2 \circ \alpha_3) = (\alpha_1 \circ \alpha_2) \circ \alpha_3$
\end{proposition}

\begin{example}
    \cref{fig: basic_shape_comp} illustrates an example of shape composition in the simplified case. Observe how the shapes $\sig \circ \sig'^T$ and $\sig \circ \tau \circ \sig'^T$ are obtained from the shapes $\sig, \tau$ and $\sig'^T$.
\end{example}

\begin{example}
    \cref{fig: shape_comp} illustrates an example of shape composition in the general case. We have two types of vertices that we diagrammaticaly represent by squares and circles. Observe how the shapes $\sig \circ \sig'^T$ and $\sig \circ \tau \circ \sig'^T$ are obtained from the shapes $\sig, \tau$ and $\sig'^T$.
\end{example}

\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.45, trim={4.5cm 2cm 0 2cm},clip]{machinery/images/basic_shape_comp}
    \caption{Illustration of shape composition and decomposition in the simplified case.}
    \label{fig: basic_shape_comp}
\end{figure}

\begin{figure}[!h]
    \centering
    \includegraphics[scale=0.38, trim={8cm 2cm 0 2cm},clip]{machinery/images/shape_comp}
    \caption{Illustration of shape composition and decomposition in the general case.}
    \label{fig: shape_comp}
\end{figure}

\subsection{Decomposition of Shapes into Left, Middle, and Right parts}
In this subsection, we describe how shapes can be decomposed into left, middle, and right parts based on the leftmost and rightmost \emph{minimum vertex separators}, which is a crucial idea for the analysis.
\begin{definition}[Paths]
	A \emph{path} in a shape $\alpha$ is a sequence of vertices $v_1,\ldots,v_t$ such that $v_i, v_{i+1}$ are in some edge/hyperedge together.
	A pair of paths is vertex-disjoint if the corresponding sequences of vertices are disjoint.
\end{definition}
\begin{definition}[Vertex separators]
	Let $\alpha$ be a shape and let $U$ and $V$ be sets of vertices in $\alpha$. We say that a set of vertices $S \subseteq V(\alpha)$ is a \emph{vertex separator} of $U$ and $V$ if every path in $\alpha$ from $U$ to $V$ contains at least one vertex in $S$. Note that any vertex separator $S$ of $U$ and $V$ must contain all of the vertices in $U \cap V$.

	As a special case, we say that $S$ is a vertex separator of $\alpha$ if $S$ is a vertex separator of $U_{\alpha}$ and $V_{\alpha}$
\end{definition}
We define the weight of a set of vertices $S \subseteq V(\alpha)$ in the same way that weight is defined for index shapes.
\begin{definition}[Simplified Weight]
	When there is only one type of index, the weight of a set of vertices $S \subseteq V(\alpha)$ is simply $|S|$.
\end{definition}
\begin{definition}[General Weight*]
	In general, given a set of vertices $S \subseteq V(\alpha)$, writing $S = \cup_{t}{S_t}$ where $S_t$ is the set of vertices of type $t$ in $S$, we define the weight of $S$ to be $w(S) = \sum_{t}{|S_t|log_{n}(n_t)}$
\end{definition}
\begin{remark}[*]
	Again, if necessary, we add an infinitesimal perturbation to $n_1,n_2,\ldots,n_{t_{max}}$ so that if two separators $S$ and $S'$ have the same weight then $S$ and $S'$ have the same number of each type of vertex.
\end{remark}
\begin{definition}[Leftmost and rightmost minimum vertex separators]
	The \emph{leftmost} minimum vertex separator is the vertex separator $S$ of minimum weight such that for every other minimum-weight vertex separator $S'$, $S$ is a separator of $U_\alpha$ and $S'$.
	The \emph{rightmost} minimum vertex separator is the vertex separator $T$ of minimum weight such that for every other minimum-weight vertex separator $T'$, $T$ is a separator of $T'$ and $V_{\alpha}$
\end{definition}
The work \cite{BHKKMP16} showed that under the simplifying assumptions, leftmost and rightmost minimum vertex separators are well defined. For a general proof that leftmost and rightmost minimum vertex separators are well defined, see \cite{potechin2020machinery}.

We now have the following crucial idea. Every shape $\alpha$ can be decomposed into the composition of three composable shapes $\sigma,\tau,{\sigma'}^T$ based on the leftmost and rightmost minimum vertex separators $S,T$ of $\alpha$ together with orderings of $S$ and $T$.
\begin{definition}[Simplified Separators With Orderings]
	Under our simplifying assumptions, given a set of vertices $S \subseteq V(\alpha)$ and an ordering $O_S = s_1,\ldots,s_{|S|}$ of the vertices of $S$, we define the index shape $(S, O_S)$ to be $(S, O_S) = (s_1,\ldots,s_{|S|})$.
\end{definition}
\begin{definition}[General Separators With Orderings*]
	In the general case, we need to give an ordering for each type of vertex. Let $S \subseteq V(\alpha)$ be a subset of the vertices of $\alpha$ and write $S = \cup_{t}{S_t}$ where $S_t$ is the set of vertices in $S$ of type $t$. Given $O_S = \{O_t\}$ where $O_t = s_{t1},\ldots,s_{t|S_t|}$ is an ordering of the vertices of $S_t$, we define the index shape piece $(S_t, O_t)$ to be $(S_t, O_t) = ((s_{t1},\ldots,s_{t|S_t|}), t, 1)$ and we define the index shape $(S,O_S)$ to be $(S,O_S) = \{(S_t,O_t)\}$.
\end{definition}
\begin{proposition}
	The number of possible orderings $O$ for $S$ is equal to $|Aut((S,O_S))|$
\end{proposition}
\begin{definition}[Shape transposes]
	Given a shape $\alpha$, we define $\alpha^{T}$ to be the shape $\alpha$ with $U_{\alpha}$ and $V_{\alpha}$ swapped i.e. $U_{\sigma^{T}} = V_{\sigma}$ and $V_{\sigma^{T}} = U_{\sigma}$.
\end{definition}
\begin{definition}[Left, middle, and right parts]
	Let $\alpha$ be a shape. Let $S$ and $T$ be the leftmost and rightmost minimal vertex separators of $\alpha$ together with orderings $O_S,O_T$ of $S$ and $T$.
	\begin{itemize}
		\item We define the \emph{left part} $\sigma_{\alpha}$ of $\alpha$ to be the shape such that
		\begin{enumerate}
			\item $H_{\sigma_{\alpha}}$ is the induced subgraph of $H_{\alpha}$ on all of the vertices of $\alpha$ reachable from $U_{\alpha}$ without passing through $S$ (note that $H_{\sigma_{\alpha}}$ includes the vertices of $S$) except that we remove any edges/hyperedges which are contained entirely within $S$.
			\item $U_{\sigma_{\alpha}} = U_{\alpha}$ and $V_{\sigma_{\alpha}} = (S,O_S)$
		\end{enumerate}
		\item We define the \emph{right part} ${\sigma'}^T_{\alpha}$ of $\alpha$ to be the shape such that
		\begin{enumerate}
			\item $H_{{\sigma'}^T_{\alpha}}$ is the induced subgraph of $H_{\alpha}$ on all of the vertices of $\alpha$ reachable from $V_{\alpha}$ without passing through $T$ (note that $H_{{\sigma'}^T_{\alpha}}$ includes the vertices of $T$) except that we remove any edges/hyperedges which are contained entirely within $T$.
			\item $V_{{\sigma'}^T_{\alpha}} = V_{\alpha}$ and $U_{{\sigma'}^T_{\alpha}} = (T,O_T)$
		\end{enumerate}
		\item We define the \emph{middle part} $\tau_{\alpha}$ of $\alpha$ to be the shape such that
		\begin{enumerate}
			\item $H_{\tau_{\alpha}}$ is the induced subgraph of $H_{\alpha}$ on all of the vertices of $\alpha$ which are not reachable from $U_{\alpha}$ and $V_{\alpha}$ without touching $S$ and $T$ (note that $H_{\tau_{\alpha}}$ includes the vertices of $S$ and $T$). $H_{\tau_{\alpha}}$ also includes the hyperedges entirely within $S$ and the hyperedges entirely within $T$.
			\item $U_{\tau_{\alpha}} = (S,O_S)$ and $V_{\tau_{\alpha}} = (T,O_T)$
		\end{enumerate}
	\end{itemize}.
\end{definition}

\begin{example}
    \cref{fig: basic_shape_comp} illustrates an example decomposition in the simplified case.
    \begin{enumerate}
        \item If we start with the shape $\al$ denoted as $\sig \circ \sig'^T$, observe that there is a unique minimum vertex separator, which consists of the middle vertex of degree $5$, i.e. the one that's not in either $U_{\sig \circ \sig'^T}$ or $V_{\sig \circ \sig'^T}$.
        Then, $\al$ is decomposed in to the left part $\sig$, a trivial middle part $\tau$ (not shown in this figure) which has $V(\tau) = \{u\}, U_{\tau} = V_{\tau} = (u), E(\tau) = \emptyset$, and the right part $\sig'^T$.
        \item If we start with the shape $\al$ denoted as $\sig \circ \tau \circ \sig'^T$, then the leftmost minimum vertex separator is the vertex of degree $4$ and the rightmost minimum vertex separator is the vertex of degree $5$. Then, $\al$ is decomposed into the left part $\sig$, the middle part $\tau$ and the right part $\sig'^T$, which are all shown in this figure.
    \end{enumerate}
\end{example}


\begin{example}
    \cref{fig: shape_comp} illustrates an example decomposition in the general case. We have two types of vertices that we diagrammatically represent by squares and circles. In this example, we assume that the set containing a single circle vertex has a lower weight compared to a set of two square vertices.
    \begin{enumerate}
        \item If we start with the shape $\sig \circ \sig'^T$, then it can be decomposed uniquely in to the composition of the left shape $\sig$, the right shape $\sig'^T$. In this case, the middle shape (not shown in this figure) is trivial.
        \item If we start with the shape $\sig \circ \tau \circ \sig'^T$, then it can be decomposed uniquely into the composition of the left shape $\sig$, the middle shape $\tau$ and the right shape $\sig'^T$, which are all shown in this figure.
    \end{enumerate}
\end{example}

\begin{proposition}
	If $\sigma,\tau,{\sigma'}^{T}$ are the left, middle, and rights parts for $\alpha$ for given orderings $O_S,O_T$ of $S$ and $T$ then $\alpha = \sigma \circ \tau \circ {\sigma'}^T$.
\end{proposition}
\begin{remark}
	One may ask which ordering(s) we should take of $S$ and $T$. The answer is that we will take all of the possible orderings of $S$ and $T$ simultaneously, giving equal weight to each.
\end{remark}
Based on this decomposition and the following claim, we make the following definitions for what it means for a shape to be a left, middle, or right part.
\begin{claim}[Proved in Section 6.1 in \cite{BHKKMP16}]
	\footnote{The proof in \cite{BHKKMP16} only explicitly treats the case when the shapes $\alpha$ are graphs, but the proof easily generalizes to the case when the $\alpha$ are hypergraphs.}
	\begin{itemize}
		\item Every shape $\sigma$ which is the left part of some other shape $\alpha$ has that $V_\sigma$ is its left-most and right-most minimum-weight separator.
		\item Every shape ${\sigma}^T$ which is the right part of some other shape $\alpha$ has that $U_{{\sigma}^T}$ is its left-most and right-most minimum-weight separator.
		\item Every shape $\tau$ which is the middle part of some other shape $\alpha$ has $U_\tau$ as its left-most minimum size separator and $V_{\tau}$ as its right-most minimum-weight separator.
	\end{itemize}
\end{claim}
\begin{definition}\label{leftmiddlerightshapedefinitions} \
	\begin{enumerate}
		\item We say that a shape $\sigma$ is a left shape if $\sigma$ is a proper shape, $V_{\sigma}$ is the left-most and right-most minimum-weight separator of $\sigma$, every vertex in $V(\sigma) \setminus V_{\sigma}$ is reachable from $U_{\sigma}$ without touching $V_{\sigma}$, and $\sigma$ has no hyperedges entirely within $V_{\sigma}$.
		\item We say that a shape $\tau$ is a proper middle shape if $\tau$ is a proper shape, $U_{\tau}$ is the left-most minimum-weight separator of $\tau$, and $V_{\tau}$ is the right most minimum-weight separator of $\tau$. In the analysis, we will also need to consider improper middle shapes $\tau$ which may not be proper shapes and which may have smaller separators between $U_{\tau}$ and $V_{\tau}$.
		\item We say that a shape ${\sigma}^{T}$ is a right shape if ${\sigma}^{T}$ is a proper shape, $U_{{\sigma}^{T}}$ is the left-most and right-most minimum-weight separator of ${\sigma}^{T}$, every vertex in $V({\sigma}^{T}) \setminus U_{{\sigma}^{T}}$ is reachable from $V_{{\sigma}^{T}}$ without touching $U_{{\sigma}^{T}}$, and ${\sigma}^{T}$ has no hyperedges entirely within $U_{{\sigma}^{T}}$.
	\end{enumerate}
\end{definition}
\begin{proposition}
	For all shapes $\sigma$, $\sigma$ is a left shape if and only if $\sigma^{T}$ is a right shape.
\end{proposition}
\begin{remark}
	As the reader has likely guessed, throughout this section we use $\sigma$ to denote left parts and $\tau$ to denote middle parts. Instead of having a separate letter for right parts, we express right parts as the transpose of a left part.
\end{remark}
\subsection{Coefficient matrices}\label{fullcoefficientmatrixsubsection}
We will have that $\Lambda = \sum_{\alpha}{\lambda_{\alpha}M_{\alpha}}$. To analyze $\Lambda$, it is extremely useful to express these coefficients in terms of matrices. To do this, we will need a few more definitions. We start by defining the sets of index shapes that can appear when analyzing $\Lambda$.
\begin{definition}
	Given a moment matrix $\Lambda$, we define the following sets of index shapes.
	\begin{enumerate}
		\item We define $\mathcal{I}(\Lambda) = \{U: \exists \text{ matrix index } A: A \text{ is a row index of } \Lambda, A \text{ has shape } U\}$ to be the set of index shapes which describe row and column indices of $\Lambda$.
		\item We define $w_{max}$ to be $w_{max} = \max{\{w(U):U \in \mathcal{I}(\Lambda)\}}$.
		\item With our simplifying assumptions, we define $\mathcal{I}_{mid}$ to be $\mathcal{I}_{mid} = \{U: |U| \leq w_{max}\}$
		\item[3*.] In general, we define $\mathcal{I}_{mid}$ to be $\mathcal{I}_{mid} = \{U: w(U) \leq w_{max}, \forall U_i \in U, p_i = 1\}$
	\end{enumerate}
\end{definition}
We also need to define the sets of shapes which can appear when analyzing $\Lambda$.
\begin{definition}[Truncation Parameters]
	Given a moment matrix $\Lambda = \sum_{\alpha}{\lambda_{\alpha}M_{\alpha}}$, we define $D_V,D_E$ to be the smallest natural numbers such that for all shapes $\alpha$ such that $\lambda_{\alpha} \neq 0$, decomposing $\alpha$ as $\alpha = \sigma \circ \tau \circ {\sigma'}^T$,
	\begin{enumerate}
		\item $|V(\sigma)| \leq D_V$, $|V(\tau)| \leq D_V$, and $|V(\sigma')| \leq D_V$.
		\item[2.*] For all edges $e \in E(\sigma) \cup E(\tau) \cup E(\sigma')$, $l_e \leq D_E$.
	\end{enumerate}
\end{definition}
\begin{remark}
	Under our simplifying assumptions, all edges have label $1$ so we will take $D_E = 1$ and ignore conditions involving $D_E$.
\end{remark}
\begin{definition}
	Given a moment matrix $\Lambda$, we define the following sets of shapes:
	\begin{enumerate}
		\item $\mathcal{L} = \{\sigma: \sigma \text{ is a left shape}, U_{\sigma} \in \mathcal{I}(\Lambda), V_{\sigma} \in \mathcal{I}_{mid}, |V(\sigma)| \leq D_V, \forall e \in E(\sigma), l_e \leq D_E\}$
		\item Given $V \in \mathcal{I}_{mid}$, we define $\mathcal{L}_V = \{\sigma \in \mathcal{L}: V_{\sigma} \equiv V\}$
		\item Given $U \in \mathcal{I}_{mid}$, we define $\mathcal{M}_U = \{\tau: \tau \text{ is a non-trivial proper middle shape}, U_{\tau} \equiv V_{\tau} \equiv U,
		|V(\tau)| \leq D_V, \forall e \in E(\tau), l_e \leq D_E\}$
	\end{enumerate}
\end{definition}
\begin{definition}
	Given a moment matrix $\Lambda$, we define a $\Lambda$-coefficient matrix (which we call a coefficient matrix for brevity) to be a matrix whose rows and columns are indexed by left shapes $\sigma,\sigma' \in \mathcal{L}$.

	We say that a coefficient matrix $H$ is SOS-symmetric if $H(\sigma,\sigma')$ is invariant under permuting the vertices of $U_{\sigma}$ and permuting the vertices of $U_{\sigma'}$ (*more precisely, for the general case we permute the vertices within each index shape piece of $U_{\sigma}$ and permute the vertices within each index shape piece of $U_{\sigma'}$).
\end{definition}
\begin{definition}
	Given a shape $\tau$, we say that a coefficient matrix $H$ is a $\tau$-coefficient matrix if $H(\sigma,\sigma') = 0$ whenever $V_{\sigma} \not\equiv U_{\tau}$ or $V_{\tau} \not\equiv U_{{\sigma'}^T}$.
\end{definition}
\begin{definition}
	Given an index shape $U$, we define $Id_{U}$ to be the shape with $U_{Id_{U}} = V_{Id_{U}} = U$, no other vertices, and no edges.
\end{definition}
Given a shape $\tau$ and a $\tau$-coefficient matrix $H$, for convenience, we create a different matrix-valued functions $M^{fact}_{\tau}(H)$ as follows.

%and $M^{orth}_{\tau}(H)$. As we will see, we can express $\Lambda$ in terms of $M^{orth}$ but to show PSDness we will need to shift to $M^{fact}$. We analyze the difference betweem $M^{fact}$ and $M^{orth}$ in subsections \ref{qualitativeintersectionpatternssection}, \ref{intersectiontermanalysissection}, and \ref{boundingdifferencesection}.

\begin{definition}
	Given a shape $\tau$ and a $\tau$-coefficient matrix $H$, define
	\[
	M^{fact}_{\tau}(H) = \sum_{\sigma \in \mathcal{L}_{U_{\tau}},\sigma' \in \mathcal{L}_{V_{\tau}}}{H(\sigma,\sigma')M_{\sigma}M_{\tau}M_{\sigma'}^T}
	\]
\end{definition}
%\begin{proposition}
%	For all $A$ and $B$ with shapes in $\mathcal{I}(\Lambda)$,
%	\begin{align*}
%		&\left(M^{fact}_{\tau}(H)\right)(A,B) = \\
%		&\sum_{\sigma \in \mathcal{L}_{U_{\tau}},\sigma' \in \mathcal{L}_{V_{\tau}}}{H(\sigma,\sigma')\sum_{A',B'}{
%				\sum_{R_1 \in \mathcal{R}(\sigma,A,A'), R_2 \in \mathcal{R}(\tau,A',B'), \atop R_3 \in \mathcal{R}({\sigma'}^T,B',B)}M_{R_1}(A,A')M_{R_2}(A',B')M_{R_3}(B',B)}}
%	\end{align*}
%\end{proposition}
%If $R_1,R_2,R_3$ are properly composable then $R = R_1 \circ R_2 \circ R_3$ has the expected shape $\sigma \circ \tau \circ {\sigma'}^T$. Otherwise, $R_1 \circ R_2 \circ R_3$ will have a different shape. We define $M^{orth}_{\tau}(H)$ to be the same sum as $M^{fact}_{\tau}(H)$ except that it is restricted to properly composable ribbons $R_1,R_2,R_3$.
%\begin{definition}
%	We define $M^{orth}_{\tau}(H)$ so that for all $A$ and $B$ with shapes in $\mathcal{I}(\Lambda)$,
%	\begin{align*}
%		&\left(M^{orth}_{\tau}(H)\right)(A,B) \\
%		&= \sum_{\sigma \in \mathcal{L}_{U_{\tau}},\sigma' \in \mathcal{L}_{V_{\tau}}}{H(\sigma,\sigma')\sum_{A',B'}{
%				\sum_{R_1 \in \mathcal{R}(\sigma,A,A'), R_2 \in \mathcal{R}(\tau,A',B'), \atop {R_3 \in \mathcal{R}({\sigma'}^T,B',B), R_1,R_2,R_3 \text{ are properly composable}}}M_{R_1}(A,A')M_{R_2}(A',B')M_{R_3}(B',B)}} \\
%		&=  \sum_{\sigma \in \mathcal{L}_{U_{\tau}},\sigma' \in \mathcal{L}_{V_{\tau}}}{H(\sigma,\sigma')\sum_{A',B'}{
%				\sum_{R_1 \in \mathcal{R}(\sigma,A,A'), R_2 \in \mathcal{R}(\tau,A',B'), \atop {R_3 \in \mathcal{R}({\sigma'}^T,B',B), R_1,R_2,R_3 \text{ are properly composable}}}M_{R_1 \circ R_2 \circ R_3}(A,B)}}
%	\end{align*}
%\end{definition}
%It would be nice if we had that $M^{orth}_{\tau}(H) = \sum_{\sigma \in \mathcal{R}_{U_{\tau}},\sigma' \in \mathcal{R}_{V_{\tau}}}{H(\sigma,\sigma')M_{\sigma \circ \tau \circ {\sigma'}^T}}$. However, this is not quite correct because there is an additional term related to automorphism groups.
%\begin{definition}
%	Given a shape $\alpha$, define $Aut(\alpha)$ to be the set of mappings from $\alpha$ to itself which keep $U_{\alpha}$ and $V_{\alpha}$ fixed.
%\end{definition}

%\begin{example}
%Consider the shape $\sigma$ where $U_{\sigma} = (u_1,u_2,u_3)$, $V_{\sigma} = (v_1,v_2,v_3)$, and $V(\sigma) = U_{\sigma} \cup V_{\sigma} \cup \{w_1,w_2,w_3\}$ with edges
%\begin{align*} E(\alpha) = &\{(u_1,w_1),(u_2,w_1),(u_3,w_1),(u_1,w_2),(u_2,w_2),(u_3,w_2),(u_1,w_3),(u_2,w_3),(u_3,w_3)\} \\
%&\cup \{(w_1,v_1), (w_1,v_2), (w_2,v_1), (w_2,v_2),(w_3,v_1), (w_3,v_2)\}
%\end{align*}
%where all edges have label $1$. Then, $Aut(\sigma) = Aut(\sigma^{T}) = S_3$ and $Aut(\sigma \circ \sigma^{T}) = S_3 \times S_2 \times S_3$. Note that in this case $Aut(\sigma \circ \sigma^{T})/(Aut(\sigma) \times Aut(\sigma^{T})) = S_2$. The last computation will be useful for the definition that follows.
%\end{example}
%
%\begin{definition}
%	Given composable shapes $\sigma,\tau,{\sigma'}^T$, we define
%	\[
%	Decomp(\sigma,\tau,\sigma') = Aut(\sigma \circ \tau \circ {\sigma'})/(Aut(\sigma) \times Aut(\tau) \times Aut({\sigma'}^T))
%	\]
%\end{definition}
%\begin{remark}
%	Each element $\pi \in Decomp(\sigma,\tau,\sigma')$ decomposes $\sigma \circ \tau \circ {\sigma'}^T$ into $\sigma$, $\tau$, and ${\sigma'}^T$ by specifying copies $\pi(\sigma)$, $\pi(\tau)$, $\pi({\sigma'}^T)$ of $\sigma$, $\tau$, and ${\sigma'}^T$ such that $\pi(\sigma) \circ \pi(\tau) \circ \pi({\sigma'}^T) = \pi(\sigma \circ \tau \circ {\sigma'}^T) = \sigma \circ \tau \circ {\sigma'}^T$. Thus, $|Decomp(\sigma,\tau,\sigma')|$ is the number of ways to decompose $\sigma \circ \tau \circ {\sigma'}^T$ into $\sigma$, $\tau$, and ${\sigma'}^T$.
%	% by specifying $U_{\tau} = V_{\sigma}$ and $U_{{\sigma'}^T} = V_{\tau}$
%\end{remark}
%\begin{lemma}\label{lm:morthsimplereexpression}
%	\[
%	M^{orth}_{\tau}(H) = \sum_{\sigma \in \mathcal{L}_{U_{\tau}},\sigma' \in \mathcal{L}_{V_{\tau}}}{H(\sigma,\sigma')|Decomp(\sigma,\tau,{\sigma'}^T)|M_{\sigma \circ \tau \circ {\sigma'}^T}}
%	\]
%\end{lemma}
%\begin{proof}[Proof sketch]
%	Observe that there is a bijection between ribbons $R$ with shape $\sigma \circ \tau \circ {\sigma'}^T$ together with an element $\pi \in Decomp(\sigma,\tau,\sigma')$ and triples of ribbons $(R_1,R_2,R_3)$ such that
%	\begin{enumerate}
%		\item $R_1,R_2,R_3$ have shapes $\sigma$, $\tau$, and ${\sigma'}^T$, respectively.
%		\item $V(R_1) \cap V(R_2) = A_{R_2} = B_{R_1}$,  $V(R_2) \cap V(R_3) = A_{R_3} = B_{R_2}$, and $V(R_1) \cap V(R_3) = A_{R_2} \cap B_{R_2}$
%	\end{enumerate}
%	To see this, note that given such ribbons $R_1,R_2,R_3$, the ribbon $R = R_1 \circ R_2 \circ R_3$ has shape $\sigma \circ \tau \circ {\sigma'}^T$ and the ribbons $R_1,R_2,R_3$ specify a decomposition of $\sigma \circ \tau \circ {\sigma'}^T$ into $\sigma$, $\tau$, and ${\sigma'}^T$.
%
%	Conversely, given $R$ and an element $\pi \in Decomp(\sigma,\tau,\sigma')$, $\pi$ specifies how to decompose $R$ into ribbons $R_1,R_2,R_3$ of shapes $\sigma$, $\tau$, and ${\sigma'}^T$.
%
%	For a more rigorous proof, see Appendix \ref{canonicalmapsection}.
%\end{proof}
%\begin{remark}
%	As this lemma shows, we have to be very careful about symmetry groups in our analysis. For accuracy, it is safest to check that the coefficients for each individual ribbon match.
%\end{remark}
Given a matrix-valued function $\Lambda$, we can associate coefficient matrices to $\Lambda$ as follows:
\begin{definition}
	Given a matrix-valued function $\Lambda = \sum_{\alpha: \alpha \text{ is proper}}{\lambda_{\alpha}M_{\alpha}}$,
	\begin{enumerate}
		\item For each index shape $U \in \mathcal{I}_{mid}$ and every $\sigma,\sigma' \in \mathcal{L}_{U}$, we take $H_{Id_U}(\sigma,\sigma') = \frac{1}{|Aut(U)|}\lambda_{\sigma \circ {\sigma'}^T}$
		\item For each $U \in \mathcal{I}_{mid}$, $\tau \in \mathcal{M}_U$ and $\sigma, \sigma' \in \mathcal{L}_{U}$, we take
		$H_{\tau}(\sigma,\sigma') = \frac{1}{|Aut(U_{\tau})|\cdot|Aut(V_{\tau})|}\lambda_{\sigma \circ \tau \circ {\sigma'}^T}$
	\end{enumerate}
\end{definition}
%\begin{lemma}\label{lm:determiningcoefficientmatrices}
%	$\Lambda = \sum_{U \in \mathcal{I}_{mid}}{M^{orth}_{Id_U}(H_{Id_U})} + \sum_{U \in \mathcal{I}_{mid}}{\sum_{\tau \in \mathcal{M}_U}{M^{orth}_{\tau}(H_{\tau})}}$
%\end{lemma}
%\begin{proof}
%	We check that the coefficients for each individual ribbon $R$ match. There are two cases to consider.
%
%	If $R$ has shape $\alpha$ where $\alpha$ has a unique minimum vertex separator $S$, then there is a bijection between orderings $O_S$ for $S$ and pairs of ribbons $R_1,R_2$ such that $R_1 \circ R_2 = R$ and the shapes $\sigma,{\sigma'}^T$ of $R_1,R_2$ are left and right shapes respectively.
%
%	To see this, observe that when we concatenate $R_1$ and $R_2$, this assigns the matrix index $B_{R_1} = A_{R_2}$ to $S$, which is equivalent to specifying an ordering $O_S$ for $S$. Conversely, given an ordering $O_S$ for $S$, we take $R_1$ to be the part of $R$ between $A_R$ and $(S,O_S)$ and we take $R_2$ to be the part of $R$ between $(S,O_S)$ and $B_R$.
%
%	From this bijection, it follows that the coefficient of $M_R$ is $\lambda_{\alpha}$ on both sides of the equation.
%
%	Similarly, if $R$ has shape $\alpha$ where $\alpha$ does not have a unique minimal vertex separator, then there is a bijection between orderings $O_S,O_T$ for the leftmost and rightmost minimum vertex separators $S,T$ of $R$ and triples of ribbons $R_1,R_2,R_3$ such that $R_1 \circ R_2 \circ R_3 = R$ and the shapes $\sigma,\tau,{\sigma'}^T$ of $R_1,R_2,R_3$ are left, proper middle, and right shapes respectively.
%
%	To see this, observe that when we concatenate $R_1$, $R_2$, and $R_3$, this assigns the matrix index $B_{R_1} = A_{R_2}$ to $S$ and assigns the matrix index
%	$B_{R_2} = A_{R_3}$ to $T$, which is equivalent to specifying orderings $O_S,O_T$ for $S,T$. Conversely, given orderings $O_S,O_T$ for $S,T$, we take $R_1$ to be the part of $R$ between $A_R$ and $(S,O_S)$, we take $R_2$ to be the part of $R$ between $(S,O_S)$ and $(T,O_T)$, and we take $R_2$ to be the part of $R$ between $(T,O_T)$ and $B_R$.
%
%	From this bijection, it again follows that the coefficient of $M_R$ is $\lambda_{\alpha}$ on both sides of the equation.
%\end{proof}
\subsection{The $-\gamma,-\gamma$ operation and qualitative theorem statement}
In the intersection term analysis, we will need to further decompose left shapes $\sigma$ as $\sigma = \sigma_2 \circ \gamma$ where $\sigma_2$ and $\gamma$ are themselves left shapes. Accordingly, we make the following definitions
\begin{definition} Given a moment matrix $\Lambda$, we define the following sets of left shapes:
	\begin{enumerate}
		\item $\Gamma = \{\gamma: \gamma \text{ is a non-trivial left shape}, U_{\gamma}, V_{\gamma} \in \mathcal{I}_{mid}, |V(\gamma)| \leq D_V, \forall e \in E(\gamma), l_e \leq D_E\}$
		\item Given $U,V \in \mathcal{I}_{mid}$ such that $w(U) > w(V)$, define $\Gamma_{U,V} = \{\gamma \in \Gamma: U_{\gamma} \equiv U, V_{\gamma} \equiv V\}$.
		\item Given $U \in \mathcal{I}_{mid}$, define $\Gamma_{U,*} = \{\gamma \in \Gamma: U_{\gamma} \equiv U\}$
		\item Given $V \in \mathcal{I}_{mid}$, define $\Gamma_{*,V} = \{\gamma \in \Gamma: V_{\gamma} \equiv V\}$
	\end{enumerate}
	\begin{remark}
		Under our simplifying assumptions, $\Gamma$ is the same as $\mathcal{L}$ except that $\Gamma$ excludes the trivial shapes. In general, while $\mathcal{L}$ requires that $U_{\sigma} \in \mathcal{I}(\Lambda)$, $\Gamma$ requires that $U_{\gamma} \in \mathcal{I}_{mid}$. Note that $\mathcal{I}(\Lambda)$ and $\mathcal{I}_{mid}$ may be incomparable because
		\begin{enumerate}
			\item There may be index shapes $U \in \mathcal{I}_{mid}$ such that no matrix index of $\Lambda$ has shape $U$.
			\item All index shape pieces $U_i$ for index shapes $U \in \mathcal{I}_{mid}$ must have $p_i = 1$ while this is not the case for $\mathcal{I}(\Lambda)$.
		\end{enumerate}
	\end{remark}
\end{definition}
We now state the theorem qualitatively after giving one more definition.
\begin{definition}
	Given a shape $\tau$, left shapes $\gamma \in {\Gamma}_{*,U_{\tau}}$ and $\gamma' \in {\Gamma}_{*,V_{\tau}}$, and a $\tau$-coefficient matrix $H$, define $H^{-\gamma,\gamma'}$ to be the $(\gamma \circ \tau \circ {\gamma'}^T)$-coefficient matrix with entries
	\begin{enumerate}
		\item $H^{-\gamma,\gamma'}(\sigma,\sigma') = H(\sigma \circ \gamma,\sigma' \circ \gamma')$ if $|V(\sigma \circ \gamma)| \leq D_V$ and $|V(\sigma' \circ \gamma')| \leq D_V$.
		\item $H^{-\gamma,\gamma'}(\sigma,\sigma') = 0$ if $|V(\sigma \circ \gamma)| > D_V$ or $|V(\sigma' \circ \gamma')| > D_V$.
	\end{enumerate}
\end{definition}
\begin{remark}
	For the theorem, we will only need the case when $\gamma' = \gamma$
\end{remark}
The qualitative theorem statement is as follows:
\begin{theorem}\label{thm:mainqualitative}
	Let $\Lambda = \sum_{U \in \mathcal{I}_{mid}}{M^{orth}_{Id_U}(H_{Id_U})} + \sum_{U \in \mathcal{I}_{mid}}{\sum_{\tau \in \mathcal{M}_U}{M^{orth}_{\tau}(H_{\tau})}}$ be an SOS-symmetric matrix valued function.

	There exist functions $f(\tau)$ and $f(\gamma)$ depending on $n$ and other parameters such that if the following conditions hold:
	\begin{enumerate}
		\item For all $U \in \mathcal{I}_{mid}$,  $H_{Id_{U}} \succeq 0$
		\item For all $U \in \mathcal{I}_{mid}$ and all $\tau \in \mathcal{M}_{U}$,
		\[
		\left[ {\begin{array}{cc}
				H_{Id_{U}} & f(\tau)H_{\tau} \\
				f(\tau)H^T_{\tau} & H_{Id_{U}}
		\end{array}} \right] \succeq 0
		\]
		\item For all $U,V \in \mathcal{I}_{mid}$ where $w(U) > w(V)$ and all $\gamma \in \Gamma_{U,V}$, $H^{-\gamma,\gamma}_{Id_{V}} \preceq f(\gamma)H_{Id_{U}}$
	\end{enumerate}
	then with high probability $\Lambda \succeq 0$
\end{theorem}
\begin{remark}
	Roughly speaking, conditions 1 and 2 give us an approximate PSD decomposition for the moment matrix $M$. Condition 3 comes from the intersection term analysis, which is the most technically intensive part of the proof.
\end{remark}
\begin{remark}
    As we will demonstrate in this work, the machinery works well when the coefficients $\lambda_{\alpha}$ has a polynomial decay for each vertex or edge in the shape. In many settings, this can be done quite easily by adding noise to the distribution, such as resampling part of the input, or by lowering the parameters slightly, such as $m \le n^{k/4 - \eps}$ instead of $m \le n^{k/4}$.
%    That said, it's possible to optimize many of our functions so that a significantly better bound can be obtained (say for example $m \le n^{k/4} / polylog(n)$ is potentially feasible), we do not attempt this in this work.
    % However, since our machinery is highly technical with many different parts, it does not work as well if the coefficients have a different kind of decay.
\end{remark}
\subsubsection{Choice of functions $f(\tau)$ and $f(\gam)$ in the simplified case}

We will describe some intuition for the functions $f(\tau), f(\gam)$. For simplicity, consider the simplified case.

In a rough sense, $f(\tau)$ measures the blow-up in the norm by using $M_{\tau}$ instead of $M_{Id_U}$ in the corresponding term of the Fourier decomposition. So we choose $f(\tau)$ to be $\norm{M_{\tau}}$, upto lower order terms. Our second condition verifies that the coefficients that arise because of this $\tau$ (which are encoded in $H_{\tau}$) are sufficiently small to overpower this norm blowup.

The fact that $\norm{M_{\tau}}$ is equal to $\tilde{O}(n^{\frac{|V(\tau)|-|U_{\tau}|}{2}})$ has been shown in previous works \cite{BHKKMP16, AMP20}. So, we choose $f(\tau)$ to be $\tilde{O}(n^{\frac{|V(\tau)|-|U_{\tau}|}{2}})$ where the problem instance is on $G_{n, 1/2}$. For problems with Gaussian or other inputs, similar forms of $f(\tau)$ can be used, which have been shown formally in the work of \cite{AMP20}. When we state the main theorem in general, we use a single $f(\tau)$ that incorporates all of these settings.

$f(\gam)$ is a bit trickier to describe. In the machinery analysis, we roughly collect intersection terms from the approximate PSD decomposition and charge them to shapes of the form $\sig \circ \gam \circ \gam^T \circ \sig'^T$. Using the same idea as the previous step, we charge these to shapes with trivial middle shapes. Roughly, $f(\gam)$ for a fixed $\gam$ upper bounds the blowup from the norms of the original shape as compared to the new intersection shape. And the third condition argues that the the original coefficients are sufficiently small to compensate for these blowups.

For problems on $G_{n, 1/2}$, we set $f(\gam) = \tilde{O}(n^{|V(\gamma) \setminus U_{\gamma}|})$. For problems with Gaussian inputs, we choose essentially the same function, but they fall under the umbrella of generalized graph matrices, where $V(\gam)$ and $U_{\gam}$ are defined accordingly. Indeed, in the main theorem, we encompass both these settings with a single choice of $f(\gam)$.

\subsection{Quantitative theorem statement}\label{quantitativetheoremstatementsection}
To state the theorem quantitatively, we will need a few more things. First, the conditions of the theorem will involve functions $B_{norm}(\alpha)$, $B(\gamma)$, $N(\gamma)$, and $c(\alpha)$. Roughly speaking, these functions will be used as follows in the analysis:
\begin{enumerate}
	\item $B_{norm}(\alpha)$ will bound the norms of the matrices $M_{\alpha}$
	\item $B(\gamma)$ and $N(\gamma)$ will help us bound the intersection terms.
	\item $c(\alpha)$ will help us sum over the possible $\gamma$ and $\tau$.
\end{enumerate}
Second, for technical reasons it turns out that comparing $H^{-\gamma,\gamma}_{Id_{V_{\gamma}}}$ to $H_{Id_{U_{\gamma}}}$ doesn't quite work. Instead, we compare $H^{-\gamma,\gamma}_{Id_{V_{\gamma}}}$ to a matrix $H'_{\gamma}$ of our choice where $H'_{\gamma}$ is very close to $H_{Id_{U_{\gamma}}}$ ($H'_{\gamma}$ will be the same as $H_{Id_{U_{\gamma}}}$ up to truncation error).
\begin{definition}
	Given a function $B_{norm}(\alpha)$, we define the distance $d_{\tau}(H_{\tau},H'_{\tau})$ between two $\tau$-coefficient matrices $H_{\tau}$ and $H'_{\tau}$ to be
	\[
	d_{\tau}(H_{\tau},H'_{\tau}) = \sum_{\sigma \in \mathcal{L}_{U_{\tau}},\sigma' \in \mathcal{L}_{V_{\tau}}}{|H'_{\tau}(\sigma,\sigma') - H_{\tau}(\sigma,\sigma')|B_{norm}(\sigma)B_{norm}(\tau)B_{norm}(\sigma')}
	\]
\end{definition}
Third, we need an SOS-symmetric analogue of the identity matrix.
\begin{definition}
	We define $Id_{Sym}$ to be the matrix such that
	\begin{enumerate}
		\item The rows and columns of $Id_{Sym}$ are indexed by the matrix indices $A,B$ whose index shape is in $\mathcal{I}(\Lambda)$.
		\item $Id_{Sym}(A,B) = 1$ if $p_A = p_B$ and $Id_{Sym}(A, B) = 0$ if $p_A \neq p_B$.
	\end{enumerate}
\end{definition}
\begin{proposition}
	If $M$ has SOS-symmetry and the rows and columns of $Id_{Sym}$ are indexed by matrix indices $A,B$ whose index shape is in $\mathcal{I}(\Lambda)$ then $M \preceq \norm{M}Id_{Sym}$
\end{proposition}
\begin{corollary}\label{distanceboundingcorollary}
	For all $\tau$ and all SOS-symmetric $\tau$-coefficient matrices $H_{\tau}$ and $H'_{\tau}$,
	\[
	M^{fact}_{\tau}(H'_{\tau}) + M^{fact}_{{\tau}^T}(H'_{{\tau}^T}) - M^{fact}_{\tau}(H_{\tau}) - M^{fact}_{{\tau}^T}(H_{{\tau}^T}) \preceq 2d_{\tau}(H_{\tau},H'_{\tau})Id_{Sym}
	\]
	Note that if $\tau$, $H_{\tau}$ and $H'_{\tau}$ are all symmetric then
	\[
	M^{fact}_{\tau}(H'_{\tau}) - M^{fact}_{\tau}(H_{\tau}) \preceq d_{\tau}(H_{\tau},H'_{\tau})Id_{Sym}
	\]
\end{corollary}
Finally, we need a few more definitions about shapes $\alpha$.
\begin{definition}[$\mathcal{M}'$]
	We define $\mathcal{M}'$ to be the set of all shapes $\alpha$ such that
	\begin{enumerate}
		\item[1.] $|V(\alpha)| \leq 3D_V$
		\item[2.*] $\forall e \in E(\alpha), l_e \leq D_E$
		\item[3.*] All edges $e \in E(\alpha)$ have multiplicity at most $3D_V$.
	\end{enumerate}
\end{definition}
\begin{definition}[$S_{\alpha}$]
	Given a shape $\alpha$, define $S_{\alpha}$ to be the leftmost minimum vertex separator of $\alpha$
\end{definition}
\begin{definition}[$I_{\alpha}$]
	Given a shape $\alpha$, define $I_{\alpha}$ to be the set of vertices in $V(\alpha) \setminus (U_{\alpha} \cup V_{\alpha})$ which are isolated.
\end{definition}
We can now state the main theorem.
\begin{theorem}\label{simplifiedmaintheorem}
	Given the moment matrix $\Lambda = \sum_{\alpha}{\lambda_{\alpha}M_{\alpha}}$,
	for all $\epsilon > 0$, if we take
	\begin{enumerate}
		\item $q = 3\left\lceil{{D_V}ln(n) + \frac{ln(\frac{1}{\epsilon})}{3} + {D_V}ln(5) + 3{D^2_V}ln(2)}\right\rceil$
		\item $B_{vertex} = 6{D_V}\sqrt[4]{2eq}$
		\item $B_{norm}(\alpha) = {B_{vertex}^{|V(\alpha) \setminus U_{\alpha}| + |V(\alpha) \setminus V_{\alpha}|}}n^{\frac{w(V(\alpha)) + w(I_{\alpha}) - w(S_{\alpha})}{2}}$
		\item $B(\gamma) = B_{vertex}^{|V(\gamma) \setminus U_{\gamma}| + |V(\gamma) \setminus V_{\gamma}|}n^{\frac{w(V(\gamma) \setminus U_{\gamma})}{2}}$
		\item $N(\gamma) = (3D_V)^{2|V(\gamma) \setminus V_{\gamma}| + |V(\gamma) \setminus U_{\gamma}|}$
		\item $c(\alpha) = 100(3D_V)^{|U_{\alpha} \setminus V_{\alpha}| + |V_{\alpha} \setminus U_{\alpha}| + 2|E(\alpha)|}2^{|V(\alpha) \setminus (U_{\alpha} \cup V_{\alpha})|}$
	\end{enumerate}
	and we have SOS-symmetric coefficient matrices $\{H'_{\gamma}: \gamma \in \Gamma\}$ such that the following conditions hold:
	\begin{enumerate}
		\item For all $U \in \mathcal{I}_{mid}$,  $H_{Id_{U}} \succeq 0$
		\item For all $U \in \mathcal{I}_{mid}$ and $\tau \in \mathcal{M}_U$,
		\[
		\left[ {\begin{array}{cc}
				\frac{1}{|Aut(U)|c(\tau)}H_{Id_{U}} & B_{norm}(\tau)H_{\tau} \\
				B_{norm}(\tau)H^T_{\tau} & \frac{1}{|Aut(U)|c(\tau)}H_{Id_{U}}
		\end{array}} \right] \succeq 0
		\]
		\item For all $U,V \in \mathcal{I}_{mid}$ where $w(U) > w(V)$ and all $\gamma \in \Gamma_{U,V}$,
		\[
		c(\gamma)^2{N(\gamma)}^2{B(\gamma)^2}H^{-\gamma,\gamma}_{Id_{V}} \preceq H'_{\gamma}
		\]
	\end{enumerate}
	then with probability at least $1 - \epsilon$,
	\[
	\Lambda \succeq \frac{1}{2}\left(\sum_{U \in \mathcal{I}_{mid}}{M^{fact}_{Id_U}{(H_{Id_U})}}\right) - 3\left(\sum_{U \in \mathcal{I}}{\sum_{\gamma \in \Gamma_{U,*}}{\frac{d_{Id_{U}}(H'_{\gamma},H_{Id_{U}})}{|Aut(U)|c(\gamma)}}}\right)Id_{sym}
	\]
	If it is also true that whenever $\norm{M_{\alpha}} \leq B_{norm}(\alpha)$ for all $\alpha \in \mathcal{M}'$,
	\[
	\sum_{U \in \mathcal{I}_{mid}}{M^{fact}_{Id_U}{(H_{Id_U})}} \succeq 6\left(\sum_{U \in \mathcal{I}}{\sum_{\gamma \in \Gamma_{U,*}}{\frac{d_{Id_{U}}(H'_{\gamma},H_{Id_{U}})}{|Aut(U)|c(\gamma)}}}\right)Id_{sym}
	\]
	then with probability at least $1 - \epsilon$, $\Lambda \succeq 0$.
\end{theorem}
\subsubsection{General Main Theorem}\label{generalmaintheoremstatementsection}
Before stating the general main theorem, we need to modify a few definitions for $\alpha$ and give a few definitions for $\Omega$
\begin{definition}[$S_{\alpha,min}$ and $S_{\alpha,max}$]
	Given a shape $\alpha \in \mathcal{M}'$, define $S_{\alpha,min}$ to be the leftmost minimum vertex separator of $\alpha$ if all edges with multiplicity at least $2$ are deleted and define $S_{\alpha,max}$ to be the leftmost minimum vertex separator of $\alpha$ if all edges with multiplicity at least $2$ are present.
\end{definition}
\begin{definition}[General $I_{\alpha}$]
	Given a shape $\alpha$, define $I_{\alpha}$ to be the set of vertices in $V(\alpha) \setminus (U_{\alpha} \cup V_{\alpha})$ such that all edges incident with that vertex have multplicity at least $2$.
\end{definition}
\begin{definition}[$B_{\Omega}$]
	We take $B_{\Omega}(j)$ to be a non-decreasing function such that for all $j \in \mathbb{N}$, $E_{\Omega}[x^{j}] \leq B_{\Omega}(j)^{j}$
\end{definition}
\begin{definition}[$h^{+}_j$]
	For all $j$, we define $h^{+}_j$ to be the polynomial $h_j$ where we make all of the coefficients have positive sign.
\end{definition}
\begin{lemma}
If $\Omega = N(0,1)$ then we can take $B_{\Omega}(j) = \sqrt{j}$ and we have that
	\[
	h^{+}_j(x) \leq \frac{1}{\sqrt{j!}}(x^2 + j)^{\frac{j}{2}} \leq \left(\frac{e}{j}(x^2 + j)\right)^{\frac{j}{2}}
	\]
\end{lemma}

For a proof, see \cite[Lemma 8.15]{AMP20}.

\begin{theorem}\label{generalmaintheorem}
	Given the moment matrix $\Lambda = \sum_{\alpha}{\lambda_{\alpha}M_{\alpha}}$,
	for all $\epsilon > 0$, if we take
	\begin{enumerate}
		\item $q = \left\lceil{3{D_V}ln(n) + ln(\frac{1}{\epsilon}) + {(3D_V)^k}ln(D_E + 1) + 3{D_V}ln(5)}\right\rceil$
		\item $B_{vertex} = 6q{D_V}$
		\item $B_{edge}(e) = 2h^{+}_{l_e}(B_{\Omega}(6{D_V}D_E))
		\max_{j \in [0,3{D_V}D_E]}{\left\{\left(h^{+}_{j}(B_{\Omega}(2qj))\right)^{\frac{l_e}{\max{\{j,l_e\}}}}\right\}}$

		As a special case, if $\Omega = N(0,1)$ then we can take $B_{edge}(e) = \left(400{D^2_V}{D^2_E}q\right)^{l_e}$
		\item $B_{norm}(\alpha) =
		2e{B_{vertex}^{|V(\alpha) \setminus U_{\alpha}| + |V(\alpha) \setminus V_{\alpha}|}}\left(\prod_{e \in E(\alpha)}{B_{edge}(e)}\right)n^{\frac{w(V(\alpha)) + w(I_{\alpha}) - w(S_{\alpha,min})}{2}}$
		\item $B(\gamma) = B_{vertex}^{|V(\gamma) \setminus U_{\gamma}| + |V(\gamma) \setminus V_{\gamma}|}\left(\prod_{e \in E(\gamma)}{B_{edge}(e)}\right)n^{\frac{w(V(\gamma) \setminus U_{\gamma})}{2}}$
		\item $N(\gamma) = (3D_V)^{2|V(\gamma) \setminus V_{\gamma}| + |V(\gamma) \setminus U_{\gamma}|}$
		\item $c(\alpha) = 100(3{t_{max}}D_V)^{|U_{\alpha} \setminus V_{\alpha}| + |V_{\alpha} \setminus U_{\alpha}| + k|E(\alpha)|}(2t_{max})^{|V(\alpha) \setminus (U_{\alpha} \cup V_{\alpha})|}$
	\end{enumerate}
	and we have SOS-symmetric coefficient matrices $\{H'_{\gamma}: \gamma \in \Gamma\}$ such that the following conditions hold:
	\begin{enumerate}
		\item For all $U \in \mathcal{I}_{mid}$,  $H_{Id_{U}} \succeq 0$
		\item For all $U \in \mathcal{I}_{mid}$ and $\tau \in \mathcal{M}_U$,
		\[
		\left[ {\begin{array}{cc}
				\frac{1}{|Aut(U)|c(\tau)}H_{Id_{U}} & B_{norm}(\tau)H_{\tau} \\
				B_{norm}(\tau)H^T_{\tau} & \frac{1}{|Aut(U)|c(\tau)}H_{Id_{U}}
		\end{array}} \right] \succeq 0
		\]
		\item For all $U,V \in \mathcal{I}_{mid}$ where $w(U) > w(V)$ and all $\gamma \in \Gamma_{U,V}$,
		\[
		c(\gamma)^2{N(\gamma)}^2{B(\gamma)^2}H^{-\gamma,\gamma}_{Id_{V}} \preceq H'_{\gamma}
		\]
	\end{enumerate}
	then with probability at least $1 - \epsilon$,
	\[
	\Lambda \succeq \frac{1}{2}\left(\sum_{U \in \mathcal{I}_{mid}}{M^{fact}_{Id_U}{(H_{Id_U})}}\right) - 3\left(\sum_{U \in \mathcal{I}}{\sum_{\gamma \in \Gamma_{U,*}}{\frac{d_{Id_{U}}(H'_{\gamma},H_{Id_{U}})}{|Aut(U)|c(\gamma)}}}\right)Id_{sym}
	\]
	If it is also true that whenever $\norm{M_{\alpha}} \leq B_{norm}(\alpha)$ for all $\alpha \in \mathcal{M}'$,
	\[
	\sum_{U \in \mathcal{I}_{mid}}{M^{fact}_{Id_U}{(H_{Id_U})}} \succeq 6\left(\sum_{U \in \calI_{mid}}{\sum_{\gamma \in \Gamma_{U,*}}{\frac{d_{Id_{U}}(H'_{\gamma},H_{Id_{U}})}{|Aut(U)|c(\gamma)}}}\right)Id_{sym}
	\]
	then with probability at least $1 - \epsilon$, $\Lambda \succeq 0$.
\end{theorem}
The full proof of the main theorems can be found in \cite{potechin2020machinery}. In this work, we will  apply the machinery to prove our main SoS lower bounds.
\subsection{Choosing $H'_{\gamma}$ and Truncation Error}\label{sec: choosing_hgamma}
A canonical choice for $H'_{\gamma}$ is to take
\begin{enumerate}
	\item $H'_{\gamma}(\sigma,\sigma') = H_{Id_U}(\sigma, \sigma')$ whenever $|V(\sigma \circ \gamma)| \leq D_V$ and $|V(\sigma' \circ \gamma)| \leq D_V$.
	\item $H'_{\gamma}(\sigma,\sigma') = 0$ whenever $|V(\sigma \circ \gamma)| > D_V$ or $|V(\sigma' \circ \gamma)| > D_V$.
\end{enumerate}
With this choice, the truncation error is
\[
d_{Id_{U_{\gamma}}}(H_{Id_{U_{\gamma}}},H'_{\gamma}) = \sum_{\sigma,\sigma' \in \mathcal{L}_{U_{\gamma}}: V(\sigma) \leq D_V, V(\sigma') \leq D_V,
	\atop |V(\sigma \circ \gamma)| > D_V \text{ or } |V(\sigma' \circ \gamma)| > D_V}{B_{norm}(\sigma)B_{norm}(\sigma')H_{Id_{U_{\gamma}}}(\sigma,\sigma')}
\]

\end{comment}

==> sherrington_kirkpatrick/chapter_notes.tex <==
\section{Chapter Notes}

The technical results in this chapter are adapted from \cite{sklowerbounds}, joint work with Mrinalkanti Ghosh, Fernando Granha Jeronimo, Chris Jones and Aaron Potechin.

\input{sherrington_kirkpatrick/open_problems}

==> sherrington_kirkpatrick/exact-constraints.tex <==
\section{Satisfying the Constraints Exactly}
\label{sec:exact-constraints}

After pseudocalibration, the PAP constraints ``$\ip{v}{d_u}^2 = 1$'' are not exactly
satisfied by the pseudocalibration,
but they are satisfied up to truncation error $\pE[\ip{v}{d_u}^2 -1] = n^{-\Omega(n^\tau)}$. This is enough to produce a Sherrington-Kirkpatrick solution that is \textit{almost} boolean, meaning $\pE[x_i^2] = 1 \pm n^{-\Omega(n^\tau)}$ where the pseudocalibration is truncated to degree $n^\tau$. To satisfy the constraints exactly, and produce an SK solution which is \textit{exactly} boolean, we can project the pseudocalibration operator. The goal of this section is to prove the following lemma for the PAP problem,

\begin{lemma}\label{lem:pseudoexpectation-rounding}
W.h.p. for the PAP problem there is $\pE' \in \RR^{\binom{[n]}{\leq D}}$ such that $\norm{\pE - \pE'}_2 \leq \frac{1}{n^{\Omega(n^\tau)}}$ and $\pE'$ exactly satisfies the constraints ``$\ip{v}{d_u}^2 = 1"$.
\end{lemma}
\begin{remark}
Note that $\pE'$ is syntactically guaranteed to still satisfy the constraints ``$v_i^2 = \frac{1}{n}$".
\end{remark}

\begin{corollary}\label{lem:constraint-fixing}
There is an $\binom{[n]}{\leq D/2} \times \binom{[n]}{\leq D/2}$ matrix $\calE$ with $\norm{\calE} \leq \frac{1}{n^{\Omega(n^\tau)}}$ such that the matrix $M_{fix}~\defeq~M~+~\calE$ is SoS-symmetric and exactly satisfies the constraints ``$\ip{v}{d_u}^2 = 1$".
\end{corollary}

We view the operators $\pE$ as vectors in $\RR^{\binom{[n]}{\leq D}}$. The approach we take is to define a ``check matrix" $Q$ such that $\pE$ satisfies the necessary constraints iff $\pE \in \nullspace(Q)$. When the constraints are functions of $v$ only, the matrix $Q$ would be filled with constants. Since the constraints depend on the inputs $d_u$, the matrix $Q$ is also a function of the $d_u$. This allows us to deconstruct it as a sum of graph matrices -- and in fact it is made out of graph matrices which we have seen already.

\begin{definition}
We let $Q$ be the matrix
\[Q \defeq \displaystyle\sum_{k=2}^{D}L_k^\T \]
where the matrices $L_k$ are defined in~\cref{sec:psd}.
\end{definition}

\begin{lemma}
$Q\pE = 0$ iff $\pE$ exactly satisfies the constraints ``$\ip{v}{d_u}^2 = 1$".
\end{lemma}
\begin{proof}
One can see in the proof of~\cref{lem:completed-left-side} that the entries of $Q\pE$ measure exactly the error in the constraints.
\end{proof}

The natural choice of $\pE'$ is therefore the projection of $\pE$ to the nullspace. This is defined by
\[\pE' \defeq \pE - Q^\T(QQ^\T)^+Q\pE \]
where we take the pseudo-inverse of $QQ^\T$ as it will turn out not to be invertible. 
%Note also that, for any constraint which is purely a function of $v$ and was satisfied by $\pE$, the constraint will also be satisfied by $\pE'$. This can seen by writing the constraint as a vector and taking the inner product on the right.

To prove~\cref{lem:pseudoexpectation-rounding}, we must decompose the second 
term in terms of graph matrices and show it has small norm.

As a warm-up, we end this outline by 
showing a simpler projection argument in the Planted Boolean Vector domain is 
sufficient if one just wants to satisfy the boolean constraints in the Planted Boolean Vector problem rather than the constraints of the PAP problem.\footnote{Using the translation between the two problems in~\cref{sec:sk}, this would allow us to exactly satisfy ``$\ip{v}{d_u}^2 =1"$ for the PAP problem. Unfortunately, the constraints ``$v_i^2 =\frac{1}{n}$" might be broken.}


Let $\pE_{\text{PBV}}$ be a candidate, not-yet-boolean, degree-$D$ pseudoexpectation operator for the Planted Boolean Vector problem, $D = 2\cdot n^\delta$. $\pE_{\text{PBV}}$ has an entry for each monomial $b^\alpha$, therefore it 
is $\multiset{n}{\leq D}$-dimensional. Let $Q_{bool}$ be the ``check  
matrix'' for the boolean constraints. $Q_{bool}$ has $n~\cdot~\multiset{n}{\leq D-2}$ rows. The $(i, \alpha)$ row checks $\pE[b^\alpha \cdot b_i^2] = \pE[b^\alpha]$. It has entry 1 in column $\alpha$ and entry $-1$ in column $\alpha \cup \{i, i\}$. 

\begin{lemma}
Assume that $\pE_{\text{PBV}}$ approximately satisfies the boolean constraints:
\[\pE_{\text{PBV}} [b^\alpha \cdot (b_i^2 - 1)] \leq n^{-\Omega(n^\tau)}\]
for any $b^\alpha$ with degree at most $D-2$. Then letting $\pE_{\text{PBV}}'$ be the projection to $\nullspace(Q_{bool})$, we have
\[\norm{\pE_{\text{PBV}} - \pE_{\text{PBV}}'}_2 \leq n^{-\Omega(n^\tau)}.\]
\end{lemma}
\begin{proof}
The effect of projecting $\pE$ to $\nullspace(Q_{bool})$ is to symmetrize $\pE[b^{\alpha + 2\beta}]$ across all $\beta$; average all entries $\pE[1], \pE[b_1^2], \pE[b_2^2], \pE[b_1^6b_7^4b_{10}^2]$ etc, average $\pE[b_1], \pE[b_1b_3^2], \pE[b_1b_3^4b_4^4]$ etc, and so on. One can see this because this is a linear map which fixes $\nullspace(Q_{bool})$ and takes all vectors into $\nullspace(Q_{bool})$.

By assumption, there is additive error $n^{-\Omega(n^\tau)}$ between $\pE_{\text{PBV}}[b^\alpha]$ and 
$\pE_{\text{PBV}}[b^\alpha \cdot b_i^2]$. As the size of $\beta$ is at most $D \ll n^\tau$, we still easily have $\pE_{\text{PBV}}[b^{\alpha + 2\beta}] = \pE_{\text{PBV}}[b^\alpha] \pm n^{-\Omega(n^\tau)}$ for all $\beta$. 
Therefore 
averaging these entries changes each of them by at most 
$n^{-\Omega(n^\tau)}$. Thus,
\[\norm{\pE_{\text{PBV}} - \pE_{\text{PBV}}'}_2 \leq \multichoose{n}{\leq D} \cdot \norm{\pE_{\text{PBV}} - \pE_{\text{PBV}}'}_\infty\]
\[\leq n^{O(n^{\delta})} \cdot n^{-\Omega(n^\tau)} = n^{-\Omega(n^\tau)}\]
\end{proof}

\subsection{Truncation error in the pseudocalibration}

The constraint ``$\ip{v}{d_u}^2 = 1$'' isn't exactly satisfied, but a general property of pseudocalibration is that it's satisfied up to truncation error, which is small w.h.p. We show a quantitative version of this bound.

We introduce the notation
\[\mu_{I, \alpha} \defeq \E_{\text{pl}} [v^I \chi_{\alpha}(d)] \]
where $\chi_\alpha(d) = h_\alpha(d)$ in the Gaussian case and $\chi_\alpha(d) = d^\alpha$ in the boolean case.

\begin{lemma}\label{lem:boolean-approximate-constraints}
    Let $p(d,v)$ such that $p$ is uniformly zero on the planted distribution. Let $\deg_d(p) = D$. For any $I \subseteq [n]$, the only nonzero Fourier coefficients of $\pE[v^I p]$ are those with size between $n^\tau \pm D$.

    Furthermore, the nonzero coefficients are bounded in absolute value by
    \[ M \cdot L \cdot 2^D  e^{mn}\cdot \max_I\max_{\abs{\alpha} \in n^\tau \pm 2D} \abs{\mu_{I, \alpha}} \]
    where $M$ is the number of nonzero monomials of $p$ and $L$ is the largest coefficient of $p$ (in absolute value).
\end{lemma}

\begin{proof} We divide the calculations into boolean and Gaussian cases. For each case we compute that Fourier coefficients below the truncation threshold neatly cancel and bound the coefficients at the threshold.

\noindent\textbf{(Boolean case)} 
Expand $p(d,v) = \displaystyle\sum_{\abs{J} \leq D} d^J p_J(v)$. By linearity,
\[\pE[v^Ip] =  \displaystyle\sum_{\abs{J} \leq D} d^J \pE[v^Ip_J(v)].\]
The $\alpha$-th Fourier coefficient gets a contribution from the $J$-th term equal to the $(\alpha \oplus J)$-th Fourier coefficient of $\pE[v^Ip_J(v)]$. Expand the polynomial $p_J$ in the $J$-th term,
\[ \pE[v^Ip_J(v)] = \sum_{K} c_{J,K} \pE[v^Iv^K]\]
The $(\alpha \oplus J)$-th coefficient of $\pE[v^Iv^K]$ is defined by pseudocalibration to be
\begin{equation}\label{eq:boolean-fourier-cases}
\left\{
\begin{array}{lr}
    \mu_{I+K,\alpha\oplus J} & \abs{\alpha \oplus J} \leq n^\tau\\
    0 & \abs{\alpha \oplus J} > n^\tau
\end{array}\right.
\end{equation}
For $\abs{\alpha} \leq n^\tau - D$ we are guaranteed to be in the first case. For this case the total $\alpha$-th Fourier coefficient is
\begin{align*}
    \displaystyle\sum_{\abs{J} \leq D} \sum_K c_{J,K}\mu_{I+K, \alpha \oplus J} &= \sum_{\abs{J} \leq D} \sum_K c_{J,K}\E_{\text{pl}}[v^{I}v^K d^{J \oplus \alpha}]\\
    &= \sum_{\abs{J} \leq D} \sum_K c_{J,K}\E_{\text{pl}}[v^{I}v^K d^\alpha d^{J}]\\
    &= \E_{\text{pl}}[v^{I}d^{\alpha}p(d,v)]\\
    & = 0.
\end{align*}
For $\abs{\alpha} > n^\tau + D$, we are guaranteed to be in the second case of~\cref{eq:boolean-fourier-cases}, in which case the total Fourier coefficient will also be zero. For $\abs{\alpha}$ within $D$ of the truncation parameter, some terms $J$ will not contribute their coefficients towards cancellation. We bound the Fourier coefficient for these $\alpha$,
\begin{align*}
    \abs{\displaystyle\sum_{\substack{J:\abs{J} \leq D,\\ \abs{\alpha \oplus J} \leq n^\tau}} \sum_K c_{J,K}\cdot\mu_{I+K, \alpha \oplus J}} &\leq \displaystyle\sum_{\abs{J} \leq D} \sum_K \abs{c_{J,K}\cdot\mu_{I+K, \alpha \oplus J}}\\
    &\leq M \cdot L \cdot \max_{I} \max_{\abs{\alpha} \in n^\tau \pm 2D} \abs{\mu_{I,\alpha}}.
\end{align*}

\noindent\textbf{(Gaussian case)} Expand $p(d, v) = \displaystyle\sum_{\abs{\beta} \leq D}h_\beta(d) p_\beta(v) = \sum_{\abs{\beta} \leq D}h_\beta(d) \sum_K c_{\beta, K} v^K$. The pseudoexpectation is
\begin{align*}
\pE[v^I p(d, v)] &= \displaystyle\sum_{\abs{\beta} \leq D}h_\beta(d) \pE[v^Ip_\beta(v)]\\
&= \sum_{\abs{\beta} \leq D}h_\beta(d) \sum_{K}c_{\beta,K}\pE[v^Iv^K]\\
&= \sum_{\abs{\beta} \leq D}h_\beta(d) \sum_K c_{\beta, K}\sum_{\abs{\alpha} \leq n^\tau} \mu_{I+K, \alpha}\frac{h_\alpha(d)}{\alpha!}.
\end{align*}
Let $l_{\alpha,\beta,\gamma}$ be the coefficient of $h_\gamma$ in the Hermite product $h_\alpha \cdot h_\beta$.
\begin{align*}
   \pE[v^I p(d, v)] &= \displaystyle\sum_{\abs{\beta} \leq D} \sum_K c_{\beta, K}\sum_{\abs{\alpha} \leq n^\tau} \mu_{I+K, \alpha}\sum_{\gamma} l_{\alpha,\beta,\gamma}\frac{h_\gamma(d)}{\alpha!} 
\end{align*}
In the case $\abs{\gamma} > n^\tau + D$, the coefficient of $h_\gamma(d)$ is zero because the max degree of a Hermite polynomial appearing in $h_{\alpha}\cdot h_{\beta}$ is at most $\abs{\alpha}+\abs{\beta} \leq n^\tau + D$. We show cancellations occur when $\abs{\gamma} \leq n^\tau - D$.
Moving the summations around, the coefficient of $h_\gamma$ is,
\begin{align*}
    &\displaystyle\sum_{\abs{\beta} \leq D} \sum_K c_{\beta, K}\sum_{\abs{\alpha} \leq n^\tau} \mu_{I+K, \alpha} \cdot  l_{\alpha,\beta,\gamma}\frac{1}{\alpha!}\\
    = & \sum_{\abs{\beta} \leq D} \sum_K c_{\beta, K}\sum_{\abs{\alpha} \leq n^\tau} \E_{\text{pl}}[v^Iv^K h_{\alpha}(d)] \cdot l_{\alpha,\beta,\gamma}\frac{1}{\alpha!}\\
    = & \E_{\text{pl}}v^I\sum_{\abs{\beta} \leq D} \sum_K c_{\beta, K}v^K\sum_{\abs{\alpha} \leq n^\tau} l_{\alpha,\beta,\gamma}\frac{h_{\alpha}(d) }{\alpha!}.
\end{align*}

We need an explicit formula for $l_{\alpha, \beta, \gamma}$ from~\cite[p.~92]{roman2005umbral},

\begin{proposition}\label{prop:multiply-coefficients}
\[l_{\alpha,\beta,\alpha+\beta - 2\delta} = \displaystyle\prod_{u,i}\binom{\alpha_{ui}}{\delta_{ui}}\binom{\beta_{ui}}{\delta_{ui}} \delta_{ui}! \]
\end{proposition}

\begin{proposition}\label{prop:hermite-product}
\[\sum_{\alpha} l_{\alpha,\beta,\gamma}\frac{h_{\alpha}(d) }{\alpha!} = h_{\beta}(d)\cdot \frac{h_\gamma(d)}{\gamma!}\]
\end{proposition}
\begin{proof}
Compute using~\cref{prop:multiply-coefficients}.
\end{proof}

In~\cref{prop:hermite-product}, the summation is actually finite. The largest $\alpha$ with $l_{\alpha,\beta,\gamma}$ nonzero has $\abs{\alpha}~\leq~\abs{\beta}~+~\abs{\gamma}$. Since we have $\abs{\beta}\leq D$ (the constraint only has degree $D$), as long as $\abs{\gamma} \leq n^\tau - D$, the above equality applies, in which case continuing the calculation for this case,
\begin{align*}
   \pE[v^Ip] &= \E_{\text{pl}}v^I\sum_{\abs{\beta} \leq D} \sum_K c_{\beta, K}v^K \cdot h_{\beta}(d)\cdot \frac{h_\gamma(d)}{\gamma!}\\
   &=  \E_{\text{pl}}v^I \cdot \frac{h_\gamma(d)}{\gamma!} \cdot \sum_{\abs{\beta} \leq D} \sum_K c_{\beta, K}v^K \cdot h_{\beta}(d)\\
   &= \E_{\text{pl}}v^I \cdot \frac{h_\gamma(d)}{\gamma!} \cdot p(d,v)\\
   &= 0.
\end{align*}
We now bound the coefficients that appear in the remaining case when $n^\tau - D < \abs{\gamma} \leq n^\tau + D$.
\begin{align*}
    \abs{\displaystyle\sum_{\abs{\beta} \leq D} \sum_K c_{\beta, K}\sum_{\abs{\alpha} \leq n^\tau} \mu_{I+K, \alpha} \cdot  l_{\alpha,\beta,\gamma}\frac{1}{\alpha!}} & \leq \displaystyle\sum_{\abs{\beta} \leq D} \sum_K \abs{c_{\beta, K}}\sum_{\abs{\alpha} \leq n^\tau} \abs{\mu_{I+K, \alpha}} \cdot  l_{\alpha,\beta,\gamma}\frac{1}{\alpha!}
\end{align*}
If $l_{\alpha,\beta,\gamma}> 0$ then we must have $\abs{\alpha} \geq \abs{\gamma} - \abs{\beta} \geq n^\tau - 2D$.
\begin{align*}
    &\leq \sum_{\abs{\beta} \leq D} \sum_K \abs{c_{\beta, K}} \cdot \left(\max_I \max_{\abs{\alpha} \in n^\tau \pm 2D}\abs{\mu_{I, \alpha}} \right) \sum_{\alpha}   l_{\alpha,\beta,\gamma}\frac{1}{\alpha!}
\end{align*}

\begin{proposition}
   \[\sum_{\alpha} l_{\alpha,\beta,\gamma}\frac{1}{\alpha!} = e^{mn} \prod_{u,i}\binom{\beta_{ui}}{\frac{\alpha_{ui} + \beta_{ui} -\gamma_{ui}}{2}}\]
\end{proposition}
\begin{proof}
Compute using~\cref{prop:multiply-coefficients}.
\end{proof}
Using the proposition,
\[\leq \sum_{\abs{\beta} \leq D} \sum_K \abs{c_{\beta, K}} \cdot \left(\max_I \max_{\abs{\alpha} \in n^\tau \pm 2D}\abs{\mu_{I, \alpha}} \right)  e^{mn}\prod_{u,i}\binom{\beta_{ui}}{\frac{\alpha_{ui} + \beta_{ui} -\gamma_{ui}}{2}}  \]
We can bound 
\[\prod_{u,i}\binom{\beta_{ui}}{k_{ui}} \leq \prod_{u,i} 2^{\beta_{ui}} = 2^{\abs{\beta}} \leq 2^D.\]
In total, letting $M$ be the number of nonzero coefficients in the constraint $p$ and $L$ be the largest coefficient, this Fourier coefficient is at most,
\[ M \cdot L \cdot 2^D  e^{mn}\cdot \max_I\max_{\abs{\alpha}\in n^\tau \pm 2D} \abs{\mu_{I+K,\alpha}} .\]
\end{proof}


\begin{lemma}\label{lem:approximate-constraints}
W.h.p. $\norm{Q\pE} \leq \frac{1}{n^{\Omega(n^\tau)}}$
\end{lemma}
\begin{proof}
    Via~\cref{lem:boolean-approximate-constraints} the only nonzero Fourier characters that appear in $Q\pE$ are those of size $n^\tau \pm 2$. Their coefficient in the lemma is at most 
    \begin{align*}
        & C \cdot  e^{mn}\cdot \max_I\max_{\abs{\alpha}\in n^\tau \pm 4} \abs{\mu_{I+K,\alpha}}\\
        \leq & C \cdot e^{mn} \cdot \frac{(n^{\tau} - 4)^{3(n^\tau - 4)}}{n^{(n^\tau - 4)/2}} && (\text{\cref{prop:coefficient-bound}})\\
        \leq & \frac{n^{3\tau n^\tau}}{n^{(\frac{1}{2} + o(1)) n^\tau }}
    \end{align*}
    Therefore we can express $Q\pE$ as a sum of graph matrices\footnote{Graph vectors, since $Q\pE$ is a vector.} of this size, with coefficients bounded by the above quantity. Now we bound the total norm by summing over all graphs.
    
    The number of graph matrices of this size is at most $n^{O(\tau) \cdot n^\tau}$.
    
    The norm of each term can be bounded using norm bounds by $n^{\frac{w(V(\alpha)) - w(S_{\min}) + w(W_{iso})}{2}}$ w.h.p. Note that there is no minimum vertex separator since $V = \emptyset$, and there are $O(1)$ isolated vertices when multiplying graphs in $Q$ with graphs in the pseudocalibration (which have no isolated vertices). The number of circle vertices can be bounded by $\frac{1}{4}\abs{E(\alpha)} \leq \frac{1}{4}n^\tau$. The number of square vertices can be bounded by $O(n^\delta) + \frac{1}{2}\abs{E(\alpha)} \leq 0.52n^\tau$. Therefore the norms are at most $m^{\frac{1}{8}n^\tau}~n^{0.26n^\tau + O(1)}~\leq~n^{0.49n^\tau}$. Notably this is significantly less than the denominator of the graph matrix coefficient, which is $n^{(0.5+o(1))n^\tau}$. Assuming $\delta$ and $\tau$ are small enough, the denominator is enough to overpower all terms multiplied together.
\end{proof}


\subsection{Analyzing $Q{Q^T}$}
The main theorem of this subsection is that the minimum nonzero eigenvalue of $QQ^T$ is large.

\begin{theorem}\label{lem:pseudoinverse-lower-bound}
The minimum nonzero eigenvalue of $QQ^T$ is $\frac{n^2}{2} - \tilde{O}(n\sqrt{m})$. 
\end{theorem}

\begin{proof}[Proof of~\cref{lem:pseudoexpectation-rounding} assuming~\cref{lem:pseudoinverse-lower-bound}]
\begin{align*}
    \norm{\pE - \pE'} & = \norm{Q^\T (QQ^\T)^+ Q\pE} \leq \norm{Q} \cdot \norm{(QQ^\T)^+} \cdot\norm{Q\pE}\\
    & \leq n^{O(1)} \cdot \frac{1}{n^2} \cdot \frac{1}{n^{\Omega(n^\tau)}}\\
    & = \frac{1}{n^{\Omega(n^\tau)}}
\end{align*}
\end{proof}

% Before we prove the theorem, we describe the strategy. Interestingly, the high-level strategy is similar to the overall proof of PSD-ness. Using the expression for $Q$ in terms of graph matrices, we can express 
% $QQ^\T$ as a sum of graph matrices. One of these terms will be an identity matrix which has coefficient $2n^2$. It would be ideal if the 
% remaining terms had norms $\littleoh_n(n^2)$ w.h.p., but as $QQ^\T$ has a nontrivial null space, this is not the case.

% We explicitly give a basis for the null space of $QQ^\T$; it will be a collection of vectors $\{N_t\}_{t \in \calT}$. Then we appeal 
% to~\cref{fact:null-space}: for $x \perp \nullspace(QQ^\T)$, it is equivalent to consider the matrix $QQ^\T~+~\sum_{t \in \calT}~N_tN_t^\T$. 
% This will essentially cancel the non-identity terms with $\Omega(n^2)$ norm in $QQ^\T$, showing that $QQ^\T$ is dominated by an identity matrix with coefficient $\Theta(n^2)$ on $\nullspace(QQ^\T)$.

Recall that $Q = \sum_{k}{L^T_k}$. Let us refer to the five shapes in~\cref{def:lk} as $\alpha_1$ through $\alpha_5$, and their coefficients as $c_{\alpha_i}$. Observe that the dominant part of $L_k$ is $2M_{\alpha_1}$ which has norm $\tilde{O}(n)$. The norm bounds for the other components of $L_k$ are as follows:
\begin{enumerate}
\item $\norm{c_{\alpha_2}M_{\alpha_2}}$ is $\tilde{O}\left(\frac{1}{n} \cdot \sqrt{mn}\right) = \tilde{O}\left(\frac{\sqrt{m}}{\sqrt{n}}\right)$
\item $\norm{c_{\alpha_3}M_{\alpha_3}}$ is $\tilde{O}\left(\frac{1}{n^2} \cdot n\sqrt{m}\right) = \tilde{O}\left(\frac{\sqrt{m}}{n}\right)$
\item $\norm{c_{\alpha_4}M_{\alpha_4}}$ is $\tilde{O}\left(\frac{1}{n} \cdot \sqrt{mn}\right) = \tilde{O}\left(\frac{\sqrt{m}}{\sqrt{n}}\right)$
\item $\norm{c_{\alpha_5}M_{\alpha_5}}$ is $\tilde{O}\left(\frac{1}{n} \cdot \sqrt{m}\right) = \tilde{O}\left(\frac{\sqrt{m}}{n}\right)$
\end{enumerate}

We start by analyzing $QQ^T = \sum_{k}{L^T_k{L_k}}$.

From the above, taking $\alpha = \alpha_1$, the dominant term of $L_k$ is $2M_{\alpha}$ where $U_{\alpha} = \{j_1,\ldots,j_{k}\}$, $V_{\alpha} = \{j_3,\ldots,j_{k}\} \cup \{u\}$, and $E(\alpha) = \{(j_1,u),(j_2,u)\}$. Since $\norm{M_{\alpha}}$ is $\tilde{O}(n)$ and $\norm{L_k - 2M_{\alpha}}$ is $\tilde{O}(\frac{\sqrt{m}}{\sqrt{n}})$, this implies that for each $k$, $\norm{L_{k}^T{L_k} - 4M^T_{\alpha}M_{\alpha}}$ is $\tilde{O}(\sqrt{mn})$. Thus, it is sufficient to analyze $M^T_{\alpha}M_{\alpha}$.

\begin{lemma}\label{QQTdecompositionlemma}
Taking $\alpha$ to be the shape such that $U_{\alpha} \setminus V_{\alpha} = \{j_1,j_2\}$, $U_{\alpha} \cap V_{\alpha} = \{j_3,j_4,\ldots,j_{k}\}$, $V_{\alpha} \setminus U_{\alpha} = \{i_{circ}\}$, and $E(\alpha) = \{(j_1,i),(j_2,i)\}$,
\[
M^{T}_{\alpha}M_{\alpha} = M_{\alpha_1} + M_{\alpha_2} + M_{\alpha_3} + M_{\alpha_4} + M_{\alpha_5} + M_{\alpha_6}
\] where $\alpha_1,\alpha_2,\alpha_3,\alpha_4,\alpha_5,\alpha_6$ are the following shapes. Note that $\alpha_1$ and $\alpha_2$ are improper shapes.
\begin{enumerate}
\item $U_{\alpha_1} \setminus V_{\alpha_1} = \emptyset$, $U_{\alpha_1} \cap V_{\alpha_1} = \{j_3,j_4,\ldots,j_{k}\} \cup \{i_{circ}\}$, $V_{\alpha_1} \setminus U_{\alpha_1} = \emptyset$, $V(\alpha_1) \setminus (U_{\alpha_1} \cup V_{\alpha_1}) = \{j_1,j_2\}$, and $E(\alpha_1) = \{(i,j_1),(i,j_1),(i,j_2),(i,j_2)\}$.
\item $U_{\alpha_2} \setminus V_{\alpha_2} = \{j_1\}$, $U_{\alpha_2} \cap V_{\alpha_2} = \{j_4,\ldots,j_{k}\} \cup \{i_{circ}\}$, $V_{\alpha_2} \setminus U_{\alpha_2} = \{j'_1\}$, $V(\alpha_2) \setminus (U_{\alpha_2} \cup V_{\alpha_2}) = \{j_2\}$, and $E(\alpha_2) = \{(i,j_1),(i,j'_1),(i,j_2),(i,j_2)\}$.
\item $U_{\alpha_3} \setminus V_{\alpha_3} = \{j_1,j_2\}$, $U_{\alpha_3} \cap V_{\alpha_3} = \{j_5,\ldots,j_{k}\} \cup \{i_{circ}\}$, $V_{\alpha_3} \setminus U_{\alpha_3} = \{j'_1,j'_2\}$, and $E(\alpha_3) = \{(i,j_1),(i,j_2),(i,j'_1),(i,j'_2)\}$.
\item $U_{\alpha_4} \setminus V_{\alpha_4} = \{i_{circ}\}$, $U_{\alpha_4} \cap V_{\alpha_4} = \{j_3,j_4,\ldots,j_{k}\}$, $V_{\alpha_4} \setminus U_{\alpha_4} = \{i'_{circ}\}$, $V(\alpha_4) \setminus (U_{\alpha_4} \cup V_{\alpha_4}) = \{j_1,j_2\}$, and $E(\alpha_4) = \{(i,j'_1),(i,j'_2),(i',j_1),(i',j_2)\}$.
\item $U_{\alpha_5} \setminus V_{\alpha_5} = \{j_1\} \cup \{i_{circ}\}$, $U_{\alpha_5} \cap V_{\alpha_5} = \{j_4,\ldots,j_{k}\}$, $V_{\alpha_5} \setminus U_{\alpha_5} = \{j'_1\} \cup \{i'_{circ}\}$, $V(\alpha_5) \setminus (U_{\alpha_5} \cup V_{\alpha_5}) = \{j_2\}$, and $E(\alpha_5) = \{(i,j'_1),(i,j_2),(i',j_1),(i',j_2)\}$.
\item $U_{\alpha_6} \setminus V_{\alpha_6} = \{j_1,j_2\} \cup \{i_{circ}\}$, $U_{\alpha_6} \cap V_{\alpha_6} = \{j_5,\ldots,j_{k}\}$, $V_{\alpha_6} \setminus U_{\alpha_6} = \{j'_1,j'_2\}  \cup \{i'_{circ}\}$, and $E(\alpha_6) = \{(i',j_1),(i',j_2),(i,j'_1),(i,j'_2)\}$.
\end{enumerate}
\end{lemma}
For pictures of these shapes, see~\cref{fig:QQTdominantfigure} below.
\begin{figure}[ht]
\centerline{\includegraphics[height=10cm]{sherrington_kirkpatrick/QQTFull}}
\caption{This figure shows the decomposition of $M^T_{\alpha}M_{\alpha}$.}
\label{fig:QQTdominantfigure}
\end{figure}
\begin{remark}
For $k = 2$, only shapes $\alpha_1$ and $\alpha_4$ are present and for $k = 3$, only shapes $\alpha_1,\alpha_2,\alpha_4,\alpha_5$ are present.
\end{remark}
\begin{proof}[Proof of Lemma \ref{QQTdecompositionlemma}]
We compute $M_{\alpha^T}M_{\alpha}$ by considering the ribbons which appear in $M_{\alpha^T}M_{\alpha}$.
\begin{enumerate}
\item Each ribbon $R$ with $A_R \setminus B_R = \emptyset$, $A_R \cap B_R = \{j_3,j_4,\ldots,j_{k}\} \cup \{i_{circ}\}$, $B_R \setminus A_R = \emptyset$, $V(R) \setminus (A_R \cup B_R) = \{j_1,j_2\}$, and $E(R) = \{(i,j_1),(i,j_1),(i,j_2),(i,j_2)\}$ appears in exactly one way as the composition of the ribbons $R_1$ and $R_2$ where 
\begin{enumerate}
\item $A_{R_1} \setminus B_{R_1} = \{i_{circ}\}$, $A_{R_1} \cap B_{R_1} = \{j_3,j_4,\ldots,j_{k}\}$, $B_{R_1} \setminus A_{R_1} = \{j_1,j_2\}$, and $E(R_1) = \{(i,j_1),(i,j_2)\}$.
\item $A_{R_2} \setminus B_{R_2} = \{j_1,j_2\}$, $A_{R_2} \cap B_{R_2} = \{j_3,j_4,\ldots,j_{k}\}$, $B_{R_2} \setminus A_{R_2} = \{i_{circ}\}$, and $E(R_2) = \{(i,j_1),(i,j_2)\}$.
\end{enumerate}
\item Each ribbon $R$ with $A_R \setminus B_R = \{j_1\}$, $A_R \cap B_R = \{j_4,\ldots,j_{k}\} \cup \{i_{circ}\}$, $B_R \setminus A_R = \{j'_1\}$, $V(R) \setminus (A_R \cup B_R) = \{j_2\}$, and $E(R) = \{(i,j_1),(i,j'_1),(i,j_2),(i,j_2)\}$ appears in exactly one way as the composition of the ribbons $R_1$ and $R_2$ where 
\begin{enumerate}
\item $A_{R_1} \setminus B_{R_1} = \{i_{circ}\}$, $A_{R_1} \cap B_{R_1} = \{j_1,j_4,\ldots,j_{k}\}$, $B_{R_1} \setminus A_{R_1} = \{j'_1,j_2\}$, and $E(R_1) = \{(i,j'_1),(i,j_2)\}$.
\item $A_{R_2} \setminus B_{R_2} = \{j_1,j_2\}$, $A_{R_2} \cap B_{R_2} = \{j'_1,j_4,\ldots,j_{k}\}$, $B_{R_2} \setminus A_{R_2} = \{i_{circ}\}$, and $E(R_2) = \{(i,j_1),(i,j_2)\}$.
\end{enumerate}
\item Each ribbon $R$ with $A_R \setminus B_R = \{j_1,j_2\}$, $A_R \cap B_R = \{j_5,\ldots,j_{k}\} \cup \{i_{circ}\}$, $B_R \setminus A_R = \{j'_1,j'_2\}$, $V(R) \setminus (A_R \cup B_R) = \emptyset$, and $E(R) = \{(i,j_1),(i,j'_1),(i,j_2),(i,j'_2)\}$ appears in exactly one way as the composition of the ribbons $R_1$ and $R_2$ where 
\begin{enumerate}
\item $A_{R_1} \setminus B_{R_1} = \{i_{circ}\}$, $A_{R_1} \cap B_{R_1} = \{j_1,j_2,j_5,\ldots,j_{k}\}$, $B_{R_1} \setminus A_{R_1} = \{j'_1,j'_2\}$, and $E(R_1) = \{(i,j'_1),(i,j'_2)\}$.
\item $A_{R_2} \setminus B_{R_2} = \{j_1,j_2\}$, $A_{R_2} \cap B_{R_2} = \{j'_1,j'_2,j_5,\ldots,j_{k}\}$, $B_{R_2} \setminus A_{R_2} = \{i_{circ}\}$, and $E(R_2) = \{(i,j_1),(i,j_2)\}$.
\end{enumerate}
\item Each ribbon $R$ with $A_R \setminus B_R = \{j_1,j_2\} \cup  \{i_{circ}\}$, $A_R \cap B_R = \{j_5,\ldots,j_{k}\}$, $B_R \setminus A_R = \{j'_1,j'_2\}  \cup  \{i'_{circ}\}$, $V(R) \setminus (A_R \cup B_R) = \emptyset$, and $E(R) = \{(i,j'_1),(i,j'_2),(i',j_1),(i',j_2)\}$ appears in exactly one way as the composition of the ribbons $R_1$ and $R_2$ where 
\begin{enumerate}
\item $A_{R_1} \setminus B_{R_1} = \{i_{circ}\}$, $A_{R_1} \cap B_{R_1} = \{j_1,j_2,j_5,\ldots,j_{k}\}$, $B_{R_1} \setminus A_{R_1} = \{j'_1,j'_2\}$, and $E(R_1) = \{(i,j'_1),(i,j'_2)\}$.
\item $A_{R_2} \setminus B_{R_2} = \{j_1,j_2\}$, $A_{R_2} \cap B_{R_2} = \{j'_1,j'_2,j_5,\ldots,j_{k}\}$, $B_{R_2} \setminus A_{R_2} = \{i'_{circ}\}$, and $E(R_2) = \{(i,j_1),(i,j_2)\}$.
\end{enumerate}
\item Each ribbon $R$ with $A_R \setminus B_R = \{i_{circ}\}$, $A_R \cap B_R = \{j_3,j_4,\ldots,j_{k}\}$, $B_R \setminus A_R = \{i'_{circ}\}$, $V(R) \setminus (A_R \cup B_R) = \{j_1,j_2\}$, and $E(R) = \{(i,j_1),(i,j_2),(i',j_1),(i',j_2)\}$ appears in exactly one way as the composition of the ribbons $R_1$ and $R_2$ where 
\begin{enumerate}
\item $A_{R_1} \setminus B_{R_1} = \{i_{circ}\}$, $A_{R_1} \cap B_{R_1} = \{j_3,j_4,\ldots,j_{k}\}$, $B_{R_1} \setminus A_{R_1} = \{j_1,j_2\}$, and $E(R_1) = \{(i,j_1),(i,j_2)\}$.
\item $A_{R_2} \setminus B_{R_2} = \{j_1,j_2\}$, $A_{R_2} \cap B_{R_2} = \{j_3,j_4,\ldots,j_{k}\}$, $B_{R_2} \setminus A_{R_2} = \{i'_{circ}\}$, and $E(R_2) = \{(i',j_1),(i',j_2)\}$.
\end{enumerate}
\item Each ribbon $R$ with $A_R \setminus B_R = \{j_1\}$, $A_R \cap B_R = \{j_4,\ldots,j_{k}\} \cup \{i_{circ}\}$, $B_R \setminus A_R = \{j'_1\}$, $V(R) \setminus (A_R \cup B_R) = \{j_2\}$, and $E(R) = \{(i,j_1),(i,j'_1),(i,j_2),(i,j_2)\}$ appears in exactly one way as the composition of the ribbons $R_1$ and $R_2$ where 
\begin{enumerate}
\item $A_{R_1} \setminus B_{R_1} = \{i_{circ}\}$, $A_{R_1} \cap B_{R_1} = \{j_1,j_4,\ldots,j_{k}\}$, $B_{R_1} \setminus A_{R_1} = \{j'_1,j_2\}$, and $E(R_1) = \{(i,j'_1),(i,j_2)\}$.
\item $A_{R_2} \setminus B_{R_2} = \{j_1,j_2\}$, $A_{R_2} \cap B_{R_2} = \{j'_1,j_4,\ldots,j_{k}\}$, $B_{R_2} \setminus A_{R_2} = \{i_{circ}\}$, and $E(R_2) = \{(i,j_1),(i,j_2)\}$.
\end{enumerate}
\end{enumerate}
Based on these cases, we have that $M_{\alpha^T}M_{\alpha} = M_{\alpha_1} + M_{\alpha_2} + M_{\alpha_3} + M_{\alpha_4} + M_{\alpha_5} + M_{\alpha_6}$.
\end{proof}
We now analyze each of the matrices $M_{\alpha_1}, M_{\alpha_2}, M_{\alpha_3}, M_{\alpha_4}, M_{\alpha_5}, M_{\alpha_6}$.
\begin{lemma}
Taking $Id_{k-2,1}$ to be the shape where $U_{Id_{k-2,1}} \setminus V_{Id_{k-2,1}} = \emptyset$, $U_{Id_{k-2,1}} \cap V_{Id_{k-2,1}} = \{j_3,j_4,\ldots,j_{k}\} \cup \{i_{circ}\}$, $V_{Id_{k-2,1}} \setminus U_{Id_{k-2,1}} = \emptyset$, and $E(Id_{k-2,1}) = \emptyset$, $\norm{M_{\alpha_1} - \binom{n-k+2}{2}M_{Id_{k-2,1}}}$ is $\tilde{O}\left(n^{\frac{3}{2}}\right)$.
\end{lemma}
\begin{proof}
To convert an improper shape $\alpha_1$ to a sum of proper shapes, we take each ribbon of shape $\alpha_1$ and decompose it into a sum of proper ribbons. Decomposing $M_{\alpha_1}$ in this way, each ribbon $R$ with $A_R \setminus B_R = \emptyset$, $A_R \cap B_R = \{j_3,j_4,\ldots,j_{k}\} \cup \{i_{circ}\}$, $B_R \setminus A_R = \emptyset$, and $E(R) = \emptyset$ appears $\binom{n-k+2}{2}$ times, once for each pair $j_1,j_2$ such that $j_1 < j_2$ and $j_1,j_2 \notin \{j_3,\ldots,j_{k}\}$. The other ribbons which arise all have an edge with label $2$ incident with $j_1$ or $j_2$ and thus the resulting terms have norm $\tilde{O}\left(n^{\frac{3}{2}}\right)$.
\end{proof}
\begin{definition}
Define $\beta_2$ to be the shape such that $U_{\beta_2} \setminus V_{\beta_2} = \{j_1\}$, $U_{\beta_2} \cap V_{\beta_2} = \{j_4,\ldots,j_{k}\} \cup \{i_{circ}\}$, $V_{\beta_2} \setminus U_{\beta_2} = \emptyset$, and $E(\beta_1) = \{(i,j_1)\}$.
\end{definition}
\begin{lemma}
$\norm{M_{\alpha_2} - (n-k+1)M_{\beta_2}M^T_{\beta_2}}$ is $\tilde{O}\left(n^{\frac{3}{2}}\right)$.
\end{lemma}
\begin{proof}
Again, to convert an improper shape $\alpha_2$ to a sum of proper shapes, we take each ribbon of shape $\alpha_2$ and decompose it into a sum of proper ribbons. Decomposing $M_{\alpha_2}$ in this way, each ribbon $R$ with $A_R \setminus B_R = \{j_1\}$, $A_R \cap B_R = \{j_4,\ldots,j_{k}\} \cup \{i_{circ}\}$, $B_R \setminus A_R = \emptyset$, and $E(R) = \{(i,j_1),(i,j'_1)\}$ appears $(n-k+1)$ times, once for each $j_2 \in [n] \setminus \{j_1,j'_1,j_4,\ldots,j_k\}$. The other ribbons which arise have an edge with label $2$ incident with $j_2$ and thus the resulting terms have norm $\tilde{O}\left(n^{\frac{3}{2}}\right)$. This implies that if we take $\alpha'_2$ to be the shape where $U_{\alpha_2} \setminus V_{\alpha_2} = \{j_1\}$, $U_{\alpha_2} \cap V_{\alpha_2} = \{j_4,\ldots,j_{k}\} \cup \{i_{circ}\}$, $V_{\alpha_2} \setminus U_{\alpha_2} = \{j'_1\}$, and $E(\alpha_2) = \{(i,j_1),(i,j'_1)\}$ then $\norm{M_{\alpha_2} - (n-k+1)M_{\alpha'_2}}$ is $\tilde{O}\left(n^{\frac{3}{2}}\right)$.

$\norm{M_{\alpha'_2}}$ is $\tilde{O}(n)$, so this term cannot be ignored. To handle this, we observe that $M_{\alpha'_2}$ is approximately equal to a PSD matrix. More precisely, $\norm{M_{\alpha'_2} - M_{\beta_2}M^T_{\beta_2}}$ is $\tilde{O}(1)$. To see this, note that when we expand out $M_{\beta_2}M^T_{\beta_2}$, the ribbons which result when there are no collisions give $M_{\alpha'_2}$ and for each ribbon $R$ which results from a collision, $A_R \setminus B_R = B_R \setminus A_R = \emptyset$ so the resulting terms have norm $\tilde{O}(1)$. 
\end{proof}
\begin{figure}[ht]\label{BetaTwoFigure}
\centerline{\includegraphics[height=3cm]{sherrington_kirkpatrick/BetaTwo}}
\caption{This figure shows $\alpha'_2$ and $\beta_2$ for $k = 4$.}
\end{figure}
$\norm{M_{\alpha_3}}$ is $\tilde{O}(n^2)$, so this term cannot be ignored. To handle this, we observe that $M_{\alpha_3}$ is approximately equal to a PSD matrix. More precisely, we have the following lemma.
\begin{definition}
Define $\beta_3$ to be the shape such that $U_{\beta_3} \setminus V_{\beta_3} = \{j_1,j_2\}$, $U_{\beta_3} \cap V_{\beta_3} = \{j_5,\ldots,j_{k}\} \cup \{i_{circ}\}$, $V_{\beta_3} \setminus U_{\beta_3} = \emptyset$, and $E(\beta_3) = \{(i,j_1),(i,j_2)\}$.
\end{definition}
\begin{lemma}
$\norm{M_{\alpha_3} - M_{\beta_3}M^T_{\beta_3}}$ is $\tilde{O}(n)$.
\end{lemma}
\begin{proof}
To see this, note that when we expand out $M_{\beta_3}M^T_{\beta_3}$, the ribbons which result when there are no collisions give $M_{\alpha_3}$ and for each ribbon $R$ which results from a collision, $|A_R \setminus B_R| = |B_R \setminus A_R| \leq 1$ so the resulting terms have norm $\tilde{O}(n)$. 
\end{proof}
\begin{figure}[ht]\label{BetaThreeFigure}
\centerline{\includegraphics[height=3cm]{sherrington_kirkpatrick/BetaThree}}
\caption{This figure shows $\alpha_3$ and $\beta_3$ for $k = 4$.}
\end{figure}
We now consider the norms of $M_{\alpha_4}$, $M_{\alpha_5}$, and $M_{\alpha_6}$.
\begin{enumerate}
\item $\norm{M_{\alpha_4}}$ is $\tilde{O}(n\sqrt{m})$.
\item $\norm{M_{\alpha_5}}$ is $\tilde{O}(n\sqrt{m})$.
\item $\norm{M_{\alpha_6}}$ is $\tilde{O}(n^2)$.
\end{enumerate}
This means that $M_{\alpha_4}$ and $M_{\alpha_5}$ can be ignored but $M_{\alpha_6}$ cannot be ignored. In fact, there is a very good reason for this. In particular, for $k \geq 4$, $L_k$ has a non-trivial nullspace $N_k$, so we cannot show that the minimum nonzero eigenvalue of ${L_k^T}{L_k}$ is large without taking this nullspace into account. We handle this nullspace $N_k$ in the next two subsubsections.

Putting everything together, we have the following corollary:
\begin{corollary}\label{QQTapproximationcorollary} \ 
\begin{enumerate}
\item For $k = 2$, $\norm{{L_k^T}L_k - 2{n^2}M_{Id_{k-2,1}}}$ is $\tilde{O}(n\sqrt{m})$
\item For $k = 3$, $\norm{{L_k^T}L_k - 2{n^2}M_{Id_{k-2,1}} - 4nM_{\beta_2}M^T_{\beta_2}}$ is $\tilde{O}(n\sqrt{m})$
\item For $k \geq 4$, $\norm{{L_k^T}L_k - 2{n^2}M_{Id_{k-2,1}} - 4nM_{\beta_2}M^T_{\beta_2} - 4M_{\beta_3}M^T_{\beta_3} - 4M_{\alpha_6}}$ is $\tilde{O}(n\sqrt{m})$
\end{enumerate}
\end{corollary}
\begin{remark}
We replaced $\binom{n-k+2}{2}$ with $\frac{n^2}{2}$ as $\norm{M_{Id_{k-2,1}}} = 1$ and $|\frac{n^2}{2} - \binom{n-k+2}{2}|$ is $\tilde{O}(n)$. Similarly, we replaced $(n-k+1)$ with $n$ as $\norm{M_{\alpha'_2}}$ is $\tilde{O}(n)$ and $|n - (n-k+1)|$ is $\tilde{O}(1)$
\end{remark}
\subsubsection{The Null Space $N_k$}
We now construct a matrix $N_k$ for each $k \geq 4$ such that ${L_k}{N_k} = 0$ and the columns of ${N_k}$ span the nullspace of $L_k$. To do this, we construct $N_k$ so that the entries of each column of $N_k$ is indexed by a subset $S = \{j_3,\ldots,j_{k}\} \subseteq [n]$ and an ordered tuple of circle indices $(i,i')$ where $i < i'$. We then want that if we view $\tilde{E}$ as a vector,
\[
({\tilde{E}^T}{L_k}N_k)_{S,(i,i')} = \tilde{E}\left[v^{S}\left({\ip{v}{d_i}}^2 - 1\right)\left({\ip{v}{d_{i'}}}^2 - 1\right)\right] - \tilde{E}\left[v^{S}\left({\ip{v}{d_{i'}}}^2 - 1\right)\left({\ip{v}{d_i}}^2 - 1\right)\right] = 0
\]
\begin{lemma}
$N_k = c_{\alpha_1}(M_{\alpha_1^+} - M_{\alpha_1^-}) + c_{\alpha_2}(M_{\alpha_2^+} - M_{\alpha_2^-}) + c_{\alpha_3}(M_{\alpha_3^+} - M_{\alpha_3^-}) + c_{\alpha_4}(M_{\alpha_4^+} - M_{\alpha_4^-}) + c_{\alpha_5}(M_{\alpha_5^+} - M_{\alpha_5^-})$ for the following shapes $\alpha_1^{+},\ldots,\alpha_5^{+}, \alpha_1^{-},\ldots,\alpha_5^{-}$ and coefficients $c_{\alpha_1},\ldots,c_{\alpha_5}$. Unless stated otherwise, all of these shapes have no middle vertices.
\begin{enumerate}
\item $U_{\alpha_1^+} \setminus V_{\alpha_1^+} = \{j_1,j_2\}$, $U_{\alpha_1^+} \cap V_{\alpha_1^+} = \{j_3,j_4,\ldots,j_{k}\} \cup \{i'_{circ}\}$, $V_{\alpha_1^+} \setminus U_{\alpha_1^+} = \{i_{circ}\}$, $E(\alpha_1^+) = \{(j_1,i),(j_2,i)\}$, and $c_{\alpha_1} = 2$.
\item $U_{\alpha_2^+} \setminus V_{\alpha_2^+} = \{j_2\}$, $U_{\alpha_2^+} \cap V_{\alpha_2^+} = \{j_4,\ldots,j_{k}\} \cup \{i'_{circ}\}$, $V_{\alpha_2^+} \setminus U_{\alpha_2^+} = \{j_3\} \cup \{i_{circ}\}$, $E(\alpha_2^+) = \{(j_3,i),(j_2,i)\}$, and $c_{\alpha_2} = \frac{2}{n}$.
\item $U_{\alpha_3^+} \setminus V_{\alpha_3^+} = \emptyset$, $U_{\alpha_3^+} \cap V_{\alpha_3^+} = \{j_5,\ldots,j_{k}\} \cup \{i'_{circ}\}$, $V_{\alpha_3^+} \setminus U_{\alpha_3^+} = \{j_3,j_4\} \cup \{i_{circ}\}$, $E(\alpha_3^+) = \{(j_3,i),(j_4,i)\}$, and $c_{\alpha_3} = \frac{2}{n^2}$.
\item $U_{\alpha_4^+} \setminus V_{\alpha_4^+} = \emptyset$, $U_{\alpha_4^+} \cap V_{\alpha_4^+} = \{j_3,j_4,\ldots,j_{k}\} \cup \{i'_{circ}\}$, $V_{\alpha_4^+} \setminus U_{\alpha_4^+} = \{i_{circ}\}$, $V(\alpha_4^+) \setminus (U_{\alpha_4^+} \cup V_{\alpha_4^+}) = \{j_1\}$ $E(\alpha_4^+) = \{(j_1,i)_2\}$, and $c_{\alpha_4} = \frac{1}{n}$.
\item $U_{\alpha_5^+} \setminus V_{\alpha_5^+} = \emptyset$, $U_{\alpha_5^+} \cap V_{\alpha_5^+} = \{j_3,j_4,\ldots,j_{k}\} \cup \{i'_{circ}\}$, $V_{\alpha_5^+} \setminus U_{\alpha_5^+} = \{i_{circ}\}$, $E(\alpha_5^+) = \{(j_3,i)_2\}$, and $c_{\alpha_5} = \frac{1}{n}$.
\end{enumerate}
where for all of these shapes, $(i_{circ},i'_{circ})$ is a tuple in the right side and $i < i'$. $\alpha_1^{-},\ldots,\alpha_5^{-}$ are the same as $\alpha_1^{+},\ldots,\alpha_5^{+}$ except that $i$ and $i'$ are swapped.
\end{lemma}
\begin{remark}
Note that $\alpha_1^{+},\ldots,\alpha_5^{+}$ are the same shapes which appear in the decomposition of $L_k$ except that the intersection of $U$ and $V$ now contains $i'_{circ}$ and we require that $i < i'$.
\end{remark}
For pictures of these shapes, see Figure \ref{NDecompositionFigure} below.
\begin{figure}[ht]
\centerline{\includegraphics[height=10cm]{sherrington_kirkpatrick/NFull081620}}
\caption{This figure shows the decomposition of $N_k$ for $k = 4$. Here we always have that $i < i'$. If $i$ and $i'$ are swapped then this flips the signs but these parts are not shown to save space.}
\label{NDecompositionFigure}
\end{figure}
\begin{proof}
To determine $N_k$, we analyze the ribbons which $N_k$ is composed of. Let $S = \{j_3,j_4,\ldots,j_k\}$.
\begin{enumerate}
\item If we take a ribbon $R$ with $A_R = \{j_1,\ldots,j_{k}\} \cup \{i'_{circ}\}$, $B_R = \{j_3,\ldots,j_{k}\} \cup (i_{circ},i'_{circ})$, and $E(R) = \{(j_1,i),(j_2,i)\}$ where $j_1 \neq j_2$ and $j_1,j_2 \notin S$ then 
\[
({\tilde{E}^T}{L_k}M_R)_{S,i,i'} = \tilde{E}\left[v^{S}v_{j_1}v_{j_2}(d_{i})_{j_1}(d_i)_{j_2}\left({\ip{v}{d_{i'}}}^2 - 1\right)\right]
\]
Each such term appears with a coefficient of $2$ in $\tilde{E}\left[v^{S}\left({\ip{v}{d_i}}^2 - 1\right)\left({\ip{v}{d_{i'}}}^2 - 1\right)\right]$, so we want each such ribbon $R$ to appear with a coefficient of $2$ in $N_k$.

Similarly, we want each ribbon $R$ with $A_R = \{j_1,\ldots,j_{k}\} \cup \{i_{circ}\}$, $B_R = \{j_3,\ldots,j_{k}\} \cup (i_{circ},i'_{circ})$, and $E(R) = \{(j_1,i'),(j_2,i')\}$ where $j_1 \neq j_2$ and $j_1,j_2 \notin S$ to appear with a coefficient of $-2$ in $N_k$.
\item If we take a ribbon $R$ with $A_R = (\{j_1,\ldots,j_{k}\} \setminus \{j_1,j_3\}) \cup \{i'_{circ}\}$, $B_R = \{j_3,\ldots,j_{k}\} \cup (i_{circ},i'_{circ})$, and $E(R) = \{(j_3,i),(j_2,i)\}$ where $j_1 = j_3 \in S$ and $j_2 \notin S$ then 
\begin{align*}
({\tilde{E}^T}{L_k}M_R)_{S,i,i'} &= \tilde{E}\left[v^{S \setminus \{j_1,j_3\}}v_{j_2}(d_{i})_{j_3}(d_i)_{j_2}\left({\ip{v}{d_{i'}}}^2 - 1\right)\right]\\
&=n\tilde{E}\left[v^{S}v_{j_1}v_{j_2}(d_{i})_{j_1}(d_i)_{j_2}\left({\ip{v}{d_{i'}}}^2 - 1\right)\right]
\end{align*}
Each such term appears with a coefficient of $\frac{2}{n}$ in $\tilde{E}\left[v^{S}\left({\ip{v}{d_i}}^2 - 1\right)\left({\ip{v}{d_{i'}}}^2 - 1\right)\right]$, so we want each such ribbon $R$ to appear with a coefficient of $\frac{2}{n}$ in $N_k$.

Similarly, we want each ribbon $R$ with $A_R = (\{j_1,\ldots,j_{k}\} \setminus \{j_1,j_3\}) \cup \{i_{circ}\}$, $B_R = \{j_3,\ldots,j_{k}\} \cup (i_{circ},i'_{circ})$, and $E(R) = \{(j_3,i'),(j_2,i')\}$ where $j_1 = j_3 \in S$ and $j_2 \notin S$ to appear with a coefficient of $-\frac{2}{n}$ in $N_k$.
\item If we take a ribbon $R$ with $A_R = (\{j_1,\ldots,j_{k}\} \setminus \{j_1,j_2,j_3,j_4\}) \cup \{i'_{circ}\}$, $B_R = \{j_3,\ldots,j_{k}\} \cup (i_{circ},i'_{circ})$, and $E(R) = \{(j_3,i),(j_4,i)\}$ where $j_1 = j_3 \in S$ and $j_2 = j_4 \in S$ then 
\begin{align*}
({\tilde{E}^T}{L_k}M_R)_{S,i,i'} &= \tilde{E}\left[v^{S \setminus \{j_1,j_2,j_3,j_4\}}(d_{i})_{j_3}(d_i)_{j_4}\left({\ip{v}{d_{i'}}}^2 - 1\right)\right]\\
&=n^2\tilde{E}\left[v^{S}v_{j_1}v_{j_2}(d_{i})_{j_1}(d_i)_{j_2}\left({\ip{v}{d_{i'}}}^2 - 1\right)\right]
\end{align*}
Each such term appears with a coefficient of $\frac{2}{n^2}$ in $\tilde{E}\left[v^{S}\left({\ip{v}{d_i}}^2 - 1\right)\left({\ip{v}{d_{i'}}}^2 - 1\right)\right]$, so we want each such ribbon $R$ to appear with a coefficient of $\frac{2}{n^2}$ in $N_k$.

Similarly, we want each ribbon $R$ with $A_R = (\{j_1,\ldots,j_{k}\} \setminus \{j_1,j_2,j_3,j_4\}) \cup \{i_{circ}\}$, $B_R = \{j_3,\ldots,j_{k}\} \cup (i_{circ},i'_{circ})$, and $E(R) = \{(j_3,i'),(j_4,i')\}$ where $j_1 = j_3 \in S$ and $j_2 = j_4 \in S$ to appear with a coefficient of $-\frac{2}{n^2}$ in $N_k$.
\item If we take a ribbon $R$ with $A_R = (\{j_1,\ldots,j_{k}\} \setminus \{j_1,j_2\})  \cup \{i'_{circ}\}$, $B_R = \{j_3,\ldots,j_{k}\} \cup (i_{circ},i'_{circ})$, and $E(R) = \{(j_1,i)_2\}$ where $j_1 = j_2 \notin S$ then 
\begin{align*}
({\tilde{E}^T}{L_k}M_R)_{S,i,i'} &= \tilde{E}\left[v^{S \setminus \{j_1,j_2\}}((d_{i})^2_{j_1} - 1)\left({\ip{v}{d_{i'}}}^2 - 1\right)\right]\\
&=n\tilde{E}\left[v^{S}v_{j_1}^2((d_{i})^2_{j_1} - 1)\left({\ip{v}{d_{i'}}}^2 - 1\right)\right]
\end{align*}
Each such term appears with a coefficient of $\frac{1}{n}$ in $\tilde{E}\left[v^{S}\left({\ip{v}{d_i}}^2 - 1\right)\left({\ip{v}{d_{i'}}}^2 - 1\right)\right]$ so we want each such ribbon $R$ to appear with a coefficient of $\frac{1}{n}$ in $N_k$.

Similarly, we want each ribbon $R$ with $A_R = (\{j_1,\ldots,j_{k}\} \setminus \{j_1,j_2\})  \cup \{i'_{circ}\}$, $B_R = \{j_3,\ldots,j_{k}\} \cup (i_{circ},i'_{circ})$, and $E(R) = \{(j_1,i)_2\}$ where $j_1 = j_2 \notin S$ to appear with a coefficient of $-\frac{1}{n}$ in $N_k$.
\item If we take a ribbon $R$ with $A_R = (\{j_1,\ldots,j_{k}\} \setminus \{j_1,j_2\}) \cup \{i'_{circ}\}$, $B_R = \{j_3,\ldots,j_{k}\} \cup (i_{circ},i'_{circ})$, and $E(R) = \{(j_3,i)_2\}$ where $j_1 = j_2 = j_3 \in S$ then 
\begin{align*}
({\tilde{E}^T}{L_k}M_R)_{S,i,i'} &= \tilde{E}\left[v^{S \setminus \{j_1,j_2\}}((d_{i})^2_{j_3} - 1)\left({\ip{v}{d_{i'}}}^2 - 1\right)\right]\\
&=n\tilde{E}\left[v^{S}v_{j_1}^2((d_{i})^2_{j_1} - 1)\left({\ip{v}{d_{i'}}}^2 - 1\right)\right]
\end{align*}
Each such term appears with a coefficient of $\frac{1}{n}$ in $\tilde{E}\left[v^{S}\left({\ip{v}{d_i}}^2 - 1\right)\left({\ip{v}{d_{i'}}}^2 - 1\right)\right]$ so we want each such ribbon $R$ to appear with a coefficient of $\frac{1}{n}$ in $N_k$.

Similarly, we want each ribbon $R$ with $A_R = (\{j_1,\ldots,j_{k}\} \setminus \{j_1,j_2\}) \cup \{i'_{circ}\}$, $B_R = \{j_3,\ldots,j_{k}\} \cup (i_{circ},i'_{circ})$, and $E(R) = \{(j_3,i)_2\}$ where $j_1 = j_2 = j_3 \in S$ to appear with a coefficient of $-\frac{1}{n}$ in $N_k$.
\end{enumerate}
\end{proof}
Observe that the dominant part of $N_k$ is $2(M_{\alpha_1^+} - M_{\alpha_1^-})$ which has norm $\tilde{O}(n)$. The norm bounds for the other components of $N_k$ are as follows:
\begin{enumerate}
\item $\norm{c_{\alpha_2}(M_{\alpha_2^+} - M_{\alpha_2^-})}$ is $\tilde{O}\left(\frac{1}{n} \cdot \sqrt{mn}\right) = \tilde{O}\left(\frac{\sqrt{m}}{\sqrt{n}}\right)$
\item $\norm{c_{\alpha_3}(M_{\alpha_3^+} - M_{\alpha_3^-})}$ is $\tilde{O}\left(\frac{1}{n^2} \cdot n\sqrt{m}\right) = \tilde{O}\left(\frac{\sqrt{m}}{n}\right)$
\item $\norm{c_{\alpha_4}(M_{\alpha_4^+} - M_{\alpha_4^-})}$ is $\tilde{O}\left(\frac{1}{n} \cdot \sqrt{mn}\right) = \tilde{O}\left(\frac{\sqrt{m}}{\sqrt{n}}\right)$
\item $\norm{c_{\alpha_5}(M_{\alpha_5^+} - M_{\alpha_5^-})}$ is $\tilde{O}\left(\frac{1}{n} \cdot \sqrt{m}\right) = \tilde{O}\left(\frac{\sqrt{m}}{n}\right)$
\end{enumerate}
\subsubsection{Analyzing $N_k{N^T_k}$}
The dominant terms of $N_k$ are $2M_{\alpha^{+}} - 2M_{\alpha^{-}}$ where 
\begin{enumerate}
\item $U_{\alpha^{+}} \setminus V_{\alpha^{+}} = \{j_1,j_2\}$, $U_{\alpha^{+}} \cap V_{\alpha^{+}} = \{j_3,\ldots,j_{k}\} \cup \{i'_{circ}\}$, $V_{\alpha^{+}} \setminus U_{\alpha^{+}} = \{i_{circ}\}$, and $E(\alpha^{+}) = \{(j_1,i),(j_2,i)\}$. Note that here $i < i'$ and $(i_{circ},i'_{circ})$ appears as a tuple in $V_{\alpha^{+}}$.
\item $U_{\alpha^{-}} \setminus V_{\alpha^{-}} = \{j_1,j_2\}$, $U_{\alpha^{-}} \cap V_{\alpha^{-}} = \{j_3,\ldots,j_{k}\} \cup \{i_{circ}\}$, $V_{\alpha^{-}} \setminus U_{\alpha^{-}} = \{i'_{circ}\}$, and $E(\alpha^{-}) = \{(j_1,i'),(j_2,i')\}$. Note that here $i < i'$ and $(i'_{circ},i_{circ})$ appears as a tuple in $V_{\alpha^{-}}$.
\end{enumerate}
\begin{lemma}\label{NNTPluslemma}
$M_{\alpha^{+}}M_{\alpha^{+}}^T + M_{\alpha^{-}}M_{\alpha^{-}}^T = M_{\alpha_1} + M_{\alpha_2} + M_{\alpha_3}$ where $\alpha_1,\alpha_2,\alpha_3$ are the following shapes.
\begin{enumerate}
\item $U_{\alpha_1} \setminus V_{\alpha_1} = \emptyset$, $U_{\alpha_1} \cap V_{\alpha_1} = \{j_1,j_2,j_3,j_4,\ldots,j_{k}\} \cup \{i_{circ}\}$, $V_{\alpha_1} \setminus U_{\alpha_1} = \emptyset$, $V(\alpha_1) \setminus (U_{\alpha_1} \cup V_{\alpha_1}) = \{i'_{circ}\}$, and $E(\alpha_1) = \{(i',j_1),(i',j_1),(i',j_2),(i',j_2)\}$.
\item $U_{\alpha_2} \setminus V_{\alpha_2} = \{j_1\}$, $U_{\alpha_2} \cap V_{\alpha_2} = \{j_2,j_4,\ldots,j_{k}\} \cup \{i_{circ}\}$, $V_{\alpha_2} \setminus U_{\alpha_2} = \{j'_1\}$, $V(\alpha_2) \setminus (U_{\alpha_2} \cup V_{\alpha_2}) = \{i'_{circ}\}$, and $E(\alpha_2) = \{(i',j_1),(i',j'_1),(i',j_2),(i',j_2)\}$.
\item $U_{\alpha_3} \setminus V_{\alpha_3} = \{j_1,j_2\}$, $U_{\alpha_3} \cap V_{\alpha_3} = \{j_5,\ldots,j_{k}\} \cup \{i_{circ}\}$, $V_{\alpha_3} \setminus U_{\alpha_3} = \{j'_1,j'_2\}$, $V(\alpha_3) \setminus (U_{\alpha_3} \cup V_{\alpha_3}) = \{i'_{circ}\}$, and $E(\alpha_3) = \{(i',j_1),(i',j_2),(i',j'_1),(i',j'_2)\}$.
\end{enumerate}
Note that for these shapes, we do not assume that $i < i'$. Also note that $\alpha_1$ and $\alpha_2$ are improper shapes, though this does not matter for us.
\end{lemma}
\begin{remark}
Actually, we do not need to do this computation as we will just use that $M_{\alpha^{+}}M_{\alpha^{+}}^T + M_{\alpha^{-}}M_{\alpha^{-}}^T \succeq 0$, but we include it anyways to show the similarity with the decomposition of ${L_k^T}L_k$.
\end{remark}
For pictures of these shapes, see Figure \ref{NNTPlusfigure} below.
\begin{figure}[ht]\label{NNTPlusfigure}
\centerline{\includegraphics[height=6cm]{sherrington_kirkpatrick/NNTPlus}}
\caption{This figure shows the decomposition of $M_{\alpha^{+}}M_{\alpha^{+}}^T + M_{\alpha^{-}}M_{\alpha^{-}}^T$.}
\end{figure}
\begin{proof}[Proof of Lemma \ref{NNTPluslemma}]
We compute $M_{\alpha^{+}}M_{\alpha^{+}}^T + M_{\alpha^{-}}M_{\alpha^{-}}^T$ by considering the ribbons which appear in $M_{\alpha^{+}}M_{\alpha^{+}}^T + M_{\alpha^{-}}M_{\alpha^{-}}^T$. For these ribbons, we do not assume that $i < i'$.
\begin{enumerate}
\item Each ribbon $R$ with $A_R \setminus B_R = \emptyset$, $A_R \cap B_R = \{j_1,j_2,j_3,j_4,\ldots,j_{k}\} \cup \{i_{circ}\}$, $B_R \setminus A_R = \emptyset$, $V(R) \setminus (A_R \cup B_R) = \{i'_{circ}\}$, and $E(R) = \{(i',j_1),(i',j_1),(i',j_2),(i',j_2)\}$ appears in exactly one way as the composition of the ribbons $R_1$ and $R_2$ where 
\begin{enumerate}
\item $A_{R_1} \setminus B_{R_1} = \{i_{circ}\}$, $A_{R_1} \cap B_{R_1} = \{j_3,j_4,\ldots,j_{k}\}$, $B_{R_1} \setminus A_{R_1} = \{j_1,j_2\}$, and $E(R_1) = \{(i,j_1),(i,j_2)\}$.
\item $A_{R_2} \setminus B_{R_2} = \{j_1,j_2\}$, $A_{R_2} \cap B_{R_2} = \{j_3,j_4,\ldots,j_{k}\}$, $B_{R_2} \setminus A_{R_2} = \{i_{circ}\}$, and $E(R_2) = \{(i,j_1),(i,j_2)\}$.
\end{enumerate}
Whether $i < i'$ or $i' < i$ only affects whether this ribbon appears in $M_{\alpha^{+}}M_{\alpha^{+}}^T$ or $M_{\alpha^{-}}M_{\alpha^{-}}^T$.
\item Each ribbon $R$ with $A_R \setminus B_R = \{j_1\}$, $A_R \cap B_R = \{j_4,\ldots,j_{k}\} \cup \{i_{circ}\}$, $B_R \setminus A_R = \{j'_1\}$, $V(R) \setminus (A_R \cup B_R) = \{i'_{circ}\}$, and $E(R) = \{(i,j_1),(i,j'_1),(i,j_2),(i,j_2)\}$ appears in exactly one way as the composition of the ribbons $R_1$ and $R_2$ where 
\begin{enumerate}
\item $A_{R_1} \setminus B_{R_1} = \{i_{circ}\}$, $A_{R_1} \cap B_{R_1} = \{j_1,j_4,\ldots,j_{k}\}$, $B_{R_1} \setminus A_{R_1} = \{j'_1,j_2\}$, and $E(R_1) = \{(i,j'_1),(i,j_2)\}$.
\item $A_{R_2} \setminus B_{R_2} = \{j_1,j_2\}$, $A_{R_2} \cap B_{R_2} = \{j'_1,j_4,\ldots,j_{k}\}$, $B_{R_2} \setminus A_{R_2} = \{i_{circ}\}$, and $E(R_2) = \{(i,j_1),(i,j_2)\}$.
\end{enumerate}
Whether $i < i'$ or $i' < i$ only affects whether this ribbon appears in $M_{\alpha^{+}}M_{\alpha^{+}}^T$ or $M_{\alpha^{-}}M_{\alpha^{-}}^T$.
\item Each ribbon $R$ with $A_R \setminus B_R = \{j_1,j_2\}$, $A_R \cap B_R = \{j_5,\ldots,j_{k}\} \cup \{i_{circ}\}$, $B_R \setminus A_R = \{j'_1,j'_2\}$, $V(R) \setminus (A_R \cup B_R) = \{i'_{circ}\}$, and $E(R) = \{(i,j_1),(i,j'_1),(i,j_2),(i,j'_2)\}$ appears in exactly one way as the composition of the ribbons $R_1$ and $R_2$ where 
\begin{enumerate}
\item $A_{R_1} \setminus B_{R_1} = \{i_{circ}\}$, $A_{R_1} \cap B_{R_1} = \{j_1,j_2,j_5,\ldots,j_{k}\}$, $B_{R_1} \setminus A_{R_1} = \{j'_1,j'_2\}$, and $E(R_1) = \{(i,j'_1),(i,j'_2)\}$.
\item $A_{R_2} \setminus B_{R_2} = \{j_1,j_2\}$, $A_{R_2} \cap B_{R_2} = \{j'_1,j'_2,j_5,\ldots,j_{k}\}$, $B_{R_2} \setminus A_{R_2} = \{i_{circ}\}$, and $E(R_2) = \{(i,j_1),(i,j_2)\}$.
\end{enumerate}
Whether $i < i'$ or $i' < i$ only affects whether this ribbon appears in $M_{\alpha^{+}}M_{\alpha^{+}}^T$ or $M_{\alpha^{-}}M_{\alpha^{-}}^T$.
\end{enumerate}
\end{proof}
\begin{lemma}\label{NNTMinuslemma}
$M_{\alpha^{+}}M_{\alpha^{-}}^T + M_{\alpha^{-}}M_{\alpha^{+}}^T = M_{\alpha_4} + M_{\alpha_5} + M_{\alpha_6}$ where $\alpha_4,\alpha_5,\alpha_6$ are the following shapes.
\begin{enumerate}
\item $U_{\alpha_4} \setminus V_{\alpha_4} = \{i_{circ}\}$, $U_{\alpha_4} \cap V_{\alpha_4} = \{j_1,j_2,j_3,j_4,\ldots,j_{k}\}$, $V_{\alpha_4} \setminus U_{\alpha_4} = \{i'_{circ}\}$, and $E(\alpha_4) = \{(i,j_1),(i,j_2),$ $(i',j_1),(i',j_2)\}$.
\item $U_{\alpha_5} \setminus V_{\alpha_5} = \{j_1\} \cup \{i_{circ}\}$, $U_{\alpha_5} \cap V_{\alpha_5} = \{j_2,j_4,\ldots,j_{k}\}$, $V_{\alpha_5} \setminus U_{\alpha_5} = \{j'_1\} \cup \{i'_{circ}\}$, and $E(\alpha_5) = \{(i,j'_1),(i,j_2),(i',j_1),(i',j_2)\}$.
\item $U_{\alpha_6} \setminus V_{\alpha_6} = \{j_1,j_2\} \cup \{i_{circ}\}$, $U_{\alpha_6} \cap V_{\alpha_6} = \{j_5,\ldots,j_{k}\}$, $V_{\alpha_6} \setminus U_{\alpha_6} = \{j'_1,j'_2\}  \cup \{i'_{circ}\}$, and $E(\alpha_6) = \{(i',j_1),(i',j_2),(i,j'_1),(i,j'_2)\}$.
\end{enumerate}
\end{lemma}
For pictures of these shapes, see Figure \ref{NNTMinusfigure} below.
\begin{figure}[ht]\label{NNTMinusfigure}
\centerline{\includegraphics[height=6cm]{sherrington_kirkpatrick/NNTMinus}}
\caption{This figure shows the decomposition of $M_{\alpha^{+}}M_{\alpha^{+}}^T + M_{\alpha^{-}}M_{\alpha^{-}}^T$.}
\end{figure}
\begin{proof}[Proof of Lemma \ref{NNTMinuslemma}]
We compute $M_{\alpha^{+}}M_{\alpha^{-}}^T + M_{\alpha^{-}}M_{\alpha^{+}}^T$ by considering the ribbons which appear in $M_{\alpha^{+}}M_{\alpha^{-}}^T + M_{\alpha^{-}}M_{\alpha^{+}}^T$. For these ribbons, we do not assume that $i < i'$.
\begin{enumerate}
\item Each ribbon $R$ with $A_R \setminus B_R = \{i_{circ}\}$, $A_R \cap B_R = \{j_1,j_2,j_3,j_4,\ldots,j_{k}\}$, $B_R \setminus A_R = \{i'_{circ}\}$, $V(R) \setminus (A_R \cup B_R) = \emptyset$, and $E(R) = \{(i,j_1),(i,j_2),(i',j_1),(i',j_2)\}$ appears in exactly one way as the composition of the ribbons $R_1$ and $R_2$ where 
\begin{enumerate}
\item $A_{R_1} \setminus B_{R_1} = \{j_1,j_2\}$, $A_{R_1} \cap B_{R_1} = \{j_3,j_4,\ldots,j_{k}\} \cup \{i_{circ}\}$, $B_{R_1} \setminus A_{R_1} = \{i'_{circ}\}$, and $E(R_1) = \{(i',j_1),(i',j_2)\}$.
\item $A_{R_2} \setminus B_{R_2} =  \{i_{circ}\}$, $A_{R_2} \cap B_{R_2} = \{j_3,j_4,\ldots,j_{k}\} \cup \{i'_{circ}\}$, $B_{R_2} \setminus A_{R_2} = \{j_1,j_2\}$, and $E(R_2) = \{(i,j_1),(i,j_2)\}$.
\end{enumerate}
Whether $i < i'$ or $i' < i$ only affects whether this ribbon appears in $M_{\alpha^{+}}M_{\alpha^{-}}^T$ or $M_{\alpha^{-}}M_{\alpha^{+}}^T$.
\item Each ribbon $R$ with $A_R \setminus B_R = \{j_1\} \cup \{i_{circ}\}$, $A_R \cap B_R = \{j_2,j_4,\ldots,j_{k}\}$, $B_R \setminus A_R = \{j'_1\} \cup \{i'_{circ}\}$, $V(R) \setminus (A_R \cup B_R) = \emptyset$, and $E(R) = \{(i,j_1),(i,j_2),(i',j'_1),(i',j_2)\}$ appears in exactly one way as the composition of the ribbons $R_1$ and $R_2$ where 
\begin{enumerate}
\item $A_{R_1} \setminus B_{R_1} = \{j_1,j_2\}$, $A_{R_1} \cap B_{R_1} = \{j'_1,j_4,\ldots,j_{k}\} \cup \{i_{circ}\}$, $B_{R_1} \setminus A_{R_1} = \{i'_{circ}\}$, and $E(R_1) = \{(i',j_1),(i',j_2)\}$.
\item $A_{R_2} \setminus B_{R_2} =  \{i_{circ}\}$, $A_{R_2} \cap B_{R_2} = \{j_1,j_4,\ldots,j_{k}\} \cup \{i'_{circ}\}$, $B_{R_2} \setminus A_{R_2} = \{j'_1,j_2\}$, and $E(R_2) = \{(i,j'_1),(i,j_2)\}$.
\end{enumerate}
Whether $i < i'$ or $i' < i$ only affects whether this ribbon appears in $M_{\alpha^{+}}M_{\alpha^{-}}^T$ or $M_{\alpha^{-}}M_{\alpha^{+}}^T$.
\item Each ribbon $R$ with $A_R \setminus B_R = \{j_1,j_2\} \cup  \{i_{circ}\}$, $A_R \cap B_R = \{j_5,\ldots,j_{k}\}$, $B_R \setminus A_R = \{j'_1,j'_2\}  \cup  \{i'_{circ}\}$, $V(R) \setminus (A_R \cup B_R) = \emptyset$, and $E(R) = \{(i,j'_1),(i,j'_2),(i',j_1),(i',j_2)\}$ appears in exactly one way as the composition of the ribbons $R_1$ and $R_2$ where 
\begin{enumerate}
\item $A_{R_1} \setminus B_{R_1} = \{j_1,j_2\}$, $A_{R_1} \cap B_{R_1} = \{j_1,j_2,j_5,\ldots,j_{k}\} \cup \{i_{circ}\}$, $B_{R_1} \setminus A_{R_1} = \{i'_{circ}\}$, and $E(R_1) = \{(i,j'_1),(i,j'_2)\}$.
\item $A_{R_2} \setminus B_{R_2} = \{i_{circ}\}$, $A_{R_2} \cap B_{R_2} = \{j'_1,j'_2,j_5,\ldots,j_{k}\}  \cup \{i'_{circ}\}$, $B_{R_2} \setminus A_{R_2} = \{j'_1,j'_2\}$, and $E(R_2) = \{(i,j_1),(i,j_2)\}$.
\end{enumerate}
Whether $i < i'$ or $i' < i$ only affects whether this ribbon appears in $M_{\alpha^{+}}M_{\alpha^{-}}^T$ or $M_{\alpha^{-}}M_{\alpha^{+}}^T$.
\end{enumerate}
\end{proof}
We now consider the norm bounds for these terms
\begin{enumerate}
\item $\norm{M_{\alpha_4}}$ is $\tilde{O}(m)$.
\item $\norm{M_{\alpha_5}}$ is $\tilde{O}(m)$.
\item $\norm{M_{\alpha_6}}$ is $\tilde{O}(n^2)$.
\end{enumerate}
This means that $M_{\alpha_6}$ cannot be ignored, but this is fine. In fact, the $M_{\alpha_6}$ here will cancel with the $M_{\alpha_6}$ that appears in the decomposition of ${L_k^T}L_k$
\begin{corollary}\label{NNTapproximationcorollary}
For all $k \geq 4$, $\norm{{N_k}{N_k}^T - 4M_{\alpha^{+}}M_{\alpha^{+}}^T - 4M_{\alpha^{-}}M_{\alpha^{-}}^T + 4M_{\alpha_6}}$ is $\tilde{O}(m)$.
\end{corollary}
\subsubsection{Putting Everything Together}
We now put everything together to prove that for all $k$, the minimum nonzero eigenvalue of ${L_k^T}{L_k}$ is $2n^2 - \tilde{O}(n\sqrt{m})$.
\begin{enumerate}
\item For $k = 2$, by Corollary \ref{QQTapproximationcorollary}, $\norm{{L_k^T}L_k - 2{n^2}M_{Id_{k-2,1}}}$ is $\tilde{O}(n\sqrt{m})$ so the minimum eigenvalue of ${L_k^T}{L_k}$ is $2n^2 - \tilde{O}(n\sqrt{m})$.
\item For $k = 3$, by Corollary \ref{QQTapproximationcorollary}, $\norm{{L_k^T}L_k - 2{n^2}M_{Id_{k-2,1}} - 4nM_{\beta_2}M^T_{\beta_2}}$ is $\tilde{O}(n\sqrt{m})$ so the minimum eigenvalue of ${L_k^T}{L_k}$ is $2n^2 - \tilde{O}(n\sqrt{m})$.
\item For $k \geq 4$, by Corollary \ref{QQTapproximationcorollary}, $\norm{{L_k^T}L_k - 2{n^2}M_{Id_{k-2,1}} - 4nM_{\beta_2}M^T_{\beta_2} - 4M_{\beta_3}M^T_{\beta_3} - 4M_{\alpha_6}}$ is $\tilde{O}(n\sqrt{m})$. By Corollary \ref{NNTapproximationcorollary}, $\norm{{N_k}{N_k}^T - 4M_{\alpha^{+}}M_{\alpha^{+}}^T - 4M_{\alpha^{-}}M_{\alpha^{-}}^T + 4M_{\alpha_6}}$ is $\tilde{O}(m)$. Combining these equations, 
\[
\norm{{L_k^T}L_k + {N_k}{N_k}^T - 2{n^2}M_{Id_{k-2,1}} - 4nM_{\beta_2}M^T_{\beta_2} - 4M_{\beta_3}M^T_{\beta_3} - 4M_{\alpha^{+}}M_{\alpha^{+}}^T - 4M_{\alpha^{-}}M_{\alpha^{-}}^T}
\] is $\tilde{O}(n\sqrt{m})$ so the minimum eigenvalue of ${L_k^T}L_k + {N_k}{N_k}^T$ is $2n^2 - \tilde{O}(n\sqrt{m})$. Since the minimum nonzero eigenvalue of ${L_k^T}L_k$ is at least as large as the minimum eigenvalue of ${L_k^T}L_k + {N_k}{N_k}^T$, the nonzero eigenvalue of ${L_k^T}{L_k}$ is $2n^2 - \tilde{O}(n\sqrt{m})$.
\end{enumerate}
This implies that the minimum nonzero eigenvaue of $QQ^T$ is $2n^2 - \tilde{O}(n\sqrt{m})$, as needed.


==> sherrington_kirkpatrick/intro.tex <==

The Sum-of-Squares (SoS) hierarchy is a semi-definite programming
(SDP) hierarchy which provides a meta-algorithm for polynomial
optimization~\cite{Lasserre15}. Given a polynomial objective function
and a system of polynomial equalities and inequalities as constraints,
the SoS framework specifies a family of increasingly ``larger'' SDP
programs, where each program provides a convex relaxation to the
polynomial optimization problem. The family is indexed by a size
parameter $D$ called the SoS degree. Roughly speaking, the larger the
SoS degree $D$, the tighter the relaxation, but also, the greater the
computational time required to solve the convex program, with $D=O(1)$
corresponding to polynomial time and $D = n$ able to exactly solve an
optimization problem on $n$ boolean variables. Due to the versatility
of polynomials in modeling computational problems, the SoS hierarchy
can be applied to a vast range of optimization problems. It has been
shown to be quite successful in this regard, as it captures
state-of-the-art approximation guarantees for many problems such as
Sparsest Cut~\cite{AroraRV04}, MaxCut~\cite{GW94}, Tensor
PCA~\cite{HopSS15} and all Max-$k$-CSPs~\cite{Raghavendra08}.

The success of SoS for optimization confers on it an important role as
an algorithmic tool. For this reason, on the flip side, understanding
the degree range for which SoS \textit{fails} to provide a desired
guarantee to a computational problem can be useful to the algorithm
designer in two ways. Firstly and more concretely, since SoS is a
proof system capturing a broad class of algorithmic
reasoning~\cite{FKP19}, an SoS lower bound can inform the algorithm
designer not only of the minimum degree required within the SoS
hierarchy, but also to avoid methods of proof that are captured by
low-degree SoS reasoning. Secondly, an SoS lower bound can serve as
strong evidence for computational hardness~\cite{hop17,hop18}, even
though it is not a formal guarantee against all types of
algorithms. This hardness evidence is particularly relevant to
average-case problems for which we do not have NP-hardness (see, e.g.,
the SoS lower bound on the Planted Clique problem~\cite{BHKKMP16}).

Our main results concern the performance of SoS on the following basic optimization problem
\begin{equation}\label{eq:general_opt}
  \OPT(W) \defeq \max_{x \in \{\pm 1\}^n} x^\T W x,
\end{equation}
where $W$ is a symmetric matrix in $\RR^{n\times n}$. This problem
arises in the fields of computer science and statistical physics,
though the terminology can sometimes differ. Computer scientists might
regard $x \in \{\pm 1\}^n$ as encoding a bipartition of $[n] = \{1,
2, \ldots, n\}$. Note that by taking $W$ to be a graph
Laplacian~\cite[Section 4]{HooryLW06} the problem is equivalent to the
MaxCut problem, a well-known NP-hard problem in the worst
case~\cite{K72}. A statistical physicist might regard $x$ as encoding
spin values in a spin-glass model. The matrix $-W$ is regarded as
the \textit{Hamiltonian} of the underlying physical system, where
entry $-W_{i,j}$ models the interaction between spin $x_i$ and $x_j$
(with $-W_{i,j} \ge 0$ being ferromagnetic and $-W_{i,j} < 0$ being
anti-ferromagnetic). Then, the optimized $x$ corresponds to the
minimum-energy, or ground, state of the system.

Instead of considering $\OPT(W)$ for a worst-case $W$, one can consider the
average-case problem in which $W$ is sampled according to some
distribution. One of the simplest models of random matrices is the
Gaussian Orthogonal Ensemble, denoted $\GOE(n)$ for $n$-by-$n$
matrices and defined as follows.
\begin{definition}
  The Gaussian Orthogonal Ensemble, denoted $\GOE(n)$, is the distribution of $\frac{1}{\sqrt{2}}(A + A^\T)$
  where $A$ is a random $n\times n$ matrix with i.i.d. standard Gaussian entries.
\end{definition}
Taking $W \sim \GOE(n)$ for the optimization problem $\OPT(W)$
of~\cref{eq:general_opt} gives rise to the so-called
Sherrington--Kirkpatrick (SK) Hamiltonian~\cite{SK76}. Note that $\GOE(n)$ is a particular kind
of Wigner matrix ensemble, thereby satisfying the semicircle law, which
in this case establishes that the largest eigenvalue of $W$ is
$(2+\littleoh_n(1)) \cdot \sqrt{n}$ with probability
$1-\littleoh_n(1)$. Thus, a trivial spectral bound establishes
$\OPT(W) \le (2+\littleoh_n(1)) \cdot n^{3/2}$ with probability
$1-\littleoh_n(1)$. However, in a foundational work based on a
variational argument~\cite{P79}, Parisi conjectured that
$$
\E_{W \sim \GOE(n)}\left[ \OPT(W) \right] \approx 2 \cdot P^* \cdot n^{3/2},
$$
where $P^* \approx 0.7632$ is now referred to as the Parisi constant.
In a breakthrough result, Talagrand~\cite{Tal06} gave a rigorous proof
of Parisi's conjecture\footnote{The results of Talagrand~\cite{Tal06}
were for the Sherrington--Kirkpatrick and mixed $p$-spin systems with
$p$ even. In~\cite{Panchenko2014}, Panchenko generalized these results
to arbitrary mixed $p$-spin systems (also including odd $p$).}. The
question then became, ``is there a polynomial-time algorithm that
given $W \sim \GOE(n)$ computes an $x$ achieving close to $\OPT(W)$?"
As it turns out, the answer was essentially shown to be yes by
Montanari~\cite{Montanari19}!

The natural question we study is that of certification: ``is there an
efficient algorithm to certify an upper bound on $\OPT(W)$ for any
input $W$, that improves upon the trivial spectral bound?" In
particular, we can ask how well SoS does as a certification
algorithm. The natural upper bound of $(2+\littleoh_n(1)) \cdot
n^{3/2}$ obtained via the spectral norm of $W$ is also the value of
the degree-$2$ SoS relaxation~\cite{MS16}. Two independent recent
works of Mohanty--Raghavendra--Xu~\cite{MRX20} and
Kunisky--Bandeira~\cite{KuniskyBandeira19} show that degree-4 SoS does
not perform much better, and a heuristic argument from~\cite{bkw19} suggests that even degree-$(n/\log n)$ SoS cannot certify anything stronger than the trivial spectral bound. Thus we ask,

\begin{center}
  \emph{Can higher-degree SoS certify better upper bounds for the Sherrington--Kirkpatrick problem, \\
        hopefully closer to the true bound $2 \cdot P^* \cdot n^{3/2}$?}
\end{center}

\noindent \textbf{Our Results.} \enspace We answer the question above negatively by showing that even at degree as large as
$n^\delta$, SoS cannot improve upon the basic spectral
algorithm. More precisely, we have the following theorem which is our
first main result and our most important contribution.

\begin{restatable}{theorem}{SKbounds}[Main I]\label{theo:sk-bounds}
  There exists a constant $\delta > 0$ such that, w.h.p. for $W \sim \GOE(n)$, there is a degree-$n^\delta$ SoS solution
  for the Sherrington--Kirkpatrick problem with value at least $(2-\littleoh_n(1)) \cdot n^{3/2}$.
\end{restatable}

In light of the result of Montanari~\cite{Montanari19}, the situation
is intriguing. Montanari showed that for all $\eps > 0$, there is a
$\bigoh_\eps(n^2)$ time randomized algorithm that given a random $W$
drawn from the Gaussian Orthogonal Ensemble, outputs an $x$ such that
${x^T}Wx \geq (1-\eps)\OPT(W)$.  The correctness of the algorithm
assumes a widely-believed conjecture from statistical physics known as
the full replica symmetry breaking assumption. However, we show an
integrality gap for SoS.

Based on this, it is an interesting question whether SoS, together
with an appropriate rounding scheme, is optimal for the
Sherrington-Kirkpatrick problem. On the one hand, the situation could
be similar to the Feige-Schechtman integrality gap instance for
MaxCut~\cite{fs02}. For the Feige-Schechtman integrality gap instance,
SoS fails to certify the value of the optimal solution. However,
applying hyperplane rounding to the SoS solution gives an
almost-optimal solution for these instances. It could be the case that
there is a rounding scheme which takes an SoS solution for the
Sherrington-Kirkpatrick problem on a random $W$ and returns an almost
optimal solution $x$. On the other hand, we currently don't know what
this rounding scheme would be.


In order to prove~\cref{theo:sk-bounds}, we first introduce a new
average-case problem we call Planted Affine Planes (PAP) for which we directly prove a SoS lower bound. We then use
the PAP lower bound to prove a lower bound on the
Sherrington--Kirkpatrick problem. The PAP problem can be informally
described as follows (see~\cref{def:prob:pap} for the formal definition).
\begin{definition}[Informal statement of PAP]
  Given $m$ random vectors $d_1,\ldots,d_m$ in $\mathbb{R}^n$, can we
  prove that there is no vector $v \in \RR^n$ such that for all
  $u \in [m]$, $\langle v, d_u\rangle^2 = 1$? In other words, can we
  prove that $m$ random vectors are not all contained in two parallel
  hyperplanes at equal distance from the origin?
\end{definition}
This problem, when we restrict $v$ to a Boolean vector in $\set{\pm \frac{1}{\sqrt{n}}}^n$,
can be encoded as the feasibility of the polynomial system
\begin{align*}
\exists v \in \R^n~\text{s.t.} \qquad & \forall i \in [n], \; v_i^2 = \frac{1}{n},\\
& \forall u \in [m], \; \ip{v}{d_u}^2 = 1.
\end{align*}
Hence it is a ripe candidate for SoS. However, we show that SoS fails
to refute a random instance. The Boolean restriction on $v$ actually
makes the lower bound result stronger since SoS cannot refute even a
smaller subset of vectors in $\RR^n$. In this work, we will consider two
different random distributions, namely when $d_1, \ldots, d_m$ are
independent samples from the multivariate normal distribution and when
they are independent samples from the uniform distribution on the
boolean hypercube.
\begin{theorem}[Main II]\label{theo:sos-bounds}
  For both the Gaussian and Boolean settings, there exists a constant $c > 0$ such that for all $\eps > 0$ and $\delta \le c\eps$, for $m \leq n^{3/2 - \eps}$, w.h.p. there is a feasible degree-$n^\delta$ SoS solution for Planted Affine Planes.
\end{theorem}

It turns out that the Planted Affine Plane problem introduced above is
closely related to the following ``Boolean vector in a random
subspace'' problem, which we call the Planted Boolean Vector problem,
introduced by~\cite{MRX20} in the context of studying the performance
of SoS on computing the Sherrington--Kirkpatrick Hamiltonian.

The Planted Boolean Vector problem is to certify that a random subspace of $\R^n$ is far from containing a boolean vector.
Specifically, we want to certify an upper bound for
\[
\OPT(V) \defeq  \frac{1}{n}\max_{b \in \{\pm 1\}^n} b^\T \Pi_V b,
\]
where $V$ is a uniformly random $p$-dimensional subspace\footnote{$V$
can be specified by a basis, which consists of $p$ i.i.d.  samples
from $\calN(0, I)$.} of $\RR^n$, and $\Pi_V$ is the projector onto
$V$. In brief, the relationship to the Planted Affine Plane problem is
that the PAP vector $v$ represents the coefficients on a linear 
combination for the vector $b$ in the span of a basis of 
$V$.

An argument of~\cite{MRX20} shows that, when $p \ll n$, w.h.p.,
$\OPT(V) \approx \frac{2}{\pi}$, whereas they also show that
w.h.p. assuming $p \geq n^{0.99}$, there is a degree-4 SoS solution
with value $1-\littleoh_n(1)$. They ask whether or not there is a
polynomial time algorithm that can certify a tighter bound; we rule
out SoS-based algorithms for a larger regime both in terms of SoS
degree and the dimension $p$ of the random subspace.

\begin{restatable}{theorem}{booleanSubspace}[Main III]\label{theo:boolean-subspace}
	There exists a constant $c > 0$ such that, for all $\eps > 0$ and $\delta \le c\eps$, for $p \geq n^{2/3 + \eps}$, w.h.p. over $V$ there is a
  degree-$n^\delta$ SoS solution for Planted Boolean Vector of value $1$.
\end{restatable}

\noindent \textbf{Our Approach.} \enspace We now provide a brief
high-level description of our approach (see~\cref{sec:strategy} for a
more detailed overview). The bulk of our technical contribution lies
in the SoS lower bound for the Planted Affine Planes
problem,~\cref{theo:sos-bounds}. We then show that Planted Affine
Planes in the Gaussian setting is equivalent to the Planted Boolean
Vector problem. The reduction from Sherrington-Kirkpatrick to the
Planted Boolean Vector problem is due to
Mohanty--Raghavendra--Xu~\cite{MRX20}.

As a starting point to the PAP lower bound, we employ the general
techniques introduced by Barak et al.~\cite{BHKKMP16} for SoS lower
bounds. We use their pseudocalibration machinery to produce a good
candidate SoS solution $\pE$. The operator $\pE$ unfortunately does
not exactly satisfy the PAP constraints ``$\ip{v}{d_u}^2 = 1$'', it
only satisfies them up to a tiny error. We use an interesting and
rather generic approach to round $\pE$ to a nearby pseudoexpectation
operator $\pE'$ which does exactly satisfy the constraints.

For degree $D$, the candidate SoS solution can be viewed as a
(pseudo) moment matrix $\calM$ with rows and columns indexed by
subsets $I,J\subset [n]$ with size bounded by $D/2$ and with entries
\[\calM[I,J] \defeq \pE[v^{I} v^{J}].\]
The matrix $\calM$ is a random function of the inputs $d_1, \dots, d_m$, and the most challenging part of the 
analysis consists of showing that $\calM$ is positive
semi-definite (PSD) with high probability.

Similarly to~\cite{BHKKMP16}, we decompose
$\calM$ as a linear combination of graph matrices, i.e., $\calM~=~\sum_{\alpha}~\lambda_{\alpha}~\cdot~M_{\alpha}$, where $M_{\alpha}$
is the graph matrix associated with shape $\alpha$. In brief, each
graph matrix aggregates all terms with shape $\alpha$  in the Fourier expansions of the entries of $\calM$ -- the shape $\alpha$ is informally a graph with labeled edges
with size bounded by $\poly(D)$. A graph
matrix decomposition of $\calM$ is particularly handy in the PSD
analysis since the operator norm of individual graph matrices $M_{\alpha}$ is (with high probability)
determined by simple combinatorial properties of the graph
$\alpha$. One technical difference from~\cite{BHKKMP16} is that our
graph matrices have two types of vertices $\square{}$ and $\circle{}$; these graph matrices fall into the general framework developed by Ahn et al. in~\cite{AMP20}.

To show that the matrix $\calM$ is PSD, we need to study the graph matrices that appear with nonzero coefficients in the decomposition. The matrix $\calM$ can be split into blocks and each diagonal block contains in the decomposition a (scaled) identity matrix. From the graph matrix perspective, this means that certain ``trivial'' shapes appear in the decomposition, with appropriate coefficients. If we could bound the norms of all other graph matrices that appear against these trivial shapes and show that, together, they have negligible norm compared to the sum of these scaled identity blocks, then we would be in good shape.

Unfortunately, this approach will not work. The kernel of the matrix $\calM$ is nontrivial, as a consequence of satisfying the PAP constraints ``$\ip{v}{d_u}^2 = 1$", and hence there is no hope of showing that the contribution of all nontrivial shapes in the decomposition of $\calM$ has small norm. Indeed, certain shapes $\alpha$ appearing in the 
decomposition of $\calM$ are such that $\norm{\lambda_{\alpha} \cdot M_{\alpha}}$ is large. As it turns out, all such shapes have a simple graphical substructure, and so we call these shapes \textit{spiders}. 

To get around the null space issue, we restrict ourselves to $\nullspace(\calM)^\perp$, which is the complement of the nullspace of $\calM$. 
We show that the substructure present in a spider implies that the spider is close to the zero matrix in $\nullspace(\calM)^\perp$. Because of this, we can almost freely 
add and subtract $M_\alpha$ for spiders $\alpha$ while preserving the action of $\calM$ on $\nullspace(\calM)^\perp$. Our strategy is to ``kill'' the spiders 
by subtracting off $\lambda_\alpha \cdot M_\alpha$ for each spider $\alpha$. But because $M_{\alpha}$ is only approximately in $\nullspace(\calM)^\perp$, this 
strategy could potentially introduce new graph matrix terms, and in particular it could introduce new spiders. To handle this, 
we recursively kill them while carefully analyzing how the coefficients of all the graph matrices change. After all spiders
are killed, the resulting moment matrix becomes
$$
\sum_{0 \le k \le D/2} \frac{1}{n^{k}} \cdot I_k + \sum_{\gamma \colon \textup{non-spiders}} \lambda_{\gamma}' \cdot M_{\gamma},
$$
for some new coefficients $\lambda_{\gamma}'$. Here, $I_k$ is the
matrix which has an identity in the $k$th block and the remaining
entries $0$. Using a novel charging argument, we finally show that the
latter term is negligible compared to the former term, thus
establishing $\calM \succeq 0$.

\noindent \textbf{Summary of Related Work and Our Contributions.} \enspace
We now summarize the existing work on these problems and our
contributions.  Degree-$4$ SoS lower bounds on the
Sherrington-Kirkpatrick Hamiltonian problem were proved independently
by Mohanty--Raghavendra--Xu~\cite{MRX20} and
Kunisky--Bandeira~\cite{KuniskyBandeira19} whereas we prove an
improved degree-$n^{\delta}$ SoS lower bound for some constant $\delta
> 0$.  Our result is obtained by reducing the Sherrington-Kirkpatrick
problem to the ``Boolean Vector in a Random Subspace'' problem which
is equivalent to our new Planted Affine Planes problem on the normal
distribution. The reduction from Sherrington-Kirkpatrick problem to
the ``Boolean Vector in a Random Subspace'' is due to
Mohanty--Raghavendra--Xu~\cite{MRX20}. The results of
Mohanty--Raghavendra--Xu~\cite{MRX20} and
Kunisky--Bandeira~\cite{KuniskyBandeira19} build on a degree-$2$ SoS
lower bounds of Montanari and Sen~\cite{MS16}. Regarding upper bounds,
Montanari~\cite{Montanari19} gave an efficient randomized message
passing algorithm to estimate $\OPT(W)$ in the SK problem within a
$(1-\eps)$ factor under the full replica symmetry breaking assumption.

Degree-$4$ SoS lower bounds on the ``Boolean Vector in a Random
Subspace'' problem for $p~\ge~n^{0.99}$ were proved by
Mohanty--Raghavendra--Xu in~\cite{MRX20} where this problem was
introduced. We improve the dependence on $p$ to $p \ge n^{2/3
+ \epsilon}$ for any $\epsilon > 0$ and obtain a stronger
degree-$n^{c\eps}$ SoS lower bound for some absolute constant $c > 0$.



==> sherrington_kirkpatrick/open_problems.tex <==

\section{Open Problems}\label{sec:open-problems}

We conjecture that for the Planted Affine Planes problem, the problem remains difficult even with the number of vectors increased to $m = n^{2 - \epsilon}$.

\begin{conjecture}
	\cref{theo:sos-bounds} holds with the bound on the number of sampled vectors $m$ loosened to $m \leq n^{2-\eps}$.
\end{conjecture}

The reason for the upper bound comes from \cref{rmk:pe-one}. Analyzing $\pE[1]$ is an established way to hypothesize about the power of SoS in hypothesis testing problems (see \cite{hop17}, \cite{hop18}).

Dual to the Planted Affine Planes problem, we conjecture a similar
bound for Planted Boolean Vector problem whenever $d \geq
n^{1/2+\eps}$.

\begin{conjecture}
	\cref{theo:boolean-subspace} holds with the bound on the dimension $p$ of a random subspace
  loosened to $p \geq n^{1/2+\eps}$.
\end{conjecture}

We conjecture that the Planted Boolean Vector problem/Planted Affine
Planes problem is still hard for SoS if the input is no longer i.i.d.
Gaussian or boolean entries, but is drawn from a ``random enough''
distribution. For example, if in the random instance of PAP the vectors
$d_u$ are i.i.d. samples from $S^n$, or a random orthonormal system,
degree $n^\delta$ SoS should still believe the instance is satisfiable
(after appropriate normalization of $v$). Or, taking the view of Planted
Boolean Vector, if the subspace is the eigenspace of the bottom
eigenvectors of a random adjacency matrix, the instance should still be
difficult. This last setting arises in Maximum Cut, for which we conjecture the following.

\begin{conjecture}
    Let $d \geq 3$, and let $G$ be a random $d$-regular graph on $n$ vertices. For some $\delta > 0$, w.h.p. there is a degree-$n^\delta$ pseudoexpectation operator $\pE$ on boolean variables $x_i$ with maximum cut value at least
    \[ \frac{1}{2} + \frac{\sqrt{d-1}}{d}(1 - \littleoh_{d,n}(1)) \]
\end{conjecture}

The above expression is w.h.p. the value of the spectral relaxation for Maximum Cut, therefore qualitatively this conjecture expresses that degree $n^\delta$ SoS cannot significantly tighten the basic spectral relaxation.

We should remark that, with respect to the goal of showing SoS cannot significantly outperform the Goemans-Williamson relaxation, random instances are not integrality gap instances. The main difficulty in comparing (even degree 4) SoS to the Goemans-Williamson algorithm seems to be the lack of a candidate hard input distribution.

Evidence for this conjecture comes from the fact that the only property
required of the random inputs $d_1, \dots, d_m$ was that norm bounds hold for
the graph matrix with Hermite polynomial entries. When the variables
$\{d_{u,i}\}$ are i.i.d from some other distribution, if we use graph matrices
for the orthonormal polynomials under the distribution and assuming suitable
bounds on the moments of the distribution, the same norm bounds
hold~\cite{AMP20}.
When $d_u \unif S^n$ or another distribution for which the coordinates are not
i.i.d, it seems likely that if we use e.g. the spherical harmonics then
similar norm bounds hold, but this is not proven.




==> sherrington_kirkpatrick/preamble.tex <==

%%%%% FLAG FOR CONFERENCE VERSION %%%%%
\def\confversion{0}
\def\ifconf{\ifnum\confversion=1}
\def\ifnotconf{\ifnum\confversion=0}

%\documentclass[11 pt]{article}

%\input{macros}
\let\pref=\prettyref

\usepackage{tikz}
\usetikzlibrary{shapes.geometric}
\usepackage{float}

\usepackage{thm-restate}

%%%%%%% Additional macros for this paper

\newcommand{\unif}{\in_{\text{R}}}
\newcommand{\T}{\intercal}
\let\mod\relax
\DeclareMathOperator{\mod}{mod}
\DeclareMathOperator{\GOE}{GOE}
\DeclareMathOperator{\linspan}{span}
\DeclareMathOperator{\nullspace}{Null}
\DeclareMathOperator{\parents}{parents}
\renewcommand{\E}{\mathop{\mathbb{E}}}
\DeclareMathOperator{\body}{body}

%\renewcommand{\circle}{\raisebox{-0.35mm}{\scalebox{1.4}{$\circ$}}}
\renewcommand*{\circle}[1]{\scalebox{0.85}{\footnotesize
		\tikz[baseline=(char.base)]{
			\node[shape=circle,draw,inner sep=1.5pt](char) {   \ifx&#1&
				\color{white} $i$
				\else
				$#1$
				\fi};
}}}
\renewcommand*{\square}[1]{\scalebox{0.85}{\footnotesize
		\tikz[baseline=(char.base), square/.style={regular polygon,regular polygon sides=4}]{
			\node[draw,square, inner sep=0.5pt](char) {
				\ifx&#1&
				\color{white} $t$
				\else
				$#1$
				\fi};
}}}
% \renewcommand*{\square}[1]{\scalebox{0.8}{\footnotesize
%     \tikz[baseline=(char.base), square/.style={regular polygon,regular polygon sides=4}]{
%         \node[draw,square, inner sep=0.5pt](char) {
%         \resizebox{\minof{\widthof{\ifx&#1&
%         \color{white} $t$
%         \else
%         $#1$
%         \fi}}{10pt}}{!}{\ifx&#1&
%         \color{white} $t$
%         \else
%         $#1$
%         \fi}};
%     }}}

%%%%%%%%%%%%%% No bullets
\renewcommand{\labelitemi}{-}


%% \usepackage{fullpage}
%% \usepackage{color,xcolor}

%% % math packages
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{ytableau}
\usepackage{mathtools}
\usepackage{blkarray}

%\newcommand{\anote}[1]{\textcolor{yellow}{ {\textbf{(Aaron: #1)}}}}
%\newcommand{\cnote}[1]{\textcolor{green}{ {\textbf{(Chris: #1)}}}}
%\newcommand{\fnote}[1]{\textcolor{blue}{ {\textbf{(Fernando: #1)}}}}
%\newcommand{\gnote}[1]{\textcolor{magenta}{ {\textbf{(Goutham: #1)}}}}
%\newcommand{\mnote}[1]{\textcolor{lime}{ {\textbf{(Mrinal: #1)}}}}
%\newcommand{\tnote}[1]{\textcolor{orange}{ {\textbf{(Tulsiani: #1)}}}}
%
%\newcommand{\frnote}[1]{\textcolor{red}{ {\textbf{(Fernando: #1)}}}}

==> sherrington_kirkpatrick/prelim.tex <==
In this section we record problem statements, then define and discuss the main objects in our SoS
lower bound: pseudoexpectation operators, the moment matrix, and graph matrices.

For a vector or variable
$v \in \R^n$, and $I \subseteq [n]$, we use the notation
$v^I \defeq \prod_{i \in I}v_i$. When a statement holds with high
probability (w.h.p.), it means it holds with probability $1 - o_n(1)$. In
particular, there is no requirement for small $n$.

\subsection{Problem statements}

We introduce the Planted Affine Planes problem over a distribution $\calD$.
\begin{definition}[Planted Affine Planes (PAP) problem]\label{def:prob:pap}
  Given $d_1, \dots, d_m \sim \calD$ where each $d_u$ is a vector in $\RR^n$,
  determine whether there exists $v \in \set{\pm \frac{1}{\sqrt{n}}}^n$ such that
  \[
  \ip{v}{d_u}^2 = 1,
  \]
  for every $u \in [m]$.
\end{definition}
Our results hold for the Gaussian setting $\mathcal{D} = \calN(0, I)$ and the boolean setting where $\calD$ is uniformly sampled from $\{\pm 1\}^n$, though we conjecture (\cref{sec:open-problems}) that similar SoS bounds hold under more general conditions on $\calD$.

Observe that in both settings the solution vector $v$ is restricted to be Boolean (in the sense that the entries are either $\frac{1}{\sqrt{n}}$ or $\frac{-1}{\sqrt{n}}$) and an SoS lower bound for this restricted version of the problem is
stronger than when $v$ can be an arbitrary vector from $\RR^n$.

The Sherrington--Kirkpatrick (SK) problem comes from the spin-glass model
in statistical physics~\cite{SK76}.

\begin{definition}[Sherrington-Kirkpatrick problem]\label{def:prob:sk}
  Given $W \sim \GOE(n)$, compute
  \[
    \OPT(W) \defeq \max_{x \in \{\pm 1\}^n} x^\T W x.
  \]
\end{definition}

The Planted Boolean Vector problem was introduced by
Mohanty--Raghavendra--Xu~\cite{MRX20}, where it was called the
``Boolean Vector in a Random Subspace''.

\begin{definition}[Planted Boolean Vector problem]\label{def:prob:pbv}
  Given a uniformly random $p$-dimensional subspace $V$ of $\mathbb{R}^n$ in the form of
  a projector $\Pi_V$ onto $V$, compute
  \[
  \OPT(V) \defeq  \frac{1}{n}\max_{b \in \{\pm 1\}^n} b^\T \Pi_V b.
  \]
\end{definition}


\subsection{Sum-of-Squares solutions}

We will work with two equivalent definitions of a degree-$D$ SoS
solution: a pseudoexpectation operator and a moment matrix. We tailor these
definitions to our setting of feasibility of systems of polynomial
equality constraints given by the common zero set of a collection of
polynomials $\calP$ on $\pm \frac{1}{\sqrt{n}}$ Boolean variables
$v_1,\dots,v_n$.  For a degree-$D$ solution to be well defined, we
need $D$ to be at least the maximum degree of a polynomial in
$\calP$. Let $\RR^{\le D}(v_1,\dots,v_n)$ be the subset of
polynomials of degree at most $D$ from the polynomial ring
$\RR(v_1,\dots,v_n)$. We denote the degree of a polynomial
$f \in \RR(v_1,\dots,v_n)$ by $\deg(f)$.

\subsubsection{Pseudoexpectation operator}

We formally define the pseudoexpectation operators used in our setting.
\begin{definition}[Pseudoexpectation]\label{def:pseudoexpectation}
  Given a finite collection of ``constraint'' polynomials $\calP$ of degree at most $D$ on $\pm \frac{1}{\sqrt{n}}$ Boolean variables $v_1,\dots,v_n$,
  a degree-$D$ pseudoexpectation operator $\pE$ is an operator
  $\pE \colon \RR^{\le D}(v_1,\dots,v_n) \to \mathbb{R}$ satisfying:
  \begin{enumerate}
    \item $\pE[1] = 1$, \label{pe:normalized}
    \item $\pE$ is an $\RR$-linear operator, i.e., $\pE[f+g] = \pE[f] + \pE[g]$ for every $f,g \in \RR^{\le D}(v_1,\dots,v_n)$, \label{pe:linear}
    \item $\pE[f^2] \ge 0$ for every $f \in \RR^{\le D}(v_1,\dots,v_n)$ with $\deg(f^2) \le D$. \label{pe:psdness}
    \item $\pE[(v_i^2-\frac{1}{n}) \cdot f] = 0$ for all $i \in [n]$ and for every $f \in \RR^{\le D}(v_1,\dots,v_n)$ with $\deg(f) \le D-2$, and \label{pe:boolean}   
    \item $\pE[g \cdot f] = 0$ for every $g \in \calP, f \in \RR^{\le D}(v_1,\dots,v_n)$ with $\deg(f \cdot g) \le D$. \label{pe:feasible}
  \end{enumerate}
\end{definition}
Note that $\pE$ behaves similarly to an expectation operator
restricted to $\RR^{\le D}(v_1,\dots,v_n)$ with the caveat that $\pE$
is only guaranteed to be non-negative on sum-of-squares polynomials.

The degree-$D$ SoS algorithm checks feasibility of a polynomial system by 
checking whether or not a degree-$D$ pseudoexpectation operator exists. To 
show an SoS lower bound, one must construct a pseudoexpectation 
operator.

\subsubsection{Moment matrix}\label{sec:moment-mtx}

We define
the moment matrix associated with a degree-$D$
pseudoexpectation $\pE$.
\begin{definition}[Moment Matrix of $\pE$]
  The moment matrix $\calM=\calM(\pE)$ associated to a pseudoexpectation $\pE$ is a
  $\binom{[n]}{\leq D/2} \times \binom{[n]}{\leq D/2}$ matrix with rows and columns indexed
  by subsets of $I, J \subseteq [n]$ of size at most $D/2$ and defined as
  \[
  \calM[I, J] \defeq \pE\left[ v^I \cdot v^J \right].
  \]
\end{definition}

To show that a candidate pseudoexpectation satisfies~\cref{pe:psdness} in~\cref{def:pseudoexpectation}, we will rely on the following standard fact.
\begin{fact}
  In the definition of pseudoexpectation, \cref{def:pseudoexpectation}, the condition in \cref{pe:psdness} is equivalent to $\calM \succeq 0$.
\end{fact}

\subsection{Graph matrices}
To study $\calM$, we decompose it using the framework of \textit{graph matrices}. Originally developed in the context of the planted clique problem, graph matrices are random matrices whose entries are symmetric functions of an underlying random object -- in our case, the set of vectors $d_1, \dots, d_m$. We take the general presentation and results from~\cite{AMP20}. For our purposes, the following definitions are sufficient.


The graphs that we study have two types of vertices, circles $\circle{}$ and squares $\square{}$. We let $\calC_m$ be a set of $m$ circles labeled 1 through $m$, which we denote by $\circle{1}, \circle{2}, \dots, \circle{m}$, and let $\calS_n$ be a set of $n$ squares labeled 1 through $n$, which we denote by $\square{1}, \square{2}, \dots, \square{n}$. We will work with bipartite graphs with edges between circles and squares, which have positive integer labels on the edges. When there are no multiedges (the graph is simple), such graphs are in one-to-one correspondence with Fourier characters on the vectors $d_u$. An edge between $\circle{u}$ and $\square{i}$ with label $l$ represents $h_{l}(d_{u,i})$ where $\{h_k\}$ is the Fourier basis (e.g. Hermite polynomials).

\[ \text{simple graph with labeled edges} \qquad \Longleftrightarrow \qquad \displaystyle\prod_{\substack{\circle{u} \in \calC_m,\\ \square{i} \in \calS_n}} h_{l(\circle{u}, \square{i})}(d_{u,i}) \]

An example of a Fourier polynomial as a graph with labeled edges is given in~\cref{fig:fourier_graph}. Unlabeled edges are implicitly labeled 1.
\begin{figure}[h!]
\centering      
\begin{tikzpicture}[scale=0.5,every node/.style={scale=0.5}]
\draw  (-2,3) rectangle node {\huge $i_1$}(-0.5,1.5) node (v5) {};
\draw  (3,1) ellipse (1 and 1) node {\huge $u$};
\draw  (6.5,3) rectangle node (v10) {\huge $j_1$} (8,1.5);
\draw  (-2,0) rectangle node {\huge $i_2$} (-0.5,-1.5);
\draw  (6.5,0) rectangle node {\huge $j_2$} (8,-1.5);
\node (v1) at (-0.5,3) {};
\node (v4) at (-0.5,2.25) {};
\node (v6) at (6.5,2.25) {};
\node (v8) at (-0.5,-0.75) {};
\node (v9) at (6.5,-0.75) {};
\node at (-0.5,0) {};
\node (v2) at (2,1) {};
\node at (2,1.5) {};
\node (v7) at (6.5,1.5) {};
\node (v3) at (4,1) {};
%\draw  plot[smooth, tension=.7] coordinates {(v1) (1,2.5) (v2)};
\draw  plot[smooth, tension=.7] coordinates {(v3)};
\draw  plot[smooth, tension=.7] coordinates {(v3)};
\draw  plot[smooth, tension=.7] coordinates {(v2) (0.5,2) (v4)};
\node at (1,2.2) {\huge $3$};
%\draw  plot[smooth, tension=.7] coordinates {(v2) (0.5,1) (v5)};
\draw  plot[smooth, tension=.7] coordinates {(v3) (5,2) (v6)};
\draw  plot[smooth, tension=.7] coordinates {(v3)};
\draw  plot[smooth, tension=.7] coordinates {(v2) (1,-0.5) (v8)};
\draw  plot[smooth, tension=.7] coordinates {(v3) (5,-0.5) (v9)};
\node at (6.5,3) {};
\draw  plot[smooth, tension=.7] coordinates {(v3)};
\draw  plot[smooth, tension=.7] coordinates {(v3)};
\draw  plot[smooth, tension=.7] coordinates {(v10)};
\node at (6.5,3) {};
\draw  (2,5.5) rectangle node {\huge $w_1$} (3.5,4);
\node (v11) at (2.5,4) {};
\node (v13) at (3,4) {};
\node (v12) at (3,2) {};
%\draw  plot[smooth, tension=.7] coordinates {(v12) (2.5,3) (2.5,4)};
\draw  plot[smooth, tension=.7] coordinates {(v12) (3,3) (3,4)};
\node at (2.5,3) {\huge $2$};
\end{tikzpicture}
\caption{The Fourier polynomial $h_3(d_{u,i_1})h_1(d_{u,i_2})h_2(d_{u,w_1})h_1(d_{u,j_1})h_1(d_{u,j_2})$ represented as a graph.}
\label{fig:fourier_graph}
\end{figure}


Define the degree of a vertex $v$,  denoted $\deg(v)$, to be the sum of the labels incident to $v$, and $\abs{E}$ to be the sum of all labels. For 
intuition it is mostly enough to work with simple graphs, in which case these quantities make sense as the edge multiplicities in an implicit multigraph.

\begin{definition}[Proper]
We say an edge-labeled graph is \textit{proper} if it has no multiedges.
\end{definition}
The definitions allow for ``improper'' edge-labeled multigraphs which simplify multiplying graph matrices (\cref{sec:single-spider} and \cref{sec:exact-constraints}).

\begin{definition}[Matrix indices]
A \textit{matrix index} is a set $A$ of elements from $\calC_m \cup \calS_n$.
\end{definition}
We let $A(\square{i})$ or $A(\circle{u})$ be 0 or 1 to indicate if the vertex is in $A$.

\begin{definition}[Ribbons]\label{def:ribbon}
A \textit{ribbon} is an undirected, edge-labeled graph $R = (V(R), E(R), A_R, B_R)$, where $V(R) \subseteq \calC_m\cup \calS_n$ and $A_R, B_R$ are two matrix indices (possibly not disjoint) with $A_R, B_R \subseteq V(R)$, representing two distinguished sets of vertices. Furthermore, all edges in $E(R)$ go between squares and circles.
\end{definition}
We think of $A_R$ and $B_R$ as being the ``left'' and ``right'' sides of $R$, respectively. We also define the set of ``middle vertices'' $C_R \defeq V(R) \setminus (A_R \cup B_R)$. If $e \not\in E(R)$, then we define its label $l(e) = 0$. We also abuse notation and write $l(\square{i}, \circle{u})$ instead of $l(\{\square{i}, \circle{u}\})$.


Akin to the picture above, each ribbon corresponds to a Fourier polynomial.
This Fourier polynomial lives inside a single entry of the matrix $M_R$.
In the definition below, the $h_k(x)$ are the Fourier basis corresponding to the respective setting. In the Gaussian case, they are the (unnormalized) Hermite polynomials, and in the boolean case, they are just the parity function, represented by
\[h_0(x) = 1, \qquad h_1(x) = x, \qquad h_k(x) = 0 \;\; (k \geq 2) \]

\begin{definition}[Matrix for a ribbon]\label{def:ribbon-matrix}
The matrix $M_R$ has rows and columns indexed by subsets of $\calC_m~\cup~\calS_n$, with a single nonzero entry defined by
\[M_R[I, J] = \left\{\begin{array}{lr}
    \displaystyle\prod_{\substack{e \in E(R), \\ e = \{\square{i}, \circle{u}\}}} h_{l(e)}(d_{u,i}) &  I = A_R, J = B_R\\
    0 & \text{Otherwise}
\end{array}\right. \]
\end{definition}

Next we describe the shape of a ribbon, which is essentially the ribbon when we have forgotten all the vertex labels and retained only the graph structure and the distinguished sets of vertices.
\begin{definition}[Index shapes]
An \textit{index shape} is a set $U$ of formal variables. Furthermore, each variable is labeled as either a ``circle'' or a ``square''.
\end{definition}
We let $U(\square{i})$ and $U(\circle{u})$ be either 0 or 1 for whether $\square{i}$ or $\circle{u}$, respectively, is in $U$.

\begin{definition}[Shapes]\label{def:shape}
A \textit{shape} is an undirected, edge-labeled graph $\alpha = (V(\alpha), E(\alpha), U_\alpha, V_\alpha)$ where $V(\alpha)$ is a set of formal variables, each of which is labeled as either a ``circle'' or a ``square''. $U_\alpha$ and $V_\alpha$ are index shapes (possibly with variables in common) such that $U_\alpha, V_\alpha \subseteq V(\alpha)$. The edge set $E(\alpha)$ must only contain edges between the circle variables and the square variables.
\end{definition}

We'll also use $W_\alpha \defeq V(\alpha) \setminus (U_\alpha \cup V_\alpha)$ to denote the ``middle vertices'' of the shape.

\begin{remk}
	We will abuse notation and use $\square{i}, \square{j}, \circle{u}, \circle{v}, \ldots$ for both the vertices of ribbons and the vertices of shapes. If they are ribbon vertices, then the vertices are elements of $\calC_m\cup\calS_n$ and if they are shape vertices, then they correspond to formal variables with the appropriate type.
\end{remk}

\begin{definition}[Trivial shape]
	Define a shape $\alpha$ to be trivial if $U_\alpha = V_\alpha$, $W_\alpha = \emptyset$ and $E(\alpha) = \emptyset$.
\end{definition}

\begin{definition}[Transpose of a shape]
  The transpose of a shape  $\alpha = (V(\alpha), E(\alpha), U_\alpha, V_\alpha)$ is defined
  to be the shape $\alpha^{\T} = (V(\alpha), E(\alpha), V_\alpha, U_\alpha)$.
\end{definition}

For a shape $\alpha$ and an injective map $\sigma : 
V(\alpha) \to \calC_m \cup \calS_n$, we define the 
realization $\sigma(\alpha)$ as a ribbon in the natural
way, by labeling all the variables using the map 
$\sigma$. We also require $\sigma$ to be 
type-preserving i.e. it takes square variables to $\calS_n$ and circle variables to $\calC_m$. 
%
The ribbons that result are referred to as \textit{ribbons of shape $\alpha$}; notice that this partitions the set of all ribbons according to their shape\footnote{Partitions up to equality of shapes, where two shapes are equal if there is a type-preserving bijection between their variables that converts one shape to the other. When we operate on sets of shapes below, we implicitly use each distinct shape only once.}\footnote{Note that in our definition two realizations of a shape may give the same ribbon.}.

Finally, given a shape $\alpha$, the graph matrix $M_\alpha$ consists of all Fourier characters for ribbons of shape $\alpha$.
\begin{definition}[Graph matrices]\label{def:graph-matrix}
Given a shape $\alpha = (V(\alpha), E(\alpha), U_\alpha, V_\alpha)$, the \textit{graph matrix} $M_\alpha$ is
\[M_\alpha = \displaystyle\sum_{R \text{ is a ribbon of shape }\alpha} M_R\]
\end{definition}

The moment matrix for PAP will turn out to be defined using graph matrices $M_\alpha$ whose left and right sides only have square vertices, and no circles. However, in the course of the analysis we will factor and multiply graph matrices with circle vertices in the left or right.


\subsection{Norm bounds}
The spectral norm of a graph matrix is determined, up to logarithmic factors, by relatively simple combinatorial properties of the graph. For a subset $S \subseteq \calC_m \cup \calS_n$, we define the weight $w(S)~\defeq~(\#\text{ circles in }S)\cdot \log_n(m)+ (\#\text{ squares in }S)$. Observe that $n^{w(S)} = m^{\# \text{ circles in }S}\cdot n^{\#\text{ squares in }S}$.

\begin{definition}[Minimum vertex separator]
For a shape $\alpha$, a set $S_{\min}$ is a minimum vertex separator if all paths from $U_\alpha$ to $V_\alpha$ pass through $S_{\min}$ and $w(S_{\min})$ is minimized over all such separating sets.
\end{definition}

Let $W_{iso}$ denote the set of isolated vertices in $W_\alpha$. Then essentially the following norm bound holds for all shapes $\alpha$ with high probability (a formal statement can be found in~\cref{app:norm_bounds}):
\[\norm{M_\alpha} \leq  \widetilde\bigoh\left(n^{\frac{w(V(\alpha)) - w(S_{\min}) + w(W_{iso})}{2}}\right)\]

In fact, the only probabilistic property required of the inputs $d_1, \dots, d_m$ by our proof is that the above norm bounds hold for all shapes that arise in the analysis.
We henceforth assume that the norm bounds in~\cref{lem:gaussian-norm-bounds} (for the Gaussian case) and~\cref{lem:norm-bounds} (for the boolean case) hold.
